Malleable Overview-Detail Interfaces

The overview-detail design pattern, characterized by an overview of multiple items and a detailed view of a selected item, is ubiquitously implemented across software interfaces. Designers often try to account for all users, but ultimately these interfaces settle on a single form. For instance, an overview map may display hotel prices but omit other user-desired attributes. This research instead explores the malleable overview-detail interface, one that end-users can customize to address individual needs. Our content analysis of overview-detail interfaces uncovered three dimensions of variation: content, composition, and layout, enabling us to develop customization techniques along these dimensions. For content, we developed Fluid Attributes, a set of techniques enabling users to show and hide attributes between views and leverage AI to manipulate, reformat, and generate new attributes. For composition and layout, we provided solutions to compose multiple overviews and detail views and transform between various overview and overview-detail layouts. A user study on our techniques implemented in two design probes revealed that participants produced diverse customizations and unique usage patterns, highlighting the need and broad applicability for malleable overview-detail interfaces.

==> versions/R_R/1_introduction.tex <==
\section{Introduction}
\label{section:introduction}

The overview-detail design pattern describes interfaces that typically consist of two views: an overview that presents a collection of items along with their key attributes, and a detail view that provides an in-depth look at a selected item, including many, if not all, of its attributes \cite{Shneiderman1996OverviewFirst, tidwell1997pattern}. This pattern enables users to efficiently browse through a large number of information entities and delve into specific ones of interest, facilitating one of the most essential operations in information tasks \cite{Norman1986ProgressiveDisclosure, Hornbaek2001OverviewDetailBenefits}. This is perhaps why the overview-detail pattern has become ubiquitous in information systems, such as shopping, booking, and rental sites, calendars, email clients, messaging applications, news and video platforms, and numerous others (Fig. \ref{fig:teaser}A).

Typically, it is the designers and developers that determine how the overview-detail pattern is instantiated in an information system for a specific context, considering factors such as the layout and interaction of the overview and the detail view, as well as the different sets of attributes to present in these views.
% For example, some email clients arrange the overview and detail side by side, with the overview displaying the sender, subject, and time of all emails and the detail view displaying the contents of the email. Many shopping websites, on the other hand, open the selected product's detail view on a new page to avoid cluttering the overview page. Many map-based booking websites display the detail view as a pop-up and the overview underneath to provide context, and often display a single attribute of an item in the overview (e.g., the price for hotels).
While they strive to create the best design for their general user base, a single instantiation of the overview-detail pattern is inevitably not enough to match the diverse needs of all users and their usage contexts. 
For instance, separating the detail view onto another page, such as in most shopping websites, can reduce clutter in the overview but incur repetitive view switching (Figure \ref{fig:md-limitations}A). Meanwhile, displaying only the price of hotels on a map improves clarity but omits other attributes---such as ratings or the number of beds---that some users may prioritize (Figure \ref{fig:md-limitations}B). Yet, few modern interfaces are malleable, forcing the end-users to work with the design determined by their developers, regardless of the end-users' own needs and preferences. 

\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{figures/1_introduction/limitations.png}
    \caption{(A) Semantic Scholar includes a paper’s title, authors, abstract, and others, but does not include figures in the master view. To view figures for each paper, the user must open each hyperlink to the paper’s detail view and toggle through every opened page. (B) Airbnb displays pins with prices on a map, representing the nightly prices of each stay. If the user wants to view other details, such as the number of bedrooms, ratings, number of reviews, the user must click on each place and navigate to a full page of details.}
    \label{fig:md-limitations}
    \Description{This figure contains two website interfaces labeled (A) and (B). Interface A shows two screenshots of Semantic Scholar, an academic research platform.The left screenshot presents a list overview of search results showing the title, authors, abstract, and other details for research papers. The right screenshot displays the detailed view of a selected research paper. The user must open each paper’s detailed view to see figures and other specifics. The overview does not display these figures directly. Interface B shows a map with price tags pinned at different locations, representing the nightly prices of accommodations on Airbnb. If users want to view details like bedrooms, ratings, or reviews, they need to click on each pin and navigate to a full-page description of selected accommodation.}
\end{figure}

\changed{
At its core, the overview-detail design pattern is intertwined with fundamental challenges in information foraging, sense-making, and decision-making \cite{coststructuresensemaking}.
First, the overview may not present the right abstraction of individual information entities to meet users' specific needs, forcing them to forage for details from other views \cite{infoforagingtheory}. 
Second, a system may hinder sensemaking if the representation of the collection of items it provides does not adequately address users' needs \cite{zhang1994representations,Kirsh2010ThinkingWithExReps, Shneiderman1996OverviewFirst}.
Third, the spatial arrangement and interaction between the overview and the detail view may hinder necessary navigation among the different views.}
Therefore, the key question we explore is \textbf{instead of letting developers dictate how information is abstracted and presented, can we make the overview-detail design pattern malleable?} That is, can we empower end-users to flexibly customize overview-detail interfaces to \changed{form their own abstractions and spatial arrangements of information?}
We break this goal into three research questions:

\begin{enumerate}[label=\textbf{[RQ\arabic*]}, leftmargin=*]
    \item  What is the design space of various implementations of this design pattern in real-world contexts,
and how can they inform the development of malleable overview-detail interfaces? 
    \item What are the interface designs and interaction techniques that can enable end-users to flexibly transform an overview-detail interface?
    \item To what extent do end-users prefer and utilize malleable overview-detail interfaces to achieve their information tasks? What are their novel usage patterns? Is the malleability we provide enough?
\end{enumerate}

We took the following steps to address these questions. First, to understand the current variations of the overview-detail pattern (\textbf{RQ1}), we conducted a content analysis with a diverse sample of 303 instantiations of the overview-detail pattern collected from 156 websites and identified three key dimensions: \textit{content}, \textit{composition}, and \textit{layout}. Second, based on these dimensions, we developed interaction techniques that allow users to customize overview-detail interfaces along these three dimensions (\textbf{RQ2}).
\changed{
For the content dimension, we developed a set of interactions, which we label as \textit{Fluid Attributes}, that enables users to surface new attributes from the detail view to the overview (Fig. \ref{fig:teaser}C), hide unwanted attributes in the overview, and use any selected attribute to filter and sort items (Fig. \ref{fig:teaser}D). Users can also prompt AI to perform these customizations automatically, reformat existing attributes, and create new ones. 
For the composition and layout dimensions, we developed solutions for customizing how the overviews and detail views are composed, such as introducing multiple overviews in the interface, and for transforming between various overview and overview-detail layouts.
We demonstrate how our presented customizations could be designed and implemented in overview-detail interfaces through multiple applications.
}
% control attributes with AI by surfacing attributes, thereby reducing unnecessary navigation between various views.
% These interaction techniques apply broadly across many variations of overview-detail interfaces.

Finally, to study the utility and usage patterns of malleable overview-detail interfaces (\textbf{RQ3}), we conducted a user study (N=12) on two design probes to accomplish shopping and booking tasks.
\changed{
% Finally, we observed how an adoption of malleable overview-detail interfaces in our design probes can influence user workflows and usage patterns (\textbf{RQ3}).
% With two high-fidelity design probes that implement our customization techniques, we conducted a user study (N=12) to accomplish shopping and hotel booking tasks.
We found that participants given the same tasks produced diverse customizations of content, composition, and layout, highlighting the need for malleable overview-detail interfaces across these dimensions.
% Furthermore, we discovered that participant usage patterns of customizing attributes closely resembled tendencies in managing personal digital information as well as structuring task hierarchies, suggesting malleable overview-detail interfaces can provide end-users the control over their interfaces to better mold the interface to their personal needs and activities.
Furthermore, we discovered that participants' usage patterns resembled common tendencies in managing personal digital information and structuring tasks, demonstrating how malleable overview-detail interfaces integrate into broader, everyday workflows.
}
% suggesting that malleable overview-detail interfaces can be broadly and effectively utilized if widely adopted.
% ---even ones provided by the public---are able to transform into personal information spaces.
% can empower users to better mold these interfaces to their needs and activities.
% This part is not going to be clear for the reader; they won't know what personal information space is

% , namely hoarding information in their interface versus reducing unnecessary clutter \cite{Vitale2018HoardingAndMinimalism}. 
% We then discuss how malleable overview-detail interfaces can be practically adopted in the real world, which will inevitably face challenges in development costs and business incentives.



In summary, our work contributes:
\begin{enumerate}
    \item A content analysis of the overview-detail design pattern that revealed three key dimensions of the design space.
    % \item \changed{An interview with industry professionals (N designers, M product managers, and P web developers) that revealed why malleable overview-detail interfaces are not widely designed and supported in the wild.}
    % \item Interaction techniques for malleable overview-detail interfaces, including a novel technique, \technique, that enables users to directly choose what, where, and how attributes are shown the interface.
    \item \changed{Interaction techniques that enable end-users to customize overview-detail interfaces, offering diverse layouts and compositions of overviews and detail views, attribute manipulability across views, and AI-driven interactions to reformat attributes and generate new ones.}
% A set of interaction techniqeues that enable end-users to flexibly customize the overview-detail interfaces, including the content with the different views, the attribute-oriented representation within the overview, the spatial arrangment of the overview and detail view, as well as novel integration with AI
    \item A user study demonstrating that participants effectively utilized malleable overview-detail interfaces to address diverse needs and revealing emergent usage patterns that inform design suggestions for future implementations.
\end{enumerate}





% Given the generalizability of customizations for overview-detail interfaces, we also 
\changed{
Our vision is to make all aspects of interfaces malleable---to make interfaces easily, expressively, and broadly customizable by the end-user.
We approach this vision by making interfaces malleable \textit{one design pattern at a time}—analyzing variations of a single design pattern and exploring broadly generalizable customization techniques that extend beyond their originally intended scenarios and contexts.
We hope this paper not only encourages future interfaces to implement malleable overview-detail interfaces, but also for future research to adopt this paper's approach to explore how more design patterns can become malleable.
}

% building upon a single design pattern in the overview-detail interface.
% To achieve this vision, we focus this research on analyzing and building upon a single design pattern in the overview-detail interface.
% We also hope this paper communicates our approach to 

% We approach this vision by making interfaces malleable \textit{one design pattern at a time}---by analyzing variations of a single design pattern and exploring broadly generalizable customization techniques across all of its instantiations.

% However, we hope this paper additionally communicates our approach to making interfaces malleable \textit{one design pattern at a time} to encourage future research to adopt this approach to more design patterns.





% Through our analysis of enabling ways for the end-user to manipulate content in overview-detail interfaces, we discovered that the overview-detail design pattern the pattern let us realize that very simple yet expressive interaction techniques can apply to a broad range of interfaces.
% We found content dimension pretty interesting because of manipulable attributes
% key value pair... model that info into attributes
% seems simple, but it's extremely critical, because it's related to user-defined abstration, navigation costs, how information is modeled
% This simple solution addresses a bunch of fundamental challenges
% This is actually a really big deal because we are the first to formalize an instantiation of an interface that supports user-defined abstractions---interfaces that actively support the end-user to form their own abstractions of provided information seamlessly during their information task.
% provided a simple yet expressive substrate for efficiently propagating attribute manipulations across many items.



% Okay, writing very casually now
% Goal of this paragraph: It's a simple pattern, but this simple pattern is extremely critical in interfaces
% It is one of the most ubiquitous instances of abstraction in software interfaces

% What else does this cover other than abstraction

% We want to say this work is a deep analysis of ODIs and then studying this leads to a bunch more research
% Conceptually, how we can build user-defined abstractions

% This issue stems from core challenges this researhc
% People cannot form their own abstractions on the interface
% Overview-detail is the most

% , regardless of then end-users' own purposes and contexts. 
% , regardless of the end-users' own needs. 

% At the core of the overview-detail pattern is the need to view information at different levels of abstraction, for different sets of details and in different spatial arrangements during information tasks. 
% The overview-detail pattern is a ubiquitously implemented form of abstraction

% Second, this challenge of not being able to view information at the right abstraction or spatial arrangement
% : the need to view information at different levels of abstraction.
% Because they cannot view 
% this pattern carries a fundamental need and characteristic that reflects in all forms of information systems: the universal need to view information at different levels of abstraction.
% The challenges described above is saying that users are not able to view the right abstraction for their need and are instead funneled into inefficient mechanisms to view this information, such as excess navigation between views \cite{tabsdo}, \bryan{to include more issues}
% While the overview-detail pattern may appear simple on the surface, this pattern ... is quite complex, carries fundamental needs and characteristics that reflect in all kinds of information systems.
% There is a universal need to view information at different levels of abstraction---different sets of detail and in different spatial arrangements. 
% , the data model the interface reflects is a ubiquitous information model, 
% 
% 
% The overview-detail pattern, along with its interaction challenges, may appear simple on the surface. 
% However, the core of the pattern carries many fundamental problems in interfaces...
% Since the overview is an abstraction of the detail views of items, there's a challenge in users not being able to define their own abstractions, hindering ... so there's a problem in how abstractions are not dynamic enough.
% abstraction and representation has a long history of these dynamic representations, and there being issues of whatever... etc.d.sfsdafs
% There is also this issue of navigation costs when moving between different views of information. This is a long standing issue of trying to reduce navigation costs in window management, and other things...
% The model of the design pattern contains... I'm actually not too sure what he mean by this anymore...
% What did he mean by the model? Anyways, yes. this paper is a foundational paper on abstractions because it is the first paper to cover "User-Defined Abstractions" in interfaces.

% Second, the spatial representation of the collection of entities may be ineffective for users to quickly identify entities of interest or understand the overall distribution of entities along key dimensions \cite{coststructuresensemaking}.


% \bryan{Something along the lines of must consider fundamental challenges intertwined with this pattern}
% they otherwise should be able to see if provided the right abstraction.
% in a more aligned overview.
% Second, overview-detail interfaces support multiple stages of information work, from exploration, sense-making, and decision-making, yet most overview-detail interfaces do not provide multiple forms of spatial arrangements to support these wide ranging tasks .}
% \bryan{While it may appear simple,}
% It seems simple on the surface, but it involves a bunch of different kinds of problems.
% 
% seems simple, but it's extremely critical, because it's related to user-defined abstration, navigation costs, how information is modeled







% can 
% further apply to more design patterns, ultimately making more aspects of interfaces malleable.

% We hope that our approach of making .... 


% by discovering and analyzing more patterns and making them malleable.
% Through this research, our goal of making all aspects of interfaces malleable---expressively, easily, and broadly customizable by the end-user. In order to achieve this, this paper takes the approach of making interfaces malleable, one design pattern at a time.
% Then something like: We hope this approach provides a path towards making more interfaces malleable by discovering and analyzing more patterns and making them malleable.}
% I feel this can't just be introduced here all of a sudden. It's toooooo surprising. Need to talk about this once, then talk about it again at the end or something. Similar to ASCII diagrams intro





% Finally, to study the utility and usage patterns of malleable overview-detail interfaces (\textbf{RQ3}), we developed two high-fidelity design probes that implement our interaction techniques: a shopping website and a hotel booking website, and conducted a user study with 12 participants where they used both design probes to accomplish shopping and booking tasks. We found that participants given the same tasks produced diverse customizations of content, composition, and layout, highlighting the need for malleable overview-detail interfaces across these dimensions. They also found the malleable overview-detail interface preferable, sharing that it allowed them to control what they wanted to focus on, reduced unnecessary navigation, and aligned their decision-making criteria to the information they wanted. Finally, we report on the emergent usage patterns of malleable overview-detail interfaces and discuss practical implications that such interfaces may have for end-users, developers, and AI.

% For example, users could surface attributes from the detail view to the overview, displaying these attributes across all items to reduce excess navigation between the overview and detail view, and hide unwanted attributes to efficiently reduce clutter. 





% Through our analysis, we discovered that making attributes directly manipulable between the overview and detail view provided a simple yet expressive way to customize overview-detail interfaces.



% The overview-detail pattern also enables fluid attributes to be assisted by AI, by asking for attributes with natural language queries and 

% is a widely generalizable and adoptable customization technique across many diverse forms of overview-detail interfaces.  This enables 

% The power in these techniques are in that they can generalize across very diverse forms of overview-detail interfaces; we demonstrate this generalizability through multiple design probes.

% Among the interaction techniques we designed, a key novel technique we contribute is \textit{\technique}, which enables users to flexibly adjust what, where, and how information attributes are represented on the overview-detail interfaces, providing a simple yet expressive way to customize overview-detail interfaces (Fig. \ref{fig:teaser}B). For example, users can surface new attributes from the detail view to the overview (Fig. \ref{fig:teaser}C), hide unwanted attributes in the overview, and use any selected attribute to filter and sort items (Fig. \ref{fig:teaser}D). Assisted with AI, users can search attributes with natural language queries, generate synthesized attributes from existing ones, and apply a consistent format to diverse attribute values (e.g., making the titles of shopping items from different vendors consistent). We also demonstrate how \technique and allow users to integrate various overview representations.
% These interaction techniques enable users to more effectively discover and consume their desired information. We demonstrate these interaction techniques with a number of research prototypes.



% % \haijun{We also demonstrate compelling use cases of synchronizing several overviews each providing a suitable representation of the chosen attribute (poor writing, but just want to leave a note here about what should be described in the intro)}

















% Furthermore, \technique is designed for the overview-detail pattern as a whole, making it applicable across all overview-detail interfaces.

% A user study of these probes shows that users can effectively make such transformations when given the opportunity. We additionally report on emergent usage patterns that our interaction techniques enable.


% Users can also make customizations through AI, by asking for higher level queries, and even push it further by generating new attributes about items.

% We also recognize the opportunity for a malleable overview-detail interface to be used 

% For the potential of how we can interact with AI as a medium for a malleable overview-detail interface. 



% Our interaction techniques for the customizable overview-detail interfaces also serve as a medium 

% Our interaction techniques that we provide to the end-user also serve as a medium for AI to operate

% We also explore possibilities for overview-detail interfaces to be customized through AI. 


% Users can leverage these customization techniques to address personal needs, such as 

% For instance, users can leverage \technique to 

% This interaction technique provides users with the ability to pull any detail attribute from the detail view to the overview, hide unrelated attributes from the overview into the detail view, or sort and filter items directly upon selecting attributes of interest (Fig. X). Users may leverage \technique to ``pull'' additional details about homes beyond the default-provided price attribute.

% This interaction technique provides users with the ability to pull any detail attribute from the detail view to the overview, hide unrelated attributes from the overview into the detail view, or sort and filter items directly upon selecting attributes of interest (Fig. X).
% % Why?
% These interactions
% Furthermore, since \technique is an interaction technique for the overview-detail design pattern itself, it offers broad applicability across all such interfaces. For example, it directly addresses the challenge depicted in Figure \ref{fig:md-limitations}b by enabling users to pull any detailed attribute they need into the map view, 

% The elegance of \technique lies in its broad applicability across all overview-detail interfaces

% The elegance of \technique lies in its ability to personalize information shown or hidden in the interface, addressing the challenge of either missing details or being overwhelmed by excessive information, while also offering broad applicability across all overview-detail interfaces.

% \bryan{Include the possiblities of \technique with AI}

% \bryan{Intro needs a statement about how we are really trying to contribute a principle or something, to enable this underlying interaction/info architecture for AI to be better used or something}

% Detailed manipulation is 

% \textit{What is the technique? What's good about it? Why is it important?}


% This interaction directly addresses the challenges illustrated in Figure \ref{fig:md-limitations}b by allowing the user to choose to pull the number of bedrooms or ratings of a place to the map view.

% A key novel technique we contribute is \textit{pulling the details}, which enables users to select and ``pull'' details from a detail view to items in the master view (Fig. <in-teaser-figure>). A \bryan{Deeper into the interaction techniques and their benefits}


% Over the decades, many software interface design patterns have evolved dramatically, while others have remained foundational, serving as the bedrock for countless designs. One such pattern is the master-detail (MD) interface, which presents an overview of items (master) alongside detailed information about a selected item (detail) \cite{Seffah2015PatternsOH, Molina2002JustUI}. Despite being implemented since the early days of user interfaces, this pattern has become ubiquitous, seen in applications ranging from calendars to e-commerce platforms. Figure \ref{fig:md-variations} illustrates this evolution: a calendar interface from 2000 (Fig. \ref{fig:md-variations}a) and Google Calendar\footnote{} in 2024 (Fig. \ref{fig:md-variations}b) both implement the same MD pattern, though with updated visuals. Other variations of this pattern include BestBuy\footnote{}, which separates the master and detail views across different web pages (Fig. \ref{fig:md-variations}c), and Zillow\footnote{}, which displays a map-based master view with a detail popup (Fig. \ref{fig:md-variations}d).

% \begin{figure}
%     \centering
%     \includegraphics[width=0.75\linewidth]{figures/md-instances/variations.png}
%     \caption{(a) Calendar interface from a CHI 2000 Extended Abstract \cite{Laakso2000MDCalendar}. (b) Google Calendar interface (as of 2024). (c) BestBuy’s shopping interface displays the master view in one web page and the detail view in another. (d) Zillow’s interface displays a master view of listings on a map and a detail view of a selected listing in a popup.}
%     \label{fig:md-variations}
% \end{figure}

% While each implementation of the MD design pattern may tailor the needs to their general user base, a single implementation also reveals interaction constraints. For instance, separating the detail view onto another page can reduce screen clutter but forces users to repeatedly switch views (Figure \ref{fig:md-limitations}a). Meanwhile, displaying only the price of homes on a map improves clarity but omits other details—such as ratings or the number of bedrooms—that some users may prioritize instead (Figure \ref{fig:md-limitations}b).

% \begin{figure}
%     \centering
%     \includegraphics[width=0.75\linewidth]{figures/md-instances/limitations.png}
%     \caption{(a) Semantic Scholar includes a paper’s title, authors, abstract, and others, but does not include figures in the master view. To view figures for each paper, the user must open each hyperlink to the paper’s detail view and toggle through every opened page. (b) Airbnb displays pins with prices on a map, representing the nightly prices of each stay. If the user wants to view other details, such as the number of bedrooms, ratings, number of reviews, the user must click on each place and navigate to a full page of details.}
%     \label{fig:md-limitations}
% \end{figure}

% Despite the multitude of MD implementations designed to address various user needs, most interfaces typically use only a single instance of the MD design pattern. \textbf{However, a single instance is not enough for the diverse needs of all users.} Instead, users should be able to customize the MD interface to control the presentation and organization of information according to their specific needs.

% Despite the widespread use of the master-detail (MD) design pattern, our understanding of its variations remains limited. Existing research identifies variations in master view structures (e.g., list of items, single instance) and explores nested MD interfaces \cite{Seffah2015PatternsOH, Molina2002JustUI, Nguyen2012MDAndroid}. However, there is a lack of a more comprehensive, empirical analysis of these variations, leaving many aspects of MD interfaces underexplored.

% In this research, we aim to better understand current variations of the MD design pattern and provide mechanisms for users to transform these interfaces to meet their specific needs. Through a content analysis of 303 MD instantiations on desktop web interfaces, we identified three key dimensions of variation: \textit{layout}, \textit{composition}, and \textit{content}.

% Through our exploration of the design space, we developed interaction techniques that allow users to customize the MD interface along these three dimensions. A key novel technique we contribute is \textit{pulling the details}, which enables users to select and ``pull'' details from a detail view to items in the master view (Fig. <in-teaser-figure>). To demonstrate these techniques, we developed two design probes: a shopping interface and a hotel booking interface. A user study of these probes shows that users can effectively make such transformations when given the opportunity. We additionally report on emergent usage patterns that our interaction techniques enable.

% In summary, our work contributes:
% \begin{enumerate}
%     \item A content analysis of master-detail interfaces that maps variations into a design space along three dimensions.
%     \item Interaction techniques enabling transformable MD interfaces, demonstrated through two design probes: a shopping interface and a hotel booking interface.
%     \item A user study demonstrating that users can effectively utilize transformable MD interfaces to address individual needs.
% \end{enumerate}




% We do know that variations do exist, and there are various needs for them. 

% For instance, there are variations in how each of the two views arrange information, we know

% The ubiquity of the master-detail design pattern across various software interfaces makes it particularly interesting to study. Academic research and online articles have highlighted a few key variations of MD interfaces. For instance, Seffah discusses different structures a master view can have, such as a list of items or a single item instance. Additionally, case studies have explored how different screen sizes necessitate varying arrangements of the master and detail views, and how MD interfaces can be nested to create hierarchical structures within applications \cite{Seffah2015PatternsOH, Nguyen2012MDAndroid, Medium article}.

% Despite the ubiquity of the MD design pattern, we only have an informal grasp of the kinds of MD interface variations exist \cite{Seffah2015PatternsOH}. 

% \bryan{There needs to be a paragraph laying out the current state of research in MD patterns}
% There needs to be a paragraph laying out the current state of research in MD patterns
% If there is nothing, then also must say something like: despite its ubiquity, we only have an informal grasp of the variations of MD interfaces that exist in the wild and little understanding of what MD transformations are available today.




% This work unveils the interaction possibilities that can 
% I feel there needs to be this last sentence that says what this paper concludes.
% Some big moral of the story type of paragraph.
% We want to share that looking into the ubiquitous design patterns can provide ways to think of novel interaction techniques that are also very generalizable across a wide range of domains
% We want to share that this work is the foundation for .. what? idk
% Want to say this design space can be a generative tool...? --> nah that needs to be proved, through like a workshop or something. Also it's obvious that a design space is a generative tool. That's the entire point of a design space is to better see what you can implement within the space but also other variations you can explore.
% We conclude with design recommendations from our design space, design probe explorations, and user study findings.






% While many designs of software interfaces have evolved significantly, some have remained unchanged, becoming foundational interface patterns that other patterns and designs build upon. 

% Figure 2a depicts one interface implemented in the year 2000, showing a list of days of a calendar in the left pane and a detailed view of selected days in the right. Figure 2b depicts a similar interface in 2024 that displays the same pattern from Figure 2a. This pattern has been referred to by many names, one of which being the Master-Detail (MD) pattern, which is defined to present an overview of a set of items in one view (Master) and details of thea selected item in another view (Detail) []. Not only has this pattern been implemented for an extended period, but it has also grown ubiquitous over time, accumulating numerous variations in the arrangement of the two views and how information is presented in the MD interface. For example, Figure 2c depicts a variation where Master and Detail views are separated into two different web pages, while Figure 2d depicts a variation where the Master view’s items are placed on a map with the Detail view displayed in a popup panel.

% Figure 2: \textit{(a) Calendar interface from a CHI 2000 extended abstract displays a Master-Detail view in a single page []. (b) Google Calendar interface (as of 2024) displays a similar Master-Detail view. (c) BestBuy’s shopping interface displays the Master view in one webpage and the Detail view in another. (d) Zillow’s interface displays a Master view of listings on a map and a Detail view of a selected listing in a popup.}

% While the various implementations of MD interfaces may have addressed all kinds of user needs, they have also revealed more interaction constraints. For instance, while creating a separated web page for the Detail view can reduce cognitive overload from an interface, certain details may not be displayed in the Master view, forcing the user to repeatedly toggle through Detail views of each item (Fig. 3a). Additionally, while a popup view can retain the context of the Master view, it cannot retain the context of the popup view itself, potentially causing the user to lose progress on any working information in the popup (Fig. 3b). <Something about how there’s a solution for the problem in Fig. 3a, but 3a has another problem, which Fig. 3b can address, but this reveals another problem, maybe another view can address>

% Figure 3: \textit{(a) Semantic Scholar includes a paper’s title, authors, abstract, and others, but does not include figures in the Master view. To view figures for each paper, the user must open each hyperlink to the paper’s Detail view and toggle through every opened page. (b) ESPN lists articles for each highlight of a Wimbledon match and can open a popup to its video highlight. If the user wants to continue scrolling through the list of highlights, they must close the popup, losing progress of the video they are actively watching. To make things worse, each time the user reopens the popup, the video starts with an ad.}

% Despite the multitude of MD implementations that address various user challenges, each interface typically only implements a single MD instance. However, a single instance of the MD design pattern is not enough to support the diverse needs of end-users. Instead, end-users must be able to customize the MD interface to address their own needs.

% Thus, the goal of this research is to uncover the variations of MD interfaces that exist in websites and leverage this understanding to generate solutions for transforming MD interfaces that suit end-user needs.


% … content analysis … Design space

% … Interactions … user study … discuss…


% Contributions

% \begin{itemize}
%     \item Design Space of MD interfaces on what and where information is presented synthesized from content analysis \& designer interviews
%     \item Probes to demonstrate ways that a transformable MD interface can be implemented
%     \item User study observing how users interact with these probes


% \end{itemize}


==> versions/R_R/2_related_work.tex <==
\section{Related Work}
\label{section:related_work}


% Overview-Detail design pattern: there is lots of analyzis on this design pattern as a structure. We explore designs to enable end-users to customize this pattern.
% Need for malleable ODIs: lots of tasks require actions in ODIs. Their solution is to provide specific designs for each task. Instead we want to provide multiple representations, more abstractions for the user to customize.
% Ways to make interfaces customizable: Interfaces with aspects that are not customizable are not customizable because they aren't designed to be. Indeed, they can't be anticipated for these customizations. As a result, most customizations are made through browser extensions, there have even been approaches to make the web more foundationally customizable for the future. But for design patterns like ODIs, you need to change the bigger stack. So our goal is to first demonstrate these customizations to the designers first. 
% Manipulable Attributes in Software Interfaces: Our goal is to let users cusotmize ODIs by making information attributes manipulable. Making attributes manipulable has been done in content creation, data visualization, and personal information management. There's also notion and airtable for customizing ODIs. 1) also can surface UI components/widgets, leveraging AI to manipulate, 2) most importantly, we recognize these techniques generalize across the ODI pattern.

% As has been shown time and again, no matter how much designers and programmers try to anticipate and provide for what users will need, the effort always falls short because it is impossible to know it advance what may be needed.


% One of the core aspects that we enable as custmoizability is to enable users to choose which attributes to show or hide, essentially allowing them to abstract their 

\subsection{The Overview-Detail Design Pattern}
The overview-detail design pattern describes interfaces that provide two views: an overview that contains a collection of items and a detail view that provides full details of a selected item \cite{Shneiderman1996OverviewFirst}. This pattern, also referred to as ``master-detail’’ \cite{Seffah2015PatternsOH, Molina2002JustUI, Nguyen2012MDAndroid} and ``director-detail’’ \cite{Pastor2007ModelDrivenArchitecture}, visualizes information for users to view a large collection of items first before uncovering their details.
% (Fig. \ref{fig:md-definition}) .
If overview-detail interfaces are designed with progressive disclosure in mind, they can offer a more approachable interface while still allowing users to access additional details. \cite{Norman1986ProgressiveDisclosure, Shneiderman1996OverviewFirst}.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.75\linewidth]{figures/md-instances/definition.png}
%     \caption{(a) The overview that contains a collection of items. (b) The detail view that presents all details of a selected item from the overview.}
%     \label{fig:md-definition}
% \end{figure}

Prior research has explored several variations of the overview-detail pattern in user interfaces. Case studies have explored how overview-detail interfaces can be nested to create hierarchical views \cite{Molina2002JustUI, Seffah2015PatternsOH}, how several detail views can be used simultaneously \cite{Saidi2016SplittingDetailViews}, and how different screen sizes may necessitate varying arrangements of the overview and detail views  \cite{Seffah2015PatternsOH, Nguyen2012MDAndroid}. 
Cockburn \etal{} have also explored how overviews and detail views can be arranged horizontally, vertically, and also along the ``z-plane'' by layering nested overviews and detail views along the z-axis, navigable by zooming. This z-axis arrangement describes the structure of zoomable user interfaces such as Pad++ \cite{Bederson1994Padpp, Cockburn2009OverviewDetailReview}. 
A relevant but distinct design pattern also explored is ``focus+context'' interfaces \cite{FirstFocusContextInterface}, where focused content is placed seamlessly with the rest, oftentimes by reducing the view of the context space by skewing the views in 3D \cite{Mackinlay1991PerspectiveWallFocusContext}, scaling \cite{bederson2000fisheye}, and reducing the display's resolution \cite{Baudisch2001FocusPlusContext}.  

These works demonstrate the diverse implementations of the overview-detail design pattern developed through research, resulting in unique design choices tailored to specific contexts. However, our research aims to explore designs that enable users to flexibly customize the overview-detail interface according to their individual needs.

% While these works aim to design better defaults for overview-detail instances, we aim to enable users to flexibly customize the overview-detail interface to address their own needs.
% I think all previous work is about finding good defaults for specific ccontext, but our work is about eanbling flexible customization for a given context by the usesr.
% These works demonstrate the diverse implementations of the overview-detail design pattern developed through research, resulting in unique design choices tailored to specific contexts. While past studies have reviewed select cases of this pattern, we aim to explore its implementations on the most commonly used websites with a formal empirical analysis.

\subsection{The Need for Malleable Overview-Detail Interfaces in Information Tasks}
Many information tasks, such as foraging \cite{infoforagingtheory}, sensemaking \cite{coststructuresensemaking}, and decision-making \cite{mesh}, involve the iterative process of searching, browsing, collecting information across various sources, making sense of collected information through various representations, and then collecting new information based on the new insights \cite{coststructuresensemaking, Pirolli2005SensemakingProcess}. In this process, users require effective representations to organize and preview a large number of information entities and quickly determine relevant ones by inspecting their details. The overview-detail interfaces directly respond to such needs and, therefore, are ubiquitous in information systems, including information visualization systems \cite{Card1999VisionToThink, bach2016TellingStoriesGraphicComics} and academic literature exploration tools \cite{Relatedly, Kang2023Synergi}.

As mentioned earlier, a single instantiation determined by developers is not enough. Therefore, many research systems that have been created to support information tasks are essentially providing additional overview-detail instantiations to compensate what could not be supported with existing ones. For example, prior work has provided comparison tables to better organize decision-making criteria \cite{mesh}, hierarchical organizations of collected snippets to facilitate information management and re-finding \cite{Kang2022Threddy, Kang2023Synergi, fuse}, spatial canvases that scaffold the user's search and synthesis processes \cite{Ramos2022ForSense, Tashman2011LiquidText, Srishti2022InterWeave}, and node-link diagrams to contextualize users with their past browsing activities \cite{graphhistory}.

Another line of work recognizes that a single instantiation is not enough and proposes providing multiple instantiations, such as those that enable multiple levels of details or transforming information representations. Pad++ introduced semantic zooming, which offers multiple levels of detail based on different zoom levels, providing an alternative to geometric scaling techniques used in traditional zoomable interfaces. Recent research has also built on this idea to utilize AI to generate these different levels of detail \cite{Dang2022BeyongTextGeneration, Suh2023Sensecape, suh2023luminate}.
WritLarge demonstrated techniques for transforming between multiple representational axes—semantic, structural, and temporal—on a digital whiteboard \cite{Xia2017WritLarge}. 
% This enables users, for instance, to write a list of to-do items on the whiteboard, reify it into a checklist, and interact with it to mark items as complete. Transforming the checklist back to the sketch could retain the changes of marked items in digital ink.
Victor additionally illustrated the need for multiple representations through the concept of a ladder of abstraction, which demonstrates how moving between different levels of abstraction helps to gain a more comprehensive understanding of a system \cite{Victor2011LadderOfAbstraction}. 
Graphologue also explored multiple representations by leveraging AI to generate text alongside a node-link diagram side by side to facilitate information comprehension \cite{Graphologue}.
We share the spirit of these systems that aim to provide multiple representations by providing end-users the ability to transform and customize between different variations of overview-detail interfaces.


% \subsection{Designing Interfaces for Customizability}
\subsection{\changed{Designing End-User Customizable Information Systems}}
% \subsection{Recognizing the Generalizability of End-User Customizable Interfaces}

\changed{We share the research community's long-standing vision of creating malleable information systems for end-users to easily and expressively customize them to suit their preferences and information needs.
One research theme explores how to design the architecture of information systems to make them inherently customizable. For example, Haystack proposed a unified data model and a customizable interface layer to enable users to integrate diverse information sources and customize what information is presented to enable personalized information management \cite{adar1999haystack, Karger2007BDMHaystack}. Smalltalk focused on enabling users to directly modify the appearance and behavior of any object in the GUI \cite{kay1993smalltalk}. HyperCard explored enabling users to create dynamic and interactive content through a scripting language and graphical user interfaces \cite{Hypercard2024}. Finally, Webstrates treated web documents as dynamic media, enabling users to create custom representations of the same DOM element while facilitating real-time, dynamic collaboration \cite{Klokmose2015Webstrates}.
}

\changed{Another line of work explores extending existing systems to make them end-user customizable, particularly with web systems thanks to their accessible DOMs.
For instance, research has explored enabling end-users to directly customize a web interface by modifying the CSS attributes for website prototyping \cite{Kim2022Stylette, Visbug2024, Tanner2019Poirot}, embedding annotations between DOM elements to facilitate in-situ note-taking \cite{Romat2019SpaceInk}, and filtering, sorting, and making spreadsheet computations to personalize lists of items shown on a webpage \cite{Litt2020Wildcard, Huynh2006Sifter}. Research has also explored the potential of web mashups and automations enabled by direct manipulation and programming-by-demonstration techniques to automate workflows and reduce context-switching  \cite{Ghiani2016WebMashup, Bolin2005Chickenfoot, min2023masonview, Hartman2007Dmix, Zhang2018Fusion, Lin2009Vegemite}.
}

% Of the above work, most similar to our approach is Sifter \cite{Huynh2006Sifter}.

\changed{
Most of the above work, however, focuses on exploring the underlying information architecture or the technical approach to enable customization for specific activities, applications, and platforms, over concretely and conceptually scoping how broadly generalizable their customizations are.
For example, it is not readily obvious how approaches taken by personal information management systems (e.g., Haystack \cite{Karger2007BDMHaystack}, Notion \cite{Notion2024}) should be generalized to shopping websites.
Moreover, it is unclear how systems like Sifter \cite{Huynh2006Sifter}, which recognize a common DOM structure for list views, can generalize to other list variations or even extend to different patterns.
In contrast, our research focuses on investigating the overview-detail design pattern that is ubiquitous across diverse information systems and platforms. The design space of the overview-detail pattern that we propose allows interface designers to easily recognize the variations of overview-detail interfaces that exist in the wild, and also serve as a comprehensive guide of what all the possible customizations any overview-detail interface variation could theoretically support.
} 

% it is also challenging to broadly generalize system-specific or platform-dependent techniques. 
% For instance, systems like Sifter \cite{Huynh2006Sifter} identify list views through a concrete pattern in DOM structures, but this approach is not focused
% For instance, systems like Sifter \cite{Huynh2006Sifter} rely on patterns in DOM structures to identify many variations of list views, but they do this to identify technically, but recognize
% concretely define a pattern in the DOM structure to identify list views, DOM patterns alone do generalizable to all other list variations.
% sifter rely on DOM strucutre/pattern to define the scope --> enable the customatnio.
% Similarly, it is also not conceptually salient how systems like Sifter can facilitate the transformation of information between the overview and detail view, such as showing additional details in the overview to facilitate sorting and filtering.

% \changed{
% Most of the above work, however, does not focus on  might be beyond various activities and platforms, which is crucial for understanding how such customizations should be broadly implemented. The approach most similar to ours is Sifter \cite{Huynh2006Sifter}, which, in attempting to detect collections of items on websites for scraping, \textit{implicitly} leverages the overview-detail design pattern in the DOM structure by identifying a single variation of the overview-detail interface.
% % @Haijun -- btw they recognized the "new page" variation by identifying lists that contain <a> elements that link to a detail view. I thought this was too detailed, but just putting this here as context
% However, the diversity of DOM structures of overview-detail interfaces makes it challenging to rely on DOM patterns alone for consistently identifying all variations of this design pattern.
% Consequently, Sifter's customization techniques face limitations when applied broadly across interfaces that share the same design pattern but differ in their DOM structures.
% In contrast, we \textit{explicitly} define the overview-detail design pattern that is ubiquitous across diverse information systems and platforms.
% As a result, our investigation of this pattern allows us to concretely recognize all the interface variations that exist in the wild and contribute to a more comprehensive understanding of which variations to implement customization techniques for.
% % in individual instances can generalize across the entire pattern.
% }
% \bryan{One thing that I want to avoid when comparing with sifter is the technical aspect of making it possible to customize the list view. Because we don't contribute anything on how to actually make all of these list interfaces customizable technically, but with our design approach, we do know the limitations}
% \bryan{I really wanted to highlight that a technical limitation with Sifter is really that they just didn't explore the entire design pattern.}



% \changed{
% Most of the above work, however, focuses on developing specific systems for specific types of activities or relying on specific platforms, making it challenging to broadly generalize their approaches. 
% }
% \changed{
% In contrast, we focus on an interface design pattern that is ubiquitous across diverse information systems and platforms--the overview-detail pattern. 
% remain consistent across a wide range of tasks and interface platforms. Therefore, we instead approach designing interfaces for customizability by first exploring all the ways a design pattern can be made customizable.
% We first analyze the design pattern by exploring all of its variations and existing customizability features, and then provide interface solutions to making these variations transformable by the end-user. 
% The design pattern serves as both a guide for concretely identifying the broad applicability of customization techniques for interfaces and a framework for informing how to implement these customizations, whether through a browser extension, a front-end UI library, or a full-stack web framework.
% Given how closely overview-detail interfaces bind to the underlying data models, we apply this design pattern-centered approach to making overview-detail interfaces malleable.
% }


\subsection{\changed{Manipulable Attributes in Software Interfaces}}


\changed{
We build upon extensive work that has explored how manipulable attributes can be utilized in a variety of domains.
% This item-attribute model structure is ubiquitous around all forms of software interfaces, and that's why so many things are also manipulable around all software.
First, data visualization focuses on encoding data into visuals, and manipulating data and visual attributes has been a core technique that enables users to create, customize, and interact with data visualizations \cite{liu2018dataillustrator, DataInk}.
Manipulable attributes have also been used to support creative tasks, enabling users to compose new graphical styles \cite{ObjectOrientedDrawing}, search for related graphical objects based on attributes \cite{Xia2017CollectionObjects}, and make color attributes manipulable across multiple representations \cite{Chevalier2012Histomages}.
Personal information management systems such as Haystack \cite{Karger2005HaystackSystem} have enabled users to manipulate attributes to modify how their personal information is presented, and database- and table-oriented software such as MS Access \cite{MSAccess2024}, Filemaker Pro \cite{FileMakerPro2024}, Notion \cite{Notion2024}, and Airtable \cite{Airtable2024} have also allowed the end-user to show and hide attributes on their interface.
Additionally, our content analysis of overview-detail interfaces has also found e-commerce websites that allow end-users to show or hide a fixed set of attributes \cite{ebay2024}.
}

\changed{
We see the overview and the detail view as two different containers of different sets of attributes, and by making both the attributes and views accessible and manipulable, we can enable end-users to flexibly customize them.
Our formulation of the malleable overview-detail design pattern acts as an amplifier, allowing us to leverage all prior techniques for making attributes manipulable for the overview-detail pattern and making them generalizable beyond each of their originally intended scenarios and contexts.
Additionally, we also explore how AI can facilitate end-users in manipulating attributes in the overview-detail interface to achieve their diverse information needs, enabling users to prompt the interface to surface, hide, sort by, filter by, and select values in attributes.
}



% Our development for the overview-detail design pattern 
% to generate a rich set of interaction techniques
% generating a rich set of interaction techniques that can empower everyday users to customize all kinds of overview-detail interfaces, including ones that may not appear applicable.
% This also allows us to leverage all prior techniques for making attributes manipulable for the overview-detail design pattern, generating a rich set of interaction techniques that can empower everyday users to customize all kinds of overview-detail interfaces, including ones that may not appear applicable.


% \bryan{
% we demonstrate how prior techniques can be generalized beyond their originally intended scenario and context
% amplifier --. prior techniques
% }



% control how attributes and views are presented by prompting the interface.




% \changed{
% % By treating attributes as first-class citizens and
% % We share the perspective that by treating attributes as first-class citizens, we can enable users to easily and expressively create stuff.
% Our insight is that the overview and the detail view are two different containers of different sets of attributes, and by making both the attributes and views accessible and manipulable, we can enable end-users to flexibly customize them.
% We aggregate prior techniques for making attributes manipulable and leverage these techniques for the overview-detail design pattern. This enables us to explore how to empower everyday users to customize all kinds of overview-detail interfaces, including ones that may not appear applicable.
% For instance, this allows us to translate all overview-detail customization techniques in Airtable to overview-detail interfaces on shopping sites, maps, calendars, and even mobile devices.
% Additionally, we explore how end-users can manipulate attributes in the overview-detail interface with AI, enabling users to control how attributes and views are presented by prompting the interface.
% }
% By treating attributes as first-class citizens and
% We share the perspective that by treating attributes as first-class citizens, we can enable users to easily and expressively create stuff.


% For instance, this allows us to translate all overview-detail customization techniques in Airtable to overview-detail interfaces on shopping sites, maps, calendars, and even mobile devices.
% \bryan{Our goal with these two sections was to say: with 2.3 the design pattern lets you recognize the variations to make customizable, and with 2.4 the design pattern lets you easily translate customization techniques between any variation in design pattern.}

% \bryan{aggregate prior technique into overview detail. in addition, we leverage AI}
% \bryan{we share the perspective that .... can leverage these techniques into overview-detail.}
% \bryan{+ we have AI.}


% \changed{We aim to leverage manipulable attributes in interfaces similar to Haystack \cite{Karger2005HaystackSystem}, Airtable \cite{Airtable2024}, and Notion \cite{Notion2024}, all of which allow the end-user to choose which properties to show or hide in an overview of items.
% However, Fluid Attributes, which focuses on attribute manipulation in overview-detail interfaces, extends this interaction further than existing systems.
% First, users can ask to surface, filter and sort, and select items inside attributes by prompting the interface with AI (Section \ref{feature:ai-assisted-attributes}) and transform overview representations through selected attributes (Section \ref{feature:overview-representations}).
% Additionally, Fluid Attributes allows us to treat buttons and UI widgets as attributes in the overview-detail interface as well, enabling end-users to efficiently surface and hide these dynamic and interactive components across the interface (Section \ref{feature:ai-query-attributes}).
% }


% \bryan{notion, airtable}
% \bryan{compose queries in tables --> all database features have these}
% \bryan{spreadsheet surface and hide attribute but we aggregate these to all overview detail.}

% \bryan{we build upon extensive work}
% \bryan{don't want to do a feature comparison, it's overview-detail}



% Xia et al  which can allow users to compose new graphical styles and search for objects with shared attributes
% By decomposing graphics objects into attribute objects, these systems enable users to flexibly compose new graphical styles, search for graphical objects with attributes as filters, and create data visualizations by combining data and visual attribute objects as visual encodings. 


% Our focus on the overview-detail design pattern enables us to push attribute manipulation further than in existing systems, as 
% \bryan{We focus on ODIs, and we push attribute manipulation further for ODIs; This is fluid attributes.}
% However, we push attributes manipulation further than existing systems.
% However, our analysis of design space provides framework for exploring seamless transformation between its variations, enabling us to produce a set of interactions --- Fluid Attributes.
%  a framework for exploring how end-users can seamlessly transform between its variations
%  analysis of the design space of overview-detail interfaces,

% Our focus on the overview-detail design pattern enables us to push attribute manipulation further than ones in these systems, as our analysis of the design space informs 
% with our set of interactions in Fluid Attributes.
% Our set of interactions in Fluid Attributes
% aims to explore all the ways overview-detail attributes can be manipulated by the end-user. 
% how end-users can further manipulate their overview-detail interface with AI.

% Fluid Attributes pushes attribute manipulation further than ones in these systems, as we explore how end-users can further manipulate their overview-detail interface with AI. Specifically, users can ask to surface, filter and sort, and select items inside attributes by prompting the interface (see Section \ref{feature:ai-assisted-attributes}), transform overview representations through attributes (see Section \ref{feature:overview-representations}), and surface and hide dynamic and interactive attributes like buttons and image gallery UI components (see Section \ref{feature:ai-query-attributes}).}

% \changed{However, the core novelty of our paper lies not in the individual interaction techniques presented---some of which are novel---but in our demonstration of how these techniques can be generalized to the overview-detail design pattern.
% This enables us to explore the scope of which our techniques can be adopted and new design opportunities for these techniques, such as ways for the end-user easily invoke Fluid Attributes in different tasks (e.g., shopping, hotel booking, organizing emails) and different interface form-factors (e.g., desktop, mobile).}




% While these are effective in PIM and database-oriented interfaces, ...
% We 
% Prev section basically said: you're limited to how much you support cusotmization because you don't look at desgin pattern, there's a lack of guidance on what to customize
% so saying the same thing really won't provide any new perspectives. But you definitely should still say something about how design pattern is the important aspect.
% One thing I could try is that analyzing the design pattern not only helps us understand the scope of how applicable these customizations are in interfaces, but also helps us explore & generate novel interactions


==> versions/R_R/3_content_analysis.tex <==
\section{Content Analysis}
\label{section:content_analysis}

To better understand the various implementations of the overview-detail design pattern, we conducted a content analysis of overview-detail interfaces in desktop websites. Our content analysis was driven by the following questions:

\begin{enumerate}[label=\textbf{[Q\arabic*]}, leftmargin=*]
    \item What kinds of overview-detail interface arrangements exist in the wild?
    \item What types of information are presented in the overview and detail view, respectively?
    \item What aspects of overview-detail interfaces are already customizable by end-users?
\end{enumerate}

We present our findings with a design space of three dimensions of variations in overview-detail interfaces (\textbf{Q1}, \textbf{Q2}) and report existing customizability options found in our collection of websites (\textbf{Q3}).


\subsection{Methods}

\subsubsection{Data Collection}

The goal of our data collection was to collect a diverse and representative set of overview-detail interfaces that people regularly use. We initially collected the top 50 highest traffic websites in the United States based on data reported by Similarweb\footnote{\href{http://similarweb.com/}{http://similarweb.com/}. Accessed June 2024.}, a web analytics platform. However, as we analyzed this collection, we realized there were many common websites that were not included, such as flight booking or restaurant websites. To diversify our collection, we expanded to three more sources: 1) top 5 highest traffic websites in each of 33 web service categories\footnote{List of 33 categories listed by Semrush in Appendix \ref{appendix:semrush-categories}.} listed by Semrush\footnote{\href{https://www.semrush.com/website/top/united-states/all/}{https://www.semrush.com/website/top/united-states/all/}. Data last updated May 2024. Accessed July 2024.}, another web analytics platform, 2) 20 randomly sampled websites from Wordpress’ showcase page to observe non-corporate websites such as blogs\footnote{ \href{https://wordpress.org/showcase/archives/}{https://wordpress.org/showcase/archives/}. Accessed July 2024.}, and 3) 20 randomly sampled websites from Awwwards’ gallery of ``2024 Sites of the Year'' to observe favorite designs from the UI/UX design community\footnote{ \href{https://www.awwwards.com/websites/sites_of_the_year/}{https://www.awwwards.com/websites/sites\_of\_the\_year/}. Accessed July 2024.}. After filtering our list (e.g., removing duplicates), our final sample consisted of 156 websites.
The first author examined all 156 websites, identifying 303 instances of overview-detail interfaces. Some websites featured multiple overviews linked to one detail view, or vice versa. For coding purposes, we defined each instance as a single overview-to-detail relationship. Thus, interfaces with multiple connections were recorded as separate instances.

\subsubsection{Coding Procedure}

We developed a codebook of overview-detail interfaces through an iterative open coding process involving collaboration among the first three authors. In the first round of open coding, we randomly selected 20 overview-detail instances from our dataset of 303, and the first three authors individually analyzed all 20 instances. The coders discussed and clustered their categories together to develop an initial codebook. In the next round, the first two authors independently coded a second sample of 20 instances, achieving an inter-rater reliability of 94.8\% agreement between the codes, measured by Cohen’s kappa. They discussed the remaining differences and revised the dimensions to reach a consensus. Given the high agreement rate, the authors determined that it was sufficient for the second author to complete the remaining coding, continuing to code in random samples of 20. After each round, the first two authors reviewed and discussed new potential dimensions and variations, revising the codebook as necessary. This process was repeated four times, stopping when no new dimensions or variations were found in the last three stages. In total, the authors analyzed 120 overview-detail instances.


\subsection{Design Space}

Our design space presents variations of overview-detail interfaces found from the content analysis, particularly in the arrangement of overviews and detail views and the types of information presented in them. Our design space covers the following three dimensions. We describe notable cases found from the three dimensions and present the full design space in Figure \ref{fig:design-space}.
\begin{itemize}
    \item \textit{\textbf{Content}} describes whether information is presented in the overview, the detail view, or both, and how the attributes in the overview are abstracted from those in the detail view.
    \item \textit{\textbf{Composition}} describes how the multiple overviews and detail views are connected together
    \item \textit{\textbf{Layout}} describes the spatial arrangement of overview and detail views within the interface.
\end{itemize}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/3_content_analysis/design-space.png}
    \caption{Design space of overview-detail interfaces on the Web: Content, Composition, and Layout.}
    \label{fig:design-space}
    \Description{This image provides a detailed breakdown of the design space of overview-detail interfaces used on the web, broken into three categories: Content, Composition, and Layout. Here's the description of each section: First, we begin with the Content dimension. The following subsections describe where a particular attribute is shown: In Detail view only: Represents scenarios where certain attributes are only visible in the detailed view. In Overview only: Attributes visible solely in the overview. In both views: Attributes visible in both overview and detail views. There are also several Overview Abstractions: Visual: Attributes like Style and Graphic can either be available or unavailable. Semantic: Attributes related to meanings like Summary or Category can be abstracted, such as a rating summary or topic labels. Computational: Attributes like Ranking/Order, Sum/Average, or Minimum/Maximum are shown through numerical abstractions. Next, we move onto the composition dimension. These Composed relationships include the following; One-to-one: One overview leads to one detail view. Many-to-one: Multiple overview points lead to one detail view. One-to-many: A single overview leads to multiple detail views. Composition also covers the following recursion: Overview inside Detail view: A recursive structure where an overview is composed with the detailed view. Detail views in between: Multiple detail views between overviews, often in a preview or hierarchical informational structure. Finally, we also have our Layout dimension. The Overview-Detail Layouts can New page: Clicking the overview opens the detailed view in a new page. Side-by-side: Overview and detail views appear next to each other. In-place: A dropdown or a replacement of content occurs in the same space. Under Overview: Detail appears under the overview via table of contents or side menu. Above Overview: Detail appears via pop-up, pop-over, tooltip, or picture-in-picture. The Overview itself can be displayed as a List, Grid, Table, Spatial map, Hierarchy, or Timeline. Lastly, the Detail Layout is highly variable, but can either show one view at a time or many at a time.}
\end{figure}

\subsubsection{Content}
Throughout our content analysis, we realized that some attributes were displayed only in the overview, some were displayed only in the detail view, and some were displayed in both views. For example, the search results interface for job openings on Indeed showed job titles, company names, and salary ranges in both views, while the overview omitted attributes like qualifications or benefits (Fig. \ref{fig:content-dimension}A).
Although we initially coded attributes as static information elements, we also observed this pattern in interactive elements, such as `Save' buttons, text fields, and menus, with some sites including them in both the overview and detail views (Fig. \ref{fig:content-dimension}C), while others displayed them only in the detail view (Fig. \ref{fig:content-dimension}D).
Moving forward, we considered interactive elements to be attributes as well.
We also found instances in rental and housing platforms where the overview primarily presented prices for each place as pins on a map, but in Zillow, if a place had more than one unit available, the pin displayed the number of units available instead (Fig. \ref{fig:content-dimension}B).
In text-heavy overview-detail interfaces such as messaging apps and online discussion forums, we noticed long blocks of text in the overview were either cut short via ellipses (Fig. \ref{fig:content-dimension}E) or a fade-out gradient (Fig. \ref{fig:content-dimension}F).

We further found that some attributes in the overview served as an abstraction of information in the detail view. We identified three forms.
First, we found visual abstractions, which were encoded into the style and visuals of the item. For instance, Ticketmaster used color shading to indicate the number of seats available per section, with sections that had more seats shown in a saturated blue, while sections with fewer seats appeared in lighter shades.
Second, we found semantic abstractions that represented the contents in the detail view with summaries or categories. For instance, ChatGPT's conversation interface generated a title that represented each conversation.
Lastly, we found computational abstractions that computed attributes from the detail view into a value. For instance, Southwest's website presents a calendar view of the cheapest flight prices for each day.

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{figures/3_content_analysis/content-dimension.png}
    \caption{Example variations in the content dimension. (A) Indeed displays the attributes job title, company, location, and salary in both the overview and detail view. (B) Zillow's overview map presents different detail attributes (price or number of units) depending on whether a housing location has multiple units. (C) eBay provides the ``Add to Watchlist'' in both the overview and detail view. (D) Other sites, such as Etsy, only provides this button in the detail view. Long blocks of text tend to be cut off in overviews via (E) eclipses as shown in Gmail or via (F) a fade out gradient as shown in Quora.}
    \label{fig:content-dimension}

    \Description{This image contains six panels labeled A through F, each demonstrating variations in how content is handled in overview-detail interfaces across different websites or apps: A) An image of Indeed's job listings interface. Both the overview and detail\textbf{ }view display attributes of job title, company, location, and salary. B) A Zillow map showing properties. Depending on the number of units available, the overview displays different attributes like the price or number of units available. C) EBay's "Add to Watchlist" button is available in both the overview and detail views of product listings. D) Unlike eBay, Etsy shows the "Add to Favorites" option only in the detail view, not in the overview of product listings. E) Long blocks of text in Gmail's overview are truncated with ellipses (three dots), so the user has to open the detail view to see the full message. F) Here, long text is truncated in Quora's overview using a fade-out gradient instead of ellipses, prompting users to click to read more. Each panel shows different strategies for handling content visibility across overview and detail interfaces, highlighting where users see certain attributes.}
\end{figure}


\subsubsection{Composition}
During our analysis, we identified several overview-detail interfaces where multiple instances were composed together.

First, we found overview-detail relationships beyond just one-to-one. Many-to-one relationships presented multiple overviews in forms such as a list overview and a map overview presented side-by-side (Fig. \ref{fig:composition-dimension}A) or different scopes such as a five-day list (Fig. \ref{fig:composition-dimension}B) and a 30-day calendar (Fig. \ref{fig:composition-dimension}C). We also found some instances synchronized navigation across the many overviews, where selecting an item in one would trigger the navigation of another to the corresponding item.

Second, we found instances of recursion---overview-detail interfaces nested within each other. 
For instance, additional overviews such as a list of articles appeared in the detail view of New York Times (Fig. \ref{fig:composition-dimension}D). 
% We also found overview-detail interfaces that presented another overview inside the detail view, such as a hierarchical information organization on Fandom.com (Fig. X). 
This finding aligns with prior research that recognized the variation of nested overview-detail views in hierarchical menu interfaces \cite{Seffah2015PatternsOH, Cockburn2009OverviewDetailReview}.
An additional variation found were cases of ``intermediate'' detail views, which a link or button inside a detail view opened a detail view containing more or all attributes of the item. One of these variations was found in Discord's list of users in a server, where clicking on a user opened a small tooltip profile card, and clicking on the profile picture inside it opened a full-screen popup, revealing further details about mutual friends and servers (Fig. \ref{fig:composition-dimension}E).


\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{figures/3_content_analysis/composition-dimension.png}
    \caption{Example variations of the composition dimension. (A) Zillow shows a view composed of two overviews---a grid (left) and a map (right). The Southwest booking interface allows users access flight information from both (B) the 5-day table view and (C) the 30-day calendar view. (D) New York Times nests an overview inside a detail view with suggested articles. (F) Discord shows an intermediate detail view of the user profile as a tooltip, which can be expanded to show the full detail view as a pop-up.}
    \label{fig:composition-dimension}
\Description{The figure shows various examples of user interface compositions from different websites and applications. It's labeled A through E, each representing a different interface example: A) Zillow: This section shows a real estate listing interface with two parts - a grid view on the left showing property details and images, and a map view on the right displaying the locations. B) Southwest Airlines: This shows a flight booking interface with a 5-day table view of flight options, prices, and times. C) Also Southwest Airlines: This displays a 30-day calendar view of flight prices, allowing users to see price trends over a month. D) New York Times: This section shows an article view with suggested related articles nested within it. E) Discord: This displays a user profile interface, showing how a tooltip with intermediate details can be expanded into a full detail view. The image is meant to illustrate different ways that interfaces can be composed to show varying levels of detail and different views of information.}
    
\end{figure}

\subsubsection{Layout}
Our analysis revealed variations in the arrangement of overviews and detail views, the organization of items within overviews, and the number of items displayed in detail views.

\textbf{Overview-Detail}: First, we observed variations in overview-detail layout, with some websites arranging overviews and detail views side by side, while others opened detail views in a pop up or a dropdown.

\textbf{Overview}: We also observed variations of overview layout in the forms of lists, grids, and tables. Notable variations also included visualizations that plotted points that could be opened into detail (Fig. \ref{fig:layout-dimension}A) and sports stadiums to select seating sections (Fig. \ref{fig:layout-dimension}B).

\textbf{Detail}: We observed that detail views varied by how many were displayed at a time. Some instances only opened one detail view at a time, while others allowed users to open many at a time. For instance, ESPN allowed only one dropdown to be open at a time (Fig. \ref{fig:layout-dimension}C), while weather.com supported multiple (Fig. \ref{fig:layout-dimension}D).

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{figures/3_content_analysis/layout-dimension.png}
    \caption{Example variations in the layout dimension. (A) MLB’s player profile page maps batting points onto the baseball field; clicking a plot point opens a detail view of a video replay of the point. (B) Ticketmaster’s seating selection page also shows a map overview; when a particular seating section is selected, the overview list changes to match the corresponding section. (C) ESPN shows each player's stats in a game, which can be opened as a dropdown. (D) Weather.com uses a similar dropdown layout, but unlike ESPN, multiple detail views can be opened simultaneously.}
    \label{fig:layout-dimension}

\Description{This image illustrates different variations in layout design for various sports and weather-related websites. The image is divided into four sections, labeled A through D: A) MLB (Major League Baseball) Player Profile: This section shows a baseball field diagram with colored dots representing batting points. There's an arrow pointing to a larger image, which appears to be a video replay of a specific play. The concept here is that users can click on a dot to see a detailed view of that particular play. B) Ticketmaster Seating Selection: This displays a stadium seating chart on the right side. On the left, there's a list of available seats with prices. The idea is that when a user selects a section on the map, the list updates to show seats in that section. C) ESPN Player Statistics: This section shows a baseball field diagram in the center, surrounded by player statistics in a table format. There's a highlighted area suggesting that certain statistics can be expanded into a dropdown for more detailed information. D) Weather.com Forecast: This displays a daily weather forecast with multiple time slots. Each time slot shows temperature and weather conditions. The layout is similar to the ESPN dropdown, but the caption notes that multiple detailed views can be open simultaneously.}
    
\end{figure}


\subsection{Existing Customizability Features}

In addition to the previously mentioned dimensions, we separately collected and coded existing customizability features for overview-detail interfaces. We found 8.33\% (13/156) of websites provided customizations for overview-detail interfaces, with 2.56\% (4/156) providing content customization, 0\% (0/156) providing composition customization, and 7.69\% (12/156) providing layout customization. All of the instances we collected were limited in customization, with the most providing eight layout variations.

We found Craigslist offered the most variations for customizing the overview-detail interface, with five options for customizing the overview layout and three for the overview-detail layout. The choice of layout also indirectly influenced which attributes were displayed. For example, the grid view included an image thumbnail, while the list view did not, likely to maintain a more compact item presentation. In the content dimension, we observed four websites that allowed users to customize which content attributes they wanted to view. Among these, eBay offered the most customization options, though it only allowed users to toggle six attributes.


\subsection{Summary}
In summary, our content analysis of 303 overview-detail instances in 156 websites identified three dimensions of variation: content, composition, and layout. Additionally, we found that only 8.33\% (13/156) of websites in our collection supported customization features, with those offering only limited options. Our collection of samples may not be fully representative of the entire set of information systems, and we may not have captured every instance of overview-detail interfaces within each sample. Thus, we do not claim the comprehensiveness of our design space and the frequencies of customizability features beyond our collection. Nevertheless, our analysis does provide insights into variations in real-world examples, offering contributions in understanding overview-detail interfaces.



















% --- DUMP ---
% In addition to the previously mentioned dimensions, we separately collected and coded existing customizability features for overview-detail interfaces, observing the kinds of customizability options websites provided and how these options aligned with the three dimensions identified.

% In the Content dimension, we observed four websites that allowed users to customize which content attributes they wished to see. Among them, Ebay has the most content customization options, allowing users to choose between six overview detail attributes that can be checked to view or checked off to hide. Other sites have more limited options to either hide certain attributes, reorder attributes, or choose between attribute types (still image or video) in the overview. 

% Regarding the Layout dimension, we observed twelve websites with such customizations options. 

% Each of these twelve sites included some level of overview layout customization, a majority of which were shopping and booking interfaces that offer options to transform the overview between list, grid, and/or table view. Interestingly, two social media sites offered additional overview layout customizations – one allowed users to choose how compact their list was, another offered a selection between a staggered grid and an organized grid.  

% There were only three websites that provided some level of overview-detail layout customization – two were variations of the “separate page” category but allowed users to choose between opening detail views in the same tab or a new tab. Among them, we found Craigslist to have the most layout customizations with a total of five different options for customizing the overview layout and three different options for customizing overview-detail layouts (Fig. X). Customizing the layout of their interface also affected which attributes were shown. For instance, a grid view provided an image thumbnail, while the list view did not---perhaps to maintain a compact view of the items 



% * We looked, we found X\% of our websites OD from had OD customizations (content: X\%; composition: X\%; layout: X\%)
% * Craigslist... 
% * End with talking about content is preselected attributes -> ebay. 



% Finally, we did not observe any composition customizability options within our sample set of 303 – though we acknowledge that there are likely some sites that utilize this. 



% Among the many websites, we found Craigslist to have the most options for customizing the layout of overviews and detail views with seven different options (Fig. X). Customizing the layout of their interface also affects which attributes were shown. For instance, a grid view provided an image thumbnail, while the list view did not---perhaps to maintain a compact view of the items.
% From our collection of 303 overview-detail interfaces, the only site to directly provide options to customize which detail to show in the overview was eBay (Fig. X). X\%
% However, options were limited to only a few details and provided options in a separate settings panel.




% <this booking site> provided filtering features on results, which upon applying a filter, would reveal the value  of that attribute for each item (Fig. X) (filtering for reviews would show the review count and review rating details)
% found a setting for presenting the results in a list or a gird. We  a small list of attributes to show in the search results page for each item. They show a set of attributes, but there were still many attributes in the details that the website did not allow the user to show in the overview.
% \bryan{Move this section before the design space summary section, but how to talk about customizations frequency by dimension if you haven't even introduced what the dimensions are? (Minor thing, but also this is Q3, not Q1-2, so you want to switch that order as well. You can first try moving it forward and try to talk about customization features without dimensions specifically?}

% \subsection{Limitations}
% It may be possible that we did not collect all overview-detail instances that exist on each single website---human error.
% Our collection of websites are also not representative of all websites in the internet.


==> versions/R_R/4_interaction_techniques.tex <==
\section{Interaction Techniques for Malleable Overview-Detail Interfaces}
\label{section:interaction_techniques}

In this section, we describe interaction techniques to customize overview-detail interfaces along the three dimensions identified from our content analysis.

% The goal of this section is not to provide ways to turn any overview-detail interface into any other, but rather to explore the interaction techniques that provides the end-user ways to transform the overview-detail interface to best suit their needs. 
% \bryan{Don't say this as a limitation, and we don't do things. Rather, just simply justify why you ended up doing these specific dimensions}


\subsection{Content}
\label{interaction-dimension:content}
To customize overview-detail interfaces along the content dimension, we introduce Fluid Attributes, a \changed{set of} interaction techniques that allows end-users to directly interact with detail attributes in the overview-detail interface. This enables users to control what, where, and how detail attributes are shown as well as directly sort and filter by attributes. Fluid Attributes also unlocks further customizations of the overview-detail interface when paired with generative AI tools by allowing users to query for attributes, generate new ones, and reformat inconsistent attributes. To support such interactions, overview-detail interfaces can provide a dedicated ``Attributes Mode'' available to toggle on and off in a global toolbar on the website \changed{(Fig. \ref{fig:probe-shopping}D)}. Upon toggling on, the website highlights all attributes in the overview-detail interface. Users can then select and perform actions on the attributes.

% Of the many ways \technique can be implemented, such as area selection, a context menu option, or a website-wide toggle, we implemented a website-wide toggle called ``Attributes Mode'', which upon toggling, highlighted all attributes in the interface. This made \technique interactions more visually salient to the reader. \bryan{This design choice is not for the readers; it's for the end-user. Introduce this design choice properly, and justify it in terms of end-user benefits instead.}
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/4_interaction_techniques/surface-and-hide.png}
    \caption{Upon entering ``Attributes Mode'', (A) users can select attributes in the detail view to surface to the overview, and (B) hide selected attributes from the overview. \changed{Users can modify which attributes are shown and hidden through a context menu or by directly dragging selected attributes to their desired view.}}
    \label{fig:surface-and-hide}
    \Description{The figure shows five screenshots demonstrating how users might use the "Surfacing and Hiding Attributes" feature while shopping online for sofas. The first two images show a user selecting two attributes - the Year Manufactured and the Item Length - which the user surfaces. The third image shows the newly customized shopping overview - now with the selected attributes appearing alongside default attributes such as product name and price. The fourth image shows the user selecting the vendor's name and and hiding that attribute from the overview. The fifth image shows the final customized shopping overview - with two additional attributes surfaced and the vendor name hidden}
\end{figure}
\subsubsection{Surfacing and Hiding Attributes (Fig. \ref{fig:surface-and-hide})}
\label{feature:surface-hide-attributes}
In order to find details of items not shown in the overview, users must open the detail view to each individual item and locate the attribute in the interface. Fluid Attributes lets users select attributes from the detail view and directly surface them by clicking ``Surface'' (Fig. \ref{fig:surface-and-hide}A). The selected attributes then populate in every item of the overview. On the other hand, if users want to hide attributes they are not interested in seeing in the overview, they can instead ``Hide'' (Fig. \ref{fig:surface-and-hide}B) those attributes. In essence, this interaction gives users the control to \textit{get an overview of only the things they want} by manipulating attributes on their own, without the help from the developers. 
% Additionally, users can hover over an attribute to ephemerally reveal an attribute over each item.

Fluid Attributes is not only limited to static attributes but also include dynamic and interactive ones, such as widgets, buttons, and components. For instance, users can surface an image gallery component into the overview to view more images and even the \textit{Add to Wishlist} button for each item on a shopping interface.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/4_interaction_techniques/sort-and-filter.png}
    \caption{Since users can surface any attribute to the overview (1), this also gives them the ability to sort and filter by their values directly (2).
    This figure shows how a user might sort overview items via the selected attribute \textit{Year Manufactured}.}
    \label{fig:sort-and-filter}

    \Description{This figure shows how users can perform additional functions, such as sort and filter, upon any selected attribute. Since users can surface any attribute to the overview (1), this also gives them the ability to sort and filter by their values directly. Continuing with the online sofa shopping scenario, the user in the figure first surfaces the \textit{Year Manufactured} attribute, and then sorts the overview items via the selected attribute}
\end{figure}
\subsubsection{Sorting and Filtering with Attributes (Fig. \ref{fig:sort-and-filter})}
\label{feature:sort-filter-attributes}
Rather than relying on a predetermined set of sort and filter functionalities given by the interface, Fluid Attributes provides the opportunity to make any attribute sortable and filterable. Users can surface the \textit{Year Manufactured} attribute of a couch (Fig. \ref{fig:sort-and-filter}.1), then directly sort them by the latest manufactured year (Fig. \ref{fig:sort-and-filter}.2). Since Fluid Attributes also includes dynamic attributes, users can, for instance, sort by the boolean value associated with the \textit{Add to Wishlist} button to ``pin'' items to the top of the search results.

\subsubsection{AI-assisted Fluid Attributes}
\label{feature:ai-assisted-attributes}
Fluid Attributes, when assisted by AI's ability to process natural language queries to functionalities, demonstrates further interaction possibilities to customize the content in the overview-detail interface. \changed{Users can leverage AI through a prompt box provided by the interface.}
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/4_interaction_techniques/AI-queries.png}
    \caption{Users can additionally prompt AI to manipulate the attributes in the overview-detail interface. (A) Users can prompt AI to surface multiple attributes relating to the popularity of each product, (B) sort and filter for the values of a surfaced attribute, (C) and even surface specific values of attributes that contain multiple values.}
    \label{fig:AI-queries}

        \Description{This figure shows three instances of how the AI feature might be used to manipulate the attributes in the overview-detail interface while shopping online for sofas. The first image shows a use case in which a user prompts "how popular are these right now" -- which surfaces prompt AI to surface attributes relating to the popularity of each product. The second image depicts a use case in which a user wants to find the sofas that are linen textured -- prompting "give me the ones that are linen textured" to surface the upholstery fabric attribute, in which the user directly filters out non-linen options. In the third image, the user prompts "show me what the back looks like", which surfaces the Image Gallery attribute. From there, the user can select images that resemble the back of the sofa.}

\end{figure}

\paragraph{Fluid Attributes via Natural Language Queries (Fig. \ref{fig:AI-queries})}
\label{feature:ai-query-attributes}
% \Technique features can be made by AI as well.
In addition to being able to directly manipulate attributes to surface them in the overview, users can also query desired attributes with their own words instead of using names assigned by the developers and content providers.
% While user-directed \technique provides a mechanism to directly shuffle content in the overview-detail interface, there are still needs that are easiest to communicate to the interface with words. 
% We find that overview-detail interfaces can utilize AI to also map user prompts to operations (i.e., surface, hide, sort, filter).
For instance, if a user asks AI in a prompt box ``\textit{How popular are these items?}'', AI can identify the relevant attributes (i.e., \textit{Number of Watchers}, \textit{Items Sold}) and surface them to the overview (Fig. \ref{fig:AI-queries}A). This extends to the other operations in Fluid Attributes, such as adding a filter operation upon asking for ``only couches with a linen texture'' (Fig. \ref{fig:AI-queries}B). Additionally, users can ask to see ``the back of the couches'', which triggers AI to surface the \textit{Image Gallery} attribute and select images that present the back view of the couch (Fig. \ref{fig:AI-queries}C). If AI fails to show this image, the user can manually look through the images with the surfaced \textit{Image Gallery} component.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/4_interaction_techniques/AI-generated-attributes.png}
    \caption{(1) Users can also generate new attributes with AI, for instance by asking for the total cost of the item, which sums the values of the \textit{Price} and \textit{Shipping Fee} attributes. (2) They can hover over the value to view its source attributes, and (3) also drag them into the overview, (4) surfacing the source attribute alongside the newly generated one.}
    \label{fig:AI-generated-attributes}

        \Description{This figure shows how users can generate new attributes with AI, for instance by asking for the total cost of the item, which sums the values of the \textit{Price} and \textit{Shipping Fee} attributes as shown in the first image. In the second image, the user hovers over an item's Total Cost attribute to view its source attributes, and can also drag them into the overview. The final image shows the completed customization, with the newly generated attribute, total cost, alongside the source attribute, shipping fee.}

\end{figure}

\paragraph{Generating New Attributes (Fig. \ref{fig:AI-generated-attributes})}
\label{feature:ai-new-attributes}
AI is also suited to generate new attributes from user queries. Users can ask for an attribute that may require computing values for each item in the overview, For instance, if a user asks for the ``total cost'' of an item, AI can sum values of attributes such as \textit{Price} and \textit{Shipping Fee} (Fig. \ref{fig:AI-generated-attributes}.1). Users can hover over the newly generated attribute to reveal the source attributes the AI referenced (Fig. \ref{fig:AI-generated-attributes}.2), and then surface these sources as well (Fig. \ref{fig:AI-generated-attributes}.3-4). If AI cannot provide the value for an item, it responds ``Not Specified''.

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{figures/4_interaction_techniques/AI-reformatted-attributes.png}
    \caption{Many attributes of items in online marketplaces are often inconsistent in the format of the value and the attribute's name. (A) To address this, users can prompt AI to reformat the titles of items to make more consistent. (B) Additionally, surfacing attributes from items that do not contain them will trigger AI to search and fill in the missing values to that attribute. If not found, AI provides the value ``Not Specified''.}
    \label{fig:AI-reformatted-attributes}

        \Description{Many attributes of items in Ebay's online marketplaces are manually entered by vendors and are often inconsistent in their formatting. This figure shows how users can prompt AI to reformat the titles of items to make more consistent -- in this case the user prompts the AI tool to "just put the brand name and its condition" -- effectively replacing the product title with the brand name attribute and condition attribute.}

\end{figure}


% \paragraph{Reformatting and Filling Empty Attribute Values (Fig. \ref{fig:AI-reformatted-attributes})}
% \paragraph{Forming Consistent Attribute Values (Fig. \ref{fig:AI-reformatted-attributes})}
\paragraph{Establishing Consistent Attribute Values (Fig. \ref{fig:AI-reformatted-attributes})}
\label{feature:ai-reformat-attributes}
Many attributes of items in online marketplaces are not only set by developers but also by vendors. This results in a large case of inconsistent attributes and values, such as using different attribute labels, currencies, units, or title formats.
If users surface an attribute that is not found in a particular item, AI can scan through the item's data to identify the attribute from other sources (Fig. \ref{fig:AI-reformatted-attributes}B).
Users can also choose to reformat attributes upon prompting the interface to make inconsistent attribute values consistent across all items. For instance, users can either ask to simply ``make the titles consistent'' or make more precise changes and ask to ``show only the brand name and the couch's condition'', thereby making the title easier to read (Fig. \ref{fig:AI-reformatted-attributes}A).
% With AI-assisted \technique, end-users can reformat attributes upon prompting the interface, making attributes consistent across all items.


\subsection{Composition and Layout}
\label{interaction-dimension:composition-layout}

% To support transforming variations in layout and composition, m
\changed{
To customize layout and composition, malleable overview-detail interfaces can provide variations from the design space in Section \ref{section:content_analysis}.
% We offer default options that are most familiar to end-users from our design space t
To make transforming between such variations most familiar to end-users, we provide dropdown menus for overview and overview-detail layouts and tabbed views for multiple overviews (Fig. \ref{fig:overview-representations}A, Fig. \ref{fig:probe-shopping}).}
By implementing these familiar interaction techniques, we aim to keep the interface customizations end-user friendly.


\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/4_interaction_techniques/overview-representations.png}
    \caption{\changed{(A) Overview variations from the design space are available for the end-user through a dropdown menu.} Fluid Attributes \changed{additionally allows users} to invoke relevant overview representations through attributes. (\changed{B}) For instance, users can select the \textit{Price} and \textit{Vendor Feedback Score} attributes to plot items in a scatter plot, or (\changed{C}) generate a color value from the image to map items onto a color space.}
    \label{fig:overview-representations}

        \Description{This figure demonstrates how the overviews can be transformed into multiple representations with attributes. In the first image, a user selects "scatter plot" - and is able to view each overview item in a scatter plot plotted along two selected attributes as axis. The second image shows the overview items mapped onto a color space, based on a color value generated from the image.}

\end{figure}


% \subsubsection{Transforming Overview Representations with Attributes (Fig. \ref{fig:overview-representations})}
\label{feature:overview-representations}

\changed{However, other overview-detail systems may support a greater variety of overview representations to meet diverse needs, which, when listed in a dropdown menu, can become large and overwhelming for the user. We recognize that attributes are closely associated with their overview representations, as they are mapped to specific visual elements or data points within the overview.
Fluid Attributes leverages this property by enabling users to select desired properties and reveal relevant overviews in various representations.}
% Just as a map places location pins using their latitude and longitude values, other detail attributes can entail different representations best suited for their contexts.
For instance, users can select the \textit{Price} and \textit{Vendor Feedback Score} attributes to view items in a scatter plot to consider the reliability of the vendors while comparing prices (Fig. \ref{fig:overview-representations}\changed{B}).
Users also can generate a color attribute from the item image to map items onto \changed{spatial overviews such as} a color space, allowing users to cluster and explore items by color\changed{, similar to Histomages \cite{Chevalier2012Histomages}} (Fig. \ref{fig:overview-representations}\changed{C}). 
\changed{A scatter plot and color space are just two examples of overviews; other malleable overview-detail interfaces can offer additional representations and even more nuanced variations of scatter plots and color spaces. Instead of aiming to provide all possible overview representations, our goal is to offer a solution that allows users to intuitively and flexibly modify how their overview is represented.}

% \changed{A scatter plot and color space are only two example overviews, and other malleable overview-detail interfaces can further provide more overview representations and even nuanced variations of scatter plots and color spaces.
% Our goal is not to provide all possible overview representations, but to provide a solution for users to intuitively and flexibly modify the representation of their overview.}
% Nevertheless, we provide a solution for achieving such transformations, offering users a flexible way to tailor their overview-detail interface.}



% Websites implementing malleable overview-detail interfaces can further explore additional overview variations---from ones that support many attribute types (e.g., scatter plot) to ones that support specific attribute types (e.g., color values for a color space, location values for a map).



% \bryan{Get rid of this section. Just motivate composition and layout, how they can be transformed, and further customized with \technique}
% We explored various techniques to support users in customizing the composition and layout of overviews and detail views. We explored how dragging the overview and detail views to different areas in the interface could determine whether the interface shows a side-by-side view, a popup, a tooltip, and more. We also explored how resizing the overview and detail view components into different shapes and sizes could transform lists into tables, tables into grids, and more. However, we deemed the most intuitive way to switch between various forms of layout was to simply use dropdown menus. Similarly for composition, we found it was most familiar for us to manage multiple overviews with a list of tabs. Thus, rather than focusing on the customization techniques for these dimensions, we highlight how different configurations of layout and composition can support various information tasks.


% transform overview based on attributes
% --> this also brings back attributes


% \haijun{using AI to reformat detail -- title}

% \bryan{• Prompt to find properties, fill in properties that aren't formatted consistently}
% \bryan{X Prompt to pull multiple properties, sort properties}
% \bryan{X Control images. "Give me the side-profile of the monitors"}
% \bryan{X Generate new properties. Flight booking. List of flights for a single day. Ask AI for cheapest flight price and its departure time. Pull this cheapest flight price and departure time to the calendar of days.}
% \bryan{• Transform the title attribute "Format this title"}


% \bryan{• Pull, hide, sort/filter details in a standard OD interface, also pull image gallery}
% \bryan{• Pull details through semantic zoom}
% \bryan{• Shopping interface turned into a Kanban board. Pull buttons to the overview. You can even sort by the button itself, whether the item was added or not}
% \bryan{X VSCode IDE: Pull more details to the minimap scrollbar... I want to connect OD to scrollbar to read wear & edit wear... somehow}

% first ask for an attribute that requires complex computation or transformation of existing attributes. For instance, if a user asks for the ``cheapest price for afternoon flights'' from a list of flight tickets for each day of the week, AI can identify all prices with departure times in the afternoon and return the minimum value with a new attribute called \textit{Cheapest Price} (Fig. \ref{fig:AI-generated-attributes}a). Users can then surface this newly generated attribute to the overview, propagating the action of finding the cheapest afternoon flight price across the remaining available days (Fig. \ref{fig:AI-generated-attributes}b).

% \bryan{AI can make errors. So we also make it clear which attributes are AI generated and which are not --> showing the sources, etc}



% Second, attributes in online platforms such as e-commerce marketplaces may not be consistent across items; perhaps the \textit{Screen Size} attribute for a monitor may be called \textit{Display Size} for another, and the \textit{Screen Size} attribute may even be hidden in a long text description. To address this, AI can identify the value of what would be the \textit{Screen Size} attribute from each item and surface that value (Fig. Xb). If AI finds the value, it can additionally reference existing attributes it sourced from. Otherwise, AI can provide a response such as ``Not Specified''.


% filling in empty details across items
% Generate new properties for items --> populate in boths views
% Generate new properties across all times in overview (cheapest price across all items)

% detail, attribute

% Not only is surfacing attributes valuable for 
% New attributes surfaced in the overview can then be sorted and filtered. For instance, users can select the X attribute, and sort it low to high. Upon encountering a ``new'' label on an item, users can filter all items that are new.
% Other components then may also be sortable and filterable. The ``Add to cart'' button can sort by its boolean value---whether the item was added to the cart or not. This may be used to sink the items that were already added to the cart to the bottom of the list.
% This includes numerical attributes such as number of items sold or text values such as the brand name.
% Numerical values can be sorted numerically and text can be sorted alphabetically.
% This also includes buttons---sorting the button attribute can sort alphabetically, but sorting the ``Add to cart'' button can sort by its boolean value---whether the item was added to the cart or not. This may be used to sink the items that were already added to the cart to the bottom of the list.

% This statement below... it's less related to the whole section
% While we do not provide a solution for creating any representations flexibly and ad hoc, \technique provides 1) a unified mechanism to spawn these diverse representations and 2) a unified endpoint for externally developed overview representations to interoperate with malleable overview-detail interfaces.

% \Technique makes overview-detail interfaces easily interoperable with other representations. 

% I want to say, transformable representations with attributes makes it extremely easy to change the order of information.
% On a table, you drag the column to reorder, so you can see certain criteria closer together -- This allows you to compare items much easier.
% This action translates and synchronizes to other representations, such as dragging X column will also drag that attribute to the top in the list view.

% @HAIJUN
% I removed the subsubsection about syncrhonizing attributes across views becase I realized \technique is ALL about synchronization! syncrhonization across overview and detail and synthonization across items in the overview.
% Also, the usability of the scroll individual cards to show the selection wasn't very practical when testing it out

% \subsubsection{Peeking at Attributes}
% \Technique also makes it easy to peek at attributes across items. Hovering over an attribute in the detail view will temporarily lift that attribute for all other items.
% \bryan{I realized scrolling through views doesn't really work that well in terms of usability. Maybe i can bring it back for the video.}
% \subsubsection{Peeking and Navigating to Attributes}
% You can hover over an attribute for an item, and it will reveal this attribute for all other items---as a non-committal way of seeing the other items.
% If an interface makes individual items scrollable
% Since \technique  applies interactions with attributes across all items, users can leverage this property to synchronize the view of each item.
% Hover over a detail, this shows on all other items in overview

% \haijun{• hovering on details in a detail view to review details of items in the master view}
 % Click will scroll to that detail  (navigation technique)

% DIFFERENT REPRESENTATIONS VIA ATTRIBUTES
% Color Picker 

% Integrating AI into interfaces to fetch information across different pages can become cumbersome, especially when the data is unstructured. \Technique gives AI a really nice structured space to work in, 




% We should say, supporting various tasks with various interface options because pretty easy to achieve with thie malleable interface.


% \subsubsection{Multiple Overviews to Facilitate Organization (Fig. X)}
% \label{feature:many-overviews}
% Users can also utilize multiple overviews, especially for tasks that require multiple stages of consideration or evaluation, such as decision-making. By forming multiple overviews beside each other, one can move items between these views, each view possibly representing a tier list of items the user wants---similar to how a kanban board is used to manage multiple stages of tasks.\bryan{partition one's decision-making process into multiple filtering stages}




% \subsubsection{Creating Comparison Views with Multiple Detail Views (Fig. X)}
% \label{feature:comparison-views}
% % Comparing between items can be in decision-making
% Comparison views can be supported through the composition dimension of allowing users to create multiple detail views. Users can select items in the overview and open them into individual detail views to directly compare then side-by-side. 


% Creating multiple detail views to directly compare between these items. (This can also then be used as a specific collection in an overview, by forming a new overview from selected items)





% Leveraging multiple views for decision-making, saving information, organizing things better, etc.





% \subsubsection{Configuring Overviews and Detail views to Reduce Clutter}








% For managing various forms of composition, we find displaying
% \subsubsubsection{Dropdown Menus} switch among list, table, grid
% \subsubsubsection{Control Panels} create new overview, manage

% \subsubsection{Supporting Information Tasks with Different Configurations}


% in the follwoing, we talk about different configurations and what tasks they can support

% \subsubsubsection{Creating multiple overviews to facilitate Organization}


% \subsubsubsection{Configuring Overview and Detail to Reduce Clutter}


% \subsubsubsection{Creating Comparison Views}of tasks they support --> the higher level task they can support




% finding distance?


% look at mesh, what kinds 

% using This subdimension


% shopping new p-->copies over
% map search results --> in one map

% Detail view layout --> you see multiple items at once scroll through

% shopping item --> item, item 1, 2,3,4

% other view




% \bryan{"•" Means it's already developed. "X" means not yet.}
% \subsection{Menus and Tabs}
% \bryan{• Customize the entire layout dimension}
% \bryan{• Customize number of overviews (composition sub-dimension)}
% \bryan{X Google Scholar scenario: List of citations (outer list). Open one of the paper's list of citations as well (inner list). Connect the inner list out with the outer list. Hierarchical dropdown menu of citations}

% \subsection{Direct Manipulation}
% \bryan{X Dragging items out of overview to create detail view of that item to compare side-by-side}
% \bryan{X Reorder the list of many overviews}
% \bryan{X Start in List view. Change the order of table view columns. Re-ordering also applies to List view}


% % End Section.
% % Here are my reasoning for this structure & more thoughts:
% \bryan{thought 1, thought 2}


==> versions/R_R/5_applications.tex <==
\section{\changed{Applications of Malleable Overview-Detail Interfaces}}
\label{section:applications}

\changed{To demonstrate the generalizability of our presented customization techniques, we developed five overview-detail interfaces for various contexts and platforms: online shopping, booking a hotel, managing emails, reading live articles, and ordering food on a mobile app. We developed the shopping and booking websites with higher fidelity than the others to use them for design probes in our user study. These two probes are described in more detail in Section \ref{subsection:design-probes}.}

\subsection{Scenarios}

\subsubsection{Online Shopping (Fig. \ref{fig:probe-shopping})}

\changed{Online shopping websites commonly present a search result of items as a list overview with predefined attributes, including a thumbnail of each item and a button to add the item to the shopping cart (Fig. \ref{fig:probe-shopping}A), and a full view of the details in a new page (Fig. \ref{fig:probe-shopping}B). However, this default requires users to repeatedly switch between both views. A malleable overview-detail interface can provide a toolbar UI which presents options for the user to instead open detail views side-by-side or in-place with a dropdown (Fig. \ref{fig:probe-shopping}C). Users can additionally add more overviews to save items in different collections (Fig. \ref{fig:probe-shopping}D).
This can be used to compare sets of choices such as combinations of camera bodies and camera lenses to purchase. 
Furthermore, users can surface attributes in the overview by toggling on ``Attributes Mode'' to manipulate attributes in the interface (Fig. \ref{fig:probe-shopping}D).}
% \subsection{Workflow 1: Shopping for Camera Lenses}
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/6_design_probes/design-probes-shopping.png}
    \caption{A screenshot of the shopping design probe, displaying \changed{(A) the overview list and (B) the detail view opened in separate pages. (C) Overview layout can be customized through a dropdown menu in the corner of each overview. (D) The toolbar provides customizations for the overview-detail, including adding and opening multiple overviews, changing overview-detail layout, and customizing attributes.}}
    \label{fig:probe-shopping}

        \Description{This figure displays a screenshot of our shopping design probe. The shopping overview is shown on the left in a list layout, and a product detail view is shown on the right, opened as a new page.}

\end{figure}


\subsubsection{Booking Hotels (Fig. \ref{fig:probe-booking})}

\changed{Interfaces such as hotel booking, home rental, and apartment search websites often provide a list view alongside a map view (Fig. \ref{fig:probe-booking}A and B) to provide rich spatial information. However, the map often only presents zero or one attribute for each location, with the only way to view these details is to click on the pin one at a time (Fig. \ref{fig:probe-booking}C). Instead, a malleable overview-detail interface can enable the user to surface more details into the map, such as rating, ranking, and amenities (Fig. \ref{fig:probe-booking}D). Additionally, the user may customize different attributes for different overviews to leverage the benefits and affordances each overview representation provides. For instance, users can surface details about the number of reviewers in the map view to gauge which areas might be more popular (Fig. \ref{fig:probe-booking}E), while they can surface details about amenities in the list view to easily sift through preferences by scrolling.}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/6_design_probes/design-probes-booking.png}
    \caption{A screenshot of our hotel booking design probe, \changed{displaying (A) an overview list of bookmarked hotels and (B) an overview map presenting locations as pins. (C) A detail view of a selected hotel is opened as a popover left of the map. (D) The toolbar presents a way for users to jump between different searched locations and customize attributes. \changed{(E) Surfaced attributes on the map populates the pin.}}}
\label{fig:probe-booking}

    \Description{The figure shows a screenshot of the hotel booking design probe, displaying an overview map of La Jolla on the right and a overview list of bookmarked hotels on the left. A detail view of a selected hotel is opened as a popover left of the map.}

\end{figure}


\subsubsection{Reading and Managing Emails (Fig. \ref{fig:application-email})}
\changed{Oftentimes, emails contain important details in the text of their messages such as a response deadline. However, foraging through a large inbox for these details can grow extremely tedious.} Using AI-assisted Fluid Attributes, users can prompt the interface to generate an attribute \textit{Response Deadline} (Fig. \ref{fig:application-email}A), surface it in the overview, and sort the emails by upcoming deadlines (Fig. \ref{fig:application-email}B).
\changed{Users can also choose to open emails in-place rather than side-by-side or on a new page, allowing them to fully read through important ones and quickly glance at less important ones.}

% finding this specific detail across emails is tedious to find manually.'
% \changed{Upon opening an email, they can also choose to open many at a time, allowing them to scroll through their list of emails without navigating back to the overview}

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{figures/5_applications/application-email.png}
    \caption{(A) Users can prompt AI to sort by emails with the most urgent deadlines. (B) Upon doing so, the attribute \textit{Response Deadline} is surfaced and sorted by latest date.}
    \label{fig:application-email}

        \Description{This figure depicts an email inbox as a list overview. The user prompts AI for "most urgent emails to respond to", which surfaces a newly generated attribute called deadlines.}

\end{figure}

% \subsubsection{\changed{Calendar}}
% Calendar applications provide multiple forms of overviews that are scoped by time (e.g., day, week, month, year). 
% Open a month overview, then through that, open two day overviews, two weeks apart. Create an event on the first day at specifically at some time, then drag the end of the event to say it ends on this day, but then drag it through this overview and into the next day's view. This makes the even extend through those two days, but also at the same time allowing you specify the end time of the event.

% Basically, I'm trying to select objects across two overviews... and then maybe surface details through that?

% 
% In a single day view, you can choose to prioritize certain details about events over others, such as to view which events are remote and which are in-person.
% One could also zoom out to see in the week view, which days are fully remote and which days have in-person meetings.
% One could zoom out even further to the month and year views to surface events they may want to prioritize over others, such as if they want to view how many meetings there are for each day, and how many of those meetings are remote and how many are in-person.
% This application demonstrates how a customizable overview-detail interface with multiple overview representations connected by time can be linked across each other.

\subsubsection{Reading Live Articles (Fig. \ref{fig:application-live-article})}
Live news articles report on long-standing events such as presidential elections and sports games. These interfaces appear to aggregate shorter articles in a scrollable stack (Fig. \ref{fig:application-live-article}A). However, it can be challenging for users joining in the middle of the event to quickly catch up on the timeline with a long document. To address this, users can select the \textit{Published Date} attribute and bind it to a timeline overview, organizing all articles into a timeline. Users can also select which details to show in the timeline before diving into individual articles (Fig. \ref{fig:application-live-article}B).

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{figures/5_applications/applications-live-article.png}
    \caption{\changed{(A) Instead of scrolling through a long list of live updates, users can gain a broader overview of the event by selecting the \textit{Published Date} attribute and transforming the layout from a list to a timeline. (B) Users can additionally generate a \textit{Title} attribute to gain a summary of the event updates.}}
    \label{fig:application-live-article}

        \Description{This figure demonstrates the utility of layout transformation in reading live articles. The first image (A) shows a standard scrollable stack of live articles on an online news site. The second figure (B) shows the same articles in which a user has surfaced and sorted articles via the \textit{Published at} attribute effectively transforming the layout from a list to a timeline}

\end{figure}
% https://www.nytimes.com/live/2024/09/12/us/california-wildfires-idaho-oregon


% \subsubsection{\changed{Collapsing Source Code Files}}
% Something about forming new overviews from codebases, like choosing how to abstract the information, like choosing the comments attribute to collapse the code into just the comments, collapse into just the headers, or even collapse by the return statements
% You could also choose to hide certain attributes in this overview. So this becomes a dropdown variation. But you can change this dropdown OD variation into even a toolkit, or open these details side by side. You can even explore a hierarchy of function headers, or a hierarchy of comments

% Point of this application is to show that any piece of information can be abstracted and formed into an overview-detail interface.



\subsubsection{Mobile Applications: Food Delivery (Fig. \ref{fig:application-food-order})}
\changed{The overview-detail design pattern is also present in diverse platforms such as mobile devices. We recognize that our presented customization techniques can translate to these platforms as well.}
When ordering food on a mobile delivery app, some attributes are not shown in the overview. For instance, Doordash shows prices and thumbnails of menu items to show what is popular (Fig. \ref{fig:application-food-order}A), but do not show descriptions---which includes the calories. An implementation of \technique in this app could allow calorie-conscious individuals to check which items best suit their needs by surfacing the calorie count into the overview. 
\changed{Users can easily invoke Fluid Attributes on mobile devices by long-pressing an attribute (Fig. \ref{fig:application-food-order}B), which opens a context menu presenting available customizations, such as the ``Surface'' option (Fig. \ref{fig:application-food-order}C). Tapping this option instantly reveals the calories for all items, eliminating the need for further context switching (Fig. \ref{fig:application-food-order}D).}
% \changed{Users can easily invoke Fluid Attributes on mobile devices by long-pressing an attribute (Fig. \ref{fig:application-food-order}B), and open a context menu that presents available customizations such as ``Surface'' (Fig. \ref{fig:application-food-order}C). Tapping on this option instantly reveals the calories for all items, eliminating any further context switching (Fig. \ref{fig:application-food-order}D).}
% also present on other devices and raise similar challenges to those in the desktop that \technique can address.
% We have identified several challenges that \technique can address.
% \subsubsection{Food delivery applications}

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{figures/5_applications/applications-food-delivery.png}
    \caption{\changed{Our presented techniques generalize across platforms such as mobile devices. (A) Upon tapping on a menu item on a mobile delivery interface, (B) calorie-conscious users can hold down on description text of the item and (C) choose to surface the description to the menu list. (D) This automatically reveals the ingredients and calories for every option.}}
    \label{fig:application-food-order}

        \Description{This figure shows the ubiquity of manipulating attributes even on a mobile device. The image shows a standard online food delivery app, in which a health-conscious user is able to select the ingredients attribute and calorie attribute and surface them in the menu overview.}

\end{figure}


% \subsubsection{\changed{Mobile Applications: Text Selection}}

% There's a challenge when selecting large amounts of text. You need to hold, then just keep holding down until you scroll down to where you want to select to. And you of course can't select all.
% If you create two overviews, perhaps you can select \textit{through} the two overviews.
% So make an initial "anchor" selection, then save that view into an overview, then scroll all the way down, then complete the selection at the bottom.
% This is cool and useful, but it's not relevant to overview-detail interfaces lol
% Can you create two overviews to the same text, like two viewports. Then you 

% \bryan{Need to think more abnout this use case. Can you push this to be relevant to overview-detail??}

% % \subsubsection{\changed{Database GUIs}}

% % On Firebase, there are literally attributes that you want to see. but you need to click through each document



% \subsection{\changed{Other Application Scenarios}}
% \label{subsection:application-scenarios}

% To demonstrate the generalizability of our interaction techniques to all forms of overview-detail interfaces, we also describe other application scenarios using our techniques.

% \subsection{Exploring literature}
% It can be challenging to stay oriented during exploratory searching tasks such as literature search. One can explore a paper and its citations, leading to an exponentially growing search pattern with no end. One way to make this process more manageable can be to form a hierarchical layout of each paper's citations that opens information to cited papers as a dropdown instead of in a separate page---essentially collapsing the entire hierarchical search path into a dropdown menu (Fig. Xa). Another detail view can then be opened side-by-side to view individual papers in full detail (Fig. Xb).


\subsection{Implementation Details}
Desktop website application scenarios were implemented with Next.js, a React web framework, while the mobile application was implemented in SwiftUI. We used eBay's API to provide results in the shopping website and used Tripadvisors's API to provide results in the hotel booking website. Our high-fidelity probes stored all customizations on Firebase\footnote{\url{https://firebase.google.com/}. Accessed December 10, 2024.} in order to log customizations users make during our user study. Other applications stored customizations locally on the application's client.

\changed{The pipeline of the system diagram of our malleable overview-detail implementations is illustrated and detailed in Figure \ref{fig:system-diagram}. The end-user can make customizations across the three dimensions, corresponding to the system's three components. In our applications, content customization is implemented such that all data is fetched to the front-end, and the management of visible attributes is entirely client-side. However, other implementations can opt to fetch data attributes dynamically to minimize unnecessary database calls. Both composition and layout customizations are also managed on the client side.}

\changed{We implement AI to customize the content dimension only, but it can also manipulate the other two dimensions. Since all customization actions are performed through individual settings within the system, these settings can be made accessible to AI to modify based on their relevance to the user's prompt. This also enables AI to sequence multiple customization operations together across different dimensions. The prompts used in our specific AI implementations are provided in Appendix \ref{appendix:prompts}.}


\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/5_applications/system-diagram.png}
    \caption{\changed{A system diagram of malleable overview-detail interfaces. (A) First, data for the overview and detail view is fetched from the system's database. (B) The system them determines which attributes are included in the overview and detail view. This can either be determined from fetching specific attributes from the database or from the front-end client. (C) Next, the system determines the composition of the interface, such as the number of overviews to display. (D) Finally, the set of overviews and detail views are presented in the determined layout. (E) The end-user is able to customize these three stages through the interface by either directly interacting with the settings on the interface or by prompting AI.}}
    \label{fig:system-diagram}
    \Description{A system diagram of malleable overview-detail interfaces that displays stages of how data is populated to the interface. (A) contains an icon of the database, which points to the Content stage (B) which depicts JSON objects for the overview and detail views. Arrows then point to (C) which depicts views determined by composition. Finally, arrows point to (D), depicting the final interface in a particular layout. Stage (E) labels a block Direct Manipulation or Prompting which points to all three of the dimensions the user can customize.}
\end{figure}

% \subsubsection{AI-assisted \TechNique Pipeline}
% The shopping interface uses OpenAI's \texttt{gpt-4o} model to generate attributes and values. When the user requests a new attribute in the provided prompt box, the system first prompts the generative model to generate the name of the attribute based on the user's input and the contextual information of each item in the overview. It then follows up by prompting the model again to generate the corresponding values for the attribute across all items. \changed{The prompts we used for AI are in Appendix X.}



 % \changed{The detailed system pipeline for supporting our demonstrated customizations is in Appendix X. Our other web probes were implemented with the same web framework, while our mobile probe was implemented in SwiftUI.}
% The shopping website supported customizations along the three dimensions from our design space, while the booking website focused on supporting customizations for the content dimension.

% \subsubsection{MVC of Malleable Overview-Detail Interfaces}
% \bryan{The overview of our system architecture is depicted in Figure X.}
% \bryan{Malleable overview-detail interfaces in our probes are composed of two main components: 1) Overview and 2) Detail}
% \bryan{Overview is a UI component that determines how}
% \bryan{In our probes, we assign an ID to all attributes of an item. }



==> versions/R_R/7_user_study.tex <==
\section{User Study}
\label{section:user-study}

We used our two high-fidelity \changed{applications (shopping and hotel booking)} to understand how effectively users might customize malleable overview-detail interfaces and to observe emergent usage patterns as they utilize overview-detail interface transformations to best fit their needs and preferences. We aimed to answer the following questions:

\begin{enumerate}[label=\textbf{[RQ\arabic*]}]
    \item How effectively can users perform customizations on malleable overview-detail interfaces?
    \item What kinds of \changed{customization workflows and} usage patterns emerge when interacting with malleable overview-detail interfaces?
    \item What additional customizations did users seek that were not supported by our design probes?
\end{enumerate}


\subsection{\changed{Design Probes}}
\label{subsection:design-probes}

% to explore how users interact with malleable overview-detail interfaces in decision-making tasks, which, based on our content analysis, we found to be among the most common tasks involved with overview-detail interfaces.
% As depicted in Figures \ref{fig:probe-shopping} and \ref{fig:probe-booking}, we provide 
\changed{
We selected shopping and hotel booking websites in order to approximate a common yet complex, real-world scenario of using malleable overview-detail interfaces. To focus our study on observing the use of the key customization features, we selected a subset of features that were demonstrated in Section \ref{section:interaction_techniques}.}

\changed{In the shopping website's content dimension, we included surfacing, hiding, sorting, and filtering by attributes, prompting AI to surface and generate new attributes, and auto-fill attribute values.
Users can also sort and filter by attributes of each item.
For composition, we enabled users to add, remove, and rename multiple overviews. For overview layouts, we provided \textit{list}, \textit{grid}, and \textit{table} views, and for overview-detail layouts, we provided \textit{new page}, \textit{side-by-side}, \textit{dropdown}, and \textit{pop-up} layouts.
For the booking website, we focused instead on the content dimension to further investigate how users surface and hide attributes and to observe potential workflow differences compared to the shopping website. Upon surfacing attributes on the booking website, users were given the option to surface them to the map, the bookmarks list, or both.
Screenshots of our probes in different configurations are in Appendix \ref{appendix:probe-screenshots}.
}

% We detail the probes through example workflows of Alice, who is looking to purchase two new camera lenses to capture the scenic beaches of San Diego, California.
% The shopping website supported customizations along all the three dimensions from our design space, while the booking website focused on supporting customizations only in the content dimension. 
% \bryan{Also must talk about booking customizations}
% \bryan{Talk about what kinds of attributes are available to surface}


% \subsubsubsection{Workflow 1: Booking Hotels in San Diego (Fig. \ref{fig:probe-booking})}

% Alice begins by browsing through the hotels on the map. She notices that while some places have high ratings, some are quite expensive. To view both attributes in the map, she surfaces the \textit{Price} and \textit{Ranking} attributes for each hotel, allowing her to compare them more effectively (\textit{Surfacing Attributes} \ref{feature:surface-hide-attributes}). She bookmarks some promising options, which adds them to a separate overview of bookmarked places on the left side of the interface.
% After finding a list of hotels for San Diego, Alice starts a new search for hotels in La Jolla.
% However, as she adds new hotels for La Jolla, Alice realizes she is starting to confuse which hotels in her bookmarks bar are in San Diego and which are in La Jolla. To resolve this, she surfaces the \textit{City} attribute from the hotel's address to her bookmarks overview, making it easy to distinguish between the two locations. Finally, after comparing her bookmarked options across both cities, Alice decides on a hotel for each location.

% \subsubsubsection{Workflow 2: Shopping for Camera Lenses (Fig. \ref{fig:probe-shopping})}

% Upon searching for ``Canon DSLR camera lenses'' in the shopping website, Alice is presented with a list of results. To directly view the details she wants without switching between many detail views, she surfaces the attributes \textit{Focal Length}, \textit{Maximum Aperture}, and \textit{Type} to the overview (\textit{Surfacing Attributes} \ref{feature:surface-hide-attributes}). Values of some items' attributes that are named inconsistently are instead auto-filled by AI (\textit{Establishing Consistent Attribute Values} \ref{feature:ai-new-attributes}). Since Alice is specifically interested in lenses that handle low-light conditions for sunset photos, she sorts the lenses by \textit{Maximum Aperture} (\textit{Sorting with Attributes} \ref{feature:sort-filter-attributes}). Alice also recognizes that not all lenses may not be compatible with her camera, but she forgets the type of mount her camera uses. Since she knows the model of her camera, she decides to ask AI, ``Is it compatible with my camera Canon EOS R?''. AI then generates the attribute \textit{Compatibility with Canon EOS R} and provides answers ``Yes'', ``No'', and ``Not Specified'' for each lens (\textit{Generating New Attributes} \ref{feature:ai-query-attributes}).

% After exploring her options, Alice narrows her choices to two categories of lenses: a favorite but expensive lens and a less performant but cost-effective lens. To further explore these two categories, she creates two new overviews to add lenses from the search results (\textit{Customize Composition}, \ref{interaction-dimension:composition-layout}) and switches the views to tables to directly compare their attributes (\textit{Customize Layout}, \ref{interaction-dimension:composition-layout}). Finally, Alice makes her decision and takes her new lenses to San Diego.


% \subsection{Default Configurations \changed{and Selected Features}}

\subsection{Default Configurations}
We configured our overview-detail interface probes with default settings to be intuitive and easy for participants to get accustomed to. Our shopping site displayed the \textit{search results} layout as a \textit{list} overview of items. The overview-detail layout was by default a \textit{new page}, and the detail view displayed one item at a time. We additionally provided a second list overview named ``Cart'', which displayed a \textit{grid} layout of the items that were added to it. Each item in the overview displayed the following attributes: \textit{Title}, \textit{Thumbnail Image}, \textit{Vendor Username}, \textit{Vendor Feedback Score}, \textit{Vendor Feedback Percentage}, \textit{Product Price}, \textit{Product Condition}, \textit{Number of Products Sold}, and an \textit{Add to Cart} button. Our booking site utilized two different overviews: a map overview and an overview list of bookmarks. Upon entering the interface, the map view displayed the \textit{Rating} attribute of each hotel, and upon adding items the bookmark list, the \textit{Hotel Name} attribute was displayed by default. 
% Our booking site contained many attributes users would look through. 

% We are interested in studying whether users can effectively customize overview-detail interfaces to suit their needs. To do so, we implemented two high-fidelity design probes, a shopping website (Fig. \ref{fig:probe-shopping}) and a hotel booking website (Fig. \ref{fig:probe-booking}), to approximate a real world scenario of using malleable overview-detail interfaces. We selected the shopping and hotel booking domains for our example websites because our content analysis revealed distinct variations in overview-detail interfaces within these domains. 

% \bryan{SAY: Shopping website uses all three dimensions, and booking website uses only one dimension: content. We wanted to have shopping do all and booking focus on the content dimension only.}
% When designing these probes, we made sure to incorporate the key interaction techniques from the previous section. 

% \changed{We first introduce the two high-fidelity} probes through example workflows of Alice, who is looking to purchase affordable camera lenses to capture the scenic beaches of San Diego, California.




% --------



% -------


% These configurations were set as the default for the design probes, as we believed they would be the most intuitive to get accustomed to the interfaces. However, the main objective of the user study is to study whether and how participants would reconfigure these settings to better align with their own preferences.

% Customization features are often discovered as one uses the software and discovers frictions \tocite{}. 
% However, a controlled lab study doesn't
% Thus, we included key features we wanted to study
% Thus, to reduce the amount of features users would need to be introduced to 
% Among our demonstrated interactions through our probes, we focused our study on the use of key features. 

% We wanted to focus our study on the use of key features.
% Thus, we 
% To reduce the amount of features users needed to be introduced to 
% We enabled the AI feature of surfacing and creating new attributes.
% We provide the specifics of which content, layout, and composition variations are provided in Appendix X.

% \bryan{I should also include which features from section 4 are included in these probes, and which are not?}
% Moved this from design probes implementation details to the user study

\subsection{Procedure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.75\linewidth]{figures/8_results/study-procedure.png}
%     \caption{Visualization of the user study timeline}
%     \label{fig:study-procedure}
% \end{figure}

% Our 90-minute user study primarily focused on the hotel booking and shopping tasks, during which participants used our system to freely customize their layout, composition, and content attributes.

% We conducted a 90-minute study that consisted of two 35-minute sessions---one for each probe---and a 20-minute interview.
We conducted a 90-minute study, which began with a brief introduction of overview-detail interfaces to familiarize participants with the concepts and terminology used throughout the study (\textit{<1 min}). We then ran two 35-minute sessions, first on the booking task and second on the shopping task.
We began with the booking task because it contained a smaller feature set which could acclimate users to both websites easier.
During each session, users were first given a tutorial of our system, which included explanations of each feature as well as mini-tasks to acclimate participants to our probes \changed{and discover preferred customizations} (\textit{\textasciitilde 10 min}). They then proceeded with the main task, in which participants were asked to think out loud \cite{thinkaloud} (\textit{\textasciitilde20 min}). Once they completed the task, participants completed a questionnaire to share their experience with the website (\textit{\textasciitilde 5 min}).

Our hotel booking task description and criteria was as follows: 
\begin{quote}
    You are traveling to the Bay Area for meetings. You will stay in two different locations, one night per stay and will need to find a hotel for each: San Francisco and San Jose. 
    \begin{itemize}
        \item Your total budget is 350 USD,
        \item You want to eat at the hotel (or hotel room) as much as possible (strong preference for hotels with included breakfast or room service)
        \item You prefer modern and new hotels over traditional or old ones,
        \item You would like to stay one night at a premium/luxurious hotel.
    \end{itemize}
\end{quote}

Our shopping task description and criteria was as follows: 
\begin{quote}
You are choosing two monitors: one for your home and one for your workplace.
    \begin{itemize}
        \item Your total budget for two monitors is 250 USD.
        \item Criteria for monitor at home:
        \begin{itemize}
            \item You want a decent deal.
            \item You want the highest resolution possible, 4k or maybe better.
            \item The monitor should take up minimum space on your desk.
        \end{itemize}
        \item Criteria for monitor at work:
        \begin{itemize}
            \item The condition of the monitor is the most important.
            \item You want a display that’s decently sized, but also has high pixel density (resolution / display size).
            \item You don’t need a monitor stand---assume the office already provides one
        \end{itemize}
    \end{itemize}
\end{quote}

At the end of the session, participants were interviewed to reflect and share their overall experience (\textit{\textasciitilde 20 min}). These interviews helped us hear their thoughts on customization preferences, strategies, limitations, and opportunities.

\subsection{Participants}
We recruited 12 participants (5 male, 7 female) from a local university through internal communication channels. Of the participants, five were graduate students and seven were undergraduate students. All participants reported having experience with online shopping and booking. 

Initially, we asked participants to use their own laptops for the study so it is most familiar and comfortable for them, but after four participants, we deemed users may prefer a better setup than their laptop. Thus, we offered the remaining participants an external monitor (4k resolution, 31'' screen size), a keyboard, and a mouse. When offered, 7/8 participants chose to use the monitor. Participants were compensated 30 USD for 90 minutes of their time.

\subsection{Measurements}
To observe potential customization patterns during our tasks, we logged all participants' actions with timestamps with our system. 
We logged the types of customizations they made throughout their task, how frequently they made particular customizations, and which attributes they surfaced and hid from the overviews.
To capture additional context and insights into participants' behaviors, we recorded both screen activity and audio during the tutorial and think-aloud tasks for further coding and analysis. We collected responses from each post-task questionnaire (7-point Likert scale) to assess self-perceived usability and utility of our provided customization features. 


==> versions/R_R/8_results.tex <==
\section{User Study Results}
\label{section:results}

% In this section, we report on the findings from our questionnaires, interviews, and observations from their tasks.

% \bryan{SAY: Users made on average X customizations for their task, Y customizations per minute}
% \bryan{SAY: Detailed distribution of number of customizations made per user in Fig. X and logs of customizations made throughout their task in Fig. X}
% \bryan{SAY: Users made what kinds of customizations, like which layouts they used, how many overviews, which content they surfaced and used}

% P4 surfaced the attributes \textit{Pool} and \textit{Laundry Service}, while P12 surfaced \textit{Fitness Center} and \textit{Landmark View}.
% We first report on observations on the diverse customizations participants made and relied on.

\changed{First, we observed our participants made diverse customizations even when given the same shopping and booking tasks and the same starting interface configurations, suggesting that the customizations provided by malleable overview-detail interfaces are beneficial and desired.}
\changed{First, many participants surfaced attributes others had not, as illustrated in Figure \ref{fig:attributes-logs}. Some participants used multiple overviews for saving monitors into work and home lists (P1, P2, P6, P7, P12), while others created one intermediate space for candidate items (P3, P4, P8, P9, P10). While a majority of participants relied on the side-by-side overview-detail layout (P1, P2, P4\textasciitilde P12), P3 preferred to use the pop-up view, while P12 preferred both the dropdown and side-by-side views. Additionally, participants relied on a broad variety and combination of overview layouts between the list (P1\textasciitilde 4, P7, P9, P10), grid (P2\textasciitilde 5, P8, P10, P11), and table (P6, P11, P12). For instance, P4 used both grid and list views, while P6 used both table and list views together.}
% In fact, we found that participants used various combinations of list, grid, and table layouts with multiple overviews.
 
% Additionally, participants surfaced different attributes in different overviews, with P4 surfacing \textit{Price}, \textit{Number of Reviews}, \textit{Ranking}, and several hotel amenities in the bookmarks bar, but only \textit{Number of Reviews} on the map.

% On the other hand, P10 surfaced six different amenities in the map but only one in the bookmarks bar.
% Since the hotel booking interface provided participants with two overviews with different size and style, we also observed that participants surfaced different attributes for each overview. 


In the following sections, we report findings for each of our research questions.
% on the questionnaires, interviews, and observations gathered during their tasks.

% \changed{First, we observed our participants made diverse customizations even when given the same shopping and booking tasks, suggesting that participants desired the customizations provided in our probes.}
% \changed{For instance,} although we found popular attributes that many participants surfaced (e.g., \textit{Price Value}, \textit{Breakfast Available}, \textit{Maximum Resolution}), we also observed unique attributes surfaced across different participants \changed{(Fig. \ref{fig:attributes-logs})}. For example, P4 surfaced the attributes \textit{Pool}, \textit{Laundry Service}, \textit{Express Check-in / Check-out}, and \textit{VIP Room Facilities}\changed{, P12 surfaced \textit{Fitness Center}, \textit{Brand}, and \textit{Landmark View}, and P8 even surfaced the ``\textit{Add to Bookmarks}'' button.}
% Since the hotel booking interface provided participants with two overviews with different size and style, we also observed that participants surfaced different attributes for each overview. For instance, P4 surfaced \textit{Price}, \textit{Number of Reviews}, \textit{Ranking}, and several hotel amenities in the bookmarks bar, but only surfaced \textit{Number of Reviews} on the map. On the other hand, P10 surfaced six different amenities in the map but only one in the bookmarks bar. 

% We additionally observed different customizations of composition and layout. Some participants used multiple overviews for saving monitors into work and home lists (P1, P2, P6, P7, P12), while others created an intermediate space to save a sub-collection of candidate items (P3, P4, P8, P9, P10). \changed{While a majority of participants mostly relied on the side-by-side overview-detail layout (P1, P2, P4\textasciitilde P12), P3 preferred to use the pop-up view while P12 preferred both the dropdown and side-by-side views. On the other hand, we observed that participants relied on a broad variety of overview layouts between the list (P1\textasciitilde 4, P7, P9, P10), grid (P2\textasciitilde 5, P8, P10, P11), and table (P6, P11, P12).}
% In fact, we found that participants used various combinations of list, grid, and table layouts with multiple overviews. For instance, P4 used both grid and list views, while P6 used both table and list views together.



% Strongest preferences

% O-D
% sidebyside P1,2,4,5,6,7,8,9,10,11,12
% popup P3
% dropdown p12

% O
% list P1,2,3,4,7,9,10
% grid P2,3,4,5,8,10,11
% table P6,11,12


% All participants primarily utilized the separate page (5/12) and side-by-side (7/12) layouts,

% \changed{, while others surfaced \textit{Fitness Center}, \textit{Multilingual Staff}, and even the ``\textit{Add to Bookmarks}'' button.}
% attributes no other participants had surfaced.
% Participants P7\textasciitilde P12 surfaced unique attributes in the booking website as well, such as the hotel's \textit{Brand}, \textit{Multilingual Staff}, and even the ``\textit{Add to Bookmarks}'' button.
% \changed{Details on all attributes participants surfaced, hid, and generated with AI are illustrated in Figure \ref{fig:attributes-logs}.}

\subsection{RQ1. How effectively can users perform customizations on malleable overview-detail interfaces?}

\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{figures/8_results/questionnaire.png}
    \caption{Participants' responses to the utility and usability of interactions to customize the content, composition, and layout the hotel booking and shopping websites.}
    \label{fig:questionnaire}

        \Description{This image shows two stacked bar charts comparing participant responses to various aspects of customization and usability for a shopping website and a hotel booking website. The chart is divided into two sections: the Shopping Website in the top half and the Hotel Booking Website in the bottom half. The Shopping Website section has 10 different criteria being evaluated, including: Easy to customize content, Useful to customize content, Easy to customize composition, Useful to customize composition, Easy to customize overview-detail layout, Useful to customize overview-detail layout, Easy to customize overview layout, Useful to customize overview layout, Interface was easy to learn, Interface was easy to operate, and Helped more than typical shopping sites. The Hotel Booking Website measures fewer criteria, only 5: Easy to customize content, Useful to customize content, Interface was easy to learn, Interface was easy to operate, and Helped more than typical hotel booking sites. For both websites, each criterion is represented by a horizontal bar, color-coded to represent different levels of agreement, ranging from "Strongly Disagree" (1) on the left to "Strongly Agree" (7) on the right. The x-axis goes from 0 to 12, representing the number of participants or the score given. In general, both websites seem to have received positive feedback, with most bars heavily weighted towards the blue (agreement) end of the spectrum. The shopping website appears to have slightly more varied responses, especially for criteria related to customizing layouts and composition.}

\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/8_results/customization-logs.png}
    \caption{The number of customization operations made by each participant for each dimension. The shopping website supports customizations for all three dimensions, while the booking website supports surface and hide attributes. For the content dimension, we count how many new attributes were interacted with. For other dimensions, we count the total number of operations made.}
    \label{fig:dimensions-logs}

        \Description{This image shows a table comparing the number of customization operations made by participants (P1 to P12) for each dimension in two different websites: a Shopping Website and a Hotel Booking Website. Note that the hotel booking website supports surface and hide attributes, while the shopping website supports customizations for all three dimensions (content, composition, and layout). For the Shopping Website: the Content dimension includes Surface Attributes, Hide Attributes, Sort Attributes, and Filter Attributes. The Composition dimension includes Add New Overview, measuring how many times each participant added a new overview during their task. The Layout dimension includes Overview Detail Layout, Overview Layout, and Detail Layout. The Hotel Booking Website only includes the content dimension, which includes Surfacing and Hiding Attributes. The data includes numerical values for the frequency of each customization, but is also presented in a heat map style, with darker shades representing higher numbers of operations.}

\end{figure}


% \textit{How effectively can users perform customizations on malleable overview-detail interfaces?}

% BOOKING Average customizations made per user: 9.083333333333334, 2.752524094152291Average minutes:10.57901388888889, 3.9033645261280525Average c/m per user:0.9113574080059595, 0.24048349904081565
% \changed{(booking: M = 10.6 min, SD = 3.9; shopping: M = 14.8 min, SD = 7.0)}.
% 14.814390277777775, 6.968311589532828
% Average customizations made per user: 13, 9.128709291752768Average minutes: 14.814390277777775Average c/m per user:0.8592719374194197, 0.48546276509842345
% Able to learn (11/12 booking; 12/12 shopping) and operate the interface (9/12 hotel booking; 12/12 shopping)
% 11/12 participants agreed that the booking website was easy to learn, and 9/12 participants agreed it was easy to operate. All participants agreed the shopping website was both easy to learn and easy to operate. 
% Basically, all participants used our features.

All participants were able to complete both tasks within the time provided during the study.
They reported that the interfaces of both probes were easy to learn (booking: 11/12; shopping: 12/12) and operate (booking: 9/12; shopping 12/12), \changed{and most agreed that it was useful to customize content (booking: 6/12 strongly agree; shopping: 10/12 strongly agree), composition (11/12), and layout (overview-detail: 11/12; overview: 12/12) on the design probes.}
All participants surfaced attributes on both websites, while 9/12 participants hid attributes on at least one of them. 10/12 participants sorted or filtered by attributes on the shopping website.
 % (booking: 7/12; shopping: 6/12)
Most participants also customized the composition (10/12) and layout (11/12) of the shopping website (Fig. \ref{fig:dimensions-logs}).
\changed{We also measured how often participants made customization operations. On average, participants made 1.80 customizations per minute during the booking task (SD=0.74) and 0.86 customizations per minute during the shopping task (SD=0.48).
During their task, participants made an average of 22.08 content (SD=12.29), 1.33 composition (SD=0.84), and 2.17 layout (SD=1.52) customizations.}
% content: 22.083333333333332, 12.291313554249964
% composition: 1.3333333333333333, 0.8498365855987975
% layout: 2.1666666666666665, 1.5184055965240497
% \bryan{Also say these details are in Fig. \ref{fig:dimensions-logs}}
% 11/12 participants agreed the hotel booking website helped more than typical, and all participants agreed shopping helped more than typical. 
These results suggest that our participants were able to effectively utilize the customizations provided and understood the value of malleable overview-detail interfaces. 
P1 described how the customizability features allowed them to feel more in control with the interface, saying: ``\textit{The ability to choose exactly what I wanted on my screen and close everything else was super nice. You can't really do [that] with a lot of sites. Like, it is what it is.}''

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/8_results/attributes-logs.png}
    \caption{Visualization of all attributes that participants interacted with in the shopping and hotel booking website. The logs of the attributes that participants interacted with revealed common attributes Minimalists (\ref{results:hoarders-minimalists}) hid from the overview in the shopping website and the unique attributes some participants surfaced to the overview in the hotel booking website. We highlight participants who only surfaced attributes blue and participants who often hid attributes red.
    Attributes are sorted by the number of participants that interacted with them. AI-generated attributes are sorted separately.}
    \label{fig:attributes-logs}

        \Description{This image is a visualization comparing the various attributes that participants interacted with during the user study task: separated between the shopping website and the hotel booking website. The various attribute interactions are as follows: surfaced during task, hid during task, both surfaced and hid during task, and AI-generated attributed. The visualization is presented as a grid, with participants (P1 to P12) listed as the horizontal axis. The vertical axis consists of various attributes that participants had interacted with during the task. The Shopping website visualizes attributes such as Maximum Resolution, Vendor Username, Condition, Estimated Sold Quantity, while the Hotel Booking website visualizes attributes such as price value, breakfast available, room service, and restaurant. Each column (P1 to P12) shows how individual participants interacted with these different attributes in each respective task. The attributes axis are sorted by the number of participants who interacted with them, with the most interacted attributes at the top and the least interacted attributes at the bottom. AI-generated attributes sorted separately. This visualization ultimately allows for a comparison of attribute interactions across different participants and between the two types of websites.}

\end{figure}

\paragraph{\changed{Fluid Attributes reduces excessive context-switching}}
Participants explained that the utility of customizations came from its ability to avoid unnecessary navigation by bringing all details of interest into a single viewing space.
P3 stated, ``\textit{with a lot of websites that you can't really customize, you end up having to open the products one by one to look at all the specifications, which takes longer. I think it's nice to be able to just see it all as you're scrolling through.}'' P4 similarly described their experience with the hotel booking website compared to other commercial websites, saying, ``\textit{Websites like Booking.com, Expedia, and Airbnb don’t have these options. You have to literally look for each and everything. On the booking website, where only the options you want are displayed, it's very easy.}''
% I would love to have that website soon so selecting hotels won't be a hassle, taking multiple hours.

\paragraph{\changed{Fluid Attributes helps users align the interface with their decision criteria}}
Additionally, some participants shared that customizing content helped align the information they wanted to see on the website with their decision-making criteria. P12 said: ``\textit{After reading the information, I kind of have some criteria in my mind of which features I probably want, so I will only concentrate on these features. [With the hotel booking website], I can just customize what information I really want to focus on. For example, I personally really prefer the ratings.}''

\paragraph{\changed{AI-assisted Fluid Attributes reduces the need to sift through details}}

We also observed almost all participants surfaced or generated attributes with AI (11/12). P12, who surfaced 5/6 attributes by prompting AI, found prompting the interface the most convenient as it gave them direct answers, stating: ``\textit{I'm a very lazy person, so I'll rely on this feature because I don't want to click on each [item] and check whether they are 4k monitors.}'' \changed{P10 also appreciated the help from AI because they no longer felt ``\textit{confined to certain characteristics}'' provided by each item. They further described how they found one shopping item that contained the \textit{Material} attribute, but noticed it did not exist for all items. Instead of manually verifying whether items were missing the attribute or had it inconsistently named, AI provided a direct solution.}


% \bryan{Participants also used AI to check if an attribute existed in the website. Instead of reading through the details of each item, they prompt for a detail, and it either gives them the attribute, generates or calculates it, or says it's missing. Need some quote on this.}

% P11, sorta 
% P10 said they found attributes for one item but learned it didn't exist for 
% P10 said want to filter for something that's not included in the detail view
% P10: confined to certain characteristics of the item. -- one item had the attribute \textit{Material} and noticed it didn't exist for all items. Instead of looking through if the attribute didn't exist or existed but in a different name, AI provided a way out of this friction.

% \changed{AI guides unfamiliar decision-making scenarios}

% \changed{
% Training task involved searching through air conditioners on the shopping website. While P4 was familiar with the main task of what kinds of specifications a good monitor has, they were not aware of the options for air conditioners.
% }

% P4: AI is especially helpful for items you're not familiar with at all. -- in unfamiliar decision-making, you don't know what to look for.
% P4: AI would be useful if I'm not at all aware of any of the options. I see. OK. If I'm buying something very different, if I'm buying, for example, like refrigerator, yeah. Or if I'm buying air conditioner, I don't know the mechanics behind that. Maybe Mechanical Engineers would be aware of, OK, what kind of compressor works the best, etcetera, etcetera. I don't know that much. So for that those purposes maybe I can use AI. But then for monitors, for laptops, yeah, we d


% \paragraph{\changed{Customizing composition and layout }}

% When asking participants about what they liked and why they liked it
% Upon finding a customization they liked, we observed that participants mostly stayed with their setting. 
% We observed that the utility of customizing also came from the ease in which they were able to find a setting they most preferred.
% The utility of these dimensions primarily came from their ability to quickly find the preferred arrangement of the overview and detail views and their layouts.
% P9 said, ``\textit{I kind of found a layout that I liked, which was the side by side, and I just stuck to using that.}''





% \paragraph{\changed{Users made diverse customizations even when given the same task}}
% \paragraph{\changed{Users make diverse customizations even when given the same task}}
% \paragraph{\changed{\bryan{Users basically could make more granular control of their interface.}}}


% We noted diverse customizations participants had made in their tasks. 
% \bryan{Diverse customizations means participants effectively used malleable overview-detail interface, because they all converged to what they wanted.}
% \bryan{I may need additional visuals showing the different types of layout they chose}


% \paragraph{\changed{The diverse customization support gives users granular control over their interface}}
% \paragraph{\changed{Users can recognize and leverage their unique preferences}}

% \paragraph{\changed{Diverse customizations aren't overwhelming???????}}
% This suggests that participants effectively utilized the customizations provided to personalize the interface to their own needs.

% \paragraph{\changed{Users prefer similar configurations across different tasks}}
% \changed{Upon reflecting on their experience with both design probes, P6 expressed a desire for their table and list configuration on the shopping website to also be available on the booking website. They noted that, for tasks like these, they almost always default to using a spreadsheet application as their go-to tool for managing and organizing information.}
% \changed{This suggests that the utility of customizations in the overview-detail design pattern comes not only from their relevance to the task at hand but also from their broad applicability and support across many different overview-detail interfaces.}
% \changed{This suggests that the utility of customizations for the overview-detail design pattern does not only come from how relevant they are for the task but also from how widely these customizations are supported across various overview-detail interfaces.}
% that their preferred customization is shared across different instantiations of the pattern.}
% This further validates the utility of providing options to customize composition and layout of overview-detail interfaces.
% , stating, ``\textit{if this layout was able to be implemented with the booking, [it would be] so nice because you can see a [table] instead of making an [separate] excel sheet on the side.}'' 






% What kinds of \changed{customization workflows and} usage patterns emerge when interacting with malleable overview-detail interfaces?

\subsection{RQ2. What are the different \changed{workflows and} usage patterns of malleable overview-detail interfaces?}
% \subsection{RQ2. What are the different usage patterns of malleable overview-detail interfaces?}

Findings from the previous section demonstrate that malleable overview-detail interfaces are both effective and preferred by our participants, as the supported customization allowed them to achieve their desired configurations. In addition to enabling these configurations, we are also concerned with how to enable users to reach these configurations more quickly. Therefore, we aim to identify the types of overview-detail configurations users prefer, which could be provided as defaults to different user groups in future interfaces to reduce the number of customization they need to perform.

% Now htat we know our interfaces are useful and that users are able to control it well, we want to know what pattern emerge. Understanding these patterns can help us understand what kinds of overview-detail settings people would prefer the most as defaults.
% \haijun{add transition paragraph here describing why we want to observe these patterns, especially because that we did not motivate these questions when we first introduce them}
% \textit{What kinds of usage patterns emerge when interacting with malleable overview-detail interfaces?}

% \bryan{The goal of this section is to identify groups of behaviors and needs. This will form clear groups of people that will make the reader think, ``You can also start to design good defaults for these groups''}
% \bryan{We would obviously love to provide individual overview-detail for each user, so they don't have to keep customizing to their needs. but we can at least provide better defaults for individual groups. So they can select specific defaults set to their wishes.}


% What customizations did each participant prefer the most?
% Strongest preferences

% O-D
% sidebyside P1,2,4,5,6,7,8,9,10,11,12
% popup P3
% dropdown p12

% O
% list P1,2,3,4,7,9,10
% grid P2,3,4,5,8,10,11
% table P6,11,12


% Which participants customized which dimensions at the start, and which customized which dimensions throughout?

% Generally look for customizations made throughout
% Look for customizations made from beginning to end (P12 started with popup, then to side by side), so popup maybe for exploration, and side by side maybe for decision making




% composition + layout


% How did people store information?

% How did people narrow their search/results?

% How did people compare options?



% \subsubsection{\changed{Customization Workflows}}

% \subsection{\changed{RQ2. What workflows did users engage in while customizing overview-detail interfaces?}}
% \bryan{When do people customize ODIs and merge with RQ3 --> just keep it as a single RQ}

% To answer this question, we detailed what operations participants performed to achieve certain information retrieval goals, such as

% To answer this question, we detailed workflows of some participants from our study as personas


% \subsubsection{finding a comfortable layout}
\paragraph{\changed{Customizing at the start and throughout}}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/8_results/usage-shopping.png}
    \caption{\changed{Logs of customizations made by participants throughout the shopping task for surfacing and hiding attributes, adding new overviews, and transforming overview and overview-detail layouts. While many participants made initial configurations, many also continued to make more customizations throughout their decision-making processes, such as creating more overviews.}}
    \label{fig:usage-shopping}
    \Description{Log visualization of each participants' customization operations throughout their shopping task. Each horizontal row is populated with content (cyan), composition (red), and layout (indigo) data points along an x-axis by duration in minutes. The figure annotates an area highlighting initial configurations for roughly the first five minutes and specific data points where users added new overviews later in the task.}
\end{figure}


\changed{
Logs of participants' customizations made throughout their shopping task are illustrated in Figure \ref{fig:usage-shopping}.
While many participants began their task by making initial configurations of their overview-detail interface (P1\textasciitilde P5, P8\textasciitilde P12), many also continued to make customizations throughout (P1\textasciitilde P4, P6\textasciitilde P8, P10, P12).
For instance, P3 initially surfaced attributes that best aligned with their criteria, but changed their set of surfaced attributes as they compared between more choices.
% , as recorded in P3's logs of content customizations in Figure \ref{fig:usage-shopping}.
Additionally, some participants added multiple overviews from the start (P1\textasciitilde P3, P6\textasciitilde P9, P12), while some added them ad hoc when they needed to save and directly compare between choices (P1, P4, P7, P10).
% Finally, PX started with a list overview, but then later switched to grid views
% (as annotated in Fig. \ref{fig:usage-shopping}).
P1, who continuously transformed their interface throughout their task, expressed the desire to stay in Attributes Mode, while P11, who preferred to ``\textit{customize once and be done}'', suggested a dedicated customizations page to make their configurations in one place.
Furthermore, P6 even expressed a desire to use their table and list configuration from the shopping website for the booking website as well. They noted that, for tasks like these, they almost always default to using a spreadsheet application as their go-to tool for managing and organizing information.
% \changed{This suggests that the utility of customizations in the overview-detail design pattern comes not only from their relevance to the task at hand but also from their broad applicability and support across many different overview-detail interfaces.}
To support users who continuously make customizations throughout their task, interfaces could reduce the friction of making these customization options with more direct manipulation interactions, keyboard shortcuts, or in-situ settings on the interface.
On the other hand, those who make initial configurations could benefit from a central settings page with available customization options, popular default configurations that users can access at any point, and if possible, saved customizations across different tasks and websites.
}


\paragraph{\changed{Common sequences of customizations}}

% Which customizations were used in tandem?
% surface + sort, surface + filter
\changed{
Most common sequences that we observed involved semantically related customizations, such as surfacing multiple attributes all relating to hotel food services or creating a new overview and immediately changing its layout.
We also observed cases when participants sorted or filtered by values of attributes they had immediately surfaced (P2\textasciitilde 4, P6, P8, P10, P11), suggesting a common \textit{surface-then-sort} and \textit{surface-then-filter} workflow.
Interfaces can reduce the number of clicks by offering pre-composed operations, enabling users to create their own, and ensuring AI-assisted interfaces can perform these composed operations as well.
}


% \subsubsection{Revealers and Removers}
\paragraph{Hoarders and Minimalists}
\label{results:hoarders-minimalists}
% \paragraph{Removers, Revealers, and Restorers}
% In addition to observing how participants surfaced attributes, 
Prior research has identified tendencies when managing digital information along the spectrum of two extremes: hoarding and minimalism \cite{Vitale2018HoardingAndMinimalism}. We found that this behavior also emerged when users were given the ability to surface or hide attributes in our probes (Fig. \ref{fig:attributes-logs}):
% \bryan{TODO: Rephrase this section}
% https://dl.acm.org/doi/10.1145/3411764.3445585
% Fileweaver
% While all participants added attributes to the overviews with both design probes, we observed distinct behaviors in how they \textit{remove} attributes (Fig. \ref{fig:attributes-logs}). We identified two common groups:
\begin{enumerate}
    \item Hoarders (P2, P4, P10): Participants who did not hide any attributes from the overview.
    \item Minimalists (P1, P3, P6, P7): Participants who deliberately hid attributes from the overview.
\end{enumerate}

P2 (Hoarder) did not hide any attributes in the overview, including ones they surfaced manually from the detail view or by using AI . They reasoned, ``\textit{hiding it has a bigger inertia for me to overcome because if I want it back, I would feel like I wasted more effort to remove it and bring it back again.}'' They further explained that this is their natural tendency, as they also clutter their screen with many tabs. On the contrary, P3 (Minimalist), who hid five default attributes from the shopping website and one default attribute on the hotel booking website, admitted to the higher effort, but also advocated for the reward, stating, ``\textit{it probably takes longer to set it up the way I want it, but also then it's easier to look through because I'm not getting irrelevant stuff.}''
% \changed{P12 instead appeared to sit in the middle of these two extremes, where they surfaced multiple attributes but then hid ones they had surfaced initially but no longer needed because their interface felt too cluttered.}

% \bryan{Aligned with literature on hoarding and minimalism \cite{Vitale2018HoardingAndMinimalism}}
Perhaps Hoarders are more resilient to clutter in the overview and less resilient to the cost of repeatedly retrieving information from the detail view. For them, an overview interface that packs information from the start, allowing them to sift through the information themselves, would be more preferable.
On the other hand, Minimalists value the limited space the overview interface can provide and want to ``keep this space clean''. For them, a blank slate in the overview, allowing them to choose which attributes they want to see would be more preferable.
\changed{
Perhaps for those who sit in the middle of these extremes, a setting that keeps a maximum number of attributes displayed at once---automatically hiding less important attributes when more are surfaced---might also be preferable.
}
% ,  users with a higher ``clutter threshold'', 
% interfaces can design their interface to also allow end-users to set a threshold .

% \bryan{We find this this connection between managing personal digital information and customizable overview-detail interfaces particularly exciting, as it may hint at the direction for end-user customizable and malleable interfaces to essentially transform into the end-user's personal information space.}



% \paragraph{Participants utilize multiple overviews for different workflows}
% \paragraph{Participants use multiple overviews to break down tasks}
% \subsubsection{Participants use multiple overviews to break down tasks}
\paragraph{Utilizing the overview composition and layout to structure tasks}
% While 3/12 participants used the default overviews provided to them (Search Results, Cart), the remaining nine
Among the 10/12 participants that utilized multiple overviews to perform the shopping task, five of them (P1, P2, P6, P7, P12) created two overviews---one for each monitor type (work and home). P12, who created these two overviews, approached their task by opening only one overview at a time to find monitors for each type. This setup allowed them to offload important information for later, saying, ``\textit{It gives me some mental space where I can preserve it.}'' They also appreciated how they could open both spaces at once when they needed to compare between the two overviews. P6 even split their budget into each overview, allocating \$150 for the work monitor and \$100 for the home monitor.

The behaviors of these participants hint at a pattern of utilizing the overview composition and layout to manage sub-tasks.
To support this usage pattern, malleable overview-detail interfaces may provide functionalities that allow users to create nested or linked overviews based on their tasks, either manually or 
 by leveraging AI. For example, the interface can break complex tasks into more manageable, hierarchical sub-tasks or linearly order overviews to queue sequentially dependent tasks. This aligns with literature that take the task-centric approach to provide hierarchically organized browser tabs \cite{tabsdo}, dedicated desktop spaces \cite{henderson1986rooms}, and dynamically linked email threads \cite{bellotti2003taskEmailThrasks}.
% Approaches to designing task-centric interfaces have been explored by providing hierarchical organizations of tabs \cite{tabsdo}, dedicated desktop spaces on the operating system \cite{henderson1986rooms}, or dynamically linked threads of emails \cite{bellotti2003taskEmailThrasks}.

% Just as Tabs.do reflects the task structure into a hierarchical organization of tabs, users may similarly configure their overview layouts into a hierarchical structure if needed \cite{tabsdo}.
% Other tasks that may involve a more sequential process (e.g., project management), may lead users to produce overview arrangements that resemble a Gantt chart or a Kanban board.



%  ------


% P12 - , especially when I I can compare the home and the work in different spaces by opening them, opening up them together.

% This reveals a group of users who prefer to match their overview-detail interface to how they organize their task.
% suggests that this group utilizes multiple overviews to break down their task into sub-tasks.
% broke down their task into two subtasks: finding a monitor for work and finding a monitor for home. With their organization, they


\subsection{RQ3. What additional customizations did users seek that were not supported by our design probes?}
% \textit{What additional customizations did users seek that were not supported by our design probes?}

\paragraph{Choose how detail views are invoked (P6)}
% P6 shared how they wanted to change how 
% shared a notable dimension our design space did not include: navigation. 
While our design probes were implemented to open detail views by clicking, P6 suggested the probes to allow users to open details by hovering. They further described how they would also want a ``less maximized'' view of the details, suggesting the desire to invoke multiple detail views with \textit{different sets of attributes} in different ways.

% P6 - different ways to invoked details
% if you could hover over it and just like have it pop up instead of having to click on it. Like the less clicks I have to do the better just because it's like faster for me. Or if there was like a way for it to like be minimized and then be maximized instead of like it all being this like it's all being displayed and I appreciate it all being displayed. But if it was like displayed so I could like actually see the numbers or prices for all of them, would that be nice?

\paragraph{Attributes about all items in the overview (P6, P10, P12)}
Participants wanted details across all items in the overview, in addition to individual ones for each item. For instance, P6 wanted to calculate the total price of the hotels in their bookmarks bar, while P10 wanted to find a ``best price'' by balancing multiple criteria they surfaced. 
Indeed, if the detail view can have attributes about an item, the overview should also have attributes about the entire collection \cite{Xia2017CollectionObjects}. Since the shopping website provided a title of the overview, it is certainly reasonable for users to also need more attributes that describe the overview itself. 

% \subsubsection{Receive recommended attributes (P2, P11, P12)}
% Three participants also wished to see recommended attributes to surface into the overview in addition to directly surfacing and prompting AI. P11 suggested a sidebar that shows attributes relevant to what they were looking for. This could perhaps better scaffold users in information-seeking tasks, as explored in prior research that explored providing contextually relevant search query suggestions to facilitate exploratory search \cite{Selenite, Srishti2022InterWeave}.













% For malleable overview-detail interfaces to facilitate both needs, perhaps further allowing them to save customizations for future re-use.

% We recognize the importance of these different preferences, and suggest 
% While supporting one of these workflows in lieu of the other may introduce conflict in the,
% We recognize two different preferences that can both be supported in the interface.
% This suggests that larger user bases may prefer the ability to both transform their interface throughout their task as well as create overview-detail presets to support their common workflows.
% While some preferred this ability continuously transform their interface throughout their task, with P1 even expressing the desire to stay in Attributes Mode, some also preferred to ``customize once and be done'' and suggested a dedicated customizations page to make their customizations in one place (P11).
% and selecting grid or table views when starting to compare between a few choices (P1, P4, P7, P10, P11).
% Participants also used sort and filter features throughout the task, rather than just in the beginning. This suggests that interactions involving fluid attributes may see more dynamic usage throughout user tasks, similar to how sort and filter features are used in current websites.
% All participants continued to surface and hide several more attributes and some
% This indicates that interactions involving

% Perhaps users may prefer to create different overview-detail presets at different stages of decision-making or sense-making tasks. Interfaces could allow users to not only make various overview-detail customizations but also save them for future re-use.


% However, other users may want to keep this power throughout, as P1 expressed a desire to stay in Attributes Mode for their task.
% As P11 commented, ``\textit{Personally, I'd like a customization page or a separate menu for customization, something I can customize once and be done.}''
% We observed similar workflows in the booking task with all participants surfacing and hiding attributes at the start of the task, and continuing to surface and hide throughout.
% This also revealed that participants did not only customize attributes to view 
% Most participants who surfaced attributes throughout the task had simply found more attributes they would be interested in.
% P12 surfaced the \textit{Photos} UI component at the start of the task to see hotel rooms, but as they surfaced more attributes, they found the component to clutter the map view too much and chose to hide back the component.
% "This suggests that some users may prefer a more transformable workspace that they can gradually morph to fit their constantly shifting activities."
% Interfaces can provide several fixed templates, but should 
% are beneficial, 
 % rather than several, fixed templates depending on specific 
% Set up composition and layout at start of task
% 1,2,3,5,6,7,8,9,12
% We observed most participants set up multiple overviews and different layouts at the start of the task.
% But we saw almost all participants surface and hide attributes throughout the task.
% P1 started their task customizing all three dimensions at the start, but still ended up customizing attributes throughout.
% --> Descirbe which attributes they surfaced at the start, and then which attributes they surfaced later
% 


% 


% Set up composition at end of task (when decision-making)
% 1, 4, 7, 10, 11 --> when it was time to start deciding on things, they added another view near the stage of decision-making.

% \subsubsection{Users customized layout and composition before starting their task but customized content throughout}
% Most participants (X) began their task by changing the overview-detail layout and overview layout to the one they preferred most from their training task.
% When it came to attributes, X participants started out by surfacing attributes they needed first, then exploring, while other participants (X) looked through items first, then surfaced attributes as they scrolled through the options.

% Perhaps this could link fluid attributes as a default technique alongside sorting and filtering?
% However, this could also be due to the probes not providing clear mechanisms to for instance create new overviews or details through attributes...

% We also found participants often customized overview layouts after adding a new overview, 
% We additionally observed that P12
% We additionally observed participants surfaced then immediately hid attributes, 
% Additionally observed others used AI generated attributes to sort and filter by immediately too (P12)
% Additionally observed P6 had surfaced and then immediately hid the attribute, possibly suggesting a desire to only peek at a few attributes.
% Additionally, future AI-assisted malleable overview-detail interfaces should ensure their unit tests also include prompts that request such customization sequences.

% P12 appeared to have a threshold or a liimit, where they surfaced multiple attributes, but then hid several ones they had surfaced initially, but no longer wanted. Interfaces can design their interface to also allow end-users to set a threshold that automatically hides less important attributes if they surface more important ones.

% To filter out items they wanted, we found participants would surface an attribute they wanted, and then use that surfaced attribute to filter directly.

% participants surfaced N attributes they cared about, some then hid a subset of those, narrowing their interested criteria

% Felt like composition and layout customizations were used in tandem, whereas attribute customizations were used more closely to filtering and sorting.



% \paragraph{Narrowing down options}

% \subsubsection{Users }
% To compare items to choose from:
% Most saved them into a separate list
% some participants filtered out items they didn't care about, using the attributes they surfaced as information to filter out.


% One participant first searched for certain attributes in the shopping item search bar. maybe then surfaced more attributes? --> Realizing these are two similar ways of finding items that better match your criteria.
% Most participants primarily surfaced attributes.
% This action



% \subsubsection{comparing options.}
% Some participants compared options by scrolling through items with custom surfaced attributes
% Other participants compared options by adding items into anoter separate overview.
% Other participants created two overviews to compare items side by side horizontally instead.
% If this is really true (concrete action), then this could suggest also a preference for customizing the axis of O+D layout, as described in (that paper from the related work).













% P2, P11 - Recommended attributes to grab
% instead of you grabbing a detail from an existing entry, I would probably prefer there to be a sidebar showing details that are relevant, like showing fields that are relevant to this thing I'm looking for
% Selenite, CoNotate


% P6, P10 - calculations across overview items
% that would be so nice if there was like a way to have like the budget, like if you could add the budget somehow and like just because I was like using my calculator. But if like there was like a way to like do the math of like, oh, your total sum of hotels is like this much, that'd be nice.


% \paragraph{Further explanations with AI (P6, P8)}
% P8 - AI makes deeper judgments, answering questions about certain attributes


% - Way to invoke detail view --> wanted to just hover over something to peek instead of having to click. Perhaps both can be provided at the same time.. How to let users easily customize this without getting in the way of their work? How to lower that friction/barrier? \cite{Mackay1991TriggersAndBarriers}



% \bryan{Were there some things users tried to do, but then didn't work? Want to ask AI for filters or sorts.}

% \bryan{Participants also wanted features that we introduce in the interaction techniques section... Maybe this is not necessary---reviewers would say: ``Then why didn't you implement that into the probe?''}

% \bryan{Since we provided hotel booking website first---which only provided the content dimension to customize---users brought up dimensions that we had prepared for the shopping website. For instance, wanting to ....? }





% RQ1 DUMP


% AI-enthusiasts

% \subsubsection{AI-enthusiasts iteratively refine their attributes}
% P8's behavior also reveals another finding with AI-assisted \technique. While P8 over-generalized their initial prompts before reaching their desired response---a tendency commonly found in non-AI expert prompters \cite{whyjonnycantprompt}, our design probe still allowed them to iterate towards their desired attribute. Similar behaviors were also observed with P12, who initially generated the attribute \textit{High Resolution}, then landed on the attribute \textit{Is 4k}.
% P12, who surfaced 5/6 attributes in the shopping website by prompting AI, found prompting the interface the most convenient as it gave them direct answers, stating: ``\textit{I'm a very lazy person, so I'll rely on this feature because I don't want to click on each [item] and check whether they are 4k monitors.}''
% appreciated how they could prompt AI for direct answers
% This presents opportunities to provide AI-enthusiasts 

% % Also could be named Restorers
% The third group, Refiners, did not hide any default attributes but hid attributes they generated themselves. For example, P8 initially asked for free shipping, first prompting with ``free,'' which led the AI to generate the attribute \textit{Free}. This did not give them the attribute they wanted, so they prompted again, this time specifying ``free shipping,'' upon which AI generated \textit{Free Shipping}. However, they were not satisfied with the attribute, so they prompted for a third attribute, \textit{Total Price}. After generating the attribute they wanted, they hid both \textit{Free} and \textit{Free Shipping}.

% This behavior differed from the other two groups. Revealers did not hide excess attributes after iterating towards their desired attribute with AI (P2, P10). Removers on the other hand did hide excess attributes, including AI-generated ones (P3). Although Refiners did not deliberately hide default attributes, they did hide excess ones they created, suggesting a unique tendency for Refiners to ``clean up after themselves''.
% % . They instead only made an effort to hide the excess attributes
% % Although Refiners did not deliberately hide default attributes as how Removers did, they did make the effort to hide attributes they generated and no longer needed, suggesting this group's tendency to ``clean up after themselves''.
% When asked why P8 hid excess attributes but left the default attributes in the overview throughout their task, they explained that the excess attributes were distracting because they provided no more information for them. However, default attributes such as \textit{Ratings} were ``\textit{ignorable}'' enough to be kept in case they might be useful in the future.
% % This indicates that Refiners' decision to hide attributes is conditional, with specific criteria determining whether an attribute should be hidden or left visible.




%  So I think it is more adaptive to my own preference and practices.
% Like just make the correct correlation of if I'm looking for this, this is the price I'm going to be looking at. Or like if I want to include these things, this is like but I also need to be like connecting multiple details with each other.

% humble myself --> participant was talking about this when they were 
% P1 even described how customizing content encouraged them to ``\textit{humble myself}'' and tell themselves, ``\textit{Yeah, this is what I actually need to look at}'', suggesting that granular control over content on websites may have better helped P1 reflect on their criteria and needs during the task.
% This suggest providing more granular control over the attributes users may additionally 

% \bryan{Need quotes on AI attributes utility}

% \paragraph{Utility of customizing composition}
% \bryan{Todo}
% \bryan{Must find quotes about how it was useful to add new overviews. Especially how you can add as many as you want.}


% Participants made diverse customizations
% 1. Diverse attributes (Fig \ref{fig:attributes-logs}) were surfaced and hidden -- You can see that there are a lot of commonalities, there are some attributes some people surfaced, but there were quite a few attributes that no one had surfaced. Note the hotel booking as example.
% 2. Composition? but how did they use these different overviews?
% 3. Layout? but how did they use these different layouts?

% P10 added a lot in the map, but not that much in shopping

% Also, why did people surface many different things? Why were the attributes diverse, even when given the same task?




% % I can just customize what information I really want to focus. For example. I personally really prefer the ratings. So I think it is more adaptive to my own like preference and practices.''
% % So I think like what Airbnb and traditional map driven search engine usually just zoom in by only one or two section. For example, them like they're stars or like how far are they from the locations I want or the money like the rent per night. But I think the difference between this one, the concept of it is like 


% % \textbf{Starting to think more about criteria and attributes}
% % P12 - I think I kind of after reading the information, I kind of have some criteria review my mind of which which kind of features I probably want. So I will only concentrate on these features. So I think like what Airbnb and traditional map driven search engine usually just zoom in by only one or two section. For example, them like they're stars or like how far are they from the locations I want or the money like the rent per night. But I think the difference between this one, the concept of it is like I can just customize what information I really want to focus. For example. I personally really prefer the ratings. So I think it is more adaptive to my own like preference and practices. So which makes easier to use?

% % \textbf{Humble oneself; choosing what they actually need to look at}
% % P1 - I got to see all the options that made that a lot easier to do. And I could like, humble myself and be like, yeah, this is what I actually need to look at.



% % appreciated being able to ``\textit{customize what information I really want to focus on}'' (P12), 




% P1 - Being able to like look at this whole thing and see like, oh, this doesn't have a desk or oh, this has a tennis court. The fact that it's visible in multiple places is really nice. I don't have to like search through something to get to it.




% P12 - \textbf{the difference between this one, the concept of it is like I can just customize what information I really want to focus. For example, I personally really prefer the ratings. So I think it is more adaptive to my own like preference and practices. So which makes it easier to use.}



% X/12 particiapnts it was easy to use. They mention it was a bit of understanding, but once they got it, it was quick and intuitive. or something that says that.


% \textbf{You need to literally look for each and everything. This, you don't have to...}
% P4 - it was definitely very useful because most of the UK booking websites, if we see like the booking.com and the Expedia and the Airbnb, they don't have these options. I mean, there are specific things that you want to see and filter out, but then in those websites you have to literally look for each and everything. And in some of the hotels, something is good, something is bad. And in some of the hotels if something is bad, something is good. So deciding between these offsets and whether that extra price is justified or not, those decision like it's very difficult to take in the normal website versus especially the bookmarking option which you had in the booking website where you have only like only the options which you want to be displayed that is getting displayed.





% You have to look for everything manually, and some hotels are good in some ways but bad in others. Deciding if the extra price is worth it is difficult. But with the bookmarking option on your website, only the options I want are displayed, making it much easier. I’d love to have that feature soon, so selecting hotels won’t be such a hassle or take hours."

%  it was definitely very useful because most of the UK booking websites, if we see like the booking.com and the Expedia and the Airbnb, they don't have these options. I mean, there are specific things that you want to see and filter out, but then in those websites you have to literally look for each and everything. And in some of the hotels, something is good, something is bad. And in some of the hotels if something is bad, something is good. So deciding between these offsets and whether that extra price is justified or not, those decision like it's very difficult to take in the normal website versus especially the bookmarking option which you had in the booking website where you have only like only the options which you want to be displayed that is getting displayed. That is like very easy. So yeah, that's makes things definitely very useful for me to use it. So yeah, I would love to have that website hop soon so that yeah, it will be easier every time to select for the hotels, not like the hassle thing and taking like multiple hours.

% P4 - But yeah, these side by side options and also the grid ones, which typical websites don't provide, that makes things very easy. And also the I think the main benefit of both the website is selecting only the useful details and it's starting the rest


% P4 - that's makes things definitely very useful for me to use it. So yeah, I would love to have that website hop soon so that yeah, it will be easier every time to select for the hotels, not like the hassle thing and taking like multiple hours.

% P4 -  I would love to have that website soon so that it will be easier every time to select hotels, it's not a hassle and taking multiple hours.

% P4 said, "That definitely makes it very useful for me. I’d love to have that feature soon, so it’ll be easier to select hotels without the hassle of spending multiple hours."

% P5 -  I think it's just more convenient than what eBay currently has right now just because yeah, eBay is you go to, you click on something, you go to a separate page. And I don't like going back and forth.


% P5 - the options to filter [in booking] are a lot more useful than shopping just because one is like where you're going to live versus like something you're going to buy, I guess. So like the whole thing with if you want like someone who speaks Chinese, I think that's very important. And like I'm surprised it's not been implemented, I guess because that that would be very convenient for someone.


% \textbf{Needing to use other applications -- not a very strong quote though}
% P6 - ``Please make this available tomorrow. I've gone on trips with friends and looking for a place to say, and it's so tough. We end up making an excel spreadsheet [with] all of our options, like costs and everything we need. So if this layout was able to be implemented with the booking site it would be so nice, because you can see a grid instead of making an excel sheet on the side.''



% P3 - it was nice to be able to see like the things that I was looking for on each location. Yeah, Because it prevented like me from having to scroll through every place separately.


% P3 - I really like being able to customize it for both because I think if I were to get like really used to like really used to using it in a certain way, like with the list view or the grid view, then it would be a lot easier to like shop for things with like looking for specific specific criteria.





% P1 - Being able to like look at this whole thing and see like, oh, this doesn't have a desk or oh, this has a tennis court. The fact that it's visible in multiple places is really nice. I don't have to like search through something to get to it.

% P1 - Same thing with like being able to drag over the exact details I want, and then I actually really like being able to remove information I didn't need 'cause then I could just like glance through exactly what I wanted and I didn't have to like read through other stuff.




% \bryan{@Allen: Quotes on why the customizations were useful}


% \bryan{@Allen: How many participants mentioned \technique was their favorite feature?}

% \bryan{@Allen: Quotes on what their favorite feature was and why.}

% P3 - it probably takes longer to like set it up the way I want it, but also then it's easier to look through and I'm not getting like irrelevant stuff.


% P5, who does not like going back and forth between separate pages, also preferred the side-by-side layout, stating 

% , and stated this option was more convenient than standard sites because they didn
% compared the shopping website to other shopping websites, and 

% ``It's just more convenient than what eBay currently has right now just because, with eBay, you click on something, 

% a layout they individually wanted, P9 stating, ``

% As shown in Figure \ref{fig:dimensions-logs}, most participants made two or three customizations in layout and composition, likely because they were able to quickly converger

% ``I found a layout that I liked, which was the side by side and I just stuck to using that.''

% P9 - I kind of found like a layout that I liked, which was the side by side and then I'm just like, OK, I'll just stick to using that. So I guess that's sort of like customization really helps because it's like everybody has like a different way of like doing different things.

% % People talked about how they liked using multiple views, it let them do some things...
% % People liked how they could view multiple different layouts

% P6 - 

% P6 - t's like as much as as like the table, like you're saying like, oh, it's like so terrible. But I actually feel like it's like, it reminds me of like Notion and like Excel. So it's really like structured. And when you're looking for like certain qualities or like certain like features that you want, like specific like requirements that you want to meet, it's so nice to be able to just like see that instead of like making it pretty or like, oh, like I want like, I feel that the grid is like visually like more appealing. But because I was looking for these qualities that's sort of like mix and match like, oh, this goes with this and this goes with this. So just like the mental framework was very intuitive. So that's what I really liked from this. So I really strongly agree with this. I think it's really, really nice. That's awesome, yes. And the interface helped me complete the shopping task better than typical. Yes. I wish all the websites were like this. It was so nice. So nice. I'm so glad to hear that. Yeah. So I'm going to strongly agree with this because like, honestly, I wish like, I am so used to this and like, yes, this isn't pretty, but like for my own sake, if I am customizing it and I have like certain like departments I have to meet, it's like so useful to just like for me to have like mental clarity of like, yes, this is within my budget. This is like, there's my resolution. It's like like taking of things of like A to do list.


% P5 directly compared the shopping website with eBay stating: ``I think it's just more convenient than what eBay currently has right now just because, with eBay, you click on something, you go to a separate page, and I don't like going back and forth.

% But PX preferred the table because of ...

% PX preferred having both a table and a grid because of...


% 11/12 participants stated they preferred the side-by-side view for the shopping website. P3 preferred a popup instead. \bryan{Why?} P12 initially started with a dropdown, then switched to side-by-side. \bryan{Why}

% Ultimately, participants were able to find a preference in the interface, suggesting that participants were able to effectively make use of the options provided by the malleable overview-detail interface.


% RQ2 DUMP



% ---- START SYNCHRONIZERS AND SEPARATORS SECTION ----
% \paragraph{Participants either surface the same or different set of attributes across different overviews}


% \paragraph{Synchronizers and Separators}

% The hotel booking interface utilized two different forms of overviews: the bookmarks bar and the map, which allowed users to either surface attributes to both overviews or just one. We observed that the 12 participants were evenly divided between two distinct usage patterns:
% \begin{enumerate}
%     \item Synchronizers (P1\textasciitilde P3, P5\textasciitilde P9, P12): Participants who surfaced the same attributes into both overviews.
%     \item Separators (P4, P10, P11): Participants who surfaced different attributes in each overview.
% \end{enumerate}

% Synchronizers surfaced all attributes to both overviews, sometimes before opening the bookmarks bar. P12, a Synchronizer, preferred to surface attributes to all overviews with the expectation that the information ``\textit{will be important in the future}''. 

% Although surfacing too many attributes can clutter the map, 

% P8 surfaced both ways, 

% realized to surface it everywhere, if need info i prob need everywhere
% surfaced images in the tutorial
% didn't surface any of the big elements
% didn't use bookmark view


% This aligned with P8, also a Synchronizer

% surfaced all attributes with the mind that ``\textit{this will be important in the future}''

% Not aware of the feature (or just Synchronizer by default...)
% P1, P2, P5, P6, P9

% Aware of choices
% P3 - Synchronizer (Hid choice after surfacing everywhere)
% P4 - Separator (She used the bookmarks bar as a comparison space; map as viewing information) (surfaced rankings and amenities)
% P7 - Synchronizer
% P8 - Synchronizer
% P10 - Separator (Only Map)
% P11 - Separator (Only Map except one in bookmark
% P12 - Synchronizer (This will be important in the future)

% Synchronizers surfaced the same attributes in both overviews, <what motivated them to do that?>
% PX stated ``Something about surfacing the same set of attributes''
% P7 even went as far to surfacing the rating of the hotels to the bookmarks bar, even though it had already been surfaced in the map. (They must have surfaced, hid, then surfaced. Maybe don't use this, it's a little risky)

% Synchronizers:
% P8 - can I get more insights from him?
% P12 - a bit cluttered for sure, but 
% P10
% - less in bookmarks, more in map --> actually no.
% Says it did get cluttered, but they didn't find it a huge issue to zoom in and out for it.
% - Yeah, I think I would still prioritize the the criteria. It's not too bad. I think it's just because they're so close together. The hotels, it's a little cluttered, but it's not like a huge issue like I would just have to zoom in and zoom out for it.
% - Likes having pictures on the map

% Separators chose to surface attributes to 
% - To overcome the clutter issue on the map, P3 added the photo only to the bookmarks bar
% - P4 was an avid bookmarks user. Only surfaced number of reviews to the map (while keeping the default, hotel rating), and surfaced price value, ranking, and amenities about breakfast to the bookmarks bar.
% - Similarly, 

% Same
% 1 2 6 8 9 12

% More in Bookmark
% 4 5 6 11

% More in Map
% 10

% P1
% - same

% P2
% - same

% P3
% - photos
% - 

% P4
% - price, number of reviews, ranking, amenitie, a LOT more in the bookmarks
% - rating, number of reviews

% P5: morein th ebookmkars
% - languages
% - breakfast, room service, description

% P6
% - photos, price level, value
% - breakfast

% P6
% - same

% P8 -- didn't care, but used same
% - same

% P9
% - same

% P10
% - less in bookmarks, more in map --> actually no.
% Says it did get cluttered, but they didn't find it a huge issue to zoom in and out for it.
% - Yeah, I think I would still prioritize the the criteria. It's not too bad. I think it's just because they're so close together. The hotels, it's a little cluttered, but it's not like a huge issue like I would just have to zoom in and zoom out for it.
% - Likes having pictures on the map

% P11
% - More in bookmarks, less in map
% - b: photos, more ameniteies

% P12
% - same

% ---- END SYNCHRONIZERS AND SEPARATORS SECTION ----



% This suggests users who heavily rely on AI to find information 
% This suggests that users who rely on AI will leverage 
% of malleable overview-detail interfaces may

% \paragraph{Reliants}

% \bryan{TODO: Instead of restorers, it's people who were more reliant on AI.}

% \bryan{Move this to AI-assisted section right below. Talk about AI people in one group. Avid AI users}
% so it's not about how they chose not to hide any default attributes, but through refining their prompt with AI, they worked towards a final attribute they wanted.

% From this explanation, it may be reason


% \bryan{This suggests integrating AI-assisted \technique into malleable overview-detail interfaces can provide a workspace to make granular changes while still having the controls to undo those changes, make revisions, or build upon them---\technique provides this entire set of interactions.}
% This process may also be preferred over manually navigating around the overview-detail interface for some users. 

%  And sometimes I don’t care about the details I don’t fully understand, like the model number or similar specifics.

% ``I particularly like the AI feature because it helps me give me direct answers.''

% Want to say this iteration is still eventually good for the user, 

% I think it seems I have the full control over all the criteria, potential criteria I can choose.

% when users inevitably stumble upon getting the right response, 

% \bryan{What does this suggest???}



% P12 - I particularly like the AI feature because it helps me give me direct answers. I, I'm a very lazy person, so I rely on these things that I don't want to click on each tab and check whether they are four key monitors. So I think that feature really help. And sometimes I don't care about the things, the numbers that don't really understand, such as such as these things, the model, OK, these are things I don't care about. So I like how the IT only features two specific item details 4 three of them, and then I can make a decision.

% P8 started their shopping task by asking for three attributes: \textit{Total Price}, which added shipping costs to the item price, \textit{Free Shipping}, whether an item provided free shipping, and \textit{Free}, another request if the. After viewing the values of the three attributes, they then hid \textit{Free Shipping} and \textit{Free}, with \textit{Total Price} remaining in the overview.
% While P8 surfaced attributes about shipping costs, whether there's free shipping or not, P9 instead asked AI for the total cost of each item, which computed the price and shipping cost into one value.


% P2 asked for the size of the monitors...

% We gave participants the criterion ``4k or better'' monitor.
% We saw some participants surfaced the attributes such as \textit{Maximum Resolution}, but many instead asked AI, producing attributes \textit{Is 4k}, \textit{Is 4k Resolution}. P12 initially (?) asked for \textit{High Resolution}, but instead hid that attribute and generated the new attribute \textit{Is 4k}.

% While some participants (P1, P7, P12) asked AI whether monitors included a monitor stand, P11 instead made a new search, ``Monitor with monitor stand'' \bryan{or something like this!}

% P7 also asked for the condition, even though it had already been surfaced in the overview. Looks like P7 used AI to also search for attributes. This may suggest implications on the reliance of AI for other tasks



% But why didn't they hide other attributes given to them by defaut?

% , introduced by using AI to generate attributes, were Restorers: participants who generated AI attributes, but removed them as an iterative step towards their desired attribute. P8 first generated three attributes
% \bryan{What does this suggest? Does this align with other literature? Need to dig deeper into this insight.}





% Revealers: P2, P4, P10
% - people who didn't said, it's not worth their effort, you can see everything, so you may as well just keep it there. (basically, you can just ignore it)
% Removers: P1, P3, P7
% - people who wanted to hide attributes say it's too cluttered, and I just want to focus on my information
% Restorers: P11, P12
% - What did restorers say? What's their reason for hiding back attributes?
% People surfaced details, but didn't hide defaults. Does this mean they liked the defaults? or did they not bother to hide? or did they really want to hide the things they surfaced?
% look into P8, who surfaced Free Shipping but hid it back


% We also observed participants who appeared to be primarily Revealers until they wanted to remove an AI-generated attribute they did not want. For instance, P8 first generated the attribute \textit{Free}, then \textit{Free Shipping}, then finally \textit{Total Price}. 




% For instance, P8 first generated the attribute \textit{Total Price} to see the total price of the item including shipping fees, then generated \textit{Free Shipping} and \textit{Free}. They then sorted by \textit{Free}, until finally removing it and instead grabbing the actual shipping value. That's because AI just didn't work here man.


% P2 - ``I just didn't really want to waste effort of hiding it because I already took effort to add it.''
% P2 - I just didn't really want to waste effort of like because I took effort to add it. And so like hiding it has a bigger kind of like. Inertia for me to overcome because like, what if I want it back then I have to go back and then like, feel like, oh, wasted, you know, like more effort to remove it and bring it back again.


% PX did not hide default attributes, but did hide attributes they had surfaced before. 

% * does this align with past literature?

% \paragraph{Opening and closing attributes over opening and closing views}
% P8 added a lot of filters. interesting user.
% P3 and P8 surfaced attributes, then hid them. \textbf{Does this suggest a behavior of users ``opening'' and ``closing'' attributes, rather than full web pages?}
% \textbf{Perhaps, more granular control over the information on their websites allows them to still effectively find information they want?}
% Look at P3 -- They hid a lot of things. They surfaced, and then hid back a few things as well.



% We observed that 10/12 participants utilized multiple overviews to approach the shopping task in two distinct approaches:
% \begin{enumerate}
%     \item  5/12 participants (P1, P2, P6, P7, P12) created two overviews, one for each monitor type (work and home)
%     % \item ---by creating a separate overview for each.
%     \item 5/12 participants (P3, P4, P8, P9, P10) created an intermediate collection for items that best satisfied their criteria, assigning names such as ``Save for Later'', ``Wishlist'', or ``Maybe''.
%     % \item prioritized criteria, adding items that best satisfied their criteria into an intermediate collection (). Another collection was then used to add and remove finalists from the intermediate collection.
% \end{enumerate}

% divided their interface into two subtasks

% P12 - The different space is very important for me, especially when I I can compare the home and the work in different spaces by opening them, opening up them together.

% P12, who created two separated overviews for work and home, sometimes opened only one of the overviews to focus on one sub-task, but 

% P12, who created separate overviews for work and home, focused on finding a monitor for one location at a time by hiding the other overview. This setup allowed them to switch their attention between the two tasks, stating, ``It gives me some mental space where I can preserve it.'' P6, who also created two overviews, even split their budget for each overview, allocating \$150 for the work monitor and \$100 for the home monitor.
% This suggests that this group utilizes multiple overviews to break down their task into sub-tasks.
% % broke down their task into two subtasks: finding a monitor for work and finding a monitor for home. With their organization, they

% On the other hand, some participants P4, who utilized an intermediate overview, began their task by collecting items into their intermediate overview based on key criteria—such as resolution, brand, and model. They used this overview to add and remove candidates, while dedicating their Cart overview as the final collection, suggesting that other users utilize multiple overviews as a way to sift through the results to find items with the best criteria first.

% to sift through items primarily based on criteria


% On the other hand, P4, who utilized an intermediate overview, began their task by looking for items with the best resolution, best brand, and newest model of monitors. They added the monitors that best matched these criteria into their intermediate collection, then among the candidates, saved the best candidates for work and for home. They dedicated the Cart overview as their final collection, while using the intermediate space as a workspace to add and remove items, suggesting another group of users that prioritize criteria and utilize multiple overviews to sift through items that best match their criteria.



% another group of users that prioritize criteria and utilize multiple overviews to sift through items that best match their criteria.


% This approach highlights the benefit of using multiple stages of overview to enhance decision accuracy and efficiency. For design implications, consider incorporating features that support intermediate evaluations and allow users to refine their selections progressively, improving their overall experience and satisfaction.


% Among the options, P4 was willing to compromise the condition for their home monitor, so 
% P10 approached this similarly, and also mentioned, if they had much more options the would have added more lists. \bryan{But to do what? what would be the purpose to add more lists?}


% because participants oftentimes kept both the intermediate overview and Cart overview open at the same time, suggesting the value of maintaining a visual context


% P5 and P11

% While this usage pattern is similar to using the Cart overview, 

% This usage pattern differs from the the use of not using additional overviews (only using the Cart overview) 
% Cart, they added 

% P5 only used the cart, but not 


% This approach differed from

% collected items that best fit one or more of their criteria. 

% P4 - First of all I wanted to go with the like the maximum resolution, the best brand and the newest model. What's the price? Since I have the limited budget, what's the price? So since I saw that the 4K ones are like pretty expensive that itself cost like more than 250. So I cannot ever buy 2 laptops considering one having the 4K. So I just opted that option out at all. I was not choosing at all in my next steps in the maximum resolution. Then I went to the 2K. The 2K models what I saw and I wanted the condition to be new because first of all I was selecting for the workplace. So for the workplace I want something new and then the next resolution was 2K. So for the 2K then I selected what were the options in the search result. Then in the search result I found three options. One was over budget. I opted that out. I then there was two options out of that too. One was the good brand, so I selected that and discard the rest. So with the work option I have, I had the best price, newest, best resolution and also the good model.

% P4 - Then whatever the money I had left, I can compromise on my like home monitor. I see. Yeah. So then I chose the condition as used or like certified. So first I chose the certified one, the level level down one by one. I chose the open box and certified. If I'm not getting anything there, then I chose the used one. But then whatever I have, I segregate that in the list, like the non work one, the home ones. And then I made this mind that if I have more money than I can buy the open box and if I have strict budget, if I'm like poor, then I can buy the used one. Yeah.

% criteria over subtasks.

% P4 added items in their intermedi
% which led them to collect items that best satisfied one or more of their criteria. Then used the intermediate step to collect items with the best criteria



% On the other hand, P9 utilized an intermediate overview to 
% compare and contrast between all possibly options, and used another overview as a ``\textit{final list}''. 

% \bryan{Separate their space is one way to help make decisions}
% The group that separates their final spaces may work to separate their collections based on subtasks,




% P9 - adding different lists. I think for me, having one list work at like store stuff for like, OK, I like different options and then I can compare and contrast between each of those different options. And then the card is more of like a final list of like. Out of the ones that I chose, I think the list feature was the most helpful.

% P4 - So for the workplace I want something new and then the next resolution was 2K. So for the 2K then I selected what were the options in the search result. Then in the search result I found three options. One was over budget. I opted that out. I then there was two options out of that too. One was the good brand, so I selected that and discard the rest. So with the work option I have, I had the best price, newest, best resolution and also the good model.

% P11 - like the idea of having other lists as essentially like a part. And I think there are some like slight UI issues with it with kind of like, OK, let's say like I feel that because of the shopping website, the cart should always be treated specially. Yeah, instead of just a list like like list would just be less in part because like a car, you actually could like it's like you're essentially checking out. You're in the couture line, you're going to pay for it. Yeah, yeah. Whereas list is like wish list, you can just look more casual.


% \bryan{To best benefit these groups, a default MOD could be provided to allow users how many types of items they will purchase, providing enough spaces to compare within the options. Perhaps even allowing comparison between combinations of items can be provided.}
% \bryan{For the other group who organize items into intermediate collections, providing stronger synrchonization or something..... }
% \bryan{But these are like design recommendations. So all of these should just be foreshadowed... maybe?}


% \bryan{Different content in different overviews}
% Hotel booking site provided two overviews: bookmarks list and the map view. We noticed participants surfaced different attributes for the two different overviews.

% For instance, PX surfaced this on the map, but surfaced this on the bookmark.

% PX surfaced both these on map and bookmark, but the bookmark additionally had this attribute.

% P11 -- hide image in the map, but instead added to the bookmark. Didn't want clutter.

% Use of different customizations across different overviews were also observed on the shopping website. In the shopping interface, creating a new overview carried all surfaced attribute settings to the new one. By default, all add to list buttons were added in each overview. P7 instead removed add to list buttons that were not for that particular list, leaving each overview to only have a button that removed from its own list, serving as a ``delete'' button. Others used different layouts for different overviews, such as P4, who used a grid and a list and P11, who used a grid and a table.



% P2 
% P3 used maybe and then cart

% consdier candidates for the two locations

% Considered candidates in one space, as an intermediate space.
% Intermediate space contained both monitors for the two different spaces.

% This suggests, people do have different working patterns, able to customize the overviews for their different cases

% P10 - 

% ``The different space is very important for me, especially when I can compare the home and work in different spaces''

% P12 - The different space is very important for me, especially when I I can compare the home and the work in different spaces by opening them, opening up them together.

% P12 - It gives me like it gives me some mental space that I can preserve it.



% \paragraph{Surface to sort}
% \bryan{Another visual showing all the cases where participant sorts right after surfacing attribte or right after filtering}
% We commonly observed participants surface attributes, then sort or filter them right away.
% \bryan{I saw that there's a correlation in the number of attributes surfaced and the number of attributes sorted. I wonder if there's a common Surface + Sort mechanic happening?}
% \bryan{I think there's a common usage pattern of surfacing, then sorting right after.}
% \bryan{There is also one quote saying they feel they can sort by anything}
% \bryan{If you know you're able to sort or filter by every attribute possible, then there's no point it having a dedicated filter/sort area. Instead, you can just directly sort any attribute or value.}
% \bryan{This suggests an interface can support: if user surfaces an attribute, a sorting and filtering functionality shows up in the UI.}
% \bryan{Another options is to also be able to sort or filter from the detail view rather than only in the overview.}

% \textbf{Different in layout?}
% Did they use differnt layouts for different views, or did they constantly switch between many?

% What were the different layouts people created for their search? did people use two different views? Did people use the same view across different overviews? 



==> versions/R_R/9999_5_applications.tex <==
\section{Application \changed{Scenarios}}
\label{section:applications-old}

To demonstrate the generalizability of our interaction techniques to all forms of overview-detail interfaces, we describe several application scenarios using our techniques.

% \subsection{Exploring literature}
% It can be challenging to stay oriented during exploratory searching tasks such as literature search. One can explore a paper and its citations, leading to an exponentially growing search pattern with no end. One way to make this process more manageable can be to form a hierarchical layout of each paper's citations that opens information to cited papers as a dropdown instead of in a separate page---essentially collapsing the entire hierarchical search path into a dropdown menu (Fig. Xa). Another detail view can then be opened side-by-side to view individual papers in full detail (Fig. Xb).

\subsection{Reading and Managing Emails}
Oftentimes, emails can contain details such as a response deadline. However, this detail is likely not shown in the overview. Using \technique, users can prompt for an attribute \textit{Response Deadline}, and sort by emails that have the most upcoming deadlines (Fig. \ref{fig:application-email}).

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{figures/5_applications/application-email.png}
    \caption{Users can prompt AI to sort by emails with the most urgent deadlines. Upon doing so, the attribute \textit{Response Deadline} is surfaced and sorted by latest date.}
    \label{fig:application-email}

        \Description{This figure depicts an email inbox as a list overview. The user prompts AI for "most urgent emails to respond to", which surfaces a newly generated attribute called deadlines.}

\end{figure}

\subsection{Reading Live Articles}
Live news articles report on long-standing events such as presidential elections and sports games. These interfaces appear to aggregate shorter articles in a scrollable stack. However, it can be challenging for users joining in the middle of the event to quickly catch up on the timeline with a long document. To address this, users can select the \textit{Published at} attribute and bind it to a timeline overview, organizing all articles into a timeline. Users can also select which details to show in the timeline before diving into individual articles (Fig. \ref{fig:application-live-article}).
\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{figures/5_applications/applications-live-article.png}
    \caption{Users can catch up on an ongoing news event by surfacing and sorting articles via the \textit{Published at} attribute and transforming the layout from a list to a timeline.}
    \label{fig:application-live-article}

        \Description{This figure demonstrates the utility of layout transformation in reading live articles. The first image (A) shows a standard scrollable stack of live articles on an online news site. The second figure (B) shows the same articles in which a user has surfaced and sorted articles via the \textit{Published at} attribute effectively transforming the layout from a list to a timeline}

\end{figure}
% https://www.nytimes.com/live/2024/09/12/us/california-wildfires-idaho-oregon

\subsection{\changed{Calendar}}
Calendar applications provide multiple forms of overviews that are scoped by time (e.g., day, week, month, year). 
% In a single day view, you can choose to prioritize certain details about events over others, such as to view which events are remote and which are in-person.
% One could also zoom out to see in the week view, which days are fully remote and which days have in-person meetings.
% One could zoom out even further to the month and year views to surface events they may want to prioritize over others, such as if they want to view how many meetings there are for each day, and how many of those meetings are remote and how many are in-person.
% This application demonstrates how a customizable overview-detail interface with multiple overview representations connected by time can be linked across each other.


\subsection{\TechNique on Mobile: Food Delivery Applications}
% Overview-detail interfaces are also present on other devices and raise similar challenges to those in the desktop that \technique can address.
% We have identified several challenges that \technique can address.
% \subsubsection{Food delivery applications}
When ordering food on a mobile delivery app, some attributes are not shown in the overview. For instance, Doordash shows ratings and rankings of menu items to show what is popular, but do not show descriptions---which includes the calories. An implementation of \technique in this app could allow calorie-conscious individuals to check which items best suit their needs by surfacing the calorie count into the overview (Fig. \ref{fig:application-food-order}).
\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{figures/5_applications/applications-food-delivery.png}
    \caption{Calorie-conscious users can surface the descriptions of food items to view their ingredients and calories. This also demonstrates how \technique can be implemented on a mobile device.}
    \label{fig:application-food-order}

        \Description{This figure shows the ubiquity of manipulating attributes even on a mobile device. The image shows a standard online food delivery app, in which a health-conscious user is able to select the ingredients attribute and calorie attribute and surface them in the menu overview.}

\end{figure}

% \subsubsection{Catching up on unread messages}
% There may be cases when a messaging app has many with unread messages. However, current interfaces only provide two choices: 1) manually enter each conversation to read them, or 2) mark all as read without reading them. \Technique in a messaging app could enable users to select or peek at a conversation and surface the unread messages in the overview, allowing them to quickly catch up on all unread messages in a single view.








% \Technique in a messaging app could enable users to select or peek at a conversation and surface the unread messages in the overview, being able to catch up on all unread messages in a single page.

% Another case may be to catch up on unread messages across numerous chatting groups. Users can surface a specific scope of the latest conversation. Users can 
% * See unread messages all in overview with temp popup




% \subsubsection{Surfacing paper details}

% Surface paper abstract on scholar, surface figures on semantic scholar, surface other information right away for other cases too...

% \subsubsection{Organizing paper citations hierarchically}


% \paragraph{Searching text in the document}


% \subsection{Browser}
% \subsectio{Graphic design}


==> versions/R_R/9999_6_design_probes.tex <==
\section{Design Probes}
\label{section:design_probes}

We are interested in studying whether users can effectively customize overview-detail interfaces to suit their needs. To do so, we implemented two high-fidelity design probes, a shopping website (Fig. \ref{fig:probe-shopping}) and a hotel booking website (Fig. \ref{fig:probe-booking}), to approximate a real world scenario of using malleable overview-detail interfaces. We selected the shopping and hotel booking domains for our example websites because our content analysis revealed distinct variations in overview-detail interfaces within these domains. \changed{We additionally implemented other smaller design probes to demonstrate the generalizability of our techniques.}
% When designing these probes, we made sure to incorporate the key interaction techniques from the previous section. 

\changed{We first introduce the two high-fidelity} probes through example workflows of Alice, who is looking to purchase affordable camera lenses to capture the scenic beaches of San Diego, California.


\subsection{Workflow 1: Shopping for Camera Lenses}
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/6_design_probes/design-probes-shopping.png}
    \caption{A screenshot of our shopping design probe, the overview list is shown on the left and a product detail view is shown on the right}
    \label{fig:probe-shopping}

        \Description{This figure displays a screenshot of our shopping design probe. The shopping overview is shown on the left in a list layout, and a product detail view is shown on the right, opened as a new page.}

\end{figure}
Upon searching for ``Canon DSLR camera lenses'' in the shopping website, Alice is presented with a list of results. As she browses through the list, she finds it cumbersome to find how far each lens zooms in as she must repeatedly open the detail view of each product to find this detail. To address this friction, she surfaces the attribute \textit{Focal Length} to the overview (\textit{Surfacing Attributes} \ref{feature:surface-hide-attributes}). She also takes this chance to surface \textit{Maximum Aperture} and \textit{Type} so she can glance at all the basic attributes to start. As Alice reviews the results, she appreciates that some items have been auto-filled by AI (\textit{Establishing Consistent Attribute Values} \ref{feature:ai-new-attributes}). Since Alice is specifically interested in lenses that handle low-light conditions for sunset photos, she sorts the lenses by \textit{Maximum Aperture} (\textit{Sorting with Attributes} \ref{feature:sort-filter-attributes}).

Alice also recognizes that not all lenses may not be compatible with her camera, but she forgets the type of mount her camera uses. Since she knows the model of her camera, she decides to ask AI, ``Is it compatible with my camera Canon EOS R?''. AI then generates the attribute \textit{Compatibility with Canon EOS R} and provides answers ``Yes'', ``No'', and ``Not Specified'' for each lens (\textit{Generating New Attributes} \ref{feature:ai-query-attributes}).

After refining her search and identifying several lenses of interest, Alice decides to categorize them for easier comparison. She creates two new overviews and re-names their titles to ``Want, but Expensive'' and ``Okay, but Cost Effective'', and adds lenses from the search result to each overview for further consideration (\textit{Customize Composition} \ref{interaction-dimension:composition-layout}). To directly compare attributes for each item, she switches the views into tables (\textit{Customize Layout} \ref{interaction-dimension:composition-layout}). After directly comparing, Alice decides to buy an expensive zoomable lens and a cost-effective low aperture lens.

\subsection{Workflow 2: Booking Hotels in San Diego}
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/6_design_probes/design-probes-booking.png}
    \caption{A screenshot of our hotel booking design probe, displaying an overview map on the right and a overview list of bookmarked hotels on the left. A detail view of a selected hotel is opened as a popover left of the map.}
\label{fig:probe-booking}

    \Description{The figure shows a screenshot of the hotel booking design probe, displaying an overview map of La Jolla on the right and a overview list of bookmarked hotels on the left. A detail view of a selected hotel is opened as a popover left of the map.}

\end{figure}

Alice, now excited about her new camera lenses, begins looking for places to stay near San Diego with the hotel booking website.

Alice begins by browsing through the hotels on the map. She notices that while some places have high ratings, some are quite expensive. To view both attributes in the map, she surfaces the \textit{Price} and \textit{Ranking} attributes for each hotel, allowing her to compare them more effectively (\textit{Surfacing Attributes} \ref{feature:surface-hide-attributes}). She bookmarks some promising options, which adds them to a separate overview of bookmarked places on the left side of the interface. Next, Alice considers the amenities each hotel offers. She is particularly concerned with ensuring that the hotel offers 24-hour check-in since she will be arriving late at night. She surfaces this detail to the map.

After finding a list of hotels for San Diego, Alice starts a new search for hotels in La Jolla.
% The hotel interface conveniently retains all the attributes she previously surfaced during her San Diego search, saving her time as she continues browsing. 
However, as she adds new hotels for La Jolla, Alice realizes she is starting to confuse which hotels in her bookmarks bar are in San Diego and which are in La Jolla. To resolve this, she surfaces the \textit{City} attribute from the hotel's address to her bookmarks overview, making it easy to distinguish between the two locations. Finally, after comparing her bookmarked options across both cities, Alice selects a hotel for each part of her trip---one in San Diego and one in La Jolla---ready for her exciting photography journey.

\subsection{\changed{Other Application Scenarios}}
\label{subsection:application-scenarios}

To demonstrate the generalizability of our interaction techniques to all forms of overview-detail interfaces, we also describe other application scenarios using our techniques.

% \subsection{Exploring literature}
% It can be challenging to stay oriented during exploratory searching tasks such as literature search. One can explore a paper and its citations, leading to an exponentially growing search pattern with no end. One way to make this process more manageable can be to form a hierarchical layout of each paper's citations that opens information to cited papers as a dropdown instead of in a separate page---essentially collapsing the entire hierarchical search path into a dropdown menu (Fig. Xa). Another detail view can then be opened side-by-side to view individual papers in full detail (Fig. Xb).

\subsubsection{Reading and Managing Emails}
Oftentimes, emails can contain details such as a response deadline. However, this detail is likely not shown in the overview. Using \technique, users can prompt for an attribute \textit{Response Deadline}, and sort by emails that have the most upcoming deadlines (Fig. \ref{fig:application-email}).

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{figures/5_applications/application-email.png}
    \caption{Users can prompt AI to sort by emails with the most urgent deadlines. Upon doing so, the attribute \textit{Response Deadline} is surfaced and sorted by latest date.}
    \label{fig:application-email}

        \Description{This figure depicts an email inbox as a list overview. The user prompts AI for "most urgent emails to respond to", which surfaces a newly generated attribute called deadlines.}

\end{figure}

% \subsubsection{\changed{Calendar}}
% Calendar applications provide multiple forms of overviews that are scoped by time (e.g., day, week, month, year). 
% Open a month overview, then through that, open two day overviews, two weeks apart. Create an event on the first day at specifically at some time, then drag the end of the event to say it ends on this day, but then drag it through this overview and into the next day's view. This makes the even extend through those two days, but also at the same time allowing you specify the end time of the event.

% Basically, I'm trying to select objects across two overviews... and then maybe surface details through that?

% 
% In a single day view, you can choose to prioritize certain details about events over others, such as to view which events are remote and which are in-person.
% One could also zoom out to see in the week view, which days are fully remote and which days have in-person meetings.
% One could zoom out even further to the month and year views to surface events they may want to prioritize over others, such as if they want to view how many meetings there are for each day, and how many of those meetings are remote and how many are in-person.
% This application demonstrates how a customizable overview-detail interface with multiple overview representations connected by time can be linked across each other.

\subsubsection{Reading Live Articles}
Live news articles report on long-standing events such as presidential elections and sports games. These interfaces appear to aggregate shorter articles in a scrollable stack. However, it can be challenging for users joining in the middle of the event to quickly catch up on the timeline with a long document. To address this, users can select the \textit{Published at} attribute and bind it to a timeline overview, organizing all articles into a timeline. Users can also select which details to show in the timeline before diving into individual articles (Fig. \ref{fig:application-live-article}).
\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{figures/5_applications/applications-live-article.png}
    \caption{Users can catch up on an ongoing news event by surfacing and sorting articles via the \textit{Published at} attribute and transforming the layout from a list to a timeline.}
    \label{fig:application-live-article}

        \Description{This figure demonstrates the utility of layout transformation in reading live articles. The first image (A) shows a standard scrollable stack of live articles on an online news site. The second figure (B) shows the same articles in which a user has surfaced and sorted articles via the \textit{Published at} attribute effectively transforming the layout from a list to a timeline}

\end{figure}
% https://www.nytimes.com/live/2024/09/12/us/california-wildfires-idaho-oregon


% \subsubsection{\changed{Collapsing Source Code Files}}
% Something about forming new overviews from codebases, like choosing how to abstract the information, like choosing the comments attribute to collapse the code into just the comments, collapse into just the headers, or even collapse by the return statements
% You could also choose to hide certain attributes in this overview. So this becomes a dropdown variation. But you can change this dropdown OD variation into even a toolkit, or open these details side by side. You can even explore a hierarchy of function headers, or a hierarchy of comments

% Point of this application is to show that any piece of information can be abstracted and formed into an overview-detail interface.



\subsubsection{Mobile Applications: Food Delivery}
% Overview-detail interfaces are also present on other devices and raise similar challenges to those in the desktop that \technique can address.
% We have identified several challenges that \technique can address.
% \subsubsection{Food delivery applications}
When ordering food on a mobile delivery app, some attributes are not shown in the overview. For instance, Doordash shows ratings and rankings of menu items to show what is popular, but do not show descriptions---which includes the calories. An implementation of \technique in this app could allow calorie-conscious individuals to check which items best suit their needs by surfacing the calorie count into the overview (Fig. \ref{fig:application-food-order}).
\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{figures/5_applications/applications-food-delivery.png}
    \caption{Calorie-conscious users can surface the descriptions of food items to view their ingredients and calories. This also demonstrates how \technique can be implemented on a mobile device.}
    \label{fig:application-food-order}

        \Description{This figure shows the ubiquity of manipulating attributes even on a mobile device. The image shows a standard online food delivery app, in which a health-conscious user is able to select the ingredients attribute and calorie attribute and surface them in the menu overview.}

\end{figure}


% \subsubsection{\changed{Mobile Applications: Text Selection}}

% There's a challenge when selecting large amounts of text. You need to hold, then just keep holding down until you scroll down to where you want to select to. And you of course can't select all.
% If you create two overviews, perhaps you can select \textit{through} the two overviews.
% So make an initial "anchor" selection, then save that view into an overview, then scroll all the way down, then complete the selection at the bottom.
% This is cool and useful, but it's not relevant to overview-detail interfaces lol
% Can you create two overviews to the same text, like two viewports. Then you 

% \bryan{Need to think more abnout this use case. Can you push this to be relevant to overview-detail??}

% % \subsubsection{\changed{Database GUIs}}

% % On Firebase, there are literally attributes that you want to see. but you need to click through each document





\subsection{Implementation Details}
The two high-fidelity design probes were implemented with Next.js, a React web framework. We used eBay's API to provide results in the shopping website and used Tripadvisors's API to provide results in the hotel booking website. \changed{The detailed system pipeline for supporting our demonstrated customizations is in Appendix X. Our other web probes were implemented with the same web framework, while our mobile probe was implemented in SwiftUI.}
% The shopping website supported customizations along the three dimensions from our design space, while the booking website focused on supporting customizations for the content dimension.

% \subsubsection{MVC of Malleable Overview-Detail Interfaces}
% \bryan{The overview of our system architecture is depicted in Figure X.}
% \bryan{Malleable overview-detail interfaces in our probes are composed of two main components: 1) Overview and 2) Detail}
% \bryan{Overview is a UI component that determines how}
% \bryan{In our probes, we assign an ID to all attributes of an item. }

\subsubsection{Storing Customizations}
Our probes store all customizations in a real-time database (i.e., Firebase) in order to log customizations users make during our user study. In practice, customizations can be cached locally in the browser or in the client-side state to respect users' ownership of personal data.

\subsubsection{AI-assisted \TechNique Pipeline}
The shopping interface uses OpenAI's \texttt{gpt-4o} model to generate attributes and values. When the user requests a new attribute in the provided prompt box, the system first prompts the generative model to generate the name of the attribute based on the user's input and the contextual information of each item in the overview. It then follows up by prompting the model again to generate the corresponding values for the attribute across all items. \changed{The prompts we used for AI are in Appendix X.}

% \bryan{Figure out robust to present this pipeline. True to implementation or illustrate its potential as well? Full robust pipeline? We did not build that though.}





% Upon searching for ``Canon DSLR camera lenses'', Alice finds a list of results ranging 
% \bryan{Range of lenses, she already has this configuration, so she decides to look for other zoom sizes.}
% \bryan{As she looks through, she finds it cumbersome to keep looking for the zoom attribute, so she surfaces this to the overview. Also surfaces other attributes, she finds valuable to her}
% \bryan{She also realizes upon surfacing these attributes, some items are filled in with AI. Upon hovering over the value, she sees the value came from the attribute X}
% \bryan{Because she wants only these zooms, she filters these in, and sorts by the lowest aperture.}
% \bryan{She also wants lenses that fit with her current camera. So she filters all lenses with the camera mount.}
% \bryan{She finds that some lenses do not mention whether the lens can zoom, so she asks AI ``Can these lenses zoom?'', which AI creates a property \textit{Zoom Capability}.}
% % As Alice scrolls through the overview, she learns the lenses that don't have this capability to all be called ``Prime'' lenses
% %  ^ Is that necessary? I want to add to show that this attribuet could also help with learning the new concept, but maybe it's a stretch, and it's best to keep it simple.
% % \bryan{After finding a few she likes, she decides to purchase two lenses, one telephoto and one prime lens}
% \bryan{After finding a few she likes, she saves lenses into several categories she wants to compare between: ``Want, but Expensive'', ``Could Buy'', ``Must Buy''.}
% \bryan{To do so, she creates three new overviews, each with lenses shes wants.}
% \bryan{As she filters down her choices by comparing items side by side in multiple overviews, she finally decides to buy a lens in Must Buy, and another lens in Want, but Expensive.}




% Pipeline that's more modular -- basically, one that could cal more functions if needed.
% Key is to identify relevant attributes, match/generate new attribute, identify value/generate new value, perform operation



% Specifically, 1) user prompt. 2) AI interprets and identities relevant existing attributes and their values, while at the same time determining which action to perform (sort, filter, surface). 3) Generates the property name(s) if needed. 4) Generates the values if needed. 5) Calls the filter/sort operations if needed.

% 1. User prompt, 2. AI interprets and identifies two things: relelvant existing attributes and their values & select the action to make: add property, filter, sort, 3. Apply those actions back to the interface through functions


% Why design probes? What's the purpose?
% We want to use these probes to study how users use malleable overview-detail.

% Why talk about these design probes? as opposed to the interaction techniques?
% In interaction techniques, we describe all the possiblte interactions we can have with MODs

% However, for our probes, we implemented a subset of these techniques to study 

% Why did we select a subset of these techniques?
% We wanted to study a subset to be able to evaluate them within the time set up for them and not overwhelm the user with too many features.

% Certainly, a system with too many features becomes too complex for users to learn within the given time of a controlled study.
% However, we do not undermine the importance of malleable overview-detail interfaces.
% Many other features in a practical setting, could be implemented to be more discoverable through a prolonged use of the system.

% We want to study how users use malleable overview-detail interfaces.




% \section{Design Probes}
% To study customizability dimensions..... we implemented our interaction techniques into two design probes: a shopping interface and a hotel booking interface.

% \subsection{Shopping Interface}

% \bryan{Layout dimension}
% \bryan{Many overviews, Collection sub-dimension}
% \bryan{Content dimension}


% \bryan{AI interaction feature: Pull details via prompting}

% \subsection{Hotel Booking Interface}
% We were also interested in exploring how users might interact with customizable OD interfaces on a map. So we developed a hotel booking interface that implements Detailed Manipulation.

% \bryan{Content dimension}
% \bryan{Many overviews, but via search results...? Does this count?}


% \bryan{thought 1}


% ---- This is start of temp comment ----
% \section{Interactions for Malleable Overview-Detail Interfaces}


% In this section, we describe interaction solutions to customize overview-detail interfaces along the three dimensions formed from our content analysis: \textit{layout}, \textit{composition}, and \textit{content}. We then highlight key novel techniques we discovered through the process of our analysis of overview-detail interfaces.

% The goal of this section is not to provide ways to turn one overview-detail interface into any other through the design space. Rather, we are interested in the interaction techniques that will provide the end-user the most control and benefit in the interface. 

% % We do not contribute ways to transform one variation into any other in our design space. 

% % We are not interested in comprehensively providing interaction techniques for transforming across all dimension variations, but rather interested in what kinds of challenges we are able to solve among each of these dimensions.

% % We don't provide interaction techniques to transform into every variation and every combination of every variation of these dimensions.

% % Rather, we describe interaction techniques that can make a customizable OD. This section isn't organized by dimensions though. It's organized by interaction techniques that we develop

% % outline
% % first, context: the results from the content analysis is that we found three dimensions of variation in overview-detail interfaces.
% %  What are we showing? Showing how we make those transformations
% % Organize it by dimensions? 

% % The goal is to make options customizable. At its very base, the customizations we provide can be implemented in diverse ways, such as menu option interface. 
% % But through this content analysis, we find novel interaction techniques that are worth exploring.

% % Layout
% % Composition
% % Content

% \subsection{Menus and Tabs}
% \bryan{Basically, this section is for Layout and Composition sub-dimension: more than one overview}

% The simplest and most traditional interaction technique for choosing between multiple options (in this case, variations) is by providing the user with a menu to choose which dimension variation they want to have. This is a simple approach for customizing the Layout dimension (Fig. X).

% \bryan{Then talk about how you can achieve the same thing for how many overviews you want, or how many detail views you want.. This is one of the sub-dimensions in the Composition dimension.}

% \bryan{But master views can be difficult to manage, so a familiar mode is by providing a tabbed view of the many master views, and enabling direct manipulation to rearrange the order of the multiple views.}

% \subsection{Direct Manipulation}

% \subsection{Detailed Manipulation}
% bringing details from the detail view to the master view 

% This interaction technique is agnostic to the interaction mechanism and instead shines light to the opportunity to control which details are shown in different views. 

% This below describes what is possible with \technique when implemented into interaction mechanisms.


% also re-prioritizing the details within the master item, like showing the dimensions to the top of the screen, just like how you can reorder the columns in a table, reorder the details in the list or grid


% \subsubsection{Customizing Composition}

% \subsubsection{Exploring the Generalizability of Detailed Manipulation }
% \bryan{I really want to talk about all the diverse ways you can use this technique though, this is so exciting to me. For instance, you can pull details to the scrollbar on a website, showing something like a scrollable minimap --> you can even made read wear and edit wear scroll bars. You can also remove details from the vscode scrollbar minimap. Another scenario beyond websites but for the design pattern is that you can modify which details you see in your tab bar on the browser. The detail view can actually be information about the history of your tabs, like an archive, and then you can choose to pull a detail about the last time you visited this tab. Then sorting it by the last visited tab. This might even help reduce tab clutter if you know which tabs you last visited or not.}



% \subsection{Interaction through AI}

% Maybe the Southwest example you have on Figma. You can either ask for the cheapest flight across the days, and the surface that detail for all the other days, or just ask for the cheapest flight in each day. We support this flexibility because either case might happen, depending on which one is more situated in the overview or the detail view.



% The user can additionally ask for attributes to surface to the overview through prompting. This can be particularly useful when what the user wants is unclear. For instance, asking for dimensions of an air conditioner on a shopping site would prompt AI to search for width, height, and length attributes of the item results.

% \bryan{I don't think this organization is that great, because we want a separate section for AI. High level requests for AI works not only for attributes but for other controls like layout or composition.}

% pulling details to master view pulls to all the items. The underlying interaction result is that the system propagates the action done by the user of a single item. Following this, we can imagine more actions beyond just pulling details if leveraging AI's ability to understand and act upon user queries. For instance one may ask to see the side profile of monitors. AI can search and identify a side profile image of each item's list of images and display that.

% \subsubsection{Attribute Synchronization}
% Selecting a detail can reveal that detail for all other views, whether it is scrolled through the view or if it's surfaced in other ways.

% \section{Design Probes}

% We describe basically what goes into the design probes we create, and also the interaction possibilities through these implementations


% In our design probes, we implemented \technique by toggling the ``details'' mode, which upon entering highlighted all detail attributes in the overview-detail interface. \bryan{There are different ways to implement this such as selecting an area or highlighting text and showing popups, or making it a default.}

% \subsection{Shopping}

% \subsubsection{A Kanban Board in a Shopping Interface}

% Buttons are also attributes of a particular item, as they are included in the detail view. By leveraging \technique and introducing multiple overviews through dimension of composition, it becomes possible to create a custom Kanban board\bryan{footnote for kanban board!} directly on the shopping interface to partition one's decision-making process into multiple filtering stages. 


% \subsection{Hotel Booking}


==> versions/R_R/9999_drafting.tex <==

% Our audience of this paper is the designers who design these interfaces.
% Our question is: How can we enable designers to design interfaces such that they are more customizable?
% Interfaces are simply not being designed that way from the start

% How do you make interfaces malleable?
% How can we design interfaces to become more customizable?
% What are the design approaches to make interfaces more customizable?
% This RW seciton is all about the APPROACHES for making interfaces customizable.
% So what are the APPROACHES?

% Customization might be less utilized, so we want it easy to make. We make it more insitu, and also make it so that users make small customizations, then slowly expand to more and more. Discoverability and ease of customization is one aspect, but 

% I know why i'm stuck. I want to talk about how to approach the design of customizability, but it's weird to go from discoverability to not having enough to customize.

% Ideally, I would like to go from one by one, then all, but then focus on design patterns
% but it's discoverability, then everything, then provide user friendly for these, then focus on design patterns.


% Designing customizable interfaces requires understanding and balancing the costs and benefits that influence users to customize their interface. 
% Mackay observed that users may be motivated to customize their interface when they recognize and grow frustrated of repetitive patterns, while users may be less inclined when the task of customizing is too difficult or time consuming that the perceived benefits are not worth the effort \cite{Mackay1991TriggersAndBarriers}.
% \changed{To balance these trade-offs, several lines of research have taken different approaches for customizability.}

% To balance this trade-off, several approaches have been explored to design interfaces for customizability. One approach has been to bring the customization settings visually closer to the UI components. For example, Anchored Customization integrates individual setting options directly into conceptually related UI components, providing a more “in-situ” way to access customizations \cite{Ponsard2016AnchoredCustomization}.

% how to support customizability?



% Visbug, Stylette, Sifter, these are made to focus on a specific aspect of customization, such as visual style, note-taking, filtering, sorting, and making spreadsheet computations.
% Addressing customizations on a case-by-case basis.

% Systematic approach tries to make things cusomtizable from the ground up, but it's simply impossible to anticipate every customization users will need [haystack, bonnie].

% These systems approach customizability from case by case, 

% Our approach in designing interfaces for customizability is to identify all the ways a design pattern can be made customizable. This way first identifies the customizability needs, and by evaluating their utility, we justify their need.
% We focus on all the customizations needed for the design pattern, \textbf{then} we will think about how to support these customizations in the implementation.



% Another line of research has prioritized expressiveness and allowed end users to customize their interface through software ustomiziations

% Another line of research has instead prioritized \textit{expressiveness} by opening the interface code to the end-user, allowing passionate developers to extend the interface their own needs. 
% Another line of research has instead prioritized expressiveness and power by opening the interface code to the end-user, \changed{allowing developers to address features or information that designers may not provide in the interface.}
% allowing passionate developers to extend the interface to others’ and their own needs. 
% Web browsers are notable examples of this case, where compiled HTML, CSS, and Javascript code are made available for end-users to view and change. 
% Researchers and developers have capitalized on this opportunity to support a diverse array of \changed{customization scenarios}, including website prototyping \cite{Kim2022Stylette, Visbug2024, Tanner2019Poirot}, note-taking \cite{Romat2019SpaceInk}, and filtering, sorting, and making spreadsheet computations \cite{Litt2020Wildcard, Huynh2006Sifter, Hogue2005Thresher}. Research has also explored the potential of web mashups and automations \changed{enabled by direct manipulation and programming-by-demonstration techniques} \cite{Ghiani2016WebMashup, Bolin2005Chickenfoot, Hartman2007Dmix, Huynh2006Sifter, min2023masonview, Lin2009Vegemite}.
% \changed{The direction for a customizable web has even been further explored with Webstrates by enabling end-users to build web software that is shareable, modifiable, and extensible across different platforms \cite{klokmose2015webstrates, radle2017codestrates, varv}.}

% \changed{
% While these web browsers and web platforms provide the expressiveness to design customizable interfaces, they are inevitably limited by the data provided from compiled websites.
% Customizations that only involve the front-end (e.g., color, font-size, or annotations) would not are not limited in customizability, 
% Consequently, it can become challenging to provide 
% Consequently, providing customizations involving deeper changes to the software stack, such as tweaking APIs to fetch unshown information or rearranging view layouts, can become an uphill battle against the browser's environment.
% an uphill battle against the available data.
% it can be technically challenging to support information and layout-heavy customizations for the overview-detail interface that involve deeper changes to the software stack
% \bryan{There are cases of extensions receiving adoption}
% \bryan{Furthermore, without knowing what kinds of overview-detail interface variations exist in the wild, an web extension that is only compatible with a small subset of overview-detail implementations could surface technical complications when addressing more variations.}
% \bryan{Furthermore, }
% , can only be made possible from within the website.
% }

% Instead of providing a solution as browser extensions,
% Two perspectives
% Focus on enabling designers to provide customization features
% Provide customizations as part of design patterns in interfaces

% To motivate this, browser extensions problem should be focused on designers -- what do the designers do?
% Designers will design an interface with default features and functionalitites, but if it's not enough for customizations, the end-users will end up developing them.
% Some cutsomizations can be implemented and demonstrated as browser extensions, but certain desgin patterns simply can't. 

% \changed{
% In order to design for customizable interfaces that involve deeper changes to the software, we aim to help designers make more customizations in interfaces as default functionalities.
% Designers will use and implement design patterns, so our approach is to provide customization features alongside design patterns.
% We instead take the approach of designing for customizability by making individual design patterns and 
% We approach designing for customizability with the goal of presenting customization techniques to designers first and by tackling customizability one design pattern at a time.
% }

% would require changes by the designers, developers, and organizations that create website.

% UI design has many interface design patterns, and among those are many variations. Of these variations, there are many needs for customizability. And also designers utilize and implement many of these design patterns.


% \changed{
% % Basically, we find all variations, see how these variations can be made available to the end-user
% % Browser extensions can't do that because there's only so much they can allow you to customize. To achieve more expressive customizations, you need to take this approach.
% % Making things more visually closer can be good, but this is hard to keep repeating for more interfaces.
% % Our approach to designing interfaces for customizability is to provide customization techniques that generalize across all implementations of a design pattern.
% % Our approach to designing interfaces for customizability is to 
% % Lines of research have done analyses on customization features that are avaiable and how people use them (wendy)
% % Lines of research have also extensively studied many design patterns and many forms of information, representations, and interface components (Maug, ASCII, dashboards, DataParticles, Logit)
% % And many forms of research have explored transformation of representations, variations, etc (WritLarge, VizFlow)
% Our design pattern approach of making interfaces malleable brings these three stages of study, analysis, and design, and contributes a systematic methodology for researchers to realize broad applicability of customizations, and influence more designers...
% Design pattern approach takes the perspective that useful customizations that are widely adopted across many interfaces can be more commonly leveraged.
% A case of this is sorting and filtering, which are customizations of what information is shown. This customization is made on the collection design pattern.
% Similarly, we stand that choosing what kinds of attributes to show or hide can become a commonly leveraged customization on the overview-detail pattern.
% % Our approach similarly takes the design pattern approach that prior research has taken, but we explore a systematic approach to tackling this by leveraging all the variations that already exist out there today.
% % Our approach is to look at design patterns. 1) what are the customizations available already? 2) what are the variations of the interface? 3) Can we let the end-user control which variations they want under this design pattern?
% }




% \changed{One line of research has taken the perspective that certain customizations such as system settings are not discoverable enough and are too costly to access. }
% To balance this trade-off, several approaches have been explored to design interfaces for customizability. 


% Strat is to start with concrete approaches, and then evaluate them through ease, expressiveness, broadness

% Q: How to design interface that's customizable?
% 

% Making the software customizable first
% Web browsers --> extensible software, but it's not enough for everything
% We see that not only are websites cusotmizable with extensions, people are creating extensions that also provide more customization features.
% Webstrates, varv --> extensible software



% Wendy --> tradeoffs, so you need to design customizability techniques that balance these tradeoffs.
% Approach is to lessen the friction to accessing certain customizations, and allow customizations to reduce the friction to accessing certain features
% Moving settings options visually closer to their functionalities and components, and also let users customize which features/functionalities are visually closer to end user


% So the first one is not really relevant to "approaches"
% Browsers give the power to customize to the end-user
% We provide design solutions for designers to implement these customizations

% Web browser and extensions to enable end-users to extend on their own, and also provide these customizations to other users who can't make this software.
% This approach allows for developers to customize as much as what's available to them, while also letting end-users get some of the benefits if it's available.
% This approach for the browser faces limitations because the software stack is just limited in that way.

% Our approach is to enable customizability through design patterns and this would influence designers to implement customizations.

% \changed{
% Thus, other lines of research has emphasized \textit{ease} of customization with the goal of making customizations less costly to perform and more discoverable.
% \bryan{First, researchers have focused on this aspect by providing a secondary, ``Personal Interface'',
% % McGrenere et al. provided two interfaces, a ``Personal Interface'' and a ``Default Interface'', 
% which encouraged users to rearrange menu items with the original menu arrangements in tact \cite{mcgrenere2007twointerfacecustomization}.}
% }
% Ponsard et al. explored how moving setting options visually closer to conceptually related UI components could provide a more ``in-situ'' way to access customizations \cite{Ponsard2016AnchoredCustomization}.
% \changed{While these are great, these customizations can have different nuances for each application and each interface design will require specific designs to think through to enable these customizations.}




% Stylette makes it easier to make style customizations through voice and LLM basically
% 

% The goal is to make customizations broadly adopted, to make it feel like a regular interaction, similar to sorting and filtering.
% They naturally balance three aspects in designing for customization: ease of customization, expressiveness, and generalizability across many interfaces.

% So rather than letting end-users only build software for themselves, this extensible platform also enabled end-users to build extensions for other users and many kinds of websites. Customization features that are broadly applicable to many interfaces. --> to impact many users.
% the approach was to leverage the expressiveness that browsers provide and design and implement individual customization features to be broadly applicable across many websites.

% While ease of customizability makes it more discoverable
% \changed{Another approach to designing customizable interfaces is to emphasize broad applicability, and through generalizable customization techniques, can influence more interfaces to adopt them and enable end-users to grow more accustomed to those customizations.}


% \changed{Thus, designing interfaces for customizability not only require ease of use and expressivity, but also require \textit{broad} applicability.}


% While all the above approaches have their benefits,
% we emphasize broad applicability of customizations, but take the perspective of tackling broad

%  But when you look at this literature, these also are broadly applicable, like sifter is hypothetically broadly applicable across all list items on web.


% Which dimensions of software interfaces can be made customizable



% Start with saying "The web is a great place and stuff."
% I like how I can mention Bonnie Nardi, (I first need to read the book to make sure she actually says this lol). But this then turns the direction to opening the programming environment to the end-user, so I feel it should not go in that direction. At the same time, Webstrates is a very influential line of research for customization. It's made so the end-user can customize the web code itself, and enabling the software to be collaborative/shareable at the same time. In that way, there isn't really anything that's designed to be customizable here. Varv and Webstrates is more on the level of Web Browsers, so I should move these earlier possibly.
% \changed{However, it is simply too difficult for designers and developers to anticipate all forms of customizations end-users may need \cite{Nardi1993SmallMatterProgramming}.}
% \changed{Instead, lines of research have explored web platforms where end-users can write code extend software 
% \changed{Will talk about open programming systems, Zhang2018Fusion}
% collaborative dynamics with shareable, modifiable, and extensible software across multiple different platforms \cite{Klokmose2015Webstrates, varv}. }
% \changed{A notable example of this case is the Web, where web browsers provide compiled HTML, CSS, and Javascript code for end-users to view and change.}
% \changed{This has also allow end-users to p.....}
% Researchers and developers have also built upon the open programmability of web browsers to support a diverse array of tasks, including website prototyping \cite{Kim2022Stylette, Visbug2024, Tanner2019Poirot}, active reading and note-taking \cite{Romat2019SpaceInk}, and filtering, sorting, and making spreadsheet computations \cite{Litt2020Wildcard, Huynh2006Sifter, Hogue2005Thresher}. Research has also explored the potential of web mashups and automations \changed{enabled by direct manipulation and programming-by-demonstration techniques} \cite{Ghiani2016WebMashup, Bolin2005Chickenfoot, Hartman2007Dmix, Huynh2006Sifter, Lin2009Vegemite}.
% \changed{While these platforms and extensions have prioritized ease of customizability for the end-users, but have also make these customizations }


% The platforms that emphasize the expressiveness of customizability focus on opening the interface code to the end-users. Web browsers are a notable case. 
% While this approach provides an expressive way to customize interfaces, \changed{not all end-users are able to or willing to write software code to address their own needs.}
% it can be difficult for end-users who lack the time or skills to make these customizations.

% browser based --> allowing extensibility. This allows end-users to code things up to customize on their own
% Also enables them to provide UI solutions so end-users can make certain csutmoziations easier without code. For sinteadnce tehre are browser extensions that can customize this this and that.
% Designing custmoizablt interfaces throuhg open code has been pushed furhter through webstrates making wiht blah blah blah.
% While this approach is great for certain aspects of customizatino, there's limitations for certain kinds of interface customizations that require changing deeper aspects of the stoftware stack such as APIs and whether to route to a new page or to instead create a split view within the same page. We find this approach is not fully suitable and appilcable for design patterns such as overview-detail interfaces




% 1. Wendy says, it's not leveraged as much. So research has tried to make things more discoverable and easily customizable. However, there's kind of limitations on how far these customizations can go (Bonnie). You need aspects of ease, but also need expressiveness.

% 2. Indeed, there is only so much you can do in terms of expressiveness. But if you design your software to be more open, this allows programmers to extend your software, making is more expressive to enable customizations and extensions. In this line, there's even people who added wrappers to enable end-users to customize through the interface specific aspects of the interface by leveraging these open-code platform designs. However, broad applicability can be a technical challenge, especially if things need to be scraped. Indeed if customizing UI style through CSS, that's been done with Visbug and all those other tools, but customizing which information is shown through browser customizations might not be as easy. Sifter has shown a method through scraping, Wildcard has proposed a community-driven movement. These are certainly powerful, but ultimately, the fullest power to choose which features are in websites or not inevitably come from the website providers: designers, developers, and organizations. They can be convinced to implement great features from end-users (which happens all the time), but this approach is indirect compared to if you can influence the designer directly.

% 3. Thus, in order to see broad applicability and adoption of customizations in interfaces, it can start from the designers. Designers leverage design patterns to build their interfaces, it's certainly possible to recommend customizations in these design patterns to demonstrate that these customizations are available as design options. This design pattern approach involves 1) analyzing customizations available, 2) analyzing pattern variations, and 3) exploring techniques to allow end-users to transform between these variations.
% Lines of research have done analyses on customization features that are avaiable and how people use them (wendy)
% Lines of research have also extensively studied many design patterns and many forms of information, representations, and interface components (Maug, ASCII, dashboards, DataParticles, Logit)
% And many forms of research have explored transformation of representations, variations, etc (WritLarge, VizFlow)
% Our design pattern approach of making interfaces malleable brings these three stages of study, analysis, and design, and contributes a systematic methodology for researchers to realize broad applicability of customizations, and influence more designers...
% Design pattern approach takes the perspective that useful customizations that are widely adopted across many interfaces can be more commonly leveraged.
% A case of this is sorting and filtering, which are customizations of what information is shown. This customization is made on the collection design pattern.
% Similarly, we stand that choosing what kinds of attributes to show or hide can become a commonly leveraged customization on the overview-detail pattern.


% ^ the term broad shifted meaning.
% First, broad meant a customizationn can be broadly appklied to a bunch of interfaces
% But then at the end, broad was use to say you can provide many many kinds of cusotmizations/transformations.

% In this research, we aim to make the customization techniques easy to discover and achieve and also aim to make them expressive to the extent of the design pattern. But our focus is to explore how our approach for exploring and realizing broad applicability for customization techniques can be used in the overview-detail interface......

% So now I have a better draft/thought process on how I'll write this. I'll try it out, then write it out, see how it reads!
% Taking a break now, and then gonna get back to writing



% CASE BY CASE APPROACH: Implement customizations features one by one on a needs basis
% One application may implement a customization feature based on their use case, but similar applications may not implement that customization, maybe because they don't know or find it worth implementing.
% Applications will have their own unique set of settings and features implemented unique to their own app.
% But these idiosyncracies can be hard for end-users to utilize, and not every application may address the same customization need.
% So I'm like considering whether it would be relevant to add Anchored Customization to this... Not sure if it's relevant anymore
% I'll think about this tomorrow, but it makes more sense to organize these by approaches to designing interfaces.\
% But Bonnie Nardi says there's only so much you can let the end-user customize. This is true.

% In light of this, we even can try to go as far as possible, even if there is this boundary.
% OPEN APPROACH: Open the code to the end-users
% 1) End-users will program themselves. This design choice gives end-users the ability to customize their software very expressively. However, it's not the easiest to gain those skills. It also just takes time to code, even if you did have those skills.
%  2) That's why these open code platforms also support ways for end-users to find and use software custmoizations made by others. These customizations in the browser would be browser extensions that can 1) provide a particular variation of the interface, such as a software extension, like a new overview, a new UI style. 2) but there are extensions that allow the end-user to more easily access/create customizations, visbug, sifter, wildcard, vegemite, etc.
% However, browsers only provide compiled code and data, requiring end-users to scrape data, which even does not guarantee all the available data will be saved---won't reflect the real data in the application's database and model.
% So while there is merit to designing systems that enable end-users to create their own customizations through code and make them available for the wider user-base,
% If customizations can be designed from within the organizations that build these websites, it would be much more effective and stable (not to mention community/end-user created features are commonly adopted and implemented into main products).

% DESIGN PATTERN APPROACH: Explore how interfaces under a design pattern can be made customizable
% Designers leverage design patterns to create common abstractions of certain design elements in interfaces.
% So by exploring how design patterns one at a time can be made customizable:
% Design patterns helps us understand a very clear big picture applicability for customizations.
% Cause maybe oftentimes customziation is not seen as valuable as it really is for the cost to make it.
% Helps us understand how broadly implementable certain things can be
% Ultimately, users are the invariants in interaction with software.....

% One design pattern that is also considered to be a UI component is to see how menu lists can be customized.
% One is to explore need by need: on a needs basis, discover a customization feature one might need
% Old times first explored menu lists, simply making menu items rearrangeable
% Giving the user the control over this is preferred over adaptive menu lists.
% It's very clear how generalizable this can be: it at the very least generalizes to the design pattern.



% Our approach similarly takes the design pattern approach that prior research has taken, but we explore a systematic approach to tackling this by leveraging all the variations that already exist out there today.
% Our approach is to look at design patterns. 1) what are the customizations available already? 2) what are the variations of the interface? 3) Can we let the end-user control which variations they want under this design pattern?

% But not only can we do that, but we can also provide designers a systematic approach to making more of their interfaces more customizable.
% Designers rely on and leverage interface design patterns, so an approach could be to look at design patterns blah blah...

% let's call it after this. Don't make this too long.

% -----------------

% What to customize is needed by end-users, but not provided by designers. the end-users choose to make those customizations on their own.
% This is powerful for giving the control to the end-users
% One concern could be that this knowledge might not go to the designers
% And maybe there just doesn't become a guideline for what should be customizable from the start.

% We believe these customizations should be broadly applicable, and rather than doing some cat and mouse chase for end-user development.

% Customization should be thought about from the start by the designers first. Then end-users can continue to contribute more customization features.

% Basically saying, wouldn't it be nice if these customizations just came from the softwrae from the first place?

% To make these customizations from the first place, perhaps designers need a systematic approach to understanding what kinds of customizations people could be making.

% To understand what kinds of variations users may want to transform to, which customizations they would want, but also need some unified way of understanding what these customizations are for.


% All i have to find is what's the weakness of the end-user customization through open code
% First, this is done in compiled code. 
% But there's things like webstrates and varv that would make the code open by default and malleable

% Also, this end-user development perspective may not directly influence the design choices of the designers.
% Might even disincentivize them to design for customizability because end-users can do it anyways.
% Dang, i feel it there's like something that's missing in this argument though.

% if we want more customizable sfotware, it should start from designers who influence what gets implemented ultimately.
% opening up the code to end-users to customize does influence designers on what to implement, there are certainly many cases of extensions becoming realy features.

% \bryan{This one is the one to use}
% Well opening up the code is good for end-users



%  ---------

% Settings + Anchored Customization: Trying to make interfaces more customizable by tackling the discoverability side of things, but focusing on what's available in the settings pages basically.
% This could be unique settings for each application or for a common feature, such as notifications.
% This is hard to tweak because there are so many settings to go through.
% One way to address this could be with Anchored Customization, where the difficulty of finding settings and customizations that the end-user needs is addressed by placing the setting visually closer to the component that is customized...
% This is not that relevant.




% ^ Perhaps an argument for these works are that they are focused on one particular interface only?
% Settings page is unique to a single application.

% Opening the code to end-users to develop for people
% 1) this is challenging for any end-user to build their own thing
% 2) that's why people provide end-user extended/built software for others to use, such as sifter
% End-users can customize, it's broadly applicable

% We want to provide the strategies for designers
% Our approach is to understand and focus on design patterns, see what the variations of these design patterns are, and then see how we can provide end-user friendly interactions to enable the


% Right now, this section talks about how customization is enabled to the end-user. But rather, the focus should be considering WHICH aspects of customization of the interface should be enabled.
% Theme should be centered around Nardi's quote, saying you can't make everything customizable.
% This should go into which interface aspects should be made customizable, which aspects might be made adaptive by the system, and which are chosen as good defaults to begin with.
% A start to explore is in menu items. This explored whether user should customize, or let the system personalize for them.
% Then explore the other types of things that are commonly customizable.
% But ultimately can't cusotmize everything
% This paper, however, explores a very ubiquitous pattern, and making this customizable, would hopefully support more diverse needs through this simple, single pattern
% Hoping this end-user techniques are expressive enough as well

% Designing for customizability
% 1. Settings. Not easy to just access (Menu). So one line was to provide settings that are easier to access on the interface
% 2. Browser customizability. precise control over specific needs, but lots of code.
% 3. Enabling prompts for user to ask for specific changes. AI is expressive, but volatile. 

% So how can we enable easy (1), precise (2), and expressive (3)

% We need a vocabulary for users to share their needs in an easy (1), precise (2), and expressive (3) way.


% Maybe what's hard is that I just don't know the literature around customization, why software customization 

% What are all the possible forms of customization? One perspective is allowing customization at which level of the s...

% interface customization --> default is a settings panel, basically choosing to customize through settings
% Brought that more in-situ with Anchored Customization
% 



% \changed{Browsers' openness have enabled researchers to ...}

% If the framing is all about how we identify ODIs and we want to make this customizable because we have this really general technique,

% \changed{End-user programming and providing a community for end-users to create and share customizations is really powerful \tocite{Wendy's sharing customizations paper}. Providing this open code from the outside might not be viable when we want ODIs to be customized, especially moving around attributes across different views because that would require more than just the compiled code available (saying there are limitations).}

% \changed{To design customizable overview-detail interfaces, we take the approach that while not code is not available, we can achieve expressiveness of what can be customized }


% \changed{This is definitely useful, but if we want to support overview-detail interface customization, especially customizing attributes, is difficult to implement as a browser extension}


% \changed{Bonnie Nardi, a Small Matter of Programming: You simply can't make everything customizable}

% \changed{I wonder if this section is relevant at all.... }





% ~~~ TODO ~~~
% This section is really here to start arguing that our method of cusotmization is to make attributes manipulable. We say that this approach is expressive because you can control all attributes, it's comprehensive in that you control all possible attributes, so it's more expressive than these limitations of adding extensions. So it should be as expressive as open progrmaming, but it's also easy because it's no code. 
% The thing is is that our contribution is simply not that. We're not contributing a customization technique.
% So basically, this section might not be good to even bring up or emphasize as much...







% Outline
% One approach towards making interfaces reconfigurable is by lifting the attributes of items and objects to be manipulable.
% 



% Customizability is about making things that are not end-user changeable to something the end-user can change. A method for getting to this higher control has been through attributes, namely making attributes of objects and items manipulable by the end-user.

% These are all about lifting attributes to the interface to make them manipulable by the end-user.
% In data visualization interfaces, where the data is extremely closely bound to the interface, which makes it natural for end-users to manipulate and customize the visualizations by their attributes.
%  Data Visualizer CHI 2018

% Line of work explored in making attributes manipulable in content creationg tasks, creating graphical objects with attribute objects, managing many objects efficiently, and creating data visualizations with drawings and visual encodings.

% Attributes have also made its way into information management systems, such as MS Access and FileMaker Pro...
% More modern systems such as Notion and Airtable also similarly support ways to show and hide attributes from lists of items...

% Architecturally, The Haystack project has took upon such techniques to make attributes of items end-user manipulable.
% Haystack allows users to add and hide properties to the object that is displayed on the interface, even allowing them to define new properties.
% Haystack's primary datatype being a collection of objects enabling users to manipulate attributes across the entire collection.

% Our focus is on the overview-detail pattern. The uniqueness of this pattern is that this is extremely ubiquitous. 

% What's unique about overview-detail
% There are more dimensions to make customizable
% In terms of the design, the detail view presents most if not all attributes of the object. This makes it an intuitive interface for the end-user to see the attributes the user can surface in the overview.
% Compared to data visualization systems, overview-detail interfaces may not necessarily reflect the underlying data or even schema of the software system.
% While attribute manipulation is a generally common technique across different domains, we contribute designs to make manipulable attributes more intuitive and natural for end-users on everyday overview-detail interfaces.



% We focus on overview-detail, which further enables us to explore how end-users can more efficiently surface information on the interface + can also explore how different dimensions of customization such as different layouts can also support attribute manipulation.



% Using attribute to model piece of information is really common. Because things are modeled this way, that's why so many things are manipulable. 


% Our work aims to empower everyday users to customize their overview-detail interfaces




%  beyond database-oriented workspaces and personal information management systems.
% It is our recognition that these techniques can generalize across all kinds of overview-detail interfaces that makes our work a novel contribution. 
% Originality: There are so many interaction techniques for specific implementations of ODIs; we recognize that there are common interaction techniques can be implemented in many diverse ODIs.
% Significance: We provide a framework to push the design and utility of malleable ODIs for the future.


% The underlying data model that is presented by overview-detail interfaces involves different sets of attributes: one for the overview and another for the detail view. 
% Our insight is that overview-detail interfaces contain different sets of attributes for the overview and the detail view, and} by treating attributes as first-class citizens and making both the attributes and views accessible and manipulable, we can enable end-users to flexibly customize them.




%  I want to say something about how this novel direction of studying this generlizability also feeds into the value of our user study... but I think I can talk about this in the intro instead. --> I really want to emphasize the importance of the user study. It's really important imo.

% \bryan{I want to also mention that ODI is used when exploring and searching for information. When the user has first entered the website and is completely new to the information presented. I'll have to choose between one of these arguments to keep the flow of the paper.}

% It is our recognition that these techniques can generalize across all kinds of overview-detail interfaces that makes our work a novel contribution. 



% Originality: There are so many interaction techniques for specific implementations of ODIs; we recognize that there are common interaction techniques can be implemented in many diverse ODIs.
% Significance: We provide a framework to push the design and utility of malleable ODIs for the future.



% By treating attributes as first-class citizens and making both the attributes and views accessible and manipulable, we can enable end-users to flexibly customize them. This resembles the line of work on attribute objects by Xia \etal{} \cite{ObjectOrientedDrawing, Xia2017CollectionObjects, DataInk}. By decomposing graphics objects into attribute objects, these systems enable users to flexibly compose new graphical styles, search for graphical objects with attributes as filters, and create data visualizations by combining data and visual attribute objects as visual encodings. Our work arrives at a similar approach but explores interactions with attributes in the overview-detail design pattern, rather than on content creation. A unique step forward in our work is that, in addition to flexibly manipulating developer-defined attributes, we also enable end-users to leverage AI to create user-defined attributes, further expanding the expressiveness for end-user customization.

% TODO: Add Data Visualization domain of surficing and hiding attributes
% Luminate
% 

% Done in content creation, creating new graphical styles

% TODO: Discuss database-oriented interfaces (MS Access and FileMaker Pro), Notion and Airtable, and then Haystack

% These

% NOTE: Maybe I will need to frame Fluid Attributes as an interaction technique that we find to be commonly applicable to many overview-detail interfaces, and our section is not to necessarily claim novelty, but to demonstrate the broad applicability of these techniques. 


% While it can feel natural for notion or airtable to translate the show and hide columns to show and hide attributes in other representations, its nonobvious that this type of customization can translate to a shopping interface or news article website. Cause databases and tables already reveal the attribute by default. we identify that these customization techniques translates to the entire overview-detail design pattern, and in turn provides efficiency benefits in all kinds of tasks. Thus we contribute knowledge that techniques like these are extremely generalizable across diverse domains. I just need to make sure that haystack and those didn’t claim these first…

% We contribute knowledge and these variations and these customizations can be designed for and implemented across overview detail interfaces. So while applications can have designs, we demonstrate how these can be designed in these tasks

% It’s not enough to simply state a difference; you also need to explain why this difference matters. Frame your contribution as a necessary or even “obvious in hindsight” step that others had not yet taken. This positions your work as a natural progression or a gap that “had to be filled,” which can make your originality argument more compelling.



% Our goal is to demonstrate how these techniques can be adopted for use beyond database-interface products like Notion and AirTable
% The novelty of our paper does not lie in all of our presented interaction techniques, but rather our exploration of such techniques across the many domains that overview-detail interfaces are implemented in. 
% Instead, 

% \changed{}

% This is customization, so where does this paper sit relative to other customizable systems?
% This paper is NOT at all about how you customize. it's about how you design the customization.
% So it should be about what kinds of software interfaces have been made customizable
% What other aspects, not overview-detail, but just any, aspects are made customizable.

% ~~~ CLEAR DIRECTION FOR REVISING THIS SECTION ~~~
% R2 brought up the concern that this paper does not address a crucial question of "how to enable these customizations in the real world". We fully agree that this is an important and exciting challenge to explore. We realize that section 2.3 may mislead readers to think this paper explores techniques and approaches to unlock these customizations with the goal of answering the previously stated question. However, our goal for this paper is to focus on which aspects/dimensions of software interfaces have been made customizable. We revised section 2.3 to focus on the customization aspects, rather than how these customizations would be made.




% How to make the Actions customizable
% \changed{HyperCard makes events and actions composable, letting users customize actions and tasks.}

% How to make the Representation and Arrangement of Information customizable
\changed{Other work makes the style of web elements customizable}
\changed{Webstrates lets users customize web documents, their style and representation.}
\changed{Location of written notes on the Web customizable}
\changed{Making specific web components and views mashup-able and automated}
\changed{Arrangements customizable (filtering and sorting)}

% How to make the Data Model customizable
\changed{Smalltalk makes \textbf{objects} in software systems customizable}
\changed{Haystack makes \textbf{data schema} and their \textbf{views} customizable.}
\changed{Wildcard models data on websites as an \textbf{editable spreadsheet}, introducing opportunities for data customization}

% How to make interfaces in a Design Pattern customizable
% We make representation, arrangement, and data model customizable, but for the entire design pattern.
\changed{Our approach is to make design patterns customizable.}
\changed{Wildcard similarly maps collection data to a spreadsheet, saying collection items map to a table model, but they don't explore all the aspects of customizability for a spreadsheet.}

% Other work explore making Representations and Arrangments customizable, but they ultimately don't consider other aspects to customize, so there are these issues. Do these designs conflict with ways to make something implementable?
% There's making Data Models customizable, but they don't consider representations and arrangements..?
% What's the problem with only focusing on these aspects? this argument insinuates that you can't have all of these customization solutions in a single technical implementation.







% After this design space for how this design pattern can be made customizable. We then evaluate the utility of these customizations.
% Analyzing the design pattern provides a scope for exploring all of its variations tand evaluating the utility of customizing.
% how customizations can generalize to interfaces that designers might not necessarily anticipate support customizations on.
% By analyzing all variations and customizations of the design pattern and evaluating the utility of these customizations first, 
% , and then considers how these customizations can be implemented through a browser extension or a web framework.

% We decouple the design opportunities from its implementation details, 
% We decouple the design opportunities from its implementation details, allowing us to fully explore the broad  of the design pattern.


% \textit{As has been shown time and again, no matter how much designers and programmers try to anticipate and provide for what users will need, the effort always falls short because it is impossible to know in advance what may be needed.}
% However, adopting a new infrastructure can take time, especially given the widespread use of web browsers.

% \bryan{We're saying how do we make interfaces more customizable by trying to make the system itself more customizable, making it more open and all that. And from this, we've learned that basically it's impossible to build a fully customizable system because we simply can't anticipate everything users will want to customize \cite{adar1999haystack, Nardi1993SmallMatterProgramming}. Given this fundamental limitation, this means we shouldn't be aiming for this perfect customizable system in just one try. So, research explores case by case, need by need customization. This is in the example of supporting tasks or supporting specific features. However, user tasks are always transforming and features... So we should be looking at something that's more invariant; that is the design pattern. Our approach is to make design patterns customizable first. }

% \bryan{We can't anticipate all the ways an interface would want to be customized. So the design pattern gives us a bigger, task-changing-proof approach to seeing how to build systems that can be more customizable. Perhaps this design patterns actually helps us better anticipate what aspects users may want to customize.}

% \bryan{We show this approach is feasible through the many design probes we build, as well as the applicability across various tasks, but also across different devices (i.e., mobile interfaces)}
% \bryan{Basically, this section is all about how we can better anticipate the customizations we may need and figure out how broadly applicable these customizations can be.}
% \bryan{This sort of hints at novel technicaues, helps us find what new techniques are available? but that much.}



% \bryan{Idk if i can even say this here, but the main reflection here is that it's really not possible to make everything customizable. You simply can't anticipate everything.}

% \changed{Thus, another approach has explored supporting a specific task or a particular aspect of interface customization.}





% We have design pattern as a guide and a scope for the aspects to customize in the interface. Knowing the design space of customizability of design patterns, we then will know what are the technical requirements to support more expressive end-user customization.
% and provides a scope for how such customizations should be implemented, 


% Customizations are inherently context-specific, shaped by the diversity of workflows and the evolving nature of user tasks \textbackslash{}cite\{Nardi1993SmallMatterProgramming, Karger2007BDMHaystack\}. Efforts to generalize customizations based solely on software paradigms or individual tasks often struggle to capture their broader applicability. In contrast, design patterns, which remain consistent across diverse tasks and platforms, offer a more robust framework for understanding and extending customizations across varying contexts.
% While the above approaches of making fundamental aspects of a software system customizable and enabling customizability case-by-case are both effective in addressing their respective customization needs, there is no concrete guide for understanding how broadly applicable these customizations are to various other tasks and interfaces.
% Consequently, this may limit how widely a customization is adopted, making it challenging to provide these customizations after the fact.
% It is challenging to provide a comprehensive guide because every customization is unique, making it impossible to anticipate all the variations users might require due to the diversity of workflows \cite{Nardi1993SmallMatterProgramming, Karger2007BDMHaystack}. Although user tasks are constantly evolving, design patterns remain consistent across a wide range of tasks and interface platforms.



% leading to no other option to provide these customizations by refactoring the application's full-stack architecture or scraping the DOM across diversely structured websites.
% \changed{The reason there is no guide is because every customization is different, and it is simply impossible to anticipate every customization a user might need given how diverse our workflows are \cite{Nardi1993SmallMatterProgramming, Karger2007BDMHaystack}. While user needs and tasks are constantly changing, design patterns are consistently interacted with across diverse tasks and interface platforms.}

% \changed{To support customizability across these transforming user activities, to consistently provide cusotmizability should be on the materials users interact with consistently, which we identify to be design patterns.}
% \changed{Design patterns are designed based on what users commonly do to interact with our interfaces, no matter the task involved.}

% These package customization features 
% However, these system aspects on what to enable customizability are guided by the kinds of customizations their proposed system supports.
% Inevitably, 
% I should not say that you can't have all four of these at once. Let's just assume that you can support all four of these


% Another approach that takes a step towards making more aspects customizable is by identifying individual tasks that people do and individual aspects of customization to enable when it is often needed. For instance, ...
% Others look at individual tasks, such as note-taking website prototyping, and automations.
% Others look at individual aspects to customize, such as making content in websites filterable, sortable, mashup-able.

% \changed{While such case-by-case solutions are effective in their respective customization needs}
% user activities involve balancing many tasks often switching between them and \bryan{other...?} \cite{coststructuresensemaking}.}
% \changed{While such case-by-case solutions have demonstrated significant technical hurdles to achieve such customizations, they are constrained by the available web data in compiled websites. For instance, customizations tools that scrape web data through the DOM can only leverage data provided by the websites and cannot customize APIs or data schemas from the back-end. Such tweaks must instead be supported and monitored by the designers and developers of the websites.}
% \changed{However, user tasks are always transforming and features... So we should be looking at something that's more invariant; that is the design pattern. Our approach is to make design patterns customizable first.}
% \changed{Research has also pushed forward an platforms where end-users could gradually add features facilitate travel planning }

% it may be unclear how broadly applicable these customizations are to various other tasks or interfaces. Consequently, this limited understanding of broadness can constrain  
% difficult to concretely identify the scope of which these customization techniques generalize across interfaces today. 


% demonstrate value for understanding how a specific customization works on many kinds of interfaces, this is way too specific, trying to handle customizations one at a time, making it unclear how generalizable these customizations are to other kinds of tasks or websites. This could limit how widely a customization is adopted in many kinds of websites.}

% However, it is impossible to anticipate all diverse needs of end-users, which may in fact drastically differ from the provided customizability properties these systems are designed for \cite{Nardi1993SmallMatterProgramming, Karger2007BDMHaystack}.
% I shold try to say that these systems are not guided by design patterns, so it's hard to see how widely the range of interfaces these customizations generalize to.


% \changed{
% There's this tradeoff to balance in end-user customizable software, where to be more expressive with the customizations you want to make, you need to make it more programmable which requires more code. On the other hand, if you want to make it easier to customize, you need to provide case-by-case interfaces and interactions to enable this.
% Our approach 
% }
% \changed{Many lines of work have aimed at designing software with end-user customizability in mind, with a notable approach being to allow the end-user to opening the system software and data schema.}
% % Many lines of research have explored approaches to making interfaces more customizable.
% % One approach explores has been to design new infrastructures with end-user customizability in mind. 
% \changed{Systems such as Smalltalk \cite{kay1993smalltalk} and HyperCard \cite{Hypercard2024} enabled users to customize their interface by modifying objects in the GUI and creating scripts that link actions such as mouse clicks together.}
% \changed{
% Web systems such as Haystack \cite{adar1999haystack} and Webstrates \cite{klokmose2015webstrates} also explored web infrastructures that allow end-users to define their own data models, create custom views, develop different representations of the same DOM element, and extend their software to support custom functionalities.
% \bryan{I want to interweave this knowledge, that it is impossible to anticipate what end-users will need \cite{Nardi1993SmallMatterProgramming}.}
% }



% \changed{Our goal is to make interfaces malleable, and the first step to achieve this is to understand all the aspects of interfaces to be malleable for the interface.}
% \changed{We should also understand the broad applicability of these customizations.}
% \changed{A fundamental aspect of malleable interfaces is that customizations a user may want is widely available across a variety of interfaces.}
% \changed{This can be seen in many end-user programming environments, where users are able to create their own scripts to automate a task they would do in many various settings}
% \changed{This support is reflected in Smalltalk and HyperCard...}
% \changed{On the other hand, Haystack allows users to define their own data models and create custom views.}
% \changed{Webstrates allows users to create different representations of web content, enabling dynamic interaction opportunities on the Web.}
% \changed{These forms of customizations have been developed with the spirit of building systems with end-user customizability in mind...}
% Can't say these aren't end user friendly, this shouldn't matter.
% This is about discovering the broad applicability of a customization.


% \changed{
% While the above approaches of making fundamental aspects of a software system customizable and enabling customizability case-by-case are both effective in addressing their respective needs, they do not focus on scoping how broadly applicable these customizations might be across different tasks and interfaces.
% Most of the above work, however, either do not define the scope of generalizability of their customizations or provide a scope defined by the technical 
% Most of the above work, however, lack an explicit scope the customization techniques 
% They don't focus on recognizing and detecting the design patterns first. Consequently, 
% reason why i can't say this is because you haven't explained why desgin patterns is the solution.
% Most of the above work, however, focuses on developing specific systems for specific types of activities or on specific platforms, and 
% Sifter does concretely scope, just not well enough.
% do not concretely scope how broadly their customizations might apply beyond their demonstrated interfaces.
% \bryan{There is no explicit scope, there's no design pattern}
% For example, Sifter detects list items on websites by first detecting a 
% }
% While the above approaches of making fundamental aspects of a software system customizable and enabling customizability case-by-case are both effective in addressing their respective needs, they do not focus on scoping how broadly applicable these customizations might be across different tasks and interfaces.
% Haystack allows users to modify attributes shown in the interface, while Sifter detects item attributes on websites to make them sortable and filterable.
% Haystack ... idk yet
% Haystack
% Wildcard also makes collections of items customizable but demonstrates its generalizability through several augmented websites, allowing developers and end-users to identify which interface variations to support.



% Of the above work, most similar to our approach are Sifter \cite{Huynh2006Sifter} and Wildcard \cite{Litt2020Wildcard}.
% , implicitly utilizes the overview-detail
% Consequently, there becomes limitations when broadly applying their customization techniques across more interface variations that match in the design pattern, but do not match in DOM structure.
% Developers may extrapolate what other variations interfaces 

% However, Sifter detects list interfaces through the pattern in the DOM structure, while Wildcard's approach relies on developers and end-users to identify which interfaces to support.
% data extraction modules are left for programmers and end-users to 
% , not the design pattern of the interface itself.

% generalize customization techniques found in all of these interfaces to contribute 
% understanding how customizations from one overview-detail interface can generalize to all other interfaces in the pattern.
% that can apply our customization techniques in.
% We investigate the overview-detail design pattern.
% This design pattern as a guide for concretely recognizing 
% This design pattern serves the research community as a guide for both concretely recognizing all of the interface variations that exist in the wild and understanding how customizations from one overview-detail interface can generalize to all other interfaces in the pattern.
% one should implement their cusomtization features to support the whole pattern
% providing the research community 
% we explicitly identify the design pattern to provide customizability for. 
% In contrast, we focus on an interface design pattern that is ubiquitous across diverse information systems and platforms--the overview-detail pattern. 
% remain consistent across a wide range of tasks and interface platforms. Therefore, we instead approach designing interfaces for customizability by first exploring all the ways a design pattern can be made customizable.
% We first analyze the design pattern by exploring all of its variations and existing customizability features, and then provide interface solutions to making these variations transformable by the end-user. 
% The design pattern serves as both a guide for concretely identifying the broad applicability of customization techniques for interfaces and a framework for informing how to implement these customizations, whether through a browser extension, a front-end UI library, or a full-stack web framework.
% Given how closely overview-detail interfaces bind to the underlying data models, we apply this design pattern-centered approach to making overview-detail interfaces malleable.

% \bryan{dont' make the design pattern as explicit---we recognize generalizable pattern.}
% \bryan{we recognize all the variations}
% \bryan{reasonable generazliablility}
% \bryan{our investigation is more concrete}
% \bryan{it's unclear how to apply that to another overview-detail.}
% \bryan{with some extrapolation, it's not directly applicable, but it's really actionable on how to identify interfaces that work}
% \bryan{Don't forget there are two other dimensions in our space --- you can layout and composition, which means that we are exploring how all of these customizations integrate into a single design pattern..?}
% \bryan{how to manage different views}




% \bryan{For example, Haystack...}
% \bryan{Whereas Wildcard...}
% \bryan{Consequently, limited in what to customize; limited in what's implemented...}

% \bryan{food ordering on the phone is same as email, same as ...}

% \bryan{For Haystack, I don't think it's even designed to be broadly generalizable to other applications because its principle for having personalized information environments is so deeply ingrained throughout its architecture.}
% \bryan{The feeling I get is that that sentence does not necessarily apply for Wildcard or Sifter because those are pretty clearly applicable as a browser extension. And their scope is pretty clearly defined. The problem I see with these two systems  is that it's just not consistent/reliable. As in, Wildcard won't work unless the ``community'' makes these integrations, while Sifter needs to be able to successfully scrape the list website, and it claimed to only work for ``clean'' websites (not to mention, it's a system from 2006). But I guess, our system shares this limitations since it will only ``work'' if the developers actually develop these customizations.
% Wildcard probably does the best job of showing the scope of applicability since it basically says you can do this for any interfaces with a collection structure.
% The difference is that it doesn't recognize the design pattern as the core thing to enable customizability for.
% }
% \bryan{Note: There's also Visbug, which very easily generalizes to all CSS style attributes, but this is a completely different dimension of customization.}

% While the above approaches of making fundamental aspects of a software system customizable and enabling customizability case-by-case are both effective in addressing their respective needs, they do not focus on scoping how broadly applicable these customizations might be across different tasks and interfaces.
% While the approaches of making fundamental aspects of a software system customizable and enabling customizability on a case-by-case basis are effective in addressing their customization needs, they do not focus on providing a scope of how broadly these customizations might apply beyond their demonstrated interfaces.
% % This is because it is impossible to anticipate all customizations users may need in order to support their diverse workflows \cite{Nardi1993SmallMatterProgramming, Karger2007BDMHaystack}.
% Consequently, this can hinder the widespread adoption of customizations and make retrofitting them into existing systems technically challenging.

% \bryan{A counter I see with this is that if you do this, you risk designing something that's infeasible.}


% \changed{One approach is to design interfaces with the goal of making them inherently customizable by addressing their fundamental system aspects.
% Smalltalk focused on making any object in the GUI end-user customizable, enabling users to directly modify the appearance and behavior of interface elements \cite{kay1993smalltalk}. 
% HyperCard further explored customizable behaviors by allowing users to compose actions, such as mouse clicks, to automate and customize workflows \cite{Hypercard2024}. 
% In contrast, Haystack explored making the data model, types, and relationships of web interfaces end-user customizable, empowering users to create personalized views and workflows for managing their information \cite{adar1999haystack}. 
% Finally, Webstrates treated web documents as dynamic media, enabling users to create custom representations of the same DOM element while facilitating real-time, dynamic collaboration \cite{Klokmose2015Webstrates}.
% }












% To provide end-users with more granular control over the interface while maintaining a low cost, a line of work has explored techniques for manipulating attributes of drawing objects in gesture-based creativity support tools \cite{ObjectOrientedDrawing, Xia2017CollectionObjects}. This work leverages the fact that drawing objects often have multiple associated attributes, providing opportunities to select objects based on shared attributes, as well as to clone and blend them. Our work arrives at a similar approach, identifying that overview-detail interfaces contain items with many common attributes, which offers users the potential to manipulate and customize the interface.

% taking out the AI thing for now, since it's not directly relevant. 
% The recent surge in generative AI has introduced opportunities to make it both easy and expressive for end-users to customize their interface by using AI to generate and render UI code from user prompts \cite{anthropic2024claude35, vercelGenUI}. While this approach is promising, the mappings between natural language prompts and generated code are not shown to the end-user, giving no way for them to understand or adjust the generated interface \cite{whyjonnycantprompt, sarkar2022like, designguidelinesforpromptengineering}.


% as we similarly identify that overview-detail interfaces contain items with many common attributes, offering users the potential to manipulate them to customize the interface. 
% We further identify that this approach enables an expressive mechanism for customizing overview-detail interfaces 

% and this approach can also be used with AI to map user prompts to specifications \cite{vaithilingam2024dynavis, bespoke}. 


% We explore the opportunity to surface attributes for the end-user to customize their overview-detail interface


% To provide end-users with more granular control over the interface while maintaining a low cost, prior research that has explored techniques for manipulating attributes of drawing objects in gesture-based creativity support tools \cite{ObjectOrientedDrawing, Xia2017CollectionObjects}.
% Work leveraging the fact that drawing objects have many attributes associated with them, demonstrated opportunities for selecting objects of common attributes, cloning, and blending.
% Our work shares this approach, as we identify that overview-detail interfaces often contain items with many common attributes, providing an opportunity for users to directly manipulate.
% % We further explore the opportunity to leverage 


% To offer end-users more granular control over the interface while maintaining a low cost, we build on previous research that investigates techniques for attribute manipulation in gesture-based creativity support tools \cite{ObjectOrientedDrawing, Xia2017CollectionObjects}. These studies have demonstrated that manipulating attributes allows users to effectively select and transform collections of media objects \cite{Xia2017CollectionObjects}. We extend this design approach to customizable overview-detail interfaces, enabling end-users to manipulate attributes across all items, thereby facilitating interface customization.




% By bringing the control of attributes
% This approach enables users

% The ability to manipulate attributes demonstrated the ability for  to select and transform collections of media objects effectively \cite{Xia2017CollectionObjects}. 

% We extend this design approach to customizable overview-detail interfaces, enabling end-users to manipulate attributes across all items to customize the interface.


% So we want to give end-users more granular and expressive control over the interface while keeping these customizations approachable and low cost.

% Well, research has explored ways to provide users with more granular and direct control for gesture-based creativity support tools, allowing you to manipulate attributes as objects. 
% Manipulating attributes has also demonstrated the ability for users to select and transform collections of media objects \cite{Xia2017CollectionObjects}. We share this design approach for making overview-detail interfaces customizable, enabling the end-user to manipulate attributes across all items in the overview-detail interface.

% An approach to supporting both granular and ``direct'' control has been explored through


% To design an overview-detail interface that is customizable, we take the approach of leveraging the 

% i was about to talk about attribute manipulation, but then i realized it doesn't flow well with the content analysis. So I want to hint at it, but not make it the main focus. 

% I want to talk about mappings

% If we want users to customize their interface in a 

% Xia \etal{} have explored interactions for manipulating attributes of strokes and shapes digital art creation \cite{ObjectOrientedDrawing, Xia2017CollectionObjects}. Notable thing is Collection Objects, enabling users to select and transform collections of items on a sketching canvas based on the attributes \cite{Xia2017CollectionObjects}.
% We share this approach to controlling the overview-detail interface by supporting interaction techniques for users to control attributes shared across items in the overview.

% \bryan{Take parts from this RW to talk about how systems have tried making customizable software. End-user customization, all general customization}

% \subsection{Constraint-based Adaptation}
% Prior work has explored computationally adapting UIs based on various contextual factors and constraints pertinent to the device, user, or situation in domains such as accessibility, ubiquitous computing, and mixed reality \cite{dey2001conceptualcontext, abowd1999context, computationalApproachUIGen, wobbrock2011ability, gajos2010personalization}. For example, SUPPLE and SUPPLE++ computationally adjust the size, style, and layout of widgets to adapt GUIs based on device constraints (e.g., screen size, input modality) and users’ capabilities (e.g., motor and vision) \cite{gajos2004supple, gajos2010personalization, supple++}. UNIFORM and Huddle automatically generate UIs  with primitive widgets for controlling home appliances by considering users’ interaction history as well as modeling the similarities and dependencies of appliances \cite{uniformNichols, HuddleAutoGenUIAppliances}. Since mobile and Mixed Reality (MR) interfaces can be invoked in arbitrary situations, research has also explored adapting these interfaces based on various environmental factors \cite{lindlbauer2019context, dey2001conceptualcontext}. For example, Lindbauer et al. explored how applications should dynamically adapt the amount of information they show and their spatial arrangement in an MR context \cite{lindlbauer2019context}.
% With this approach, the data schema remains the same, and the encoding remains program-based but augmented with contextual constraints, resulting in context-aware dynamic interfaces. However, the scope of the dynamic behaviors is pre-defined by developers, and end-users are unable to change the underlying data scheme and encoding.
% \subsection{End-User Customization}
% Previous research has explored creating interactive systems that are both customizable and extensible, allowing end-users to tailor them to their specific needs. This work is primarily situated within the field of end-user programming or development (EUP or EUD) \cite{nardiProgramming}, where end-users can employ natural language programming \cite{PUMICE}, GUI-based interaction \cite{litt2020wildcard, Hypercard, fusion}, visual programming \cite{Scratch, DynamicLand}, and programming-by-demonstration \cite{vegemiteJames} to extend existing systems.
% For example, pioneering systems like OpenDoc \cite{Apple_OpenDoc}, HyperCard \cite{Hypercard}, Smalltalk \cite{kay1996early}, and recent system DynamicLand \cite{DynamicLand} aimed to develop dynamic and personal media for end-users to create their own dynamic content and UI. Hypercard allows users to develop interactive multimedia content by linking objects via GUI and scripting advanced behaviors using a built-in programming language \cite{Hypercard}. These systems pre-define the underlying data schema but expose the encoding mechanism to enable EUD.
% To circumvent the lack of access to the applications’ internal data schema, research has explored constructing external data schema to enable EUD. For example, with the accessible and manipulable
% Document Object Model (DOM) of webpages, Wildcard supports collecting data from and injecting data back to the webpage DOM structure, and by representing the data using an external spreadsheet, end-users can manipulate the spreadsheet to customize the web pages.\cite{litt2020wildcard}. Further leveraging the composability and transclusion of the web \cite{Nelson1995Transclusion}, prior work explored enabling end-users to create mashup applications to achieve their specific needs. For example, Fusion and C3W enables users to create mashups by extracting components from existing webpages and connecting them using transclusion, formula, and glue code \cite{fusion, fujima2004c3w}. Vegemite enables users to collect data from multiple websites; using scripts that can be generated from users’ demonstration, it can perform computation on the collected data and automatically execute web actions such as clicking links and inputting data values to web forms \cite{vegemiteJames}.
% With EUP/EUD, the applications’ internal data schemas often remain inaccessible to end users, but the encoding mechanisms are available for them to extend the applications. While external data schemas, often spreadsheet, can serves as the proxies or connectors with the original applications, these external data schemas are also pre-defined by developers, leaving end-users still with limited customizability.
% \subsection{Specification-based Synthesis}
% In addition to adapting and extending applications, prior research explored generating entire applications and UIs to support end-users’ information tasks. For example, Nichols et al. explored employing a specification language and parameterized templates that encode design conventions to automatically generate interfaces for controlling home appliances \cite{NicholsSmartTemplate, nichols2002requirements, GeneratingRemoteControl}. Based upon the specification of command-line applications, Bespoke can synthesize custom GUIs by mapping UI widgets to different types of command-line parameters \cite{bespoke}. Similarly, DynaVis composes UI widgets to create interfaces for controlling parameters inferred from users’ natural language queries to edit data visualizations \cite{vaithilingam2024dynavis}.
% Another theme in this direction is designing a programming model based on high-level specification language. This enables users to focus on composing high-level domain-specific primitives and deferring low-level execution architecture and runtime \cite{heer2010declarative}. Using a high-level declarative grammar, Vega-Lite enables rapid specification of interactive data visualizations \cite{vega-lite}.
% Inspired by the success in data visualization, Varv explored representing interactive software as a declarative data structure that describes the schema and actions of a set of concepts \cite{varv}.
% With this approach, developers carefully design the specifications, which dictate the space of possible UIs and ensure the consistency and quality of the generated UIs \cite{NicholsSmartTemplate}. Although end-users can technically generate UIs within the boundaries set by these specifications, their ability to do so is mediated by the encoding mechanisms. To enable end-users to intuitively generate the applications and UIs, prior research often provides an additional layer of graphical and natural language interfaces which are mapped to the underlying specifications \cite{vaithilingam2024dynavis, bespoke,narechania2020nl4dv, crosspower}.
% \subsection{AI-based Code Generation}
% Recent developments in AI, especially its ability to generate functional program code from natural language prompts, have sparked a new approach toward generative UI. AI products such as Claude \cite{anthropic2024claude35} and Vercel \cite{vercelGenUI} can generate and render UI code from natural language prompts. Wu et al. explored fine-tuning LLMs with automated feedback to improve the quality of the generated UI code \cite{wu2024uicoder}. As AI’s code generation capability continues to improve \cite{anthropic2024claude}, the complexity and quality of AI-generated applications and UI will likely increase.
% However, this UI generation approach can be a double-edged sword. On the one hand, AI can generate code for arbitrary user prompts. On the other hand, the lack of understandable and controllable mappings between users’ prompts and low-level code makes it challenging for end-users to customize the generated UIs when AI inevitably and probably constantly fails to meet users’ dynamic and shifting goals. For example, research has shown that end-users face considerable challenges in prompting AI to design interactive systems \cite{whyjonnycantprompt}.
% With this approach, while both the data schema and the encoding are dynamically generated, resulting in generative UIs, the low-level code representation and the obscure mappings between natural language prompts and generated code pose significant challenges for end-users to control and customize the generated results, as found in many domains of AI-generated content \cite{whyjonnycantprompt, sarkar2022like, designguidelinesforpromptengineering}.



% ----- END -----
% VizFlow supports dynamic layouts by linking text and charts, allowing users to create data-driven articles without needing programming skills \cite{Sultanum2021VizFlow}.


% Research has additionally found that users often prefer having the control to customize over system recommendations, but avoid customization features due to the complexity involved in achieving them \cite{McGrenere2007AdaptableSoftware, Park2007AdaptableVersusAdaptive}.
% while barriers such as high difficulty and lack of time may deter users from customizing if the perceived benefits are not worth the effort \cite{Mackay1991TriggersAndBarriers, Marathe2011CustomizationControlOrIdentidy}.

% Mackay also highlights barriers including high difficulty and lack of time, which deter users from making customizations if the perceived benefits are not worth the effort \cite{Mackay1991TriggersAndBarriers}.
% Additionally, research reveals trade-offs between user-controlled and system-recommended customizations, where users often prefer having control but may avoid customization features due to the complexity involved in achieving them \cite{Mackay1991TriggersAndBarriers, McGrenere2007AdaptableSoftware, Park2007AdaptableVersusAdaptive}.

% Mackay identifies key factors influencing software customization, such as users' recognition of repetitive patterns and frustration with repeated actions.


% and demonstrate interaction opportunities, it is especially important to explore this within the MD design pattern. However, there is currently a lack of comprehensive understanding regarding the range of customization options available for MD interfaces.


% Given this trade-off between customization needs and the friction to customize, researchers have explored approaches towards reducing the barriers for customizability to more interfaces. For example, Anchored Customization brings individual settings options from a separate page to conceptually related UI components, making customizations more in-situ for the interface \cite{Ponsard2016AnchoredCustomization}. Similarly, WritLarge allows the user to transform digital ink from a sketch to a grid and then to a table, each "semantic level" offering their unique respective affordances such as erasing strokes at the strokes level or turning handwriting into text \cite{Xia2017WritLarge}. VizFlow supports a range of dynamic layouts by using text-chart links, allowing users to author data-driven articles without programming \cite{Sultanum2021VizFlow}.



% While these findings serve as valuable insights for effective design for customizability, it is particularly important to explore this for the MD design pattern, something that is implemented across so many diverse tasks and where users must navigate through views in various directions while keeping an understanding of all the information presented. However, there lacks a comprehensive understanding of the various customization options that exist and are possible for MD interfaces.





% WritLarge allows the user to transform a selection of digital ink from a sketch of a table to a grid, then to a table, then back down to a grid, each ``semantic level'' affording unique functionalities, such as the sketch allowing for erasing the lines, and more structured representations like tables ....



% A mechanism we are interested in focusing on is transclusion.
% We want to focus on this because we want to support in-context

% To support web collection and management within the context of active web spaces, we utilize transclusion, a technique that involves embedding one part of an application into another \cite{Nelson1995Transclusion}. 
% We aim to support information collection and organization by aggregating web components with transclusion, a technique that involves embedding one part of an application into another \cite{Nelson1995Transclusion}.
% Methods for transcluding web components has seen real-world use and has shown interaction benefits in commercial applications and HCI research.
% For example, note-taking applications such as Notion \tocite{notion} and Confluence \tocite{Confluence} collaborate with other companies, including Figma \tocite{Figma}, to embed views from other companies' applications in their documents. In HCI research, prototypes such as inlineLink embedded iframes inside websites, allowing users to view many hypertext files in a single rendered document \cite{miura2004inlinelink}. 

% Additionally, Webstrates introduced a technique for turning web elements into shareable and modifiable media across numerous spaces through transclusion \cite{klokmose2015webstrates}. This technology has unlocked opportunities to develop and integrate transclusion in diverse domain such as programming, video creation, and videoconferencing \cite{radle2017codestrates, klokmose2019videostrates, gronbaek2021mirrorblender, gronbaek2023mirrorverse}.
% Although there has been a rich research ecosystem for transcluding web content across websites, all of these works either constrain the user to a set of web contents they can transclude and where or require technical expertise to develop custom transclusions. Our goal is thus to empower end-users to create their own transclusions by directly manipulating and moving web components across websites.



% Dynaviz? Designing for customizability --> natural language prompt, but presenting the widget that the user can use to better customize the chart directly?

% MD interfaces are widely implemented across diverse tasks, requiring users to navigate between views in various directions while maintaining an understanding of all the presented information. 


% Line of work that makes personal user interfaces automatically

% There’s work that can allow you to transform the representation of views (WritLarge, bret victor), 

% Transformable representations: WritLarge, Bret Victor, Damien Masson's work

% Customizing lists, such as reordering, 

% We explore how we can design an MD interface that enables transformations across our design space dimensions.


% While extensive research has been done understanding the various customization options available across many domains and patterns, there lacks a comprehensive understanding of the various customization options that exist and are possible for MD interfaces.

% While these studies provide valuable insights into the design of MD interfaces, they do not fully explore the potential for customization in this pattern. Our work addresses this gap by introducing new interaction techniques that enable users to directly manipulate and customize the details presented in the MD interface.



% Line of work on end-user programming and end-user customization — providing customization tools that aren’t built into the websites, allowing you to make your own filtering, sorting, or computational operations \cite{Huynh2006Sifter, Litt2020Wildcard}.



% RW1 DUMP

% \bryan{Use overview-detail, and also include the mit website hci patterns --> they are defining overview "plus" detail}

% The master-detail design pattern is a widely implemented interface pattern characterized by two distinct views: a master view that contains a collection of items and a detail view that contains details of a selected item. This pattern, also referred to as ``director-detail'' or ``master-slave'' \cite{Pastor2007ModelDrivenArchitecture}, share different interpretations of what constitutes a ``master'', such as allowing the master to be a single item instead of a collection \cite{Seffah2015PatternsOH}. Despite these variations, the core structure of the MD pattern---as illustrated in Figure \ref{fig:md-definition}---remains consistent across these definitions.

% A notable strength of the overview-detail pattern is that it aligns with the principle of progressive disclosure \cite{Norman1986ProgressiveDisclosure, Shneiderman1996OverviewFirst}. By initially presenting only the essential details and revealing more details as the user delves deeper, the overview-detail pattern helps manage complexity and reduces cognitive overload \cite{Norman1986ProgressiveDisclosure}. 

% As this pattern is closely aligned with how information is organized in software systems, this pattern is also demonstrated in the context of web development. For instance, developers often structure API routes to manage collections of items with an ``index'' route (e.g., \texttt{/admin/articles}) and support retrieving individual item details through nested routes (e.g., \texttt{/admin/articles/:id}) \cite{Rails}.

% A formal empirical analysis could reveal additional variations and interaction possibilities of the MD pattern that individual case studies may miss. To our knowledge, our work presents the first empirical analysis of MD interfaces, which we leverage to explore and develop novel interactions enabled by this design space.

% A notable strength of the Master-Detail (MD) pattern is in its alignment with the principle of progressive disclosure \cite{Norman1986ProgressiveDisclosure, Shneiderman1996OverviewFirst}. By initially presenting only the essential details and revealing more details as the user delves deeper, progressive disclosure helps manage complexity and reduces cognitive overload \cite{Norman1986ProgressiveDisclosure}. A similar principle closely aligned with the MD pattern is the overview+detail principle, which advocates for displaying both an overview and a detailed view simultaneously, allowing users to grasp the broader context while accessing specific pieces of information \cite{Card1999VisionToThink, Hornbaek2001OverviewDetailBenefits}.  These benefits of the MD pattern are also reflected in diverse applications. For instance, Baudisch \etal's \textit{focus-plus-context screen} allows users to open a detailed portion of a map while maintaining an overview of the entire area \cite{Baudisch2001FocusPlusContext}, and web developers often architect web page routes to fetch collections of items in an ``index'' route (e.g., \texttt{/admin/articles}) that then supports navigation to deeper routes to retrieve individual item details (e.g., \texttt{/admin/articles/:id}) \cite{Rails}.

% This alignment with many design principles is perhaps the reason for its widespread use, making the MD pattern particularly interesting to study. Academic research and online articles have highlighted a few key variations of MD interfaces. For instance, Molina \etal{} explores how other patterns, such as a population pattern, can compose with the MD pattern to generalize the organizational structures user interfaces \cite{Molina2002JustUI}. Additionally, case studies explore how MD interfaces can be nested to create hierarchical views in applications \cite{Molina2002JustUI, Seffah2015PatternsOH} and how different screen sizes may necessitate varying arrangements of the master and detail views  \cite{Seffah2015PatternsOH, Nguyen2012MDAndroid}.



% RW2 DUMP



% \bryan{Bring up related work systems that provide just a new OD. They are essentially ODs to support task X, Y, Z}

% \bryan{This paragraph says: Okay, well you need one more OD instantiation to help with a task. So these contribute a new instantiation. Such as new layout, new composition, new content to the OD interface.}
% and support understanding of AI generated text \cite{Graphologue}.


% While this approach provides end-users with more instantiations to interact with, these representations are ultimately instantiated by the designer, limiting any ability for users to customize.


% Aimed at providing overviews on papers sourced from related work sections in papers
% PaperWeaver and Relatedly providing overview summaries of related work sections in papers
% Graphologue provides AI generated response, but also generates interactive node-link diagram alongside the text in real-time.


% Those are overviews. Anything else for overview-detail?
% These are all sensemaking stuff. I wonder if there are ny other directions of literature for this?


% Systems have also provided a spatial canvas to 
% ForSense, InterWeave providing canvas as you collect and explore
% Threddy, Synergi, Fuse providing a hierarchical structure to manage threads and snippets of information collected.



% they are still ultimately limited by the types of instantiations made by the designer and developer.
% \bryan{final statement that we need malleability, but especially for overview-detail interfaces, to support information tasks.}
% Thus, a malleable interface is needed to complet

% Instead, we need a malleable interface that allows users to
% A malleable interface is one that ideally allows users to 
% introduces ways to transform between different representations through axes of representation...

% introduced techniques for viewing information on a zoomable user interface at different zoom levels by providing varying levels of detail, which displays information at varying levels of detail at multiple zoom levels.

% Bret Victor climbing up and down the ladder of abstraction
% WritLarge
% pad++ provide multiple levels of abstraction in a zooming interface

% Charagraph --> this is a single additional representation, so not actually relevant
% texsketch
% \haijun{talk about work along this direction, in the end, say that while these work provide multiple instantiations, end-user still manipulate them, so they are still stuck with what the developers choose}
% ^ This paragraph is not about overview detail, but transformabl rep in general? like multiple abstraction 

% ^ yes, are there relate works that explore transformable Overview, or mutliple-level overview? I mean map is one? naturally has semantic zooming?

% okay, that makes more sense.

% When you say customize how they transform --> it's customizing the representation? that's what peiling's suggestion does , there's semantic zoom which is another representation you get, but even still, you need to need  to customizations on it

% ok sounds good. I think i can finish this tomorrow 



% [cool, glad it's -as in how these two sections of RW should be restructured-clearer now! ]

% [yes, developer right now decides what to show on each zooming level, but with our approach, theoretically, we can customize what's shown on each zooming level] 

% but not customizable. yes.

% That's the point of this section. We say that there are transformable ones... but they are not customizable. what if people what to customize how they transform. like what peiling suggested, having end users to customize what's shown on each level of the semantic zooms

% and they our next section talks about customizable interfaces, so it will flow well?



% Significant research has been devoted to understanding the types of online information tasks users engage in \cite{tangledWeb, knowledgeworkerweb, tabbedbrowsing}, their usage patterns \cite{knowledgeworkerweb,tabdue}, and challenges users encounter\cite{browsingcluttered,tabdue, graphhistory}. These tasks are often involve various subtasks such as 
% The complexity and fluidity of this activity, coupled with today's software interfaces that fragment information spaces across many applications and tabs, is perhaps the reasons for interaction costs such as information overload, browsing clutter, and excessive context switching \cite{Chang2021TabComesDue, Han2022Passages, Miller1960InfoOverload}.

% Many lines of research have aimed to address subsets of frictions encountered in information tasks within specific domains. One approach explored ways to streamline the users collection processes as they dive into the details of information. Systems employed browser-level comparison tables to facilitate decision-making across online items \cite{Chang2020Mesh}, spatial canvases to help synthesize and make sense of information \cite{Ramos2022ForSense, Suh2023Sensecape}, and hierarchical organizations to efficiently structure and manage snippets of text and web content \cite{Kuznetsov2022Fuse, threaddy}. A second approach has focused on providing users an overview first in order to guide users' exploration. For example, Relatedly \cite{Relatedly} and PaperWeaver \cite{PaperWeaver} create overviews of relevant papers by leveraging semantic connections from the content of the active paper. Selenite scaffolds users’ decision-making processes by generating initial criteria about an item to purchase \cite{Selenite}. Lastly, mixed-initiative approaches leveraged the benefits of systems that facilitate both information exploration and synthesis. For instance, Synergi facilitates the both collection and synthesis of information by automatically fetching relevant threads from academic papers and placing them into hierarchical categories \cite{Synergi}. Sensecape guides users' exploration and collection processes with a hierarchical organization of canvases \cite{Sensecape}. Meanwhile, Qlarify enables users to gradually uncover more details about key concepts within a paper abstract by intelligently fetching information from the full paper \cite{Fok2024QlarifyARXIV}.

% While these solutions offer valuable insights into addressing the various challenges across their respective domains, an interface cannot only provide one solution at a time to support the dynamic nature of information tasks. Instead, a malleable interface would allow the user to choose which representation of an overview suits their understanding best and decide how they uncover and synthesize information from related or detailed sources. 
% Our work presents an opportunity to unify existing tools that facilitate information tasks with a malleable overview-detail design pattern.

% \bryan{Question: Don't malleable interface literature and our intro already motivate the need for malleable interfaces for information tasks? Or did I completely misunderstand something about this section?}



% On the other hand, malleable interfaces have




% \subsection{MD Interfaces in Information Spaces for Sensemaking}

% % This is particularly important in information-rich environments, where the MD pattern's widespread use presents unique challenges in supporting users' sensemaking activities.

% % Master-detail interfaces are ubiquitous in digital information spaces, making these interfaces a common interface users encounter during sensemaking activities.

% MD interfaces are ubiquitously integrated into everyday interfaces we use for a plethora of sensemaking tasks, some of which include collecting papers, shopping, travel planning, or even simply learning new concepts. However, due to the sheer scale of information the internet packs into MD interfaces, users must navigate through large hierarchies of master-detail web pages during these tasks. Furthermore, as the task increases in complexity, the explored information grows increasingly challenging to manage and analyze in the interface, often leading to cases of browsing clutter and fragmented information spaces \cite{Chang2021TabComesDue, Han2022Passages}. 

% Several lines of research in2 specific domains have tackled the challenges pertaining to information management and online sensemaking for their respective activities. For instance, designers have shared design recommendations on the optimal arrangement of information in overview pages (master) and item pages (detail) of e-commerce websites to reduce the excess reading costs for end-users \cite{van2007design}. Research has explored providing users with personal spaces to aggregate snippets of information (master) from full web pages (detail) \cite{Kuznetsov2022Fuse}. Other work have integrated various representations, such as a table \cite{Chang2020Mesh}, a canvas \cite{Ramos2022ForSense}, and a hierarchy \cite{Suh2023Sensecape}, as an overview (master) to aid users in comparing items, synthesizing notes, and understanding complex concepts (detail) \cite{Chang2020Mesh, Suh2023Sensecape, Ramos2022ForSense}.

% While these solutions for supporting individual tasks are valuable for directly addressing domain-specific challenges, they often lack the flexibility required for the diverse working patterns. Consequently, users may face challenges in switching between the many working spaces across various different contexts. This highlights the need for a solution that addresses these common challenges through a unified approach. We propose that making the MD interfaces more customizable provides an effective way to achieve this flexibility.




==> versions/R_R/99_conclusion.tex <==
\section{Conclusion}
\label{section:conclusion}

This research explored malleable overview-detail interfaces, ones that end-users can customize to address individual needs. We conducted a content analysis of overview-detail interfaces in the wild and identified three dimensions of variation: content, composition, and layout. Based on these dimensions, we developed interaction techniques to support customization along these dimensions. We developed a set of interaction techniques that enable end-users to customize diverse layouts, compositions of views, manipulable attributes across views, and AI-driven interactions to reformat and generate new attributes.
Our user study found that participants produced diverse customizations and surfaced usage patterns in how they managed attributes and organized multiple overviews. We hope our work paves the way for further exploration of malleable overview-detail interfaces in new contexts and inspires the expansion of malleable interfaces to additional design patterns.


==> versions/R_R/9_discussion.tex <==
\section{Discussion and Future Work}
\label{section:discussion}

Our exploration of design probes and observations from our user study reveal opportunities to further investigate malleable overview-detail interfaces. We discuss potential directions for supporting additional aspects of customization in future systems, studying their prolonged use, exploring practical approaches to implement them in real-world websites, \changed{and future opportunities to support user-defined abstractions in other contexts. Finally, we discuss how our design pattern approach for broadening end-user customizability can generalize beyond the overview-detail pattern.}


\subsection{Supporting More Variations for Malleable Overview-Detail Interfaces}
In this research, we focused primarily on the utility of the malleability of overview-detail interfaces, rather than the utility of each individual variation. As a result, we did not implement all possible variations within the design space. However, implementing the full range of variations---and potentially more variations outside of our design space---could provide a more comprehensive understanding of the value each design option offers. 
Probes could also be implemented in different contexts beyond shopping and hotel booking to offer insights into which variations and instances users prefer in diverse scenarios and gain stronger evidence of various usage patterns.
% A larger set of provided variations and contexts could open opportunities to uncover more usage patterns of malleable overview-detail interfaces than what we identified.
Future work should explore the full range of design variations, including those beyond our design space, and \changed{additionally investigate their long-term utility across a variety of} contexts.


\subsection{How Do We Bring Malleable Overview-Detail Interfaces to the Real World?}

Our user study showed promising signs of the utility and value of malleable overview-detail interfaces. 
\changed{Our work aims to serve as a concrete guide for implementing our overview-detail interface customizations across many real websites and applications.}
% However, even if our proposed customization techniques do not achieve absolute widespread adoption, they can still be integrated into websites that already support similar features, while newer websites can design their software architecture to accommodate these customizations in future development stages.
% long term goals
However, the decision to implement them ultimately rests with the developers---from individual providers to large corporations. Increasing customizability requires additional development, which \changed{can demand significant time, increase codebase complexity, and even require re-architecting the application entirely}. Therefore, the critical question becomes: \textit{How can we practically bring malleable overview-detail interfaces to the real world?}

\changed{We have seen many systems take the approach of foregoing the development cost entirely by creating an end-user tool as a browser extension \cite{Zhang2018Fusion, Visbug2024, Kim2022Stylette}, and this can be similarly done for overview-detail interfaces by scraping active websites to identify overviews, detail views, and their associated attributes. Sifter \cite{Huynh2006Sifter}, in their DOM structure detection algorithm, even identify a variation of overview-detail interfaces---our design pattern approach could perhaps improve upon such detection algorithms to identify more variations. However, such ``outside-in'' approaches often face challenges related to inconsistency and usability issues, making it technically difficult to implement them effectively.}

\changed{Another approach is to reduce the cost for developers with a developer toolkit, such as a web framework, that provides many variations and customizations out of the box. This framework can package together an architecture involving GraphQL \cite{graphql2024} to dynamically fetch attributes from the back-end and a custom UI component library that provides sets of layouts and compositions to use as defaults and for end-users to customize. 
While a toolkit may be less viable for existing websites, we aim to significantly reduce the cost for developers building new ones.}
% , enabling the future adoption of malleable overview-detail interfaces.}


% However, a toolkit that involves rebuilding the website from its very core parts of its stack would be less viable for existing websites.
% \changed{
% Considering and balancing the trade-offs of both approaches have been the main subject of prior work on customization techniques and is known to be a significant barrier. 
% Therefore, while designers and developers should consider these trade-offs when implementing our presented customizations, we nevertheless encourage them to 
% These trade-offs should guide the practical implementation of malleable overview-detail interfaces in real-world applications.
% However, we still encourage websites to implement our presented customizations as we believe...
% }


\subsection{\changed{Pushing the Possibilities of User-Defined Abstractions}}


\changed{
Diverse forms of abstractions are implemented across various information systems and digital artifacts to assist users in understanding, operating with, and communicating with complex knowledge.
For instance, scientific data, mechanical systems, and code are often abstracted into various visualizations and diagrams, which involve the use of ellipses, blocks and arrows, and graphs \cite{ASCIIDrawings, Victor2011LadderOfAbstraction, Fong2021LinkedList}.
Recent advancements in AI has also enabled the development of generating different levels of abstractions of text \cite{Suh2023Sensecape, suh2023luminate, Graphologue} and different summarizations of academic papers \cite{elicit2024}.
We have also explored dynamic abstractions in the context of overview-detail interfaces, enabling end-users to modify a custom set of attributes.
Across these various systems and contexts, there is a clear need for end-users to define abstractions that suit their unique needs. However, the mechanisms that allow users to easily abstract information extend much beyond modifying data attributes supported in our malleable overview-detail interfaces.
This opens opportunities to explore how users can go beyond modifying data attributes to creating and tailoring their own abstractions in more diverse and expressive ways. Our goal is to study user-defined abstractions as a phenomenon across these diverse contexts and variations, seeking ways to better support them through a unified interaction methodology.
}



% Across these various systems and contexts, there exists a need for end-users to define the right abstraction to suit their unique needs, and there are clearly mechanisms of abstracting information beyond use data attributes supported in our malleable overview-detail interfaces.
% Across these various systems and contexts, there is a clear need for end-users to define abstractions that suit their unique needs, but the mechanisms for end-users to easily abstract information in their own extends beyond modifying data attributes, as supported in our malleable overview-detail interfaces.

% other way of saying is useful --> provides guidance, assists
% Indeed, there are many other ways to abstract information beyond only its attributes.




% opening opportunities to explore how end-users can further create and tailor their own abstractions beyond just data attributes.
% We aim to study user-defined abstractions as a phenomenon across a diverse range of contexts and variations to explore how can further support them through a unified interaction.
% 
% We have explored dynamic abstractions under the context of overview-detail interfaces, enabling end-users to modify a custom set of attributes in overview-detail interfaces.
% Across these various systems and contexts, there remains a crucial need for end-users to view the right abstraction for their unique contexts


% a core theoretical exploring of our work was examining how evv
% Therefore, we see opportunities for future work to explore how end-users can further create and tailor their own abstractions across these different forms.


% We have also begun to see an increase of more dynamic abstractions with the advances in AI generating different levels and types of summaries of text-heavy content such as conversations, emails, and academic papers \cite{Suh2023Sensecape, suh2023luminate, elicit2024}.
% dynamic abstractions,
% On the other hand, dense, text-heavy documents—such as LLM-generated text and academic papers—are increasingly being dynamically abstracted into different levels and forms of summarization using AI, which are generated as titles, outlines, or paragraphs \cite{Suh2023Sensecape, suh2023luminate, elicit2024}.
% We explored the nuances involved dynamic abstractions for overview-detail interfaces, which we allowed end-users to create their own abstractions through a custom set of attributes.


% Across these various systems and contexts
% A core theoretical exploration of our work was examining how effectively users could create their own abstractions within the overview-detail interface by manipulating the data attributes of overview items—either through direct manipulation or by prompting.
% lots of abstraction and it's useful
% we se ein LLM as well making abstraction more dynamic
% we explored ODI is abstraction
% we need user defined


\subsection{Malleable Interfaces: Beyond the Overview-Detail Design Pattern}
This research focuses on making overview-detail interfaces malleable. While the overview-detail pattern is widely implemented across many interface systems, it is not the only design pattern in use. Research has explored the challenges and opportunities for end-users to customize various interface elements, including dashboard interfaces \cite{Sarikaya2019ReviewDashboards}, item collections in lists and spreadsheets \cite{Huynh2006Sifter,Litt2020Wildcard}, and menu list interfaces \cite{Park2007AdaptableVersusAdaptive}. We have also investigated how different representations of the overview interface can be customized in relation to the overview-detail interface. We believe that exploring other design patterns and their design spaces can offer new opportunities for making more interfaces malleable. This approach of investigating the variations and nuances of each design pattern may help us move closer to developing a general malleable interface.
% \bryan{TODO: You basically want to push further the discussion on what other design patterns you can explore. And really talk about how this approach of analyzing content, then understanding its variations, is an effective way of understanding broader applicability of customizations of interfaces.}






% it's crucial to provide right abstraction in the interface.
% overview-detail explores abstraction of whch attributes are shown
% Our core exploration was to make data attributes manipulable in the overview of overview-detial interface.
% There are many other forms of abstractions beyond attributes, such as visual/diagrams and text/semantic
% There are many opportunities for future work to exploring other ways end-users can form their own abstractions.

% D. It's crucial to provide the right abstraction in the interface.
% A. Overview-detail explores abstraction of which attributes are shown.
% C. Our core exploration was to make data attributes manipulable in the overview of the overview-detail interface.
% B. There are many other forms of abstractions beyond attributes, such as visual/diagrams and text/semantic.
% E. There are many opportunities for future work to explore other ways end-users can form their own abstractions.

% These user-defined abstractions... 
% One of our core theoretical explorations was to explore how effectively users could create their own abstractions on the overview-detail interface by making the data attributes of overview items manipulable in the interface.
% But it is known that there are many other ways of abstracting than just by their data attributes.
% And not only that, it is common behavior for users to create abstractions for their own everyday needs, such as creating titles for files to organize, 
% For instance, there exist diverse forms of visual abstractions to communicate scientific information, mechanical systems, and code \cite{ASCIIDrawings, Victor2011LadderOfAbstraction, Fong2021LinkedList}.

% A core theoretical exploration of our work was examining how effectively users could create their own abstractions within the overview-detail interface by manipulating the data attributes of overview items---either by direct manipulation or by prompting.
% Indeed, there are many other ways of abstracting data beyond just their data attributes.
% For instance, complex knowledge such as scientific data, mechanical systems, and code are often abstracted in diverse forms of visualizations and diagrams \cite{ASCIIDrawings, Victor2011LadderOfAbstraction, Fong2021LinkedList}, while dense, text-heavy documents such as LLM-generated text and academic papers have recently explored summarizing this information with AI \cite{Suh2023Sensecape, elicit2024}.
% Among all these systems and contexts, it still remains crucial to provide the right abstraction in the interface. 
% One way to achieve this is by giving control to the end-user, allowing them to better align the abstraction with their needs. We see opportunities for future work to explore ways for end-users to form their own abstractions in these different forms as well.

% Among all these systems and contexts, it remains crucial to provide the right abstraction in the interface.
% abstracting information and supporting these methods within the interface, enabling users to define and form their own abstractions.
% Among all these systems and contexts, it still remains crucial that the right abstraction in the interface is provided to the user, and one of the ways to do this would be to give this control to the end-user to allow them to align it better on their own.
% There are many opportunities for future work to explore additional ways of abstracting information and to support these methods within the interface, enabling end-users to define and form their own abstractions.
% There is an exciting road ahead basically, that we're paving to make abstraction for controllable by the end-user...
% We see many opportunities to explore more ways to enable end-users to define and form their own abstractions in the interface.
% still important for the right abstraction is provided for the end-user, and giving this control to the end-user could allow them to align it better.
% Abstractions can also be created in the form of writing, like how sensecape, pad++, and Elicit provide textual summaries in different ways --- particularly relevant for LLMs \cite{Suh2023Sensecape, pad++, elicit2024}
% Among all these systems and contexts, there still exists the need for users to view information at not only different levels of abstraction, but the right kind of abstraction. One, perhaps the only, way to address this need is to give this control to the end-user.

% \bryan{Basically, we explore UDAs by making attributes manipulable. But there are mote forms of abstractions that may not be directly manipulable through attributes. Heatmap, AI-generated content, fuzzier forms basically. There are already UDAs around, such as Elicit that allows you to ask specific questions about papers, allowing you to form your own needed aspects of papers. Not to mention there are also visual encodings that the interface may want to support. Future work can explore this larger design space of how these many kinds of UDAs can be supported through the interface...?}

% \bryan{I will discuss user-defined abstractions, and how this fits into the paper}
% \bryan{btw, the reason why I talk about this is because we want to further emphasize the importance of the design implications of better understanding ODIs and malleable ODIs, rather than the interaction technique. We need to better spell out the ODI aspect, and user-defined abstractions is a key piece to it.}

% \bryan{There are many different approaches to providing more forms of abstractions to the user}
% \bryan{sensecape, writlarge, pad++, codetoon, bret victor}
% \bryan{Normally, the kinds of abstractions in interfaces are either: 1) abstractions provided to the user predefined or 2) giving users full responsibility to create their own abstractions on an authoring space such as a spatial canvas or text-editing space.}
% \bryan{Problem with 1 is that the abstractions provided may not fully align with end-users' needs.}
% \bryan{Problem with 2 is that creating their own kinds of abstractions is not only lots of work, but they also won't know what they need.}
% \bryan{Through malleable overview-detail interfaces, we were able to explore the possibilities of \textit{user-defined abstractions}---abstractions in interfaces that end-users can form that 1) align with their needs, 2) can be easily created, and 3) can better identify the abstraction they need based on their task.}

% \bryan{Now I talk about how this research opens us researchers to think of all the ways we can make abstractions user-defined.}
% \bryan{The age of LLMs has popularized one form of abstraction---summarization---where large amount of information can be reduced into perhaps a single phrase to a few sentences.}
% \bryan{This is done by having the LLM receive an input of content, and prompt to summarize or reduce into a shorter length.}
% \bryan{If we look through the lens of user-defined abstractions, we can see that the LLM, alongside its provided summarization prompt, is defining how the content is being summarized. Instead, perhaps the interface can provide the end-user to define the kinds of abstractions to best suit their needs, such as summarizing a story into key themes, character development, or passage of time.}
% \bryan{Indeed, with LLMs, the end-user may just want to prompt these specific forms of abstractions, and it is likely that users already do this. However, it may be hard to know which kinds of abstractions they may need \cite{gulfofenvisioning}. Future interface design research can explore how to provide the kinds of abstractions users may want as well as let them tweak them to fit their unique needs.}
% \bryan{Similarly, research papers can be cited by numerous other papers with diverse approaches. For instance, one may cite this paper to reference the overview-detail design pattern, another may cite this paper to reference user-defined abstractions, and another may cite this paper for our research approach of making interfaces malleable by analyzing design patterns.}
% \bryan{By looking through the lens of user-defined abstractions, these varying forms of summaries of this work are abstractions of this paper. Perhaps future research could explore how we can leverage this database of user-defined abstractions to facilitate search and understanding of a paper through the diverse abstractions formed by research communities.}
% \bryan{We believe our research has only scratched the surface of how we can enable end-users to effectively form their own abstractions. We only explored this in overview-detail interfaces, but there are so many other challenges and nuances in other forms of interfaces that would be difficult to support through our provided customization techniques.}
% \bryan{There is much more to explore in user-defined abstractions. I hope future research could dive into user-defined abstractions to make more abstractions customizable and easily creatable by the end-user.}
% , a form of user-defined abstractions,






% \bryan{There are these other patterns}


% \bryan{By explore how we can make other design patterns malleable, we believe this research contributes an approach towards finding ways to make other design patterns malleable, ultimately working towards general malleable interfaces.}
% \bryan{We believe this research shares an approach to making more }

% \bryan{There's }

% \subsection{A Language for End-users to Customize Malleable Interfaces}

% There seems to be a common misconception that malleable software implies open code and an open architecture. End-users being able to manipulate and tweak their own software doesn’t necessarily mean they should use the same language developers and engineers use. End-users need to be able to use their own language* to manipulate and tweak their own software whenever they want to. 

% \bryan{Opening the code for users to grow acclimated to programming}
% \bryan{Using AI for prompts}
% \bryan{But what we want is a language for the end-users, }

% \subsection{Further Exploring User-Defined Abstractions}
% \subsection{Towards Malleable Interfaces with User-Defined Abstractions}
% \subsection{Towards Malleable Interfaces with User-Defined Abstractions}

% Bret Victor talks about ladder of abstraction to be able to climb up and down to facilitate understanding of systems. This argues that \textit{a single representation is not enough}, but rather interfaces must provide multiple representations. Indeed, our user study observed that users effectively leveraged the various overviews and sets of attributes provided to them. However, our user study also found that users surfaced diverse sets of attributes we could not have fully anticipated.

% Bret Victor discusses the concept of the ``ladder of abstraction,''which allows users to move up and down levels of abstraction to better understand complex systems \cite{Victor2011LadderOfAbstraction}. This perspective argues that a single representation is not sufficient; instead, interfaces must offer multiple representations to support diverse user needs. In line with this, our user study observed that participants effectively utilized the various overviews and sets of attributes provided to them. However, the study also revealed that users surfaced diverse sets of attributes that we could not have fully anticipated.

% Not only is a single representation enough, but \textit{providing} multiple representations is not enough either. Instead, we must provide \textit{user-defined abstractions}---abstractions that end-users can customize or create on their own, enabling them to engage with information in ways that best suit their needs. For instance, if a user is new to a city and wants to know popular areas for lively restaurants, the user should be able to easily augment their map to display a heat map based on restaurant the number of reviews they have. 

% However, this scenario raises two core questions. First, how does the interface provide any possible representation the user wants? One user may want a heat map, while another may want an animation illustrating change in liveliness throughout the day. Perhaps generative AI could help create these abstractions, with emerging systems being able to generate and render user interfaces on the fly \cite{anthropic2024claude35, vercelGenUI}. Though, the challenge still remains in allowing the end-user to understand and change this generated code when it inevitably fails to address the user's exact needs \cite{whyjonnycantprompt, sarkar2022like, designguidelinesforpromptengineering}. Second, how would the user know \textit{what kinds} of abstractions would best help them in their context? Our approach in this paper was to provide default abstractions that can kick-start users' path towards creating their own. However, these defaults may inevitably be insufficient in supporting all user needs. 







% \changed{Future work could also develop and deploy robust probes to observe when and how frequently users make these various overview-detail customizations. Such a study could provide deeper insights into why users make particular customizations and which variations they prefer for which scenarios.}

% Another value that long-term studies could provide is the opportunity to uncover more usage patterns we identified.

% \bryan{Explore deeper into what kinds of variations could be possible}
% \bryan{Being able to change axes and navigation, could become these transformation primitives, which AI can get change and generate UI and functionality for it to make those transformations work, for instance, generating brand new overviews, or generating more overview-detail layouts beyond those mentioned in the design space}
% Future studies could also include more probes across different contexts beyond shopping and hotel booking, offering insights into which variations and instances users prefer in diverse scenarios and why.


% \bryan{Direct manipulation to communicate AI operations}
% \bryan{Our stuff focused on direct manipulation of attributes to basically move them or filter. And most of AI was triggered by prompting.}
% \bryan{We did have one feature where you can surface, and AI would essentailly autofill values of items that aren't there.}
% \bryan{maybe somehting with direct manupulation, but these actions communicate the intent to AI, resulting in some operation.}
% \bryan{What could happen if you could drag an attribute onto another attribute}
% \bryan{What could happen if you could an attribute onto a different item?}
% \bryan{What coyld happen if you select multiple attributes and drag them to an empty space?}
% \bryan{Maybe this is backwards thinking... maybe you need to flip the thinking to needs-based, then provide DM opporunities}
% \bryan{This relates to more variations because this could make it possbile to create more variations in MOD...}



%  Moreover, there are opportunities to deeply explore these additional variations beyond the ones implemented in our probes, such as customizing how one might invoke detail views from the overview (e.g., clicking, hovering, highlighting).

% \subsection{}

% \bryan{What are other usage patterns out there?}
% \bryan{We could discover more with a prolonged study.}


% \subsection{vs or +  Defaults for malleable overview-detail interfaces}
% \subsection{Malleable overview-detail defaults: will we reach convergence or an alternating cycle?}
% \subsection{To converge or to alternate between overview-detail customizations}
% \subsection{Customizing Overview-Detail Interfaces: To Settle or To Switch?}
% \bryan{I'm going to remove this section, and basically move this discussion into the user study, sharing more details of participants making layout and composition customizations earlier, but content customizations throughout the interface.}
% \subsection{Against or for malleable overview-detail defaults?}
% \subsection{Malleable overview-detail defaults: Yes or No?}

% Our study found that some users only surface attributes to the overview while others also hide them. We also found that users will compose multiple overviews to better structure their tasks. 
% Our insights offered recommendations for better defaults by observing usage patterns of malleable overview-detail interfaces.
% Indeed, some users may only need better defaults, as they perceive customizations as merely a short-term task. 
% tehy see customizations as one-and-done thing...

%rather than toggling.
% When asked about desired features of our probes, P2 wanted to see recommendations of attributes to surface, explaining, ``\textit{Given so much power, I don't like many options to customize. I wasn't sure which ones might be more important for me for this specific task.}'' 

% These preferences suggest two potential directions for malleable overview-detail interfaces: 1) users may settle on an optimal default setting, or 2) they may continuously switch between different customizations as they navigate their tasks. This raises several questions: \textit{What factors influence users to settle on a setting, and what factors drive them to frequently customize? Does this behavior vary with different customizable dimensions? How does this behavior evolve over time?}
% One way to answer these questions is to study the prolonged use of malleable overview-detail interfaces with a larger population. Future work could involve developing and deploying a robust probe to observe when and how frequently users make overview-detail customizations. Such a study would provide insights into whether and when users find an optimal setting, or if they continue to leverage various customizations in different contexts.



% Nevertheless, if our presented customizations techniques do not reach widespread adoption, it is possible for these techniques to still be implemented in websites that already support some of our customizations, while newer websites can consider a software architecture that will support these customizations later in their development.
% But if the customization techniques do not reach widespread adoption in the future, the presented techniques can still be implemented in websites that only have some customizations and can support more. Smaller websites more closely maintained can also implement their websites to support these customizations, meaning these customizations can still be accessible one way or another. 

% \subsection{Are malleable overview-detail interfaces ready for the real world?}

% Our user study showed promising signs of the utility and value of malleable overview-detail interfaces for end-users.
% Our design probes further demonstrated that such interfaces can be effectively implemented on websites. 
% However,
% \textit{How can we make it practical for developers to implement malleable overview-detail interfaces?}

% Perhaps the approach to address this challenge is to create an end-user tool and scrape the front-end contents to reconstruct data. Recent advances in AI has demonstrated the ability to effectively fetch data across websites, so you can pull data from other pages without navigating away. We could leverage the technical approaches from prior work to see how this could be achieved.
% \changed{Perhaps an approach to address this challenge}
% \bryan{We can leverage our design space/pattern and get better at understanding and identifying more vairaitons to support customizatinos for. We could Integrate Sifter and all of these web scraping and AI things to cover a broader variety of these interfaces}
% Many works have tried to support these kinds of integrations, and supporting these takes a lot of engineering and to make sure it works well and consistently. Where there are frictions for end-users when customizing from the outside, and there a developer toolkit is not an immediate solution for all existing websites, but rather, is a solution when building new sites. Future work will need to consider these barriers...
% \changed{However, these approaches face significant barriers for widespread adoption. }

% Perhaps an approach to address this challenge is to forego the development cost entirely by creating an end-user tool as a browser extension or plug-in \changed{for overview-detail interfaces}, similar to existing end-user customization tools explored in prior research \cite{Zhang2018Fusion, Visbug2024, Kim2022Stylette}. This tool could scrape the currently active website to identify overviews and detail views along with their associated attributes. The tool can \changed{also leverage AI to fetch} missing attributes \changed{from different pages}. However, websites are constantly evolving, requiring that the tool also adapt continuously to support as many sites as possible. Additionally, the tool would be limited by the data provided by the browser-compiled website data, potentially limiting the customization capabilities for the end-user.


% While a front-end toolkit could provide many composition and layout customizations such as many overview representations, dynamically surfacing and hiding attributes may involve application stack. 
% This toolkit would then become a framework at a more architectural level, that potentially packages together GraphQL and a UI component library.



% While a package that provides many overview representations out of the box or features for end-users to create multiple overviews and detail views could be achieved solely on the front-end of applications, 

% Enabling customizability in either directions---from the outside and the inside---have faced trade-offs both approaches have tried to address, and it still remains a challenge to effectively bring these customizations to the real world.

% \bryan{I should still say, regardless, this isn't the point of this paper, the point of this paper is to influence the designers and have more people advocate for these interaction techniques.}
% The risk is adoption. So what's going to stop adoption? What happens if these larger websites don't implement this?
% \bryan{Even if these toolkits or frameworks are not widely adopted in websites, authors of this paper and more inspired researchers can implement these features in smaller and simpler websites such as research lab websites or faculty directory pages. These implementations can help realize the utility of some of these customizations and carry over to more websites.
% Ultimately, the goal of this paper is to really just say you can implement these techniques across all interfaces in the design space, not just personal information management pages, spreadsheet or database-driven interfaces.
% }

% Ultimately, adding customization features is technically challenging 

% Still, adoption is difficult and hard to predict. Even if Living
% Papers falls short of a widely-used framework, it can be deployed
% for real-world publications and websites, and also help influence
% the trajectory and feature set of other tools. For individual users,
% Living Papers provides natural escape hatches: one can produce
% a LaTeX project or interactive web page and, if desired, jettison
% Living Papers and move forward with the generated outputs.

% For instance, REST APIs face the limitation that properties in tables cannot be flexibly taken apart and put together---GraphQL instead is the solution to this.}
% Another approach is to build a developer toolkit, such as a library or framework. This toolkit could offer all the variations and customizations outlined in our design space and enable our proposed interaction techniques out of the box. While integrating this tool into websites incurs a cost for developers, it could potentially reduce this cost if the toolkit provides default layouts that developers want to implement from the start. However, providing a broadly implementable toolkit requires engineering this tool to interoperate with existing websites and become reliably extensible to more overview-detail customizations in the future. 

% Both approaches present their own engineering challenges worth investigating. Future work should delve deeper into the benefits and challenges to effectively bring our malleable overview-detail interfaces into the real world.








% Perhaps the techniques for manipulating attributes explored in this paper may provide the means to elicit the most suitable representations.

% Perhaps these defaults can be iteratively customized kick-start their path towards creating their own abstractions.




% While this makes it high potential, it is challenging to address \textit{all} possible diverse needs we can not anticipate. We identify two hurdles to fully achieve the types of

% Participants surfacing diverse attributes hints at the potential for user-defined abstractions

% , forming diverse and unique abstractions---abstractions users formed to their own preferences, sets of attributes we could not anticipate users to surface.

% Thus, not only is a single representation enough, but \textit{providing} multiple representations to the end-user is not enough either. Instead, end-users must be able to create their own abstractions in diverse forms beyond what we can anticipate. While this goal is 



% Our study found that users could customize ....
% Self constructed, and diverse variations of overviews demonstrating that user-defined abstractions
% custom abstractions users can create on their own.
% We cannot possibly provide more representations for them. Providing multiple representations may not be enough to support understanding.
% Rather, they should form any own abstractions on their own. We envision an expressive way for users to form their own abstractions, beyond just surfacing specific attributes and forming overviews provided to them.
% But create their own abstractions of any form.




% Our study found that users could effectively customize which kinds of information they wanted to surface from the detail view to the overview with \technique.
% and which overview layout they wanted to see items in.
% At the core of the overview-detail pattern is the need to view information at different levels of abstraction, for different sets of details, and in different spatial arrangements during information tasks. 
% Their self-constructed overviews demonstrated their capability to choose which information to abstract away from the detailed views of all items.
% We believe this hints at the potential for \textit{user-defined abstractions}---abstractions that end-users can customize or create on their own, enabling them to engage with information in ways that best suit their needs.

% We believe this points to the potential for user-defined abstractions—customizable abstractions that allow end-users to tailor and shape their interactions to meet their specific needs, enabling them to engage with information in ways that best suit their preferences.
% For instance, if a user is new to a city and wants to know popular areas for lively restaurants, the user should be able to augment their map to display a heat map based on restaurant attributes such as \textit{Review Count}.

% While we propose a step forward with \technique, we identify two hurdles to fully achieve the types of user-defined abstractions we envision.
% lightweight, reliable, and expressive
%  to be communicate to the interface in a lightweight, reliable, and expressive way to produce
% First, we need to effectively support the diverse forms of abstractions end-users need. One approach can be through generative AI, with emerging systems being able to generate and render user interfaces on the fly \cite{anthropic2024claude35, vercelGenUI}. Though, the challenge still remains in allowing the end-user to understand and change this generated code when it inevitably fails to address the user's exact needs \cite{whyjonnycantprompt, sarkar2022like, designguidelinesforpromptengineering}.
% Second, and arguably more importantly, end-users must know \textit{what kinds} of abstractions they need to form. One avenue can be to provide recommendations and default abstractions users can use to kick-start their path towards creating their own abstractions.
% , by first modifying the defaults.
% We believe this direction can lead to promising insights in how the end-user can form and utilize dynamic representations to suit their needs.
% We believe this direction can lead to promising insights in how the end-user can form and utilize dynamic representations to suit their needs.
%  of overview-detail interfaces 



% % \subsection{Towards user-defined abstractions}
% \subsection{Malleable Interfaces: Beyond the Overview-Detail Interface}

% \bryan{To write or not to write?}
% \bryan{This section is not very clear to me right now, but this would lay down the long term vision of malleable interfaces that we want.}

% \textbf{Outline}
% \begin{itemize}
%     \item Can our design approach extend to more design patterns? Does this work provide a step towards making more interfaces malleable?
%     \begin{itemize}
%         \item Pattern 1: Collections
%         \item Pattern 2: 
%     \end{itemize}
% \end{itemize}


% We explored the interaction technique \technique.

% We are curious whether this can apply to other interface design patterns. 

% For a collection of items, definitely. selecting by attribute

% What is my argument in this section though? I don't even know what I want to talk about here, That's the problem

% Our goal: Malleable interfaces. We want to achieve this. We want end-user customization of anything they want, including functionality or whatever. 

% Our question is actually: Does our research approach work for other design patterns?

% What are other design patterns out there?

% viewports

% dashboards

% WYSIWYG



% In this research, we were primarily interested in the utility of the malleability of overview-detail interfaces, rather than the utility of each individual variation. Therefore, we did not implement all variations in the design space. However, implementing all variations into a system could provide a more comprehensive understanding of the utility of each design option within the design space. Additionally, there are opportunities to explore and implement more dimensions beyond the ones in this paper.
% A future study could also include more probes beyond shopping and hotel booking, which could offer valuable insights into which variations and instances users prefer and why in various scenarios.

% We only implemented a few of the variations because we were interested in utility of malleability of ODs, instaed of trying to evaluate the utility of each feature and each variation.
% Implementing all variations into a system  would give us a more comprehensive understanding of the utility of each variation in the design space.
% We could also expand this to more probes in different contexts beyond shopping and hotel booking.
% Studying this may offer insights to which variations and which instances users prefer in which contexts.

% Our two design probes do not implement all variations in our entire design space.
% we don’t implement our entire design space so we don’t claim utility or ease of use of all the variations we collected
% This paper explored three dimensions of variation in malleable overview-detail interfaces and provided interaction techniques for end-users to customize them.



% Furthermore, end-users must know \textit{what kinds} of abstractions to make. When
% Thus we ask the following questions: 

% In the case of \technique, we observed that end-users, such as P12, felt the attributes they surfaced better aligned with their decisino-making criteria.

% This can lead to future designs of malleable overview-detail interfaces that support more ways to abstract information from their details.

% Questions
% 1. How do we enable end-users to create their own abstractions?
% 2. How do we enable end-users to know what kinds of abstractions they need?

% * Our design space observed more forms of abstractions that attributes took, especially visual
% * There are various other forms of overviews that could be achieved, such as
% * 


% \textbf{Outline}
% \begin{itemize}
%     \item Study findings hinted at the value of user-defined abstractions---end-users being able to customize given abstractions and even form their own---through MODs.
%     \begin{itemize}
%         \item How can we further support user-defined abstractions? Can AI support this?
%     \end{itemize}
%     \item More dimensions for MODs
%     \begin{itemize}
%         \item axis, navigation, synchronization
%     \end{itemize}
%     \item Using AI to generate and customize more aspects of MODs
% \end{itemize}

% * We proposed an interaction technique of reformatting titles of items in shopping websites to make them more consistent and easier to read. There are opportunities to reformat more things. Even re-style things, re-arrange attributes to show certain things before others. You can change the size, so you can see specific details easier than others....


% - Towards user-defined abstractions
% \bryan{Our interface hinted at the potential that users can begin to create their own abstractions to suit their needs. Our probes specifically studied how users surface and hide their own details, this being Judy Fan's definition of abstraction. While it's limited, \technique was able to support users in creating their own abstractions that overview items represented for details.}

% \bryan{How can AI help create these different abstractions that people need?}

% % \subsection{There was this one section I wanted to write about, but I don't remember...}
% % \bryan{It was something about the findings from the user study... some result or something....}


% \bryan{Different definitions of abstraction: traditional definition, as well as Judy Fan's definition (more and less details)}

% \bryan{Talk about all the work on abstractions, Damien Masson, Bret Victor, Ian's Notational Programming}

% \bryan{But creating new abstractions are still tough. An initial challenge is that people cannot easily create our own abstractions. Programming is hard. Sketching is hard. To create abstractions, it takes time and effort, costs that people most likely do not afford to spend (This is why research is such a great incubator for novel abstractions). A more crucial challenge that precedes the previous is that people may not even know \textit{what kinds} of abstractions they need.}

% \bryan{Our study has shown signs that suggest user-defined abstractions---when provided the ability to choose which attributes they want to surface---can be achieved. ... Creating different kinds of abstractions in the same interface as well. In the hotel booking website, X/12 participants finished their task with different attributes surfaced in the bookmarks overview and the map overview. When asked about }

% \bryan{Creating more visual abstractions through AI could be possible. While multiple representations are fixed in our probes, generative AI tools have the potential to construct custom abstractions based on attributes people surface in the overview.}





% Our exploration of design probes and observations from our user study reveal opportunities to support more variations of overview-detail interfaces. We discuss future steps to study these opportunities in the long term, identifying practical approaches to implement malleable overview-detail interfaces in real-world websites.

% Our exploration of our design probes and observations from our user study ---> there are opportunities to support more variations of overview-detail interfaces, future steps to further study ... in the long run, and approaches to take to practically implement malleable overview-detail interfaces in realworld websites


% In this section, we discuss how customization behaviors may differ with prolonged use of malleable overview-detail interfaces and provide how future work can further study these behaviors. We then discuss how malleable overview-detail interfaces could be practically implemented in real-world websites, and then finally explore approaches to making overview-detail interfaces even more malleable.


% Perhaps an approach to take is to scrap the plan to convince developers entirely by doing it ourselves and making an end-user tool in browsers, following the many end-user customization extensions tools from prior research \cite{}.
% + We can scrape the currently active website to identify the overview and detail view as well as all their attributes
% + Leverage AI to cover for missing attributes and make data more consistent.
% - Websites are also constantly evolving, which will require the extension to constantly evolve to support as many websites as possible.
% - We are limited by the data provided in compiled code through the browser, forcing us to reconstruct the data already constructed by the website providers
% - This is only scoped for the browser. (I might remove this argument, cause framework also scoped to browser)

% \textbf{Outline}
% \begin{itemize}
%     \item We find MODs are very useful and people really want it. How do we practically bring this to the real world?
%     \begin{itemize}
%         \item It's about reducing the burden for developers --- developer toolkit
%     \end{itemize}
% \end{itemize}


% - Practical value of malleable overview-detail interfaces
% \bryan{Transition to ``Well, inevitably, everyone is different, even within our identified groups. This means we still need malleability. How do we practically implement malleable overview-detail interfaces?''}
% But we also need these customizations to become easily accessible, become defaults of the overview-detail interface.

% \bryan{We have demonstrated that end-users can and will customize overview-detail interfaces.}
% \bryan{We have also demonstrated---through our design probes---malleable overview-detail interfaces can be built effectively.}
% \bryan{But the question remains: Is it practical to invest the time and effort to provide such malleability in real websites? Will corporations and website providers actually build this?}
% \bryan{Certainly, creating more customization features requires more time and effort to develop, which costs money. The incentive for corporations and independent website providers to create a more malleable overview-detail interface is not necessarily in their best financial or personal interest.}
% \bryan{However, the financial and user experience benefits may exceed the initial cost to build. Improved user experience increases retention, retention increases likelihood of sales (cite? more logic?).}
% \bryan{The bottleneck lies in the burden for designers and developers to build these customizations to lower the barrier to bringing malleability to these sites.}
% \bryan{One way to achieve this is to provide a developer toolkit---a library or a development framework that provides a more malleable overview-detail interfaces out of the box.}
% \bryan{Note: Mention how overview representations have the potential to be interoverable with overview-detail interfaces now, through attributes}

% \bryan{Also, how do we actually get AI into the mix of things in these websites? We're already seeing many websites use AI as chatbots with LLMs being so powerful. Websites are using LLMs to return UI components within the conversational UI. But this means you lose the interface you designed to be used --- there's a disconnect. But with AI integrated into overview-detail, it's possible to directly change the UI. (But that's already been convinced in the past sections). }


% We found in our user study that participants had strongly agreed of the utility of our customizations, suggesting that users
% Our user study showed optimistic signs of the utility and value in malleable overview-detail interfaces for end-users. We have also demonstrated through our design probes that malleable overview-detail interfaces can indeed be built in websites.
% However, providing more customizability does require more development, and for all website builders---individual website providers to large corporations---costs in time and effort are extremely valuable.

% Our designs are valuable, and we provide results that signal the utility of these customizations.
% But ultimately, the decision to implement these designs fall to the hands of the developers---individual website providers to large corporations. And providing more customizability requires more development, which costs time and effort---extremely valuable resources for orgs and businesses.
% Thus, our question then becomes: How do we make it practical for developers to bring malleable overview-detail interfaces

% Our user study showed promising signs of the utility and value of malleable overview-detail interfaces for end-users. Our design probes further demonstrated that such interfaces can be effectively implemented on websites. However, adding more customization options requires additional development, which translates to significant time and effort—valuable resources for both individual website providers and large corporations.

% Thus, the key question becomes: How can we make it practical for developers to integrate malleable overview-detail interfaces into their systems?


% \paragraph{Developer toolkit for malleable overview-detail interfaces}



% \subsection{Seamless customization}
% We proposed \technique, which allowed users to easily surface, hide, sort, and filter attributes of interest.

% Filtering and sorting aren't really considered customizations, but they are configurations on the website. Similarly, reordering tabs on a browser is so lightweight that it's not a customization basically.
% Can \technique achieve this level of seamlessness in the interface?



% slowly dwindle or remain cyclical. 

% Regardless of the outcome, the need for malleable overview-detail interfaces remains unchanged. If users continue to alternate between various customizations based on different contexts, we indeed confirm the need for malleable overview-detail interfaces in our everyday use. If users converge towards an optimal overview-detail setting, the very tool needed to reach this optimal setting is through the malleable overview-detail interface.

% Perhaps we may converge to find out that users eventually reach a final default they like and never switch away from for all dimensions. Nevertheless, the value of malleable overview-detail interfaces still remain in \textit{enabling} users to reach this optimal convergence.




% * On the other hand, other participants had mentioned the utility of customizations, for instance P1 stated they wished they could stay in ``Attributes Mode''



% \textbf{Outline}
% \begin{itemize}
%     \item We don't want participants to customize all the time. We need to provide defaults that fit user groups.
%                     \begin{itemize}
%                         \item P11 said they will customize and just be done with it.
%                         \item P2 said they didn't like too many options to customize.
%                         \item Possible defaults we can provide to these groups?
%                         \item Need to figure this out. What are some defaults that might best benefit these groups? (Groups being Revealers, Removers, and Refiners; AI-enthusiasts; sub-task creators)
%                     \end{itemize}
% \item In addition to default MOD settings, we found participants who wanted some customizations to be default.
%     \begin{itemize}
%         \item P1 wanted to just stay in Attributes Mode.
%         \item Perhaps \technique is more ``seamless'' than the others, hinting at this customization being a necessary feature for user workflows. Similar to filtering and sorting---they are customizations, but so lightweight and so necessary, it's a default way to configure the interface.
%     \end{itemize}
% \item If we do give better defaults for MODs, will users still customize? If so, what will they customize? Is there a convergence towards a user-optimal set of features, or is there an alternating cycle?
%     \begin{itemize}
%         \item Future work could study this.
%     \end{itemize}
% \end{itemize}

% From these two needs, we find that there are people who want good defaults, but there are also people who want customizations by default.
% What are the features that users want as better defaults? What are features that users will inevitably still customize?
% Future work could design and implement better defaults for usage groups, and study user behaviors of these better default probes.


% - Design implications and recommendations for the user groups we identified
% \bryan{There are barriers to customization \cite{Mackay1991TriggersAndBarriers}, and thus would be most beneficial to provide more general defaults that tailor toward these groups.}
% \bryan{This talks about for these groups, what may be the default that will help them the most}

% \bryan{X/12 participants mentioned they would have liked to stay on Attributes Mode during the whole task, PX stating, ``....'''}
% \bryan{Another participant (PX) wished to be able to right-click to select the attributes instead to access the attribute even more in-situ.}






% One way to answer these questions can be to study the prolonged use of malleable overview-detail interfaces. Future work could build and deploy a robust probe to observe when and how frequently users make customizations. 
% This study would provide insights to the if and when users will find an optimal setting or continue to leverage various customizations in different contexts.

% We could use this probe to observe whether the a long-term use will lead to users finding their optimal default or continue to leverage various customizations in different contexts.



% These preferences can take us in two directions for malleable overview-detail interfaces: 1) users either converge towards an optimal default setting or 2) users constantly alternate between various customizations throughout their tasks.

% Users' desires to stay in

% that they would prefer a ``customization page'' where they can customize once and 
% these better defaults may be the desired ultimate outcome, .

% P11 commented on the matter of convenience/, ``\textit{Personally, I'd like a customization page or a separate menu for customization, something I can customize once and be done.}'' 


% * Rec default designs
% * This may be the desired outcome, that people simply want better defaults.
% * P11 says they want to customize and just be done with it
% * P2 says they don't like being given too many options to customize.
% * Then, this might show that providing better defaults for these groups would certainly be beneficial.
% * Other participants, however, mentioned that they wanted ``Attributes Mode'' to be a default for their interface, suggesting that users may constantly use \technique throughout their task. This means other participants would want to keep customizing, changing the various dimensions.
% * These decisions can take us in two trajectories: 1) Eventual convergence towards an optimal default setting or 2) an alternating cycle between customizations based on task.
% * The behaviors after we give these user groups improved defaults can take two trajectories: User needs and overview-detail defaults can converge
% perhaps we can provide them the defaults they want, and run the study once more. Will users still customize?




% P11 - Customize and done
% It might be like personally I think I like, I like like a customization page possibly or a a separate menu for customization that I feel like I customize once and then I'm done. Yeah. But for featuring customization like the hide on and off, yeah, I if I were to hope for a way to do it, I just, I want like maybe a check box or maybe some like keywords I can type into it, Yeah.

% P2 - given so much power, I don't like like many options to customize. I think I wasn't sure which ones might be like, I have an idea like what might be more important for me, like for this specific task, but like, I don't know if I'm choosing the right ones for those, if that makes sense. I see, like, yeah, maybe I want like a recommendation of like most people sorted by price, size and weight or something like that. And like, oh, I didn't think about weight. Like I want a heavy like monitor or not, or yeah. And so like I'd want to also filter by that or like, yeah, I don't know, like being able to not only choose what filters I want to use, but also explore other useful filters for me in my use case. But I guess that's more of the like the kind of like AI powered suggestion, kind of like functionality, but maybe not what we're talking about for customization. 










% \bryan{AI Limitation: Refining Prompts}
% We also found participants who appeared to be primarily Revealers ended up hiding AI-generated attributes they no longer wanted. Likely due to the attribute and value being incorrect... they didn't want the value to distract them. However, some eventually did land on an attribute they wanted, but just through iteration. Allowing users to refine their prompt likely resolves this challenge.



% \bryan{Suggesting an equilibrium of attributes?}
% Hotel booking and shopping websites provided different number of attributes by default. The hotel booking website provided only the rating of the hotel, while the shopping website provided eight default attributes. This explains why participants hid more attributes on the shopping website as opposed to the hotel booking website, uncovering the behavior group of removers. However, some still did not remove attributes on the shopping website. This raises the question: regardless of provided defaults, will the end-user inevitably surface attributes they need, or is there a large enough barrier to stop users from surfacing all details they would need? Answering this may provide implications to the design of the defaults of malleable overview-detail interfaces.
% Although websites may converge to a subset of attributes most users may need



% \subsection{Isn't it always better to let people customize?}

% Diverse customizations can simply mean they make different changes to the interface. Giving them the same task does control, but diverse changes could just be because everyone does different things.

% Our study suggests users want diverse customizations of overview-detail, but it could also be because people just make a lot of different choices?

% \bryan{It is true. Having the option is better. But there are barriers to customization that aren't necessarily worth it. Wendy shares these barriers to customizing software, and a key barrier is simply how easy it is to customize.}
% \bryan{During our study, X/12 participants raised their score from the hotel booking website to the shopping website when rating Ease of Use on the content dimension (this might not be a valid argument). But X/12 participants DID state that \technique got easier to use because they became familiar with it during the hotel booking task.}
% \bryan{So ease of use and ease of learning are important. This might sacrifice discoverability, but once discovered, could be powerful.....? this reads weird}



% \subsection{Guidelines for practically implementing malleable overview-detail interfaces}

% \subsubsection{Practically Implementing \TechNique}
% \bryan{When designing \technique, we considered multiple interactions for users to easily select attributes. We explored area selection, standard in-browser text selection, and even simply right-clicking to open a context menu. We opted for a toggle button that highlighted all attributes to prioritize discoverability of the novel interaction technique.}
% \bryan{During our user study, while all 12 participants either agreed or strongly agreed that \technique useful, some wished for an easier way to manipulate attributes.}
% \bryan{X/12 participants mentioned they would have liked to stay on Attributes Mode during the whole task, PX stating, ``....'''}
% \bryan{Another participant (PX) wished to be able to right-click to select the attributes instead to access the attribute even more in-situ.}
% \bryan{Thus, our findings recommend designers to provide multiple ways---for discoverability and ease of access---for selecting attributes, when practically implementing \technique on websites}

% \subsubsection{Practically Implementing AI-assisted \TechNique}
% ...




% \subsection{How much malleability is enough malleability?}
% End-user customization can go as far as being able to edit the code \bryan{Reference what Geoffrey Litt and Clemens referenced in their talks --- MyWebstrates or Wildcard? Climbing step by step towards more code...?}



==> versions/R_R/9_limitations_future_work.tex <==
% \section{Limitations and Future Work}
% \label{section:limitation-future-work}


% \subsection{Content Analysis Limitations}

% \subsection{User Study}

% There may have been a learning bias from the hotel booking website to the shopping website, 


% Diverse customizations can simply mean they make different changes to the interface. Giving them the same task does control, but diverse changes could just be because everyone does different things.

% Our study suggests users want diverse customizations of overview-detail, but it could also be because people just make a lot of different choices?




% \subsection{Studying the Prolonged Use Malleable Overview-Detail Interfaces}

% % Certainly, a system with too many features becomes too complex for users to learn within the given time of a controlled study.
% % The purpose of our probes is to study the diverse customizations people make, rather if they utilize all customizations in a given time-frame. To this end, ...
% % % However, we do not undermine the importance of providing more customizability options malleable overview-detail interfaces.
% % Many other features in a practical setting, could be implemented to be more discoverable through a prolonged use of the system.


% % Since the purpose of the probes is to study the how people make diverse customizations when provided, rather than evaluating whether they can make effectively make and utilize every customization in the interface, we implemented a subset of our interaction techniques into our probes. 

% % Certainly, a system with too many features becomes too complex for users to learn within the given time of a controlled study.
% % The purpose of our probes is to study the diverse customizations people make, rather if they utilize all customizations in a given time-frame. To this end, ...
% % However, we do not undermine the importance of malleable overview-detail interfaces.
% % Many other features in a practical setting, could be implemented to be more discoverable through a prolonged use of the system.



% \subsection{Developer Toolkit for Malleable Overview-Detail Interfaces}

==> versions/initial_submission/1_introduction.tex <==
\section{Introduction}
\label{section:introduction}

The overview-detail design pattern describes interfaces that typically consist of two views: an overview that presents a collection of items along with their key attributes, and a detail view that provides an in-depth look at a selected item, including many, if not all, of its attributes \cite{Shneiderman1996OverviewFirst, tidwell1997pattern}. This pattern enables users to efficiently browse through a large number of information entities and delve into specific ones of interest, facilitating one of the most essential operations in information tasks \cite{Norman1986ProgressiveDisclosure, Hornbaek2001OverviewDetailBenefits}. This is perhaps why the overview-detail pattern has become ubiquitous in information systems, such as shopping, booking, and rental sites, calendars, email clients, messaging applications, news and video platforms, and numerous others (Fig. \ref{fig:teaser}A).

When developing an information system, designers and developers determine how the overview-detail pattern is instantiated for their specific context and purpose, considering factors such as the layout and interaction of the overview and the detail view, as well as the different sets of attributes to present in these views. For example, some email clients arrange the overview and detail side by side, with the overview displaying the sender, subject, and time of all emails and the detail view displaying the contents of the email. Many shopping websites, on the other hand, open the selected product's detail view on a new page to avoid cluttering the overview page. Many map-based booking websites display the detail view as a pop-up and the overview underneath to provide context, and often display a single attribute of an item in the overview (e.g., the price for hotels).

While these designers and developers strive to create the best design for their general user base, a single instantiation of the overview-detail pattern is not enough to match the diverse needs of all users and their usage contexts. 
For instance, separating the detail view onto another page can reduce screen clutter but may force users to repeatedly switch views (Figure \ref{fig:md-limitations}A). Meanwhile, displaying only the price of hotels on a map improves clarity but omits other attributes---such as ratings or the number of beds---that some users may prioritize (Figure \ref{fig:md-limitations}B). Yet, few modern interfaces are malleable, forcing the end-users to work with the design determined by their developers, regardless of the end-users' own needs. 
% , regardless of then end-users' own purposes and contexts. 
% , regardless of the end-users' own needs. 

\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{figures/1_introduction/limitations.png}
    \caption{(A) Semantic Scholar includes a paper’s title, authors, abstract, and others, but does not include figures in the master view. To view figures for each paper, the user must open each hyperlink to the paper’s detail view and toggle through every opened page. (B) Airbnb displays pins with prices on a map, representing the nightly prices of each stay. If the user wants to view other details, such as the number of bedrooms, ratings, number of reviews, the user must click on each place and navigate to a full page of details.}
    \label{fig:md-limitations}
    \Description{This figure contains two website interfaces labeled (A) and (B). Interface A shows two screenshots of Semantic Scholar, an academic research platform.The left screenshot presents a list overview of search results showing the title, authors, abstract, and other details for research papers. The right screenshot displays the detailed view of a selected research paper. The user must open each paper’s detailed view to see figures and other specifics. The overview does not display these figures directly. Interface B shows a map with price tags pinned at different locations, representing the nightly prices of accommodations on Airbnb. If users want to view details like bedrooms, ratings, or reviews, they need to click on each pin and navigate to a full-page description of selected accommodation. }
\end{figure}

At the core of the overview-detail pattern is the need to view information at different levels of abstraction, for different sets of details and in different spatial arrangements during information tasks. Therefore, the key question we explore is \textbf{instead of letting developers dictate how information is abstracted and presented, can we make the overview-detail design pattern malleable?} That is, can we empower end-users to flexibly customize overview-detail interfaces to meet their specific needs and preferences? We break this goal into three research questions:

\begin{enumerate}[label=\textbf{[RQ\arabic*]}, leftmargin=*]
    \item What is the design space of various implementations of this design pattern in real-world contexts, and how can they inform the development of malleable overview-detail interfaces? 
    \item What are the interface designs and interaction techniques that can enable end-users to flexibly transform an overview-detail interface?
    \item To what extent do end-users prefer and utilize malleable overview-detail interfaces to achieve their information tasks? What are the novel usage patterns? Is the malleability we provide enough?
\end{enumerate}

We take the following steps to address these questions. First, to understand the current variations of the overview-detail pattern (\textbf{RQ1}), we conducted a content analysis with a diverse sample of 303 instantiations of the overview-detail pattern collected from 156 websites and identified three key dimensions: \textit{content}, \textit{composition}, and \textit{layout}. Second, based on these dimensions, we developed interaction techniques that allow users to customize overview-detail interfaces along these three dimensions (\textbf{RQ2}). Among the interaction techniques we designed, a key novel technique we contribute is \textit{\technique}, which enables users to flexibly adjust what, where, and how information attributes are represented on the overview-detail interfaces, providing a simple yet expressive way to customize overview-detail interfaces (Fig. \ref{fig:teaser}B). For example, users can surface new attributes from the detail view to the overview (Fig. \ref{fig:teaser}C), hide unwanted attributes in the overview, and use any selected attribute to filter and sort items (Fig. \ref{fig:teaser}D). Assisted with AI, users can search attributes with natural language queries, generate synthesized attributes from existing ones, and apply a consistent format to diverse attribute values (e.g., making the titles of shopping items from different vendors consistent). We also demonstrate how \technique and allow users to integrate various overview representations.
% \haijun{We also demonstrate compelling use cases of synchronizing several overviews each providing a suitable representation of the chosen attribute (poor writing, but just want to leave a note here about what should be described in the intro)}
These interaction techniques enable users to more effectively discover and consume their desired information. We demonstrate these interaction techniques with a number of research prototypes.

Finally, to study the utility and usage patterns of malleable overview-detail interfaces (\textbf{RQ3}), we developed two high-fidelity design probes that implement our interaction techniques: a shopping website and a hotel booking website, and conducted a user study with 12 participants where they used both design probes to accomplish shopping and booking tasks. We found that participants given the same tasks produced diverse customizations of content, composition, and layout, highlighting the need for malleable overview-detail interfaces across these dimensions. They also found the malleable overview-detail interface preferable, sharing that it allowed them to control what they wanted to focus on, reduced unnecessary navigation, and aligned their decision-making criteria to the information they wanted. Finally, we report on the emergent usage patterns of malleable overview-detail interfaces and discuss practical implications that such interfaces may have for end-users, developers, and AI.

In summary, our work contributes:
\begin{enumerate}
    \item A content analysis of the overview-detail design pattern that revealed three key dimensions of the design space.
    \item Interaction techniques for malleable overview-detail interfaces, including a novel technique, \technique, that enables users to directly choose what, where, and how attributes are shown the interface.
    \item A user study demonstrating that participants effectively utilized malleable overview-detail interfaces to address diverse needs and revealing emergent usage patterns that inform design suggestions for future implementations.
\end{enumerate}























% Furthermore, \technique is designed for the overview-detail pattern as a whole, making it applicable across all overview-detail interfaces.

% A user study of these probes shows that users can effectively make such transformations when given the opportunity. We additionally report on emergent usage patterns that our interaction techniques enable.


% Users can also make customizations through AI, by asking for higher level queries, and even push it further by generating new attributes about items.

% We also recognize the opportunity for a malleable overview-detail interface to be used 

% For the potential of how we can interact with AI as a medium for a malleable overview-detail interface. 



% Our interaction techniques for the customizable overview-detail interfaces also serve as a medium 

% Our interaction techniques that we provide to the end-user also serve as a medium for AI to operate

% We also explore possibilities for overview-detail interfaces to be customized through AI. 


% Users can leverage these customization techniques to address personal needs, such as 

% For instance, users can leverage \technique to 

% This interaction technique provides users with the ability to pull any detail attribute from the detail view to the overview, hide unrelated attributes from the overview into the detail view, or sort and filter items directly upon selecting attributes of interest (Fig. X). Users may leverage \technique to ``pull'' additional details about homes beyond the default-provided price attribute.

% This interaction technique provides users with the ability to pull any detail attribute from the detail view to the overview, hide unrelated attributes from the overview into the detail view, or sort and filter items directly upon selecting attributes of interest (Fig. X).
% % Why?
% These interactions
% Furthermore, since \technique is an interaction technique for the overview-detail design pattern itself, it offers broad applicability across all such interfaces. For example, it directly addresses the challenge depicted in Figure \ref{fig:md-limitations}b by enabling users to pull any detailed attribute they need into the map view, 

% The elegance of \technique lies in its broad applicability across all overview-detail interfaces

% The elegance of \technique lies in its ability to personalize information shown or hidden in the interface, addressing the challenge of either missing details or being overwhelmed by excessive information, while also offering broad applicability across all overview-detail interfaces.

% \bryan{Include the possiblities of \technique with AI}

% \bryan{Intro needs a statement about how we are really trying to contribute a principle or something, to enable this underlying interaction/info architecture for AI to be better used or something}

% Detailed manipulation is 

% \textit{What is the technique? What's good about it? Why is it important?}


% This interaction directly addresses the challenges illustrated in Figure \ref{fig:md-limitations}b by allowing the user to choose to pull the number of bedrooms or ratings of a place to the map view.

% A key novel technique we contribute is \textit{pulling the details}, which enables users to select and ``pull'' details from a detail view to items in the master view (Fig. <in-teaser-figure>). A \bryan{Deeper into the interaction techniques and their benefits}


% Over the decades, many software interface design patterns have evolved dramatically, while others have remained foundational, serving as the bedrock for countless designs. One such pattern is the master-detail (MD) interface, which presents an overview of items (master) alongside detailed information about a selected item (detail) \cite{Seffah2015PatternsOH, Molina2002JustUI}. Despite being implemented since the early days of user interfaces, this pattern has become ubiquitous, seen in applications ranging from calendars to e-commerce platforms. Figure \ref{fig:md-variations} illustrates this evolution: a calendar interface from 2000 (Fig. \ref{fig:md-variations}a) and Google Calendar\footnote{} in 2024 (Fig. \ref{fig:md-variations}b) both implement the same MD pattern, though with updated visuals. Other variations of this pattern include BestBuy\footnote{}, which separates the master and detail views across different web pages (Fig. \ref{fig:md-variations}c), and Zillow\footnote{}, which displays a map-based master view with a detail popup (Fig. \ref{fig:md-variations}d).

% \begin{figure}
%     \centering
%     \includegraphics[width=0.75\linewidth]{figures/md-instances/variations.png}
%     \caption{(a) Calendar interface from a CHI 2000 Extended Abstract \cite{Laakso2000MDCalendar}. (b) Google Calendar interface (as of 2024). (c) BestBuy’s shopping interface displays the master view in one web page and the detail view in another. (d) Zillow’s interface displays a master view of listings on a map and a detail view of a selected listing in a popup.}
%     \label{fig:md-variations}
% \end{figure}

% While each implementation of the MD design pattern may tailor the needs to their general user base, a single implementation also reveals interaction constraints. For instance, separating the detail view onto another page can reduce screen clutter but forces users to repeatedly switch views (Figure \ref{fig:md-limitations}a). Meanwhile, displaying only the price of homes on a map improves clarity but omits other details—such as ratings or the number of bedrooms—that some users may prioritize instead (Figure \ref{fig:md-limitations}b).

% \begin{figure}
%     \centering
%     \includegraphics[width=0.75\linewidth]{figures/md-instances/limitations.png}
%     \caption{(a) Semantic Scholar includes a paper’s title, authors, abstract, and others, but does not include figures in the master view. To view figures for each paper, the user must open each hyperlink to the paper’s detail view and toggle through every opened page. (b) Airbnb displays pins with prices on a map, representing the nightly prices of each stay. If the user wants to view other details, such as the number of bedrooms, ratings, number of reviews, the user must click on each place and navigate to a full page of details.}
%     \label{fig:md-limitations}
% \end{figure}

% Despite the multitude of MD implementations designed to address various user needs, most interfaces typically use only a single instance of the MD design pattern. \textbf{However, a single instance is not enough for the diverse needs of all users.} Instead, users should be able to customize the MD interface to control the presentation and organization of information according to their specific needs.

% Despite the widespread use of the master-detail (MD) design pattern, our understanding of its variations remains limited. Existing research identifies variations in master view structures (e.g., list of items, single instance) and explores nested MD interfaces \cite{Seffah2015PatternsOH, Molina2002JustUI, Nguyen2012MDAndroid}. However, there is a lack of a more comprehensive, empirical analysis of these variations, leaving many aspects of MD interfaces underexplored.

% In this research, we aim to better understand current variations of the MD design pattern and provide mechanisms for users to transform these interfaces to meet their specific needs. Through a content analysis of 303 MD instantiations on desktop web interfaces, we identified three key dimensions of variation: \textit{layout}, \textit{composition}, and \textit{content}.

% Through our exploration of the design space, we developed interaction techniques that allow users to customize the MD interface along these three dimensions. A key novel technique we contribute is \textit{pulling the details}, which enables users to select and ``pull'' details from a detail view to items in the master view (Fig. <in-teaser-figure>). To demonstrate these techniques, we developed two design probes: a shopping interface and a hotel booking interface. A user study of these probes shows that users can effectively make such transformations when given the opportunity. We additionally report on emergent usage patterns that our interaction techniques enable.

% In summary, our work contributes:
% \begin{enumerate}
%     \item A content analysis of master-detail interfaces that maps variations into a design space along three dimensions.
%     \item Interaction techniques enabling transformable MD interfaces, demonstrated through two design probes: a shopping interface and a hotel booking interface.
%     \item A user study demonstrating that users can effectively utilize transformable MD interfaces to address individual needs.
% \end{enumerate}




% We do know that variations do exist, and there are various needs for them. 

% For instance, there are variations in how each of the two views arrange information, we know

% The ubiquity of the master-detail design pattern across various software interfaces makes it particularly interesting to study. Academic research and online articles have highlighted a few key variations of MD interfaces. For instance, Seffah discusses different structures a master view can have, such as a list of items or a single item instance. Additionally, case studies have explored how different screen sizes necessitate varying arrangements of the master and detail views, and how MD interfaces can be nested to create hierarchical structures within applications \cite{Seffah2015PatternsOH, Nguyen2012MDAndroid, Medium article}.

% Despite the ubiquity of the MD design pattern, we only have an informal grasp of the kinds of MD interface variations exist \cite{Seffah2015PatternsOH}. 

% \bryan{There needs to be a paragraph laying out the current state of research in MD patterns}
% There needs to be a paragraph laying out the current state of research in MD patterns
% If there is nothing, then also must say something like: despite its ubiquity, we only have an informal grasp of the variations of MD interfaces that exist in the wild and little understanding of what MD transformations are available today.




% This work unveils the interaction possibilities that can 
% I feel there needs to be this last sentence that says what this paper concludes.
% Some big moral of the story type of paragraph.
% We want to share that looking into the ubiquitous design patterns can provide ways to think of novel interaction techniques that are also very generalizable across a wide range of domains
% We want to share that this work is the foundation for .. what? idk
% Want to say this design space can be a generative tool...? --> nah that needs to be proved, through like a workshop or something. Also it's obvious that a design space is a generative tool. That's the entire point of a design space is to better see what you can implement within the space but also other variations you can explore.
% We conclude with design recommendations from our design space, design probe explorations, and user study findings.






% While many designs of software interfaces have evolved significantly, some have remained unchanged, becoming foundational interface patterns that other patterns and designs build upon. 

% Figure 2a depicts one interface implemented in the year 2000, showing a list of days of a calendar in the left pane and a detailed view of selected days in the right. Figure 2b depicts a similar interface in 2024 that displays the same pattern from Figure 2a. This pattern has been referred to by many names, one of which being the Master-Detail (MD) pattern, which is defined to present an overview of a set of items in one view (Master) and details of thea selected item in another view (Detail) []. Not only has this pattern been implemented for an extended period, but it has also grown ubiquitous over time, accumulating numerous variations in the arrangement of the two views and how information is presented in the MD interface. For example, Figure 2c depicts a variation where Master and Detail views are separated into two different web pages, while Figure 2d depicts a variation where the Master view’s items are placed on a map with the Detail view displayed in a popup panel.

% Figure 2: \textit{(a) Calendar interface from a CHI 2000 extended abstract displays a Master-Detail view in a single page []. (b) Google Calendar interface (as of 2024) displays a similar Master-Detail view. (c) BestBuy’s shopping interface displays the Master view in one webpage and the Detail view in another. (d) Zillow’s interface displays a Master view of listings on a map and a Detail view of a selected listing in a popup.}

% While the various implementations of MD interfaces may have addressed all kinds of user needs, they have also revealed more interaction constraints. For instance, while creating a separated web page for the Detail view can reduce cognitive overload from an interface, certain details may not be displayed in the Master view, forcing the user to repeatedly toggle through Detail views of each item (Fig. 3a). Additionally, while a popup view can retain the context of the Master view, it cannot retain the context of the popup view itself, potentially causing the user to lose progress on any working information in the popup (Fig. 3b). <Something about how there’s a solution for the problem in Fig. 3a, but 3a has another problem, which Fig. 3b can address, but this reveals another problem, maybe another view can address>

% Figure 3: \textit{(a) Semantic Scholar includes a paper’s title, authors, abstract, and others, but does not include figures in the Master view. To view figures for each paper, the user must open each hyperlink to the paper’s Detail view and toggle through every opened page. (b) ESPN lists articles for each highlight of a Wimbledon match and can open a popup to its video highlight. If the user wants to continue scrolling through the list of highlights, they must close the popup, losing progress of the video they are actively watching. To make things worse, each time the user reopens the popup, the video starts with an ad.}

% Despite the multitude of MD implementations that address various user challenges, each interface typically only implements a single MD instance. However, a single instance of the MD design pattern is not enough to support the diverse needs of end-users. Instead, end-users must be able to customize the MD interface to address their own needs.

% Thus, the goal of this research is to uncover the variations of MD interfaces that exist in websites and leverage this understanding to generate solutions for transforming MD interfaces that suit end-user needs.


% … content analysis … Design space

% … Interactions … user study … discuss…


% Contributions

% \begin{itemize}
%     \item Design Space of MD interfaces on what and where information is presented synthesized from content analysis \& designer interviews
%     \item Probes to demonstrate ways that a transformable MD interface can be implemented
%     \item User study observing how users interact with these probes


% \end{itemize}


==> versions/initial_submission/2_related_work.tex <==
\section{Related Work}
\label{section:related_work}

\subsection{The Overview-Detail Design Pattern}
The overview-detail design pattern describes interfaces that provide two views: an overview that contains a collection of items and a detail view that provides full details of a selected item \cite{Shneiderman1996OverviewFirst}. This pattern, also referred to as ``master-detail’’ \cite{Seffah2015PatternsOH, Molina2002JustUI, Nguyen2012MDAndroid} and ``director-detail’’ \cite{Pastor2007ModelDrivenArchitecture}, is designed to manage and visualize information such that users are able to view a large collection of items first before uncovering their details.
% (Fig. \ref{fig:md-definition}) .
If overview-detail interfaces are designed with progressive disclosure in mind, they can offer a more approachable experience while still allowing users to access additional details. \cite{Norman1986ProgressiveDisclosure, Shneiderman1996OverviewFirst}.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.75\linewidth]{figures/md-instances/definition.png}
%     \caption{(a) The overview that contains a collection of items. (b) The detail view that presents all details of a selected item from the overview.}
%     \label{fig:md-definition}
% \end{figure}

Prior research has explored several variations of the overview-detail pattern in user interfaces. Case studies have explored how overview-detail interfaces can be nested to create hierarchical views \cite{Molina2002JustUI, Seffah2015PatternsOH}, how several detail views can be used simultaneously \cite{Saidi2016SplittingDetailViews}, and how different screen sizes may necessitate varying arrangements of the overview and detail views  \cite{Seffah2015PatternsOH, Nguyen2012MDAndroid}. 
Cockburn \etal{} have also explored how overviews and detail views can be arranged horizontally, vertically, and also along the ``z-plane'' by layering nested overviews and detail views along the z-axis, navigable by zooming. This z-axis arrangement describes the structure of zoomable user interfaces such as Pad++ \cite{Bederson1994Padpp, Cockburn2009OverviewDetailReview}. 
A relevant but distinct design pattern also explored is ``focus+context'' interfaces \cite{FirstFocusContextInterface}, where focused content is placed seamlessly with the rest, oftentimes by reducing the view of the context space by skewing the views in 3D \cite{Mackinlay1991PerspectiveWallFocusContext}, scaling \cite{bederson2000fisheye}, and reducing the display's resolution \cite{Baudisch2001FocusPlusContext}.  

These works demonstrate the diverse implementations of the overview-detail design pattern developed through research, resulting in unique design choices tailored to specific contexts. However, our research aims to explore designs that enable users to flexibly customize the overview-detail interface according to their individual needs.

% While these works aim to design better defaults for overview-detail instances, we aim to enable users to flexibly customize the overview-detail interface to address their own needs.
% I think all previous work is about finding good defaults for specific ccontext, but our work is about eanbling flexible customization for a given context by the usesr.
% These works demonstrate the diverse implementations of the overview-detail design pattern developed through research, resulting in unique design choices tailored to specific contexts. While past studies have reviewed select cases of this pattern, we aim to explore its implementations on the most commonly used websites with a formal empirical analysis.

\subsection{The Need for Malleable Overview-Detail Interfaces in Information Tasks}
Many information tasks, such as foraging \cite{infoforagingtheory}, sensemaking \cite{coststructuresensemaking}, and decision-making \cite{mesh}, involve the iterative process of searching, browsing, collecting information across various sources, making sense of collected information through various representations, and then collecting new information based on the new insights \cite{coststructuresensemaking, Pirolli2005SensemakingProcess}. In this process, users require effective representations to organize and preview a large number of information entities and quickly determine relevant ones by inspecting their details. The overview-detail interfaces directly respond to such needs and, therefore, are ubiquitous in information systems, including information visualization systems \cite{Card1999VisionToThink, bach2016TellingStoriesGraphicComics} and academic literature exploration tools \cite{Relatedly, kang2023synergi}.

As mentioned earlier, a single instantiation determined by developers is not enough. Therefore, many research systems that have been created to support information tasks are essentially providing additional overview-detail instantiations to compensate what could not be supported with existing ones. For example, prior work has provided comparison tables to better organize decision-making criteria \cite{mesh}, hierarchical organizations of collected snippets to facilitate information management and re-finding \cite{threaddy, Synergi, fuse}, spatial canvases that scaffold the user's search and synthesis processes \cite{Ramos2022ForSense, Tashman2011LiquidText, Srishti2022InterWeave}, and node-link diagrams to contextualize users with their past browsing activities \cite{graphhistory}.

Another line of work recognizes that a single instantiation is not enough and proposes providing multiple instantiations, such as those that enable multiple levels of details or transforming information representations. Pad++ introduced semantic zooming, which offers multiple levels of detail based on different zoom levels, providing an alternative to geometric scaling techniques used in traditional zoomable interfaces. Recent research has also built on this idea to utilize AI to generate these different levels of detail \cite{Dang2022BeyongTextGeneration, Suh2023Sensecape, suh2023luminate}.
WritLarge demonstrated techniques for transforming between multiple representational axes—semantic, structural, and temporal—on a digital whiteboard \cite{Xia2017WritLarge}. This enables users, for instance, to write a list of to-do items on the whiteboard, reify it into a checklist, and interact with it to mark items as complete. Transforming the checklist back to the sketch could retain the changes of marked items in digital ink.
Bret Victor additionally illustrated the need for multiple representations through the concept of a ladder of abstraction, which demonstrates how moving between different levels of abstraction helps to gain a more comprehensive understanding of a system \cite{Victor2011LadderOfAbstraction}. 
Graphologue also explored multiple representations by leveraging AI to generate text alongside a node-link diagram side by side to facilitate information comprehension \cite{Graphologue}.
We share the spirit of these systems that aim to provide multiple representations by providing end-users the ability to transform and customize between different variations of overview-detail interfaces.


\subsection{Designing Interfaces for Customizability}

% Designing for customizability
% 1. Settings. Not easy to just access (Menu). So one line was to provide settings that are easier to access on the interface
% 2. Browser customizability. precise control over specific needs, but lots of code.
% 3. Enabling prompts for user to ask for specific changes. AI is expressive, but volatile. 

% So how can we enable easy (1), precise (2), and expressive (3)

% We need a vocabulary for users to share their needs in an easy (1), precise (2), and expressive (3) way.


Designing customizable interfaces requires understanding and balancing the costs and benefits that influence users to customize their interface. 
Mackay observed that users may be motivated to customize their interface when they recognize and grow frustrated of repetitive patterns, while users may be less inclined when the task of customizing is too difficult or time consuming that the perceived benefits are not worth the effort \cite{Mackay1991TriggersAndBarriers}. 

To balance this trade-off, several approaches have been explored to design interfaces for customizability. One approach has been to bring the customization settings visually closer to the UI components. For example, Anchored Customization integrates individual setting options directly into conceptually related UI components, providing a more ``in-situ'' way to access customizations \cite{Ponsard2016AnchoredCustomization}. 

Another line of research has instead prioritized expressiveness and power by opening the interface code to the end-user, allowing passionate developers to extend the interface to others' and their own needs. Web browsers are notable examples of this case, where compiled HTML, CSS, and Javascript code are made available for end-users to view and change. Researchers and developers have capitalized on this opportunity to support a diverse array of tasks, including website prototyping \cite{Kim2022Stylette, Visbug2024, Tanner2019Poirot, Zhang2018Fusion}, active reading and note-taking \cite{Romat2019SpaceInk}, and filtering, sorting, and making spreadsheet computations \cite{Litt2020Wildcard, Huynh2006Sifter, Hogue2005Thresher}. Research has also explored the potential of web mashups and automations with dedicated programming and direct-manipulation environments \cite{Ghiani2016WebMashup, Bolin2005Chickenfoot, Hartman2007Dmix, Huynh2006Sifter, Lin2009Vegemite} and collaborative dynamics with shareable, modifiable, and extensible software across multiple different platforms \cite{Klokmose2015Webstrates, varv}. While this approach provides an expressive way to customize interfaces, it can be difficult for end-users who lack the time or skills to make these customizations.

Our work aims to empower everyday users to customize their overview-detail interfaces. Our insight is that the overview and the detail view are two different containers of different sets of attributes. By treating attributes as first-class citizens and making both the attributes and views accessible and manipulable, we can enable end-users to flexibly customize them. This resembles the line of work on attribute objects by Xia \etal{} \cite{ObjectOrientedDrawing, Xia2017CollectionObjects, DataInk}. By decomposing graphics objects into attribute objects, these systems enable users to flexibly compose new graphical styles, search for graphical objects with attributes as filters, and create data visualizations by combining data and visual attribute objects as visual encodings. Our work arrives at a similar approach but explores interactions with attributes in the overview-detail design pattern, rather than on content creation. A unique step forward in our work is that, in addition to flexibly manipulating developer-defined attributes, we also enable end-users to leverage AI to create user-defined attributes, further expanding the expressiveness for end-user customization.



















% To provide end-users with more granular control over the interface while maintaining a low cost, a line of work has explored techniques for manipulating attributes of drawing objects in gesture-based creativity support tools \cite{ObjectOrientedDrawing, Xia2017CollectionObjects}. This work leverages the fact that drawing objects often have multiple associated attributes, providing opportunities to select objects based on shared attributes, as well as to clone and blend them. Our work arrives at a similar approach, identifying that overview-detail interfaces contain items with many common attributes, which offers users the potential to manipulate and customize the interface.

% taking out the AI thing for now, since it's not directly relevant. 
% The recent surge in generative AI has introduced opportunities to make it both easy and expressive for end-users to customize their interface by using AI to generate and render UI code from user prompts \cite{anthropic2024claude35, vercelGenUI}. While this approach is promising, the mappings between natural language prompts and generated code are not shown to the end-user, giving no way for them to understand or adjust the generated interface \cite{whyjonnycantprompt, sarkar2022like, designguidelinesforpromptengineering}.


% as we similarly identify that overview-detail interfaces contain items with many common attributes, offering users the potential to manipulate them to customize the interface. 
% We further identify that this approach enables an expressive mechanism for customizing overview-detail interfaces 

% and this approach can also be used with AI to map user prompts to specifications \cite{vaithilingam2024dynavis, bespoke}. 


% We explore the opportunity to surface attributes for the end-user to customize their overview-detail interface


% To provide end-users with more granular control over the interface while maintaining a low cost, prior research that has explored techniques for manipulating attributes of drawing objects in gesture-based creativity support tools \cite{ObjectOrientedDrawing, Xia2017CollectionObjects}.
% Work leveraging the fact that drawing objects have many attributes associated with them, demonstrated opportunities for selecting objects of common attributes, cloning, and blending.
% Our work shares this approach, as we identify that overview-detail interfaces often contain items with many common attributes, providing an opportunity for users to directly manipulate.
% % We further explore the opportunity to leverage 


% To offer end-users more granular control over the interface while maintaining a low cost, we build on previous research that investigates techniques for attribute manipulation in gesture-based creativity support tools \cite{ObjectOrientedDrawing, Xia2017CollectionObjects}. These studies have demonstrated that manipulating attributes allows users to effectively select and transform collections of media objects \cite{Xia2017CollectionObjects}. We extend this design approach to customizable overview-detail interfaces, enabling end-users to manipulate attributes across all items, thereby facilitating interface customization.




% By bringing the control of attributes
% This approach enables users

% The ability to manipulate attributes demonstrated the ability for  to select and transform collections of media objects effectively \cite{Xia2017CollectionObjects}. 

% We extend this design approach to customizable overview-detail interfaces, enabling end-users to manipulate attributes across all items to customize the interface.


% So we want to give end-users more granular and expressive control over the interface while keeping these customizations approachable and low cost.

% Well, research has explored ways to provide users with more granular and direct control for gesture-based creativity support tools, allowing you to manipulate attributes as objects. 
% Manipulating attributes has also demonstrated the ability for users to select and transform collections of media objects \cite{Xia2017CollectionObjects}. We share this design approach for making overview-detail interfaces customizable, enabling the end-user to manipulate attributes across all items in the overview-detail interface.

% An approach to supporting both granular and ``direct'' control has been explored through


% To design an overview-detail interface that is customizable, we take the approach of leveraging the 

% i was about to talk about attribute manipulation, but then i realized it doesn't flow well with the content analysis. So I want to hint at it, but not make it the main focus. 

% I want to talk about mappings

% If we want users to customize their interface in a 

% Xia \etal{} have explored interactions for manipulating attributes of strokes and shapes digital art creation \cite{ObjectOrientedDrawing, Xia2017CollectionObjects}. Notable thing is Collection Objects, enabling users to select and transform collections of items on a sketching canvas based on the attributes \cite{Xia2017CollectionObjects}.
% We share this approach to controlling the overview-detail interface by supporting interaction techniques for users to control attributes shared across items in the overview.

% \bryan{Take parts from this RW to talk about how systems have tried making customizable software. End-user customization, all general customization}

% \subsection{Constraint-based Adaptation}
% Prior work has explored computationally adapting UIs based on various contextual factors and constraints pertinent to the device, user, or situation in domains such as accessibility, ubiquitous computing, and mixed reality \cite{dey2001conceptualcontext, abowd1999context, computationalApproachUIGen, wobbrock2011ability, gajos2010personalization}. For example, SUPPLE and SUPPLE++ computationally adjust the size, style, and layout of widgets to adapt GUIs based on device constraints (e.g., screen size, input modality) and users’ capabilities (e.g., motor and vision) \cite{gajos2004supple, gajos2010personalization, supple++}. UNIFORM and Huddle automatically generate UIs  with primitive widgets for controlling home appliances by considering users’ interaction history as well as modeling the similarities and dependencies of appliances \cite{uniformNichols, HuddleAutoGenUIAppliances}. Since mobile and Mixed Reality (MR) interfaces can be invoked in arbitrary situations, research has also explored adapting these interfaces based on various environmental factors \cite{lindlbauer2019context, dey2001conceptualcontext}. For example, Lindbauer et al. explored how applications should dynamically adapt the amount of information they show and their spatial arrangement in an MR context \cite{lindlbauer2019context}.
% With this approach, the data schema remains the same, and the encoding remains program-based but augmented with contextual constraints, resulting in context-aware dynamic interfaces. However, the scope of the dynamic behaviors is pre-defined by developers, and end-users are unable to change the underlying data scheme and encoding.
% \subsection{End-User Customization}
% Previous research has explored creating interactive systems that are both customizable and extensible, allowing end-users to tailor them to their specific needs. This work is primarily situated within the field of end-user programming or development (EUP or EUD) \cite{nardiProgramming}, where end-users can employ natural language programming \cite{PUMICE}, GUI-based interaction \cite{litt2020wildcard, Hypercard, fusion}, visual programming \cite{Scratch, DynamicLand}, and programming-by-demonstration \cite{vegemiteJames} to extend existing systems.
% For example, pioneering systems like OpenDoc \cite{Apple_OpenDoc}, HyperCard \cite{Hypercard}, Smalltalk \cite{kay1996early}, and recent system DynamicLand \cite{DynamicLand} aimed to develop dynamic and personal media for end-users to create their own dynamic content and UI. Hypercard allows users to develop interactive multimedia content by linking objects via GUI and scripting advanced behaviors using a built-in programming language \cite{Hypercard}. These systems pre-define the underlying data schema but expose the encoding mechanism to enable EUD.
% To circumvent the lack of access to the applications’ internal data schema, research has explored constructing external data schema to enable EUD. For example, with the accessible and manipulable
% Document Object Model (DOM) of webpages, Wildcard supports collecting data from and injecting data back to the webpage DOM structure, and by representing the data using an external spreadsheet, end-users can manipulate the spreadsheet to customize the web pages.\cite{litt2020wildcard}. Further leveraging the composability and transclusion of the web \cite{Nelson1995Transclusion}, prior work explored enabling end-users to create mashup applications to achieve their specific needs. For example, Fusion and C3W enables users to create mashups by extracting components from existing webpages and connecting them using transclusion, formula, and glue code \cite{fusion, fujima2004c3w}. Vegemite enables users to collect data from multiple websites; using scripts that can be generated from users’ demonstration, it can perform computation on the collected data and automatically execute web actions such as clicking links and inputting data values to web forms \cite{vegemiteJames}.
% With EUP/EUD, the applications’ internal data schemas often remain inaccessible to end users, but the encoding mechanisms are available for them to extend the applications. While external data schemas, often spreadsheet, can serves as the proxies or connectors with the original applications, these external data schemas are also pre-defined by developers, leaving end-users still with limited customizability.
% \subsection{Specification-based Synthesis}
% In addition to adapting and extending applications, prior research explored generating entire applications and UIs to support end-users’ information tasks. For example, Nichols et al. explored employing a specification language and parameterized templates that encode design conventions to automatically generate interfaces for controlling home appliances \cite{NicholsSmartTemplate, nichols2002requirements, GeneratingRemoteControl}. Based upon the specification of command-line applications, Bespoke can synthesize custom GUIs by mapping UI widgets to different types of command-line parameters \cite{bespoke}. Similarly, DynaVis composes UI widgets to create interfaces for controlling parameters inferred from users’ natural language queries to edit data visualizations \cite{vaithilingam2024dynavis}.
% Another theme in this direction is designing a programming model based on high-level specification language. This enables users to focus on composing high-level domain-specific primitives and deferring low-level execution architecture and runtime \cite{heer2010declarative}. Using a high-level declarative grammar, Vega-Lite enables rapid specification of interactive data visualizations \cite{vega-lite}.
% Inspired by the success in data visualization, Varv explored representing interactive software as a declarative data structure that describes the schema and actions of a set of concepts \cite{varv}.
% With this approach, developers carefully design the specifications, which dictate the space of possible UIs and ensure the consistency and quality of the generated UIs \cite{NicholsSmartTemplate}. Although end-users can technically generate UIs within the boundaries set by these specifications, their ability to do so is mediated by the encoding mechanisms. To enable end-users to intuitively generate the applications and UIs, prior research often provides an additional layer of graphical and natural language interfaces which are mapped to the underlying specifications \cite{vaithilingam2024dynavis, bespoke,narechania2020nl4dv, crosspower}.
% \subsection{AI-based Code Generation}
% Recent developments in AI, especially its ability to generate functional program code from natural language prompts, have sparked a new approach toward generative UI. AI products such as Claude \cite{anthropic2024claude35} and Vercel \cite{vercelGenUI} can generate and render UI code from natural language prompts. Wu et al. explored fine-tuning LLMs with automated feedback to improve the quality of the generated UI code \cite{wu2024uicoder}. As AI’s code generation capability continues to improve \cite{anthropic2024claude}, the complexity and quality of AI-generated applications and UI will likely increase.
% However, this UI generation approach can be a double-edged sword. On the one hand, AI can generate code for arbitrary user prompts. On the other hand, the lack of understandable and controllable mappings between users’ prompts and low-level code makes it challenging for end-users to customize the generated UIs when AI inevitably and probably constantly fails to meet users’ dynamic and shifting goals. For example, research has shown that end-users face considerable challenges in prompting AI to design interactive systems \cite{whyjonnycantprompt}.
% With this approach, while both the data schema and the encoding are dynamically generated, resulting in generative UIs, the low-level code representation and the obscure mappings between natural language prompts and generated code pose significant challenges for end-users to control and customize the generated results, as found in many domains of AI-generated content \cite{whyjonnycantprompt, sarkar2022like, designguidelinesforpromptengineering}.



% ----- END -----
% VizFlow supports dynamic layouts by linking text and charts, allowing users to create data-driven articles without needing programming skills \cite{Sultanum2021VizFlow}.


% Research has additionally found that users often prefer having the control to customize over system recommendations, but avoid customization features due to the complexity involved in achieving them \cite{McGrenere2007AdaptableSoftware, Park2007AdaptableVersusAdaptive}.
% while barriers such as high difficulty and lack of time may deter users from customizing if the perceived benefits are not worth the effort \cite{Mackay1991TriggersAndBarriers, Marathe2011CustomizationControlOrIdentidy}.

% Mackay also highlights barriers including high difficulty and lack of time, which deter users from making customizations if the perceived benefits are not worth the effort \cite{Mackay1991TriggersAndBarriers}.
% Additionally, research reveals trade-offs between user-controlled and system-recommended customizations, where users often prefer having control but may avoid customization features due to the complexity involved in achieving them \cite{Mackay1991TriggersAndBarriers, McGrenere2007AdaptableSoftware, Park2007AdaptableVersusAdaptive}.

% Mackay identifies key factors influencing software customization, such as users' recognition of repetitive patterns and frustration with repeated actions.


% and demonstrate interaction opportunities, it is especially important to explore this within the MD design pattern. However, there is currently a lack of comprehensive understanding regarding the range of customization options available for MD interfaces.


% Given this trade-off between customization needs and the friction to customize, researchers have explored approaches towards reducing the barriers for customizability to more interfaces. For example, Anchored Customization brings individual settings options from a separate page to conceptually related UI components, making customizations more in-situ for the interface \cite{Ponsard2016AnchoredCustomization}. Similarly, WritLarge allows the user to transform digital ink from a sketch to a grid and then to a table, each "semantic level" offering their unique respective affordances such as erasing strokes at the strokes level or turning handwriting into text \cite{Xia2017WritLarge}. VizFlow supports a range of dynamic layouts by using text-chart links, allowing users to author data-driven articles without programming \cite{Sultanum2021VizFlow}.



% While these findings serve as valuable insights for effective design for customizability, it is particularly important to explore this for the MD design pattern, something that is implemented across so many diverse tasks and where users must navigate through views in various directions while keeping an understanding of all the information presented. However, there lacks a comprehensive understanding of the various customization options that exist and are possible for MD interfaces.





% WritLarge allows the user to transform a selection of digital ink from a sketch of a table to a grid, then to a table, then back down to a grid, each ``semantic level'' affording unique functionalities, such as the sketch allowing for erasing the lines, and more structured representations like tables ....



% A mechanism we are interested in focusing on is transclusion.
% We want to focus on this because we want to support in-context

% To support web collection and management within the context of active web spaces, we utilize transclusion, a technique that involves embedding one part of an application into another \cite{Nelson1995Transclusion}. 
% We aim to support information collection and organization by aggregating web components with transclusion, a technique that involves embedding one part of an application into another \cite{Nelson1995Transclusion}.
% Methods for transcluding web components has seen real-world use and has shown interaction benefits in commercial applications and HCI research.
% For example, note-taking applications such as Notion \tocite{notion} and Confluence \tocite{Confluence} collaborate with other companies, including Figma \tocite{Figma}, to embed views from other companies' applications in their documents. In HCI research, prototypes such as inlineLink embedded iframes inside websites, allowing users to view many hypertext files in a single rendered document \cite{miura2004inlinelink}. 

% Additionally, Webstrates introduced a technique for turning web elements into shareable and modifiable media across numerous spaces through transclusion \cite{klokmose2015webstrates}. This technology has unlocked opportunities to develop and integrate transclusion in diverse domain such as programming, video creation, and videoconferencing \cite{radle2017codestrates, klokmose2019videostrates, gronbaek2021mirrorblender, gronbaek2023mirrorverse}.
% Although there has been a rich research ecosystem for transcluding web content across websites, all of these works either constrain the user to a set of web contents they can transclude and where or require technical expertise to develop custom transclusions. Our goal is thus to empower end-users to create their own transclusions by directly manipulating and moving web components across websites.



% Dynaviz? Designing for customizability --> natural language prompt, but presenting the widget that the user can use to better customize the chart directly?

% MD interfaces are widely implemented across diverse tasks, requiring users to navigate between views in various directions while maintaining an understanding of all the presented information. 


% Line of work that makes personal user interfaces automatically

% There’s work that can allow you to transform the representation of views (WritLarge, bret victor), 

% Transformable representations: WritLarge, Bret Victor, Damien Masson's work

% Customizing lists, such as reordering, 

% We explore how we can design an MD interface that enables transformations across our design space dimensions.


% While extensive research has been done understanding the various customization options available across many domains and patterns, there lacks a comprehensive understanding of the various customization options that exist and are possible for MD interfaces.

% While these studies provide valuable insights into the design of MD interfaces, they do not fully explore the potential for customization in this pattern. Our work addresses this gap by introducing new interaction techniques that enable users to directly manipulate and customize the details presented in the MD interface.



% Line of work on end-user programming and end-user customization — providing customization tools that aren’t built into the websites, allowing you to make your own filtering, sorting, or computational operations \cite{Huynh2006Sifter, Litt2020Wildcard}.



% RW1 DUMP

% \bryan{Use overview-detail, and also include the mit website hci patterns --> they are defining overview "plus" detail}

% The master-detail design pattern is a widely implemented interface pattern characterized by two distinct views: a master view that contains a collection of items and a detail view that contains details of a selected item. This pattern, also referred to as ``director-detail'' or ``master-slave'' \cite{Pastor2007ModelDrivenArchitecture}, share different interpretations of what constitutes a ``master'', such as allowing the master to be a single item instead of a collection \cite{Seffah2015PatternsOH}. Despite these variations, the core structure of the MD pattern---as illustrated in Figure \ref{fig:md-definition}---remains consistent across these definitions.

% A notable strength of the overview-detail pattern is that it aligns with the principle of progressive disclosure \cite{Norman1986ProgressiveDisclosure, Shneiderman1996OverviewFirst}. By initially presenting only the essential details and revealing more details as the user delves deeper, the overview-detail pattern helps manage complexity and reduces cognitive overload \cite{Norman1986ProgressiveDisclosure}. 

% As this pattern is closely aligned with how information is organized in software systems, this pattern is also demonstrated in the context of web development. For instance, developers often structure API routes to manage collections of items with an ``index'' route (e.g., \texttt{/admin/articles}) and support retrieving individual item details through nested routes (e.g., \texttt{/admin/articles/:id}) \cite{Rails}.

% A formal empirical analysis could reveal additional variations and interaction possibilities of the MD pattern that individual case studies may miss. To our knowledge, our work presents the first empirical analysis of MD interfaces, which we leverage to explore and develop novel interactions enabled by this design space.

% A notable strength of the Master-Detail (MD) pattern is in its alignment with the principle of progressive disclosure \cite{Norman1986ProgressiveDisclosure, Shneiderman1996OverviewFirst}. By initially presenting only the essential details and revealing more details as the user delves deeper, progressive disclosure helps manage complexity and reduces cognitive overload \cite{Norman1986ProgressiveDisclosure}. A similar principle closely aligned with the MD pattern is the overview+detail principle, which advocates for displaying both an overview and a detailed view simultaneously, allowing users to grasp the broader context while accessing specific pieces of information \cite{Card1999VisionToThink, Hornbaek2001OverviewDetailBenefits}.  These benefits of the MD pattern are also reflected in diverse applications. For instance, Baudisch \etal's \textit{focus-plus-context screen} allows users to open a detailed portion of a map while maintaining an overview of the entire area \cite{Baudisch2001FocusPlusContext}, and web developers often architect web page routes to fetch collections of items in an ``index'' route (e.g., \texttt{/admin/articles}) that then supports navigation to deeper routes to retrieve individual item details (e.g., \texttt{/admin/articles/:id}) \cite{Rails}.

% This alignment with many design principles is perhaps the reason for its widespread use, making the MD pattern particularly interesting to study. Academic research and online articles have highlighted a few key variations of MD interfaces. For instance, Molina \etal{} explores how other patterns, such as a population pattern, can compose with the MD pattern to generalize the organizational structures user interfaces \cite{Molina2002JustUI}. Additionally, case studies explore how MD interfaces can be nested to create hierarchical views in applications \cite{Molina2002JustUI, Seffah2015PatternsOH} and how different screen sizes may necessitate varying arrangements of the master and detail views  \cite{Seffah2015PatternsOH, Nguyen2012MDAndroid}.



% RW2 DUMP



% \bryan{Bring up related work systems that provide just a new OD. They are essentially ODs to support task X, Y, Z}

% \bryan{This paragraph says: Okay, well you need one more OD instantiation to help with a task. So these contribute a new instantiation. Such as new layout, new composition, new content to the OD interface.}
% and support understanding of AI generated text \cite{Graphologue}.


% While this approach provides end-users with more instantiations to interact with, these representations are ultimately instantiated by the designer, limiting any ability for users to customize.


% Aimed at providing overviews on papers sourced from related work sections in papers
% PaperWeaver and Relatedly providing overview summaries of related work sections in papers
% Graphologue provides AI generated response, but also generates interactive node-link diagram alongside the text in real-time.


% Those are overviews. Anything else for overview-detail?
% These are all sensemaking stuff. I wonder if there are ny other directions of literature for this?


% Systems have also provided a spatial canvas to 
% ForSense, InterWeave providing canvas as you collect and explore
% Threddy, Synergi, Fuse providing a hierarchical structure to manage threads and snippets of information collected.



% they are still ultimately limited by the types of instantiations made by the designer and developer.
% \bryan{final statement that we need malleability, but especially for overview-detail interfaces, to support information tasks.}
% Thus, a malleable interface is needed to complet

% Instead, we need a malleable interface that allows users to
% A malleable interface is one that ideally allows users to 
% introduces ways to transform between different representations through axes of representation...

% introduced techniques for viewing information on a zoomable user interface at different zoom levels by providing varying levels of detail, which displays information at varying levels of detail at multiple zoom levels.

% Bret Victor climbing up and down the ladder of abstraction
% WritLarge
% pad++ provide multiple levels of abstraction in a zooming interface

% Charagraph --> this is a single additional representation, so not actually relevant
% texsketch
% \haijun{talk about work along this direction, in the end, say that while these work provide multiple instantiations, end-user still manipulate them, so they are still stuck with what the developers choose}
% ^ This paragraph is not about overview detail, but transformabl rep in general? like multiple abstraction 

% ^ yes, are there relate works that explore transformable Overview, or mutliple-level overview? I mean map is one? naturally has semantic zooming?

% okay, that makes more sense.

% When you say customize how they transform --> it's customizing the representation? that's what peiling's suggestion does , there's semantic zoom which is another representation you get, but even still, you need to need  to customizations on it

% ok sounds good. I think i can finish this tomorrow 



% [cool, glad it's -as in how these two sections of RW should be restructured-clearer now! ]

% [yes, developer right now decides what to show on each zooming level, but with our approach, theoretically, we can customize what's shown on each zooming level] 

% but not customizable. yes.

% That's the point of this section. We say that there are transformable ones... but they are not customizable. what if people what to customize how they transform. like what peiling suggested, having end users to customize what's shown on each level of the semantic zooms

% and they our next section talks about customizable interfaces, so it will flow well?



% Significant research has been devoted to understanding the types of online information tasks users engage in \cite{tangledWeb, knowledgeworkerweb, tabbedbrowsing}, their usage patterns \cite{knowledgeworkerweb,tabdue}, and challenges users encounter\cite{browsingcluttered,tabdue, graphhistory}. These tasks are often involve various subtasks such as 
% The complexity and fluidity of this activity, coupled with today's software interfaces that fragment information spaces across many applications and tabs, is perhaps the reasons for interaction costs such as information overload, browsing clutter, and excessive context switching \cite{Chang2021TabComesDue, Han2022Passages, Miller1960InfoOverload}.

% Many lines of research have aimed to address subsets of frictions encountered in information tasks within specific domains. One approach explored ways to streamline the users collection processes as they dive into the details of information. Systems employed browser-level comparison tables to facilitate decision-making across online items \cite{Chang2020Mesh}, spatial canvases to help synthesize and make sense of information \cite{Ramos2022ForSense, Suh2023Sensecape}, and hierarchical organizations to efficiently structure and manage snippets of text and web content \cite{Kuznetsov2022Fuse, threaddy}. A second approach has focused on providing users an overview first in order to guide users' exploration. For example, Relatedly \cite{Relatedly} and PaperWeaver \cite{PaperWeaver} create overviews of relevant papers by leveraging semantic connections from the content of the active paper. Selenite scaffolds users’ decision-making processes by generating initial criteria about an item to purchase \cite{Selenite}. Lastly, mixed-initiative approaches leveraged the benefits of systems that facilitate both information exploration and synthesis. For instance, Synergi facilitates the both collection and synthesis of information by automatically fetching relevant threads from academic papers and placing them into hierarchical categories \cite{Synergi}. Sensecape guides users' exploration and collection processes with a hierarchical organization of canvases \cite{Sensecape}. Meanwhile, Qlarify enables users to gradually uncover more details about key concepts within a paper abstract by intelligently fetching information from the full paper \cite{Fok2024QlarifyARXIV}.

% While these solutions offer valuable insights into addressing the various challenges across their respective domains, an interface cannot only provide one solution at a time to support the dynamic nature of information tasks. Instead, a malleable interface would allow the user to choose which representation of an overview suits their understanding best and decide how they uncover and synthesize information from related or detailed sources. 
% Our work presents an opportunity to unify existing tools that facilitate information tasks with a malleable overview-detail design pattern.

% \bryan{Question: Don't malleable interface literature and our intro already motivate the need for malleable interfaces for information tasks? Or did I completely misunderstand something about this section?}



% On the other hand, malleable interfaces have




% \subsection{MD Interfaces in Information Spaces for Sensemaking}

% % This is particularly important in information-rich environments, where the MD pattern's widespread use presents unique challenges in supporting users' sensemaking activities.

% % Master-detail interfaces are ubiquitous in digital information spaces, making these interfaces a common interface users encounter during sensemaking activities.

% MD interfaces are ubiquitously integrated into everyday interfaces we use for a plethora of sensemaking tasks, some of which include collecting papers, shopping, travel planning, or even simply learning new concepts. However, due to the sheer scale of information the internet packs into MD interfaces, users must navigate through large hierarchies of master-detail web pages during these tasks. Furthermore, as the task increases in complexity, the explored information grows increasingly challenging to manage and analyze in the interface, often leading to cases of browsing clutter and fragmented information spaces \cite{Chang2021TabComesDue, Han2022Passages}. 

% Several lines of research in2 specific domains have tackled the challenges pertaining to information management and online sensemaking for their respective activities. For instance, designers have shared design recommendations on the optimal arrangement of information in overview pages (master) and item pages (detail) of e-commerce websites to reduce the excess reading costs for end-users \cite{van2007design}. Research has explored providing users with personal spaces to aggregate snippets of information (master) from full web pages (detail) \cite{Kuznetsov2022Fuse}. Other work have integrated various representations, such as a table \cite{Chang2020Mesh}, a canvas \cite{Ramos2022ForSense}, and a hierarchy \cite{Suh2023Sensecape}, as an overview (master) to aid users in comparing items, synthesizing notes, and understanding complex concepts (detail) \cite{Chang2020Mesh, Suh2023Sensecape, Ramos2022ForSense}.

% While these solutions for supporting individual tasks are valuable for directly addressing domain-specific challenges, they often lack the flexibility required for the diverse working patterns. Consequently, users may face challenges in switching between the many working spaces across various different contexts. This highlights the need for a solution that addresses these common challenges through a unified approach. We propose that making the MD interfaces more customizable provides an effective way to achieve this flexibility.




==> versions/initial_submission/3_content_analysis.tex <==
\section{Content Analysis}
\label{section:content_analysis}

To better understand the various implementations of the overview-detail design pattern, we conducted a content analysis of overview-detail interfaces in desktop websites. Our content analysis was driven by the following questions:

\begin{enumerate}[label=\textbf{[Q\arabic*]}, leftmargin=*]
    \item What kinds of overview-detail interface arrangements exist in the wild?
    \item What types of information are presented in the overview and detail view, respectively?
    \item What aspects of overview-detail interfaces are already customizable by end-users?
\end{enumerate}

We present our findings with a design space of three dimensions of variations in overview-detail interfaces (\textbf{Q1}, \textbf{Q2}) and report existing customizability options found in our collection of websites (\textbf{Q3}).


\subsection{Methods}

\subsubsection{Data Collection}

The goal of our data collection was to collect a diverse and representative set of overview-detail interfaces that people regularly use. We initially collected the top 50 highest traffic websites in the United States based on data reported by Similarweb\footnote{\href{http://similarweb.com/}{http://similarweb.com/}. Accessed June 2024.}, a web analytics platform. However, as we analyzed this collection, we realized there were many common websites that were not included, such as flight booking or restaurant websites. To diversify our collection, we expanded to three more sources: 1) top 5 highest traffic websites in each of 33 web service categories\footnote{List of 33 categories listed by Semrush in Appendix \ref{appendix:semrush-categories}} listed by Semrush\footnote{\href{https://www.semrush.com/website/top/united-states/all/}{https://www.semrush.com/website/top/united-states/all/}. Data last updated May 2024. Accessed July 2024.}, another web analytics platform, 2) 20 randomly sampled websites from Wordpress’ showcase page to observe non-corporate websites such as blogs\footnote{ \href{https://wordpress.org/showcase/archives/}{https://wordpress.org/showcase/archives/}. Accessed July 2024.}, and 3) 20 randomly sampled websites from Awwwards’ gallery of ``2024 Sites of the Year'' to observe favorite designs from the UI/UX design community\footnote{ \href{https://www.awwwards.com/websites/sites_of_the_year/}{https://www.awwwards.com/websites/sites\_of\_the\_year/}. Accessed July 2024.}. After filtering our list (e.g., removing duplicates), our final sample consisted of 156 websites.
The first author examined all 156 websites, identifying 303 instances of overview-detail interfaces. Some websites featured multiple overviews linked to one detail view, or vice versa. For coding purposes, we defined each instance as a single overview-to-detail relationship. Thus, interfaces with multiple connections were recorded as separate instances.

\subsubsection{Coding Procedure}

We developed a codebook of overview-detail interfaces through an iterative open coding process involving collaboration among the first three authors. In the first round of open coding, we randomly selected 20 overview-detail instances from our dataset of 303, and the first three authors individually analyzed all 20 instances. The coders discussed and clustered their categories together to develop an initial codebook. In the next round, the first two authors independently coded a second sample of 20 instances, achieving an inter-rater reliability of 94.8\% agreement between the codes, measured by Cohen’s kappa. They discussed the remaining differences and revised the dimensions to reach a consensus. Given the high agreement rate, the authors determined that it was sufficient for the second author to complete the remaining coding, continuing to code in random samples of 20. After each round, the first two authors reviewed and discussed new potential dimensions and variations, revising the codebook as necessary. This process was repeated four times, stopping when no new dimensions or variations were found in the last three stages. In total, the authors analyzed 120 overview-detail instances.


\subsection{Design Space}

Our design space presents variations of overview-detail interfaces found from the content analysis, particularly in the arrangement of overviews and detail views and the types of information presented in them. Our design space covers the following three dimensions. We describe notable cases found from the three dimensions and present the full design space in Figure \ref{fig:design-space}.
\begin{itemize}
    \item \textit{\textbf{Content}} describes whether information is presented in the overview, the detail view, or both, and how the attributes in the overview are abstracted from those in the detail view.
    \item \textit{\textbf{Composition}} describes how the multiple overviews and detail views are connected together
    \item \textit{\textbf{Layout}} describes the spatial arrangement of overview and detail views within the interface.
\end{itemize}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/3_content_analysis/design-space.png}
    \caption{Design space of overview-detail interfaces on the Web: Content, Composition, and Layout.}
    \label{fig:design-space}
    \Description{This image provides a detailed breakdown of the design space of overview-detail interfaces used on the web, broken into three categories: Content, Composition, and Layout. Here's the description of each section: First, we begin with the Content dimension. The following subsections describe where a particular attribute is shown: In Detail view only: Represents scenarios where certain attributes are only visible in the detailed view. In Overview only: Attributes visible solely in the overview. In both views: Attributes visible in both overview and detail views. There are also several Overview Abstractions: Visual: Attributes like Style and Graphic can either be available or unavailable. Semantic: Attributes related to meanings like Summary or Category can be abstracted, such as a rating summary or topic labels. Computational: Attributes like Ranking/Order, Sum/Average, or Minimum/Maximum are shown through numerical abstractions. Next, we move onto the composition dimension. These Composed relationships include the following; One-to-one: One overview leads to one detail view. Many-to-one: Multiple overview points lead to one detail view. One-to-many: A single overview leads to multiple detail views. Composition also covers the following recursion: Overview inside Detail view: A recursive structure where an overview is composed with the detailed view. Detail views in between: Multiple detail views between overviews, often in a preview or hierarchical informational structure. Finally, we also have our Layout dimension. The Overview-Detail Layouts can New page: Clicking the overview opens the detailed view in a new page. Side-by-side: Overview and detail views appear next to each other. In-place: A dropdown or a replacement of content occurs in the same space. Under Overview: Detail appears under the overview via table of contents or side menu. Above Overview: Detail appears via pop-up, pop-over, tooltip, or picture-in-picture. The Overview itself can be displayed as a List, Grid, Table, Spatial map, Hierarchy, or Timeline. Lastly, the Detail Layout is highly variable, but can either show one view at a time or many at a time.}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{figures/3_content_analysis/content-dimension.png}
    \caption{Example variations in the content dimension. (A) Indeed displays the attributes job title, company, location, and salary in both the overview and detail view. (B) Zillow's overview map presents different detail attributes (price or number of units) depending on whether a housing location has multiple units. (C) eBay provides the ``Add to Watchlist'' in both the overview and detail view. (D) Other sites, such as Etsy, only provides this button in the detail view. Long blocks of text tend to be cut off in overviews via (E) eclipses as shown in Gmail or via (F) a fade out gradient as shown in Quora.}
    \label{fig:content-dimension}

    \Description{This image contains six panels labeled A through F, each demonstrating variations in how content is handled in overview-detail interfaces across different websites or apps: A) An image of Indeed's job listings interface. Both the overview and detail\textbf{ }view display attributes of job title, company, location, and salary. B) A Zillow map showing properties. Depending on the number of units available, the overview displays different attributes like the price or number of units available. C) EBay's "Add to Watchlist" button is available in both the overview and detail views of product listings. D) Unlike eBay, Etsy shows the "Add to Favorites" option only in the detail view, not in the overview of product listings. E) Long blocks of text in Gmail's overview are truncated with ellipses (three dots), so the user has to open the detail view to see the full message. F) Here, long text is truncated in Quora's overview using a fade-out gradient instead of ellipses, prompting users to click to read more. Each panel shows different strategies for handling content visibility across overview and detail interfaces, highlighting where users see certain attributes.}
\end{figure}

\subsubsection{Content}
Throughout our content analysis, we realized that some attributes were displayed only in the overview, some were displayed only in the detail view, and some were displayed in both views. For example, the search results interface for job openings on Indeed showed job titles, company names, and salary ranges in both views, while the overview omitted attributes like qualifications or benefits (Fig. \ref{fig:content-dimension}A).
Although we initially coded attributes as static information elements, we also observed this pattern in interactive elements, such as `Save' buttons, text fields, and menus, with some sites including them in both the overview and detail views (Fig. \ref{fig:content-dimension}C), while others displayed them only in the detail view (Fig. \ref{fig:content-dimension}D).
Moving forward, we considered interactive elements to be attributes as well.
We also found instances in rental and housing platforms where the overview primarily presented prices for each place as pins on a map, but in Zillow, if a place had more than one unit available, the pin displayed the number of units available instead (Fig. \ref{fig:content-dimension}B).
In text-heavy overview-detail interfaces such as messaging apps and online discussion forums, we noticed long blocks of text in the overview were either cut short via ellipses (Fig. \ref{fig:content-dimension}E) or a fade-out gradient (Fig. \ref{fig:content-dimension}F).

We further found that some attributes in the overview served as an abstraction of information in the detail view. We identified three forms.
First, we found visual abstractions, which were encoded into the style and visuals of the item. For instance, Ticketmaster used color shading to indicate the number of seats available per section, with sections that had more seats shown in a saturated blue, while sections with fewer seats appeared in lighter shades.
Second, we found semantic abstractions that represented the contents in the detail view with summaries or categories. For instance, ChatGPT's conversation interface generated a title that represented each conversation.
Lastly, we found computational abstractions that computed attributes from the detail view into a value. For instance, Southwest's website presents a calendar view of the cheapest flight prices for each day.


\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{figures/3_content_analysis/composition-dimension.png}
    \caption{Example variations of the composition dimension. (A) Zillow shows a view composed of two overviews---a grid (left) and a map (right). The Southwest booking interface allows users access flight information from both (B) the 5-day table view and (C) the 30-day calendar view. (D) New York Times nests an overview inside a detail view with suggested articles. (F) Discord shows an intermediate detail view of the user profile as a tooltip, which can be expanded to show the full detail view as a pop-up.}
    \label{fig:composition-dimension}
\Description{The figure shows various examples of user interface compositions from different websites and applications. It's labeled A through E, each representing a different interface example: A) Zillow: This section shows a real estate listing interface with two parts - a grid view on the left showing property details and images, and a map view on the right displaying the locations. B) Southwest Airlines: This shows a flight booking interface with a 5-day table view of flight options, prices, and times. C) Also Southwest Airlines: This displays a 30-day calendar view of flight prices, allowing users to see price trends over a month. D) New York Times: This section shows an article view with suggested related articles nested within it. E) Discord: This displays a user profile interface, showing how a tooltip with intermediate details can be expanded into a full detail view. The image is meant to illustrate different ways that interfaces can be composed to show varying levels of detail and different views of information.}
    
\end{figure}

\subsubsection{Composition}
During our analysis, we identified several overview-detail interfaces where multiple instances were composed together.

First, we found overview-detail relationships beyond just one-to-one. Many-to-one relationships presented multiple overviews in forms such as a list overview and a map overview presented side-by-side (Fig. \ref{fig:composition-dimension}A) or different scopes such as a five-day list (Fig. \ref{fig:composition-dimension}B) and a 30-day calendar (Fig. \ref{fig:composition-dimension}C). We also found that some instances synchronized navigation across the many overviews, where selecting an item in one would trigger the navigation of another to the corresponding item.

Second, we found instances of recursion---overview-detail interfaces nested within each other. 
For instance, additional overviews such as a list of articles appeared in the detail view of New York Times (Fig. \ref{fig:composition-dimension}D). 
% We also found overview-detail interfaces that presented another overview inside the detail view, such as a hierarchical information organization on Fandom.com (Fig. X). 
This finding aligns with prior research that recognized the variation of nested overview-detail views in hierarchical menu interfaces \cite{Seffah2015PatternsOH, Cockburn2009OverviewDetailReview}.
An additional variation found were cases of ``intermediate'' detail views, which a link or button inside a detail view opened a detail view containing more or all attributes of the item. One of these variations was found in Discord's list of users in a server, where clicking on a user opened a small tooltip profile card, and clicking on the profile picture inside it opened a full-screen popup, revealing further details about mutual friends and servers (Fig. \ref{fig:composition-dimension}E).


\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{figures/3_content_analysis/layout-dimension.png}
    \caption{Example variations in the layout dimension. (A) MLB’s player profile page maps batting points onto the baseball field; clicking a plot point opens a detail view of a video replay of the point. (B) Ticketmaster’s seating selection page also shows a map overview; when a particular seating section is selected, the overview list changes to match the corresponding section. (C) ESPN shows each player's stats in a game, which can be opened as a dropdown. (D) Weather.com uses a similar dropdown layout, but unlike ESPN, multiple detail views can be opened simultaneously.}
    \label{fig:layout-dimension}

\Description{This image illustrates different variations in layout design for various sports and weather-related websites. The image is divided into four sections, labeled A through D: A) MLB (Major League Baseball) Player Profile: This section shows a baseball field diagram with colored dots representing batting points. There's an arrow pointing to a larger image, which appears to be a video replay of a specific play. The concept here is that users can click on a dot to see a detailed view of that particular play. B) Ticketmaster Seating Selection: This displays a stadium seating chart on the right side. On the left, there's a list of available seats with prices. The idea is that when a user selects a section on the map, the list updates to show seats in that section. C) ESPN Player Statistics: This section shows a baseball field diagram in the center, surrounded by player statistics in a table format. There's a highlighted area suggesting that certain statistics can be expanded into a dropdown for more detailed information. D) Weather.com Forecast: This displays a daily weather forecast with multiple time slots. Each time slot shows temperature and weather conditions. The layout is similar to the ESPN dropdown, but the caption notes that multiple detailed views can be open simultaneously.}
    
\end{figure}

\subsubsection{Layout}
Our analysis revealed variations in the arrangement of overviews and detail views, the organization of items within overviews, and the number of items displayed in detail views.

\textbf{Overview-Detail}: First, we observed variations in overview-detail layout, with some websites arranging overviews and detail views side by side, while others opened detail views in a pop up or a dropdown.

\textbf{Overview}: We also observed variations of overview layout in the forms of lists, grids, and tables. Notable variations also included visualizations that plotted points that could be opened into detail (Fig. \ref{fig:layout-dimension}A) and sports stadiums to select seating sections (Fig. \ref{fig:layout-dimension}B).

\textbf{Detail}: We observed that detail views varied by how many were displayed at a time. Some instances only opened one detail view at a time, while others allowed users to open many at a time. For instance, ESPN allowed only one dropdown to be open at a time (Fig. \ref{fig:layout-dimension}C), while weather.com supported multiple (Fig. \ref{fig:layout-dimension}D).


\subsection{Existing Customizability Features}

In addition to the previously mentioned dimensions, we separately collected and coded existing customizability features for overview-detail interfaces. We found 8.33\% (13/156) websites provided customizations for overview-detail interfaces, with 2.56\% (4/156) providing content customization, 0\% (0/156) providing composition customization, and 7.69\% (12/156) providing layout customization. All of the instances we collected were limited in customization, with the most providing eight layout variations.

We found Craigslist offered the most variations for customizing the overview-detail interface, with five options for customizing the overview layout and three for the overview-detail layout. The choice of layout also indirectly influenced which attributes were displayed. For example, the grid view included an image thumbnail, while the list view did not, likely to maintain a more compact item presentation. In the Content dimension, we observed four websites that allowed users to customize which content attributes they wanted to view. Among these, eBay offered the most customization options, though it only allowed users to toggle six attributes.


\subsection{Summary}
In summary, our content analysis of 303 overview-detail instances in 156 websites identified three dimensions of variation: content, composition, and layout. Additionally, we found that only 8.33\% (13/156) websites in our collection supported customization features, with those offering only limited options. Our collection of samples may not be fully representative of the entire set of information systems, and we may not have captured every instance of overview-detail interfaces within each sample. Thus, we do not claim the comprehensiveness of our design space and the frequencies of customizability features beyond our collection. Nevertheless, our analysis does provide insights into variations in real-world examples, offering contributions in understanding overview-detail interfaces.



















% --- DUMP ---
% In addition to the previously mentioned dimensions, we separately collected and coded existing customizability features for overview-detail interfaces, observing the kinds of customizability options websites provided and how these options aligned with the three dimensions identified.

% In the Content dimension, we observed four websites that allowed users to customize which content attributes they wished to see. Among them, Ebay has the most content customization options, allowing users to choose between six overview detail attributes that can be checked to view or checked off to hide. Other sites have more limited options to either hide certain attributes, reorder attributes, or choose between attribute types (still image or video) in the overview. 

% Regarding the Layout dimension, we observed twelve websites with such customizations options. 

% Each of these twelve sites included some level of overview layout customization, a majority of which were shopping and booking interfaces that offer options to transform the overview between list, grid, and/or table view. Interestingly, two social media sites offered additional overview layout customizations – one allowed users to choose how compact their list was, another offered a selection between a staggered grid and an organized grid.  

% There were only three websites that provided some level of overview-detail layout customization – two were variations of the “separate page” category but allowed users to choose between opening detail views in the same tab or a new tab. Among them, we found Craigslist to have the most layout customizations with a total of five different options for customizing the overview layout and three different options for customizing overview-detail layouts (Fig. X). Customizing the layout of their interface also affected which attributes were shown. For instance, a grid view provided an image thumbnail, while the list view did not---perhaps to maintain a compact view of the items 



% * We looked, we found X\% of our websites OD from had OD customizations (content: X\%; composition: X\%; layout: X\%)
% * Craigslist... 
% * End with talking about content is preselected attributes -> ebay. 



% Finally, we did not observe any composition customizability options within our sample set of 303 – though we acknowledge that there are likely some sites that utilize this. 



% Among the many websites, we found Craigslist to have the most options for customizing the layout of overviews and detail views with seven different options (Fig. X). Customizing the layout of their interface also affects which attributes were shown. For instance, a grid view provided an image thumbnail, while the list view did not---perhaps to maintain a compact view of the items.
% From our collection of 303 overview-detail interfaces, the only site to directly provide options to customize which detail to show in the overview was eBay (Fig. X). X\%
% However, options were limited to only a few details and provided options in a separate settings panel.




% <this booking site> provided filtering features on results, which upon applying a filter, would reveal the value  of that attribute for each item (Fig. X) (filtering for reviews would show the review count and review rating details)
% found a setting for presenting the results in a list or a gird. We  a small list of attributes to show in the search results page for each item. They show a set of attributes, but there were still many attributes in the details that the website did not allow the user to show in the overview.
% \bryan{Move this section before the design space summary section, but how to talk about customizations frequency by dimension if you haven't even introduced what the dimensions are? (Minor thing, but also this is Q3, not Q1-2, so you want to switch that order as well. You can first try moving it forward and try to talk about customization features without dimensions specifically?}

% \subsection{Limitations}
% It may be possible that we did not collect all overview-detail instances that exist on each single website---human error.
% Our collection of websites are also not representative of all websites in the internet.


==> versions/initial_submission/4_interaction_techniques.tex <==
\section{Interaction Techniques for Malleable Overview-Detail Interfaces}
\label{section:interaction_techniques}

In this section, we describe interaction techniques to customize overview-detail interfaces along the three dimensions identified from our content analysis.

% The goal of this section is not to provide ways to turn any overview-detail interface into any other, but rather to explore the interaction techniques that provides the end-user ways to transform the overview-detail interface to best suit their needs. 
% \bryan{Don't say this as a limitation, and we don't do things. Rather, just simply justify why you ended up doing these specific dimensions}


\subsection{Content}
\label{interaction-dimension:content}
To customize overview-detail interfaces along the content dimension, we introduce \textit{\technique}, a novel interaction technique that allows end-users to directly interact with detail attributes in the overview-detail interface. This enables users to control what, where, and how detail attributes are shown as well as directly sort and filter by attributes. \Technique also unlocks further customizations of the overview-detail interface when paired with generative AI tools by allowing users to query for attributes, generate new ones, and reformat inconsistent attributes. To support such interactions, overview-detail interfaces can provide a dedicated ``Attributes Mode'' available to toggle on and off in a global toolbar on the website. Upon toggling on, the website highlights all attributes in the overview-detail interface. Users can then select and perform actions on the attributes.

% Of the many ways \technique can be implemented, such as area selection, a context menu option, or a website-wide toggle, we implemented a website-wide toggle called ``Attributes Mode'', which upon toggling, highlighted all attributes in the interface. This made \technique interactions more visually salient to the reader. \bryan{This design choice is not for the readers; it's for the end-user. Introduce this design choice properly, and justify it in terms of end-user benefits instead.}
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/4_interaction_techniques/surface-and-hide.png}
    \caption{Upon entering ``Attributes Mode'', (A) users can select attributes in the detail view to surface to the overview, and (B) hide selected attributes from the overview.}
    \label{fig:surface-and-hide}
    \Description{The figure shows five screenshots demonstrating how users might use the "Surfacing and Hiding Attributes" feature while shopping online for sofas. The first two images show a user selecting two attributes - the Year Manufactured and the Item Length - which the user surfaces. The third image shows the newly customized shopping overview - now with the selected attributes appearing alongside default attributes such as product name and price. The fourth image shows the user selecting the vendor's name and and hiding that attribute from the overview. The fifth image shows the final customized shopping overview - with two additional attributes surfaced and the vendor name hidden}
\end{figure}
\subsubsection{Surfacing and Hiding Attributes (Fig. \ref{fig:surface-and-hide})}
\label{feature:surface-hide-attributes}
In order to find details of items not shown in the overview, users must open the detail view to each individual item and locate the attribute in the interface. \Technique lets users select attributes from the detail view and directly surface them by clicking ``Surface'' (Fig. \ref{fig:surface-and-hide}A). The selected attributes then populate in every item of the overview. On the other hand, if users want to hide attributes they are not interested in seeing in the overview, they can instead ``Hide'' (Fig. \ref{fig:surface-and-hide}B) those attributes. In essence, this interaction gives users the control to \textit{get an overview of only the things they want} by manipulating attributes on their own, without the help from the developers. 
% Additionally, users can hover over an attribute to ephemerally reveal an attribute over each item.

\Technique are not only limited to static attributes but also include dynamic and interactive ones, such as widgets, buttons, and components. For instance, users can surface an image gallery component into the overview to view more images and even the \textit{Add to Wishlist} button for each item on a shopping interface.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/4_interaction_techniques/sort-and-filter.png}
    \caption{Since users can surface any attribute to the overview (1), this also gives them the ability to sort and filter by their values directly (2).
    This figure shows how a user might sort overview items via the selected attribute \textit{Year Manufactured}.}
    \label{fig:sort-and-filter}

    \Description{This figure shows how users can perform additional functions, such as sort and filter, upon any selected attribute. Since users can surface any attribute to the overview (1), this also gives them the ability to sort and filter by their values directly. Continuing with the online sofa shopping scenario, the user in the figure first surfaces the \textit{Year Manufactured} attribute, and then sorts the overview items via the selected attribute}
\end{figure}
\subsubsection{Sorting and Filtering with Attributes (Fig. \ref{fig:sort-and-filter})}
\label{feature:sort-filter-attributes}
Rather than only using a predetermined set of sort and filter functionalities given by the interface, \technique provide the added opportunity to make any attribute sortable and filterable. For example, users can surface the \textit{Year Manufactured} attribute of a couch (Fig. \ref{fig:sort-and-filter}.1), then directly sort them by the latest manufactured year (Fig. \ref{fig:sort-and-filter}.2). Again, since \technique also includes dynamic attributes, users can, for instance, sort by the boolean value associated with the \textit{Add to Wishlist} button to ``pin'' items to the top of the search results.

\subsubsection{AI-assisted \TechNique}
\label{feature:ai-assisted-attributes}
\Technique, when assisted by AI's ability to process natural language queries to functionalities, demonstrates further interaction possibilities to customize the content in the overview-detail interface.
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/4_interaction_techniques/AI-queries.png}
    \caption{Users can additionally prompt AI to manipulate the attributes in the overview-detail interface. (A) Users can prompt AI to surface multiple attributes relating to the popularity of each product, (B) sort and filter for the values of a surfaced attribute, (C) and even surface specific values of attributes that contain multiple values.}
    \label{fig:AI-queries}

        \Description{This figure shows three instances of how the AI feature might be used to manipulate the attributes in the overview-detail interface while shopping online for sofas. The first image shows a use case in which a user prompts "how popular are these right now" -- which surfaces prompt AI to surface attributes relating to the popularity of each product. The second image depicts a use case in which a user wants to find the sofas that are linen textured -- prompting "give me the ones that are linen textured" to surface the upholstery fabric attribute, in which the user directly filters out non-linen options. In the third image, the user prompts "show me what the back looks like", which surfaces the Image Gallery attribute. From there, the user can select images that resemble the back of the sofa.}

\end{figure}

\paragraph{\TechNique via Natural Language Queries (Fig. \ref{fig:AI-queries})}
\label{feature:ai-query-attributes}
% \Technique features can be made by AI as well.
In addition to being able to directly manipulate attributes to surface them in the overview, users can also query desired attributes with their own words instead of using names assigned by the developers and content providers.
% While user-directed \technique provides a mechanism to directly shuffle content in the overview-detail interface, there are still needs that are easiest to communicate to the interface with words. 
% We find that overview-detail interfaces can utilize AI to also map user prompts to operations (i.e., surface, hide, sort, filter).
For instance, if a user asks AI in a prompt box ``\textit{How popular are these items?}'', AI can identify the relevant attributes (i.e., \textit{Number of Watchers}, \textit{Items Sold}) and surface them to the overview (Fig. \ref{fig:AI-queries}A). This extends to the other operations in \technique, such as adding a filter operation upon asking for ``only couches with a linen texture'' (Fig. \ref{fig:AI-queries}B). Additionally, users can ask to see ``the back of the couches'', which triggers AI to surface the \textit{Image Gallery} attribute and select images that present the back view of the couch (Fig. \ref{fig:AI-queries}C). If AI fails to show this image, the user can manually look through the images with the surfaced \textit{Image Gallery} component.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/4_interaction_techniques/AI-generated-attributes.png}
    \caption{(1) Users can also generate new attributes with AI, for instance by asking for the total cost of the item, which sums the values of the \textit{Price} and \textit{Shipping Fee} attributes. (2) They can hover over the value to view its source attributes, and (3) also drag them into the overview, (4) surfacing the source attribute alongside the newly generated one.}
    \label{fig:AI-generated-attributes}

        \Description{This figure shows how users can generate new attributes with AI, for instance by asking for the total cost of the item, which sums the values of the \textit{Price} and \textit{Shipping Fee} attributes as shown in the first image. In the second image, the user hovers over an item's Total Cost attribute to view its source attributes, and can also drag them into the overview. The final image shows the completed customization, with the newly generated attribute, total cost, alongside the source attribute, shipping fee.}

\end{figure}

\paragraph{Generating New Attributes (Fig. \ref{fig:AI-generated-attributes})}
\label{feature:ai-new-attributes}
AI is also suited to generate new attributes from user queries. Users can ask for an attribute that may require computing values for each item in the overview, For instance, if a user asks for the ``total cost'' of an item, AI can sum values of attributes such as \textit{Price} and \textit{Shipping Fee} (Fig. \ref{fig:AI-generated-attributes}.1). Users can hover over the newly generated attribute to reveal the source attributes the AI referenced (Fig. \ref{fig:AI-generated-attributes}.2), and then surface these sources as well (Fig. \ref{fig:AI-generated-attributes}.3-4). If AI cannot provide the value for an item, it responds ``Not Specified''.

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{figures/4_interaction_techniques/AI-reformatted-attributes.png}
    \caption{Many attributes of items in online marketplaces are often inconsistent in the format of the value and the attribute's name. (A) To address this, users can prompt AI to reformat the titles of items to make more consistent. (B) Additionally, surfacing attributes from items that do not contain them will trigger AI to search and fill in the missing values to that attribute. If not found, AI provides the value ``Not Specified''.}
    \label{fig:AI-reformatted-attributes}

        \Description{Many attributes of items in Ebay's online marketplaces are manually entered by vendors and are often inconsistent in their formatting. This figure shows how users can prompt AI to reformat the titles of items to make more consistent -- in this case the user prompts the AI tool to "just put the brand name and its condition" -- effectively replacing the product title with the brand name attribute and condition attribute.}

\end{figure}


% \paragraph{Reformatting and Filling Empty Attribute Values (Fig. \ref{fig:AI-reformatted-attributes})}
% \paragraph{Forming Consistent Attribute Values (Fig. \ref{fig:AI-reformatted-attributes})}
\paragraph{Establishing Consistent Attribute Values (Fig. \ref{fig:AI-reformatted-attributes})}
\label{feature:ai-reformat-attributes}
Many attributes of items in online marketplaces are not only set by developers but also by vendors. This results in a large case of inconsistent attributes and values, such as using different attribute labels, currencies, units, or title formats.
If users surface an attribute that is not found in a particular item, AI can scan through the item's data to identify the attribute from other sources (Fig. \ref{fig:AI-reformatted-attributes}B).
Users can also choose to reformat attributes upon prompting the interface to make inconsistent attribute values consistent across all items. For instance, users can either ask to simply ``make the titles consistent'' or make more precise changes and ask to ``show only the brand name and the couch's condition'', thereby making the title easier to read (Fig. \ref{fig:AI-reformatted-attributes}A).
% With AI-assisted \technique, end-users can reformat attributes upon prompting the interface, making attributes consistent across all items.


\subsection{Composition and Layout}
\label{interaction-dimension:composition-layout}

To support transforming variations in layout and composition, we offer default options that are most familiar to end-users from our design space through dropdown menus to select layouts and tabbed views to visualize the collection of multiple overviews. By implementing these familiar interaction techniques, we aim to keep the interface customizations end-user friendly.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/4_interaction_techniques/overview-representations.png}
    \caption{\Technique provides a technique to invoke diverse overview representations. (A) For instance, users can select the \textit{Price} and \textit{Vendor Feedback Score} attributes to plot items in a scatter plot, or (B) generate a color value from the image to map items onto a color space.}
    \label{fig:overview-representations}

        \Description{This figure demonstrates how the overviews can be transformed into multiple representations with attributes. In the first image, a user selects "scatter plot" - and is able to view each overview item in a scatter plot plotted along two selected attributes as axis. The second image shows the overview items mapped onto a color space, based on a color value generated from the image.}

\end{figure}


\subsubsection{Transforming Overview Representations with Attributes (Fig. \ref{fig:overview-representations})}
\label{feature:overview-representations}
In addition to the default interactions provided to customize composition and layout, \technique provides a direct solution in the interface to transform the overview into various representations by providing relevant overviews based on attributes users select. Just as a map interface positions items using their latitude and longitude values, other detail attributes can entail different representations best suited for their contexts. For instance, users can select the \textit{Price} and \textit{Vendor Feedback Score} attributes to view items in a scatter plot to consider the reliability of the vendors while comparing prices (Fig. \ref{fig:overview-representations}A).
Users also can generate a color attribute from the item image to map items onto a color space, allowing users to cluster and explore items by color (Fig. \ref{fig:overview-representations}B).






% \bryan{Get rid of this section. Just motivate composition and layout, how they can be transformed, and further customized with \technique}
% We explored various techniques to support users in customizing the composition and layout of overviews and detail views. We explored how dragging the overview and detail views to different areas in the interface could determine whether the interface shows a side-by-side view, a popup, a tooltip, and more. We also explored how resizing the overview and detail view components into different shapes and sizes could transform lists into tables, tables into grids, and more. However, we deemed the most intuitive way to switch between various forms of layout was to simply use dropdown menus. Similarly for composition, we found it was most familiar for us to manage multiple overviews with a list of tabs. Thus, rather than focusing on the customization techniques for these dimensions, we highlight how different configurations of layout and composition can support various information tasks.


% transform overview based on attributes
% --> this also brings back attributes


% \haijun{using AI to reformat detail -- title}

% \bryan{• Prompt to find properties, fill in properties that aren't formatted consistently}
% \bryan{X Prompt to pull multiple properties, sort properties}
% \bryan{X Control images. "Give me the side-profile of the monitors"}
% \bryan{X Generate new properties. Flight booking. List of flights for a single day. Ask AI for cheapest flight price and its departure time. Pull this cheapest flight price and departure time to the calendar of days.}
% \bryan{• Transform the title attribute "Format this title"}


% \bryan{• Pull, hide, sort/filter details in a standard OD interface, also pull image gallery}
% \bryan{• Pull details through semantic zoom}
% \bryan{• Shopping interface turned into a Kanban board. Pull buttons to the overview. You can even sort by the button itself, whether the item was added or not}
% \bryan{X VSCode IDE: Pull more details to the minimap scrollbar... I want to connect OD to scrollbar to read wear & edit wear... somehow}

% first ask for an attribute that requires complex computation or transformation of existing attributes. For instance, if a user asks for the ``cheapest price for afternoon flights'' from a list of flight tickets for each day of the week, AI can identify all prices with departure times in the afternoon and return the minimum value with a new attribute called \textit{Cheapest Price} (Fig. \ref{fig:AI-generated-attributes}a). Users can then surface this newly generated attribute to the overview, propagating the action of finding the cheapest afternoon flight price across the remaining available days (Fig. \ref{fig:AI-generated-attributes}b).

% \bryan{AI can make errors. So we also make it clear which attributes are AI generated and which are not --> showing the sources, etc}



% Second, attributes in online platforms such as e-commerce marketplaces may not be consistent across items; perhaps the \textit{Screen Size} attribute for a monitor may be called \textit{Display Size} for another, and the \textit{Screen Size} attribute may even be hidden in a long text description. To address this, AI can identify the value of what would be the \textit{Screen Size} attribute from each item and surface that value (Fig. Xb). If AI finds the value, it can additionally reference existing attributes it sourced from. Otherwise, AI can provide a response such as ``Not Specified''.


% filling in empty details across items
% Generate new properties for items --> populate in boths views
% Generate new properties across all times in overview (cheapest price across all items)

% detail, attribute

% Not only is surfacing attributes valuable for 
% New attributes surfaced in the overview can then be sorted and filtered. For instance, users can select the X attribute, and sort it low to high. Upon encountering a ``new'' label on an item, users can filter all items that are new.
% Other components then may also be sortable and filterable. The ``Add to cart'' button can sort by its boolean value---whether the item was added to the cart or not. This may be used to sink the items that were already added to the cart to the bottom of the list.
% This includes numerical attributes such as number of items sold or text values such as the brand name.
% Numerical values can be sorted numerically and text can be sorted alphabetically.
% This also includes buttons---sorting the button attribute can sort alphabetically, but sorting the ``Add to cart'' button can sort by its boolean value---whether the item was added to the cart or not. This may be used to sink the items that were already added to the cart to the bottom of the list.

% This statement below... it's less related to the whole section
% While we do not provide a solution for creating any representations flexibly and ad hoc, \technique provides 1) a unified mechanism to spawn these diverse representations and 2) a unified endpoint for externally developed overview representations to interoperate with malleable overview-detail interfaces.

% \Technique makes overview-detail interfaces easily interoperable with other representations. 

% I want to say, transformable representations with attributes makes it extremely easy to change the order of information.
% On a table, you drag the column to reorder, so you can see certain criteria closer together -- This allows you to compare items much easier.
% This action translates and synchronizes to other representations, such as dragging X column will also drag that attribute to the top in the list view.

% @HAIJUN
% I removed the subsubsection about syncrhonizing attributes across views becase I realized \technique is ALL about synchronization! syncrhonization across overview and detail and synthonization across items in the overview.
% Also, the usability of the scroll individual cards to show the selection wasn't very practical when testing it out

% \subsubsection{Peeking at Attributes}
% \Technique also makes it easy to peek at attributes across items. Hovering over an attribute in the detail view will temporarily lift that attribute for all other items.
% \bryan{I realized scrolling through views doesn't really work that well in terms of usability. Maybe i can bring it back for the video.}
% \subsubsection{Peeking and Navigating to Attributes}
% You can hover over an attribute for an item, and it will reveal this attribute for all other items---as a non-committal way of seeing the other items.
% If an interface makes individual items scrollable
% Since \technique  applies interactions with attributes across all items, users can leverage this property to synchronize the view of each item.
% Hover over a detail, this shows on all other items in overview

% \haijun{• hovering on details in a detail view to review details of items in the master view}
 % Click will scroll to that detail  (navigation technique)

% DIFFERENT REPRESENTATIONS VIA ATTRIBUTES
% Color Picker 

% Integrating AI into interfaces to fetch information across different pages can become cumbersome, especially when the data is unstructured. \Technique gives AI a really nice structured space to work in, 




% We should say, supporting various tasks with various interface options because pretty easy to achieve with thie malleable interface.


% \subsubsection{Multiple Overviews to Facilitate Organization (Fig. X)}
% \label{feature:many-overviews}
% Users can also utilize multiple overviews, especially for tasks that require multiple stages of consideration or evaluation, such as decision-making. By forming multiple overviews beside each other, one can move items between these views, each view possibly representing a tier list of items the user wants---similar to how a kanban board is used to manage multiple stages of tasks.\bryan{partition one's decision-making process into multiple filtering stages}




% \subsubsection{Creating Comparison Views with Multiple Detail Views (Fig. X)}
% \label{feature:comparison-views}
% % Comparing between items can be in decision-making
% Comparison views can be supported through the composition dimension of allowing users to create multiple detail views. Users can select items in the overview and open them into individual detail views to directly compare then side-by-side. 


% Creating multiple detail views to directly compare between these items. (This can also then be used as a specific collection in an overview, by forming a new overview from selected items)





% Leveraging multiple views for decision-making, saving information, organizing things better, etc.





% \subsubsection{Configuring Overviews and Detail views to Reduce Clutter}








% For managing various forms of composition, we find displaying
% \subsubsubsection{Dropdown Menus} switch among list, table, grid
% \subsubsubsection{Control Panels} create new overview, manage

% \subsubsection{Supporting Information Tasks with Different Configurations}


% in the follwoing, we talk about different configurations and what tasks they can support

% \subsubsubsection{Creating multiple overviews to facilitate Organization}


% \subsubsubsection{Configuring Overview and Detail to Reduce Clutter}


% \subsubsubsection{Creating Comparison Views}of tasks they support --> the higher level task they can support




% finding distance?


% look at mesh, what kinds 

% using This subdimension


% shopping new p-->copies over
% map search results --> in one map

% Detail view layout --> you see multiple items at once scroll through

% shopping item --> item, item 1, 2,3,4

% other view




% \bryan{"•" Means it's already developed. "X" means not yet.}
% \subsection{Menus and Tabs}
% \bryan{• Customize the entire layout dimension}
% \bryan{• Customize number of overviews (composition sub-dimension)}
% \bryan{X Google Scholar scenario: List of citations (outer list). Open one of the paper's list of citations as well (inner list). Connect the inner list out with the outer list. Hierarchical dropdown menu of citations}

% \subsection{Direct Manipulation}
% \bryan{X Dragging items out of overview to create detail view of that item to compare side-by-side}
% \bryan{X Reorder the list of many overviews}
% \bryan{X Start in List view. Change the order of table view columns. Re-ordering also applies to List view}


% % End Section.
% % Here are my reasoning for this structure & more thoughts:
% \bryan{thought 1, thought 2}


==> versions/initial_submission/5_applications.tex <==
\section{Applications}
\label{section:applications}

To demonstrate the generalizability of our interaction techniques to all forms of overview-detail interfaces, we describe several application scenarios using our techniques.

% \subsection{Exploring literature}
% It can be challenging to stay oriented during exploratory searching tasks such as literature search. One can explore a paper and its citations, leading to an exponentially growing search pattern with no end. One way to make this process more manageable can be to form a hierarchical layout of each paper's citations that opens information to cited papers as a dropdown instead of in a separate page---essentially collapsing the entire hierarchical search path into a dropdown menu (Fig. Xa). Another detail view can then be opened side-by-side to view individual papers in full detail (Fig. Xb).

\subsection{Reading and Managing Emails}
Oftentimes, emails can contain details such as a response deadline. However, this detail is likely not shown in the overview. Using \technique, users can prompt for an attribute \textit{Response Deadline}, and sort by emails that have the most upcoming deadlines (Fig. \ref{fig:application-email}).

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{figures/5_applications/application-email.png}
    \caption{Users can prompt AI to sort by emails with the most urgent deadlines. Upon doing so, the attribute \textit{Response Deadline} is surfaced and sorted by latest date.}
    \label{fig:application-email}

        \Description{This figure depicts an email inbox as a list overview. The user prompts AI for "most urgent emails to respond to", which surfaces a newly generated attribute called deadlines.}

\end{figure}

\subsection{Reading Live Articles}
Live news articles report on long-standing events such as presidential elections and sports games. These interfaces appear to aggregate shorter articles in a scrollable stack. However, it can be challenging for users joining in the middle of the event to quickly catch up on the timeline with a long document. To address this, users can select the \textit{Published at} attribute and bind it to a timeline overview, organizing all articles into a timeline. Users can also select which details to show in the timeline before diving into individual articles (Fig. \ref{fig:application-live-article}).
\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{figures/5_applications/applications-live-article.png}
    \caption{Users can catch up on an ongoing news event by surfacing and sorting articles via the \textit{Published at} attribute and transforming the layout from a list to a timeline.}
    \label{fig:application-live-article}

        \Description{This figure demonstrates the utility of layout transformation in reading live articles. The first image (A) shows a standard scrollable stack of live articles on an online news site. The second figure (B) shows the same articles in which a user has surfaced and sorted articles via the \textit{Published at} attribute effectively transforming the layout from a list to a timeline}

\end{figure}
% https://www.nytimes.com/live/2024/09/12/us/california-wildfires-idaho-oregon

\subsection{\TechNique on Mobile: Food Delivery Applications}
% Overview-detail interfaces are also present on other devices and raise similar challenges to those in the desktop that \technique can address.
% We have identified several challenges that \technique can address.
% \subsubsection{Food delivery applications}
When ordering food on a mobile delivery app, some attributes are not shown in the overview. For instance, Doordash shows ratings and rankings of menu items to show what is popular, but do not show descriptions---which includes the calories. An implementation of \technique in this app could allow calorie-conscious individuals to check which items best suit their needs by surfacing the calorie count into the overview (Fig. \ref{fig:application-food-order}).
\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{figures/5_applications/applications-food-delivery.png}
    \caption{Calorie-conscious users can surface the descriptions of food items to view their ingredients and calories. This also demonstrates how \technique can be implemented on a mobile device.}
    \label{fig:application-food-order}

        \Description{This figure shows the ubiquity of manipulating attributes even on a mobile device. The image shows a standard online food delivery app, in which a health-conscious user is able to select the ingredients attribute and calorie attribute and surface them in the menu overview.}

\end{figure}

% \subsubsection{Catching up on unread messages}
% There may be cases when a messaging app has many with unread messages. However, current interfaces only provide two choices: 1) manually enter each conversation to read them, or 2) mark all as read without reading them. \Technique in a messaging app could enable users to select or peek at a conversation and surface the unread messages in the overview, allowing them to quickly catch up on all unread messages in a single view.








% \Technique in a messaging app could enable users to select or peek at a conversation and surface the unread messages in the overview, being able to catch up on all unread messages in a single page.

% Another case may be to catch up on unread messages across numerous chatting groups. Users can surface a specific scope of the latest conversation. Users can 
% * See unread messages all in overview with temp popup




% \subsubsection{Surfacing paper details}

% Surface paper abstract on scholar, surface figures on semantic scholar, surface other information right away for other cases too...

% \subsubsection{Organizing paper citations hierarchically}


% \paragraph{Searching text in the document}


% \subsection{Browser}
% \subsectio{Graphic design}


==> versions/initial_submission/6_design_probes.tex <==
\section{Design Probes}
\label{section:design_probes}

We are interested in studying whether users can effectively customize overview-detail interfaces to suit their needs. To do so, we implemented two design probes, a shopping website (Fig. \ref{fig:probe-shopping}) and a hotel booking website (Fig. \ref{fig:probe-booking})---to approximate a real world scenario of using malleable overview-detail interfaces. We selected the shopping and hotel booking domains for our example websites because our content analysis revealed distinct variations in overview-detail interfaces within these domains. When designing these probes, we made sure to incorporate the key interaction techniques from the previous section. 

We introduce the probes through example workflows of Alice, who is looking to purchase affordable camera lenses to capture the scenic beaches of San Diego, California.


\subsection{Workflow 1: Shopping for Camera Lenses}
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/6_design_probes/design-probes-shopping.png}
    \caption{A screenshot of our shopping design probe, the overview list is shown on the left and a product detail view is shown on the right}
    \label{fig:probe-shopping}

        \Description{This figure displays a screenshot of our shopping design probe. The shopping overview is shown on the left in a list layout, and a product detail view is shown on the right, opened as a new page.}

\end{figure}
Upon searching for ``Canon DSLR camera lenses'' in the shopping website, Alice is presented with a list of results. As she browses through the list, she finds it cumbersome to find how far each lens zooms in as she must repeatedly open the detail view of each product to find this detail. To address this friction, she surfaces the attribute \textit{Focal Length} to the overview (\textit{Surfacing Attributes} \ref{feature:surface-hide-attributes}). She also takes this chance to surface \textit{Maximum Aperture} and \textit{Type} so she can glance at all the basic attributes to start. As Alice reviews the results, she appreciates that some items have been auto-filled by AI (\textit{Establishing Consistent Attribute Values} \ref{feature:ai-new-attributes}). Since Alice is specifically interested in lenses that handle low-light conditions for sunset photos, she sorts the lenses by \textit{Maximum Aperture} (\textit{Sorting with Attributes} \ref{feature:sort-filter-attributes}).

Alice also recognizes that not all lenses may not be compatible with her camera, but she forgets the type of mount her camera uses. Since she knows the model of her camera, she decides to ask AI, ``Is it compatible with my camera Canon EOS R?''. AI then generates the attribute \textit{Compatibility with Canon EOS R} and provides answers ``Yes'', ``No'', and ``Not Specified'' for each lens (\textit{Generating New Attributes} \ref{feature:ai-query-attributes}).

After refining her search and identifying several lenses of interest, Alice decides to categorize them for easier comparison. She creates two new overviews and re-names their titles to ``Want, but Expensive'' and ``Okay, but Cost Effective'', and adds lenses from the search result to each overview for further consideration (\textit{Customize Composition} \ref{interaction-dimension:composition-layout}). To directly compare attributes for each item, she switches the views into tables (\textit{Customize Layout} \ref{interaction-dimension:composition-layout}). After directly comparing, Alice decides to buy an expensive zoomable lens and a cost-effective low aperture lens.

\subsection{Workflow 2: Booking Hotels in San Diego}
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/6_design_probes/design-probes-booking.png}
    \caption{A screenshot of our hotel booking design probe, displaying an overview map on the right and a overview list of bookmarked hotels on the left. A detail view of a selected hotel is opened as a popover left of the map.}
\label{fig:probe-booking}

    \Description{The figure shows a screenshot of the hotel booking design probe, displaying an overview map of La Jolla on the right and a overview list of bookmarked hotels on the left. A detail view of a selected hotel is opened as a popover left of the map.}

\end{figure}

Alice, now excited about her new camera lenses, begins looking for places to stay near San Diego with the hotel booking website.

Alice begins by browsing through the hotels on the map. She notices that while some places have high ratings, some are quite expensive. To view both attributes in the map, she surfaces the \textit{Price} and \textit{Ranking} attributes for each hotel, allowing her to compare them more effectively (\textit{Surfacing Attributes} \ref{feature:surface-hide-attributes}). She bookmarks some promising options, which adds them to a separate overview of bookmarked places on the left side of the interface. Next, Alice considers the amenities each hotel offers. She is particularly concerned with ensuring that the hotel offers 24-hour check-in since she will be arriving late at night. She surfaces this detail to the map.

After finding a list of hotels for San Diego, Alice starts a new search for hotels in La Jolla.
% The hotel interface conveniently retains all the attributes she previously surfaced during her San Diego search, saving her time as she continues browsing. 
However, as she adds new hotels for La Jolla, Alice realizes she is starting to confuse which hotels in her bookmarks bar are in San Diego and which are in La Jolla. To resolve this, she surfaces the \textit{City} attribute from the hotel's address to her bookmarks overview, making it easy to distinguish between the two locations. Finally, after comparing her bookmarked options across both cities, Alice selects a hotel for each part of her trip---one in San Diego and one in La Jolla---ready for her exciting photography journey.

\subsection{Implementation Details}
The two design probes were implemented with Next.js, a React web framework. We used eBay's API to provide results in the shopping website and used Tripadvisors's API to provide results in the hotel booking website. The shopping website supported customizations along the three dimensions from our design space, while the booking website focused on supporting customizations for the content dimension.

% \subsubsection{MVC of Malleable Overview-Detail Interfaces}
% \bryan{The overview of our system architecture is depicted in Figure X.}
% \bryan{Malleable overview-detail interfaces in our probes are composed of two main components: 1) Overview and 2) Detail}
% \bryan{Overview is a UI component that determines how}
% \bryan{In our probes, we assign an ID to all attributes of an item. }

\subsubsection{Storing Customizations}
Our probes store all customizations in a real-time database (i.e., Firebase) in order to log customizations users make during our user study. In practice, customizations can be cached locally in the browser or in the client-side state to respect users' ownership of personal data.

\subsubsection{AI-assisted \TechNique Pipeline}
The shopping interface uses OpenAI's \texttt{gpt-4o} model to generate attributes and values. When the user requests a new attribute in the provided prompt box, the system first prompts the generative model to generate the name of the attribute based on the user's input and the contextual information of each item in the overview. It then follows up by prompting the model again to generate the corresponding values for the attribute across all items.

% \bryan{Figure out robust to present this pipeline. True to implementation or illustrate its potential as well? Full robust pipeline? We did not build that though.}





% Upon searching for ``Canon DSLR camera lenses'', Alice finds a list of results ranging 
% \bryan{Range of lenses, she already has this configuration, so she decides to look for other zoom sizes.}
% \bryan{As she looks through, she finds it cumbersome to keep looking for the zoom attribute, so she surfaces this to the overview. Also surfaces other attributes, she finds valuable to her}
% \bryan{She also realizes upon surfacing these attributes, some items are filled in with AI. Upon hovering over the value, she sees the value came from the attribute X}
% \bryan{Because she wants only these zooms, she filters these in, and sorts by the lowest aperture.}
% \bryan{She also wants lenses that fit with her current camera. So she filters all lenses with the camera mount.}
% \bryan{She finds that some lenses do not mention whether the lens can zoom, so she asks AI ``Can these lenses zoom?'', which AI creates a property \textit{Zoom Capability}.}
% % As Alice scrolls through the overview, she learns the lenses that don't have this capability to all be called ``Prime'' lenses
% %  ^ Is that necessary? I want to add to show that this attribuet could also help with learning the new concept, but maybe it's a stretch, and it's best to keep it simple.
% % \bryan{After finding a few she likes, she decides to purchase two lenses, one telephoto and one prime lens}
% \bryan{After finding a few she likes, she saves lenses into several categories she wants to compare between: ``Want, but Expensive'', ``Could Buy'', ``Must Buy''.}
% \bryan{To do so, she creates three new overviews, each with lenses shes wants.}
% \bryan{As she filters down her choices by comparing items side by side in multiple overviews, she finally decides to buy a lens in Must Buy, and another lens in Want, but Expensive.}




% Pipeline that's more modular -- basically, one that could cal more functions if needed.
% Key is to identify relevant attributes, match/generate new attribute, identify value/generate new value, perform operation



% Specifically, 1) user prompt. 2) AI interprets and identities relevant existing attributes and their values, while at the same time determining which action to perform (sort, filter, surface). 3) Generates the property name(s) if needed. 4) Generates the values if needed. 5) Calls the filter/sort operations if needed.

% 1. User prompt, 2. AI interprets and identifies two things: relelvant existing attributes and their values & select the action to make: add property, filter, sort, 3. Apply those actions back to the interface through functions


% Why design probes? What's the purpose?
% We want to use these probes to study how users use malleable overview-detail.

% Why talk about these design probes? as opposed to the interaction techniques?
% In interaction techniques, we describe all the possiblte interactions we can have with MODs

% However, for our probes, we implemented a subset of these techniques to study 

% Why did we select a subset of these techniques?
% We wanted to study a subset to be able to evaluate them within the time set up for them and not overwhelm the user with too many features.

% Certainly, a system with too many features becomes too complex for users to learn within the given time of a controlled study.
% However, we do not undermine the importance of malleable overview-detail interfaces.
% Many other features in a practical setting, could be implemented to be more discoverable through a prolonged use of the system.

% We want to study how users use malleable overview-detail interfaces.




% \section{Design Probes}
% To study customizability dimensions..... we implemented our interaction techniques into two design probes: a shopping interface and a hotel booking interface.

% \subsection{Shopping Interface}

% \bryan{Layout dimension}
% \bryan{Many overviews, Collection sub-dimension}
% \bryan{Content dimension}


% \bryan{AI interaction feature: Pull details via prompting}

% \subsection{Hotel Booking Interface}
% We were also interested in exploring how users might interact with customizable OD interfaces on a map. So we developed a hotel booking interface that implements Detailed Manipulation.

% \bryan{Content dimension}
% \bryan{Many overviews, but via search results...? Does this count?}


% \bryan{thought 1}


% ---- This is start of temp comment ----
% \section{Interactions for Malleable Overview-Detail Interfaces}


% In this section, we describe interaction solutions to customize overview-detail interfaces along the three dimensions formed from our content analysis: \textit{layout}, \textit{composition}, and \textit{content}. We then highlight key novel techniques we discovered through the process of our analysis of overview-detail interfaces.

% The goal of this section is not to provide ways to turn one overview-detail interface into any other through the design space. Rather, we are interested in the interaction techniques that will provide the end-user the most control and benefit in the interface. 

% % We do not contribute ways to transform one variation into any other in our design space. 

% % We are not interested in comprehensively providing interaction techniques for transforming across all dimension variations, but rather interested in what kinds of challenges we are able to solve among each of these dimensions.

% % We don't provide interaction techniques to transform into every variation and every combination of every variation of these dimensions.

% % Rather, we describe interaction techniques that can make a customizable OD. This section isn't organized by dimensions though. It's organized by interaction techniques that we develop

% % outline
% % first, context: the results from the content analysis is that we found three dimensions of variation in overview-detail interfaces.
% %  What are we showing? Showing how we make those transformations
% % Organize it by dimensions? 

% % The goal is to make options customizable. At its very base, the customizations we provide can be implemented in diverse ways, such as menu option interface. 
% % But through this content analysis, we find novel interaction techniques that are worth exploring.

% % Layout
% % Composition
% % Content

% \subsection{Menus and Tabs}
% \bryan{Basically, this section is for Layout and Composition sub-dimension: more than one overview}

% The simplest and most traditional interaction technique for choosing between multiple options (in this case, variations) is by providing the user with a menu to choose which dimension variation they want to have. This is a simple approach for customizing the Layout dimension (Fig. X).

% \bryan{Then talk about how you can achieve the same thing for how many overviews you want, or how many detail views you want.. This is one of the sub-dimensions in the Composition dimension.}

% \bryan{But master views can be difficult to manage, so a familiar mode is by providing a tabbed view of the many master views, and enabling direct manipulation to rearrange the order of the multiple views.}

% \subsection{Direct Manipulation}

% \subsection{Detailed Manipulation}
% bringing details from the detail view to the master view 

% This interaction technique is agnostic to the interaction mechanism and instead shines light to the opportunity to control which details are shown in different views. 

% This below describes what is possible with \technique when implemented into interaction mechanisms.


% also re-prioritizing the details within the master item, like showing the dimensions to the top of the screen, just like how you can reorder the columns in a table, reorder the details in the list or grid


% \subsubsection{Customizing Composition}

% \subsubsection{Exploring the Generalizability of Detailed Manipulation }
% \bryan{I really want to talk about all the diverse ways you can use this technique though, this is so exciting to me. For instance, you can pull details to the scrollbar on a website, showing something like a scrollable minimap --> you can even made read wear and edit wear scroll bars. You can also remove details from the vscode scrollbar minimap. Another scenario beyond websites but for the design pattern is that you can modify which details you see in your tab bar on the browser. The detail view can actually be information about the history of your tabs, like an archive, and then you can choose to pull a detail about the last time you visited this tab. Then sorting it by the last visited tab. This might even help reduce tab clutter if you know which tabs you last visited or not.}



% \subsection{Interaction through AI}

% Maybe the Southwest example you have on Figma. You can either ask for the cheapest flight across the days, and the surface that detail for all the other days, or just ask for the cheapest flight in each day. We support this flexibility because either case might happen, depending on which one is more situated in the overview or the detail view.



% The user can additionally ask for attributes to surface to the overview through prompting. This can be particularly useful when what the user wants is unclear. For instance, asking for dimensions of an air conditioner on a shopping site would prompt AI to search for width, height, and length attributes of the item results.

% \bryan{I don't think this organization is that great, because we want a separate section for AI. High level requests for AI works not only for attributes but for other controls like layout or composition.}

% pulling details to master view pulls to all the items. The underlying interaction result is that the system propagates the action done by the user of a single item. Following this, we can imagine more actions beyond just pulling details if leveraging AI's ability to understand and act upon user queries. For instance one may ask to see the side profile of monitors. AI can search and identify a side profile image of each item's list of images and display that.

% \subsubsection{Attribute Synchronization}
% Selecting a detail can reveal that detail for all other views, whether it is scrolled through the view or if it's surfaced in other ways.

% \section{Design Probes}

% We describe basically what goes into the design probes we create, and also the interaction possibilities through these implementations


% In our design probes, we implemented \technique by toggling the ``details'' mode, which upon entering highlighted all detail attributes in the overview-detail interface. \bryan{There are different ways to implement this such as selecting an area or highlighting text and showing popups, or making it a default.}

% \subsection{Shopping}

% \subsubsection{A Kanban Board in a Shopping Interface}

% Buttons are also attributes of a particular item, as they are included in the detail view. By leveraging \technique and introducing multiple overviews through dimension of composition, it becomes possible to create a custom Kanban board\bryan{footnote for kanban board!} directly on the shopping interface to partition one's decision-making process into multiple filtering stages. 


% \subsection{Hotel Booking}


==> versions/initial_submission/7_user_study.tex <==
\section{User Study}
\label{section:user-study}

We used our two design probes to understand how effectively users might customize malleable overview-detail interfaces and to observe emergent usage patterns as they utilize overview-detail interface transformations to best fit their needs and preferences. We aimed to answer the following questions:

\begin{enumerate}[label=\textbf{[RQ\arabic*]}]
    \item How effectively can users perform customizations on malleable overview-detail interfaces?
    \item What kinds of usage patterns emerge when interacting with malleable overview-detail interfaces?
    \item What additional customizations did users seek that were not supported by our design probes?
\end{enumerate}

\subsection{Default Configurations}

Our shopping site displayed the \textit{search results} layout as a \textit{list} overview of items. The overview-detail layout was by default a \textit{separate page}, and the detail view displayed one detail item at a time. We additionally provided a second list overview named ``Cart'', which displayed a \textit{grid} layout of the items that were added to it. Each item in the overview displayed the following attributes: \textit{Title}, \textit{Thumbnail Image}, \textit{Vendor Username}, \textit{Vendor Feedback Score}, \textit{Vendor Feedback Percentage}, \textit{Product Price}, \textit{Product Condition}, \textit{Number of Products Sold}, and an \textit{Add to Cart} button.

Our booking site utilized two different overviews: a map overview and an overview list of bookmarks. Upon entering the interface, the map view displayed the \textit{rating} attribute of each hotel, and the bookmark list, upon adding items displayed the \textit{hotel name} attribute by default. 
% Our booking site contained many attributes users would look through. 

These configurations were set as the default for the design probes, as we believed they would be the most intuitive to get accustomed to the interfaces. However, the main objective of the user study is to study whether and how participants would reconfigure these settings to better align with their own preferences.

\subsection{Procedure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.75\linewidth]{figures/8_results/study-procedure.png}
%     \caption{Visualization of the user study timeline}
%     \label{fig:study-procedure}
% \end{figure}

Our 90 minute user study primarily consisted of two tasks---a hotel booking task and an online shopping task---in which users used our system to freely customize their layout, composition, and content attributes throughout the task.

\paragraph{Introduction <1 min}
The study began with a brief introduction of overview-detail interfaces to familiarize participants with the concepts and terminology used throughout the study. We ran two 35-minute sessions, one for each task. We began with the hotel booking task because it contained a smaller feature set which could acclimate users to both websites easier. For each task, users were first given a tutorial of our system, which included explanations of each feature as well as mini-tasks to acclimate participants to our probes (\textit{\textasciitilde 10 min}). They then proceeded with the main task, which participants were asked to think out loud \cite{thinkaloud} (\textit{\textasciitilde20 min}). Once they completed the task, participants completed a questionnaire to share their experience with the website (\textit{\textasciitilde 5 min}).

Our hotel booking task description and criteria was as follows: 
\begin{quote}
    You are traveling to the Bay Area for meetings. You will stay in two different locations, one night per stay and will need to find a hotel for each: San Francisco and San Jose. 
    \begin{itemize}
        \item Your total budget is \$350 USD,
        \item You want to eat at the hotel (or hotel room) as much as possible (strong preference for hotels with included breakfast or room service)
        \item You prefer modern and new hotels over traditional or old ones,
        \item You would like to stay one night at a premium/luxurious hotel.
    \end{itemize}
\end{quote}

Our shopping task description and criteria was as follows: 
\begin{quote}
You are choosing two monitors: one for your home and one for your workplace.
    \begin{itemize}
        \item Your total budget for two monitors is \$250.
        \item Criteria for monitor at home:
        \begin{itemize}
            \item You want a decent deal.
            \item You want the highest resolution possible, 4k or maybe better.
            \item The monitor should take up minimum space on your desk.
        \end{itemize}
        \item Criteria for monitor at work:
        \begin{itemize}
            \item The condition of the monitor is the most important.
            \item You want a display that’s decently sized, but also has high pixel density (resolution / display size).
            \item You don’t need a monitor stand---assume the office already provides one
        \end{itemize}
    \end{itemize}
\end{quote}

At the end of the session, participants were interviewed to provide qualitative feedback on their overall experience (\textit{\textasciitilde 20 min}). These interviews helped us hear their thoughts on customization preferences, strategies, limitations, and opportunities.
% The full list of interview questions is provided in Appendix  \ref{appendix:interview-questions}.

\subsection{Participants}
We recruited 12 participants (5 male, 7 female) from a local university through internal communication channels. Of the participants, five were graduate students and seven were undergraduate students. All participants reported having experience with online shopping and booking. 

Initially, we asked participants to use their own laptops for the study so it is most familiar and comfortable for them, but after four participants, we deemed users may prefer better setup than their laptop. Thus, we offered the remaining participants an external monitor (4k resolution, 31'' screen size), a keyboard, and a mouse. When offered, 7/8 participants chose to use the monitor. Participants were compensated \$30 USD for 90 minutes of their time.

\subsection{Measurements}
To observe potential customization patterns during our tasks, we logged all participants' actions with timestamps with our system. 
We logged the types of customizations they made throughout their task, how frequently they made particular customizations, and which attributes they surfaced and hid from the overviews.
To capture additional context and insights into participants' behaviors, we recorded both screen activity and audio during the tutorial and think-aloud tasks for further coding and analysis.

We collected responses from each post-task questionnaire (7-point Likert scale) to assess self-perceived usability and utility of our provided customization features. 
% The full list of questionnaire questions for each task is provided in Appendix \ref{appendix:posttask-questionnaire}.


==> versions/initial_submission/8_results.tex <==
\section{User Study Results}
\label{section:results}

In this section, we report on the findings from our questionnaires, interviews, and observations from their tasks.

\subsection{RQ1. How effectively can users perform customizations on malleable overview-detail interfaces?}

\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{figures/8_results/questionnaire.png}
    \caption{Participants' responses to the utility and usability of interactions to customize the content, composition, and layout the hotel booking and shopping websites.}
    \label{fig:questionnaire}

        \Description{This image shows two stacked bar charts comparing participant responses to various aspects of customization and usability for a shopping website and a hotel booking website. The chart is divided into two sections: the Shopping Website in the top half and the Hotel Booking Website in the bottom half. The Shopping Website section has 10 different criteria being evaluated, including: Easy to customize content, Useful to customize content, Easy to customize composition, Useful to customize composition, Easy to customize overview-detail layout, Useful to customize overview-detail layout, Easy to customize overview layout, Useful to customize overview layout, Interface was easy to learn, Interface was easy to operate, and Helped more than typical shopping sites. The Hotel Booking Website measures fewer criteria, only 5: Easy to customize content, Useful to customize content, Interface was easy to learn, Interface was easy to operate, and Helped more than typical hotel booking sites. For both websites, each criterion is represented by a horizontal bar, color-coded to represent different levels of agreement, ranging from "Strongly Disagree" (1) on the left to "Strongly Agree" (7) on the right. The x-axis goes from 0 to 12, representing the number of participants or the score given. In general, both websites seem to have received positive feedback, with most bars heavily weighted towards the blue (agreement) end of the spectrum. The shopping website appears to have slightly more varied responses, especially for criteria related to customizing layouts and composition.}

\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/8_results/customization-logs.png}
    \caption{The number of customization operations made by each participant for each dimension. The hotel booking website supports surface and hide attributes, and the shopping website supports customizations for all three dimensions. For the content dimension, we count how many new attributes were interacted with. For other dimensions, we count the total number of operations participants made.}
    \label{fig:dimensions-logs}

        \Description{This image shows a table comparing the number of customization operations made by participants (P1 to P12) for each dimension in two different websites: a Shopping Website and a Hotel Booking Website. Note that the hotel booking website supports surface and hide attributes, while the shopping website supports customizations for all three dimensions (content, composition, and layout). For the Shopping Website: the Content dimension includes Surface Attributes, Hide Attributes, Sort Attributes, and Filter Attributes. The Composition dimension includes Add New Overview, measuring how many times each participant added a new overview during their task. The Layout dimension includes Overview Detail Layout, Overview Layout, and Detail Layout. The Hotel Booking Website only includes the content dimension, which includes Surfacing and Hiding Attributes. The data includes numerical values for the frequency of each customization, but is also presented in a heat map style, with darker shades representing higher numbers of operations.}

\end{figure}


% \textit{How effectively can users perform customizations on malleable overview-detail interfaces?}

All participants were able to complete both tasks within the time provided during the study.
They reported that the interfaces of both probes were easy to learn (booking: 11/12; shopping: 12/12) and operate (booking: 9/12; shopping 12/12). 
% Able to learn (11/12 booking; 12/12 shopping) and operate the interface (9/12 hotel booking; 12/12 shopping)
% 11/12 participants agreed that the booking website was easy to learn, and 9/12 participants agreed it was easy to operate. All participants agreed the shopping website was both easy to learn and easy to operate. 
% Basically, all participants used our features.
All participants surfaced attributes on both websites, while 9/12 participants hid attributes on at least one of the websites. 10/12 participants sorted or filtered by attributes on the shopping website.
 % (booking: 7/12; shopping: 6/12)
Most participants also customized the composition (10/12) and layout (11/12) of the shopping website (Fig. \ref{fig:dimensions-logs}).
% \bryan{Also say these details are in Fig. \ref{fig:dimensions-logs}}
% 11/12 participants agreed the hotel booking website helped more than typical, and all participants agreed shopping helped more than typical. 
These results suggest that our participants were able to utilize the customizations provided and understood the value of malleable overview-detail interfaces. 
P1 described how the customizability features allowed them to feel more in control with the interface, saying: ``\textit{The ability to choose exactly what I wanted on my screen and close everything else was super nice. You can't really do [that] with a lot of sites. Like, it is what it is.}''
% P6 described using the design probes as being similar to ``\textit{cooking a meal,}'' stating: ``\textit{It's like having all of the ingredients ready before starting, so you have everything that you need.}'' 

% This suggests participants understood the value of malleable overview-detail interfaces.

\subsubsection{Users made diverse customizations even when given the same task}

% \bryan{Diverse customizations means participants effectively used malleable overview-detail interface, because they all converged to what they wanted.}
% \bryan{I may need additional visuals showing the different types of layout they chose}

Although we found popular attributes that many participants surfaced (e.g., \textit{Price Value}, \textit{Breakfast Available}, \textit{Maximum Resolution}), we also observed that individual participants surfaced different sets of attributes for their individual needs. For example, P4 surfaced the attributes \textit{Pool}, \textit{Laundry Service}, \textit{Express Check-in / Check-out}, and \textit{VIP Room Facilities}---attributes no other participants has surfaced.
Participants P7\textasciitilde P12 surfaced unique attributes in the booking website as well, such as the hotel's \textit{Brand}, \textit{Multilingual Staff}, and even the ``\textit{Add to Bookmarks}'' button (Fig. \ref{fig:attributes-logs}).

Since the hotel booking interface provided participants with two overviews with different size and style, we also observed that participants surfaced different attributes for each overview. For instance, P4 surfaced \textit{Price}, \textit{Number of Reviews}, \textit{Ranking}, and several hotel amenities in the bookmarks bar, but only surfaced \textit{Number of Reviews} on the map. On the other hand, P10 surfaced six different amenities in the map but only one in the bookmarks bar. 

We additionally observed different customizations of composition and layout. Some participants used multiple overviews for saving monitors into work and home lists (P1, P2, P6, P7, P12), while others created an intermediate space to save a sub-collection of candidate items (P3, P4, P8, P9, P10). We additionally found that participants used various combinations of list, grid, and table layouts with multiple overviews. For instance, P4 used both grid and list views, while P6 used the list and table views. This suggests that participants effectively utilized the customizations provided to personalize the interface to their own needs.
% All participants primarily utilized the separate page (5/12) and side-by-side (7/12) layouts,


\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/8_results/attributes-logs.png}
    \caption{Visualization of all attributes that participants interacted with in the shopping and hotel booking website. The logs of the attributes that participants interacted with revealed common attributes Minimalists (\ref{results:hoarders-minimalists}) hid from the overview in the shopping website and the unique attributes some participants surfaced to the overview in the hotel booking website. We highlight participants who only surfaced attributes blue and participants who often hid attributes red.
    Attributes are sorted by the number of participants that interacted with them. AI-generated attributes are sorted separately.}
    \label{fig:attributes-logs}

        \Description{This image is a visualization comparing the various attributes that participants interacted with during the user study task: separated between the shopping website and the hotel booking website. The various attribute interactions are as follows: surfaced during task, hid during task, both surfaced and hid during task, and AI-generated attributed. The visualization is presented as a grid, with participants (P1 to P12) listed as the horizontal axis. The vertical axis consists of various attributes that participants had interacted with during the task. The Shopping website visualizes attributes such as Maximum Resolution, Vendor Username, Condition, Estimated Sold Quantity, while the Hotel Booking website visualizes attributes such as price value, breakfast available, room service, and restaurant. Each column (P1 to P12) shows how individual participants interacted with these different attributes in each respective task. The attributes axis are sorted by the number of participants who interacted with them, with the most interacted attributes at the top and the least interacted attributes at the bottom. AI-generated attributes sorted separately. This visualization ultimately allows for a comparison of attribute interactions across different participants and between the two types of websites.}

\end{figure}

\subsubsection{Utility of customizing content}
All participants agreed that it was useful to customize content on the design probes (booking: 6/12 strongly agree; shopping: 10/12 strongly agree). 
Participants explained that its utility came from its ability to avoid unnecessary navigation by bringing all details of interest into a single viewing space.
P3 stated, ``\textit{with a lot of websites that you can't really customize, you end up having to open the products one by one to look at all the specifications, which takes longer. I think it's nice to be able to just see it all as you're scrolling through.}'' P4 similarly described their experience with the hotel booking website compared to other commercial websites:
\begin{quote}
``\textit{Websites like Booking.com, Expedia, and Airbnb don’t have these options. You have to literally look for each and everything. On the booking website, where only the options you want are displayed, it's very easy.}''
\end{quote}
% I would love to have that website soon so selecting hotels won't be a hassle, taking multiple hours.

Additionally, some participants shared that customizing content helped align their decision-making criteria with the information they wanted to see on the website. P12 shared, 
\begin{quote}
``\textit{After reading the information, I kind of have some criteria in my mind of which features I probably want, so I will only concentrate on these features. [With the hotel booking website], I can just customize what information I really want to focus on. For example, I personally really prefer the ratings.}''
\end{quote}

We also observed almost all participants generate attributes with AI (11/12). P12, who surfaced 5/6 attributes by prompting AI, found prompting the interface the most convenient as it gave them direct answers, stating: ``\textit{I'm a very lazy person, so I'll rely on this feature because I don't want to click on each [item] and check whether they are 4k monitors.}''


\subsubsection{Utility of customizing composition and layout}
Participants agreed it was useful to customize composition (11/12) and layout (overview-detail: 11/12; overview: 12/12). 
% When asking participants about what they liked and why they liked it
% Upon finding a customization they liked, we observed that participants mostly stayed with their setting. 
% We observed that the utility of customizing also came from the ease in which they were able to find a setting they most preferred.
The utility of these dimensions primarily came from their ability to quickly find the preferred arrangement of the overview and detail views and their layouts.
P9 said, ``\textit{I kind of found a layout that I liked, which was the side by side, and I just stuck to using that.}''

Furthermore, upon reflecting on their experience with both design probes, P6 mentioned that they had wished their composition and layout settings on the shopping website were also available in the booking website. Specifically, they wanted to see a table overview while collecting hotels to better compare attributes they were interested in.
% , stating, ``\textit{if this layout was able to be implemented with the booking, [it would be] so nice because you can see a [table] instead of making an [separate] excel sheet on the side.}'' 
This further validates the utility of providing options to customize composition and layout of overview-detail interfaces.

\subsection{RQ2. What are the different usage patterns of malleable overview-detail interfaces?}
Findings from the previous section demonstrate that malleable overview-detail interfaces are both effective and preferred by our participants, as the supported customization allowed them to achieve their desired configurations. In addition to enabling these configurations, we are also concerned with how to enable users to reach these configurations more quickly. Therefore, we aim to identify the types of overview-detail configurations users prefer, which could be provided as defaults to different user groups in future interfaces to reduce the number of customization steps one needs to perform.

% Now htat we know our interfaces are useful and that users are able to control it well, we want to know what pattern emerge. Understanding these patterns can help us understand what kinds of overview-detail settings people would prefer the most as defaults.
% \haijun{add transition paragraph here describing why we want to observe these patterns, especially because that we did not motivate these questions when we first introduce them}
% \textit{What kinds of usage patterns emerge when interacting with malleable overview-detail interfaces?}

% \bryan{The goal of this section is to identify groups of behaviors and needs. This will form clear groups of people that will make the reader think, ``You can also start to design good defaults for these groups''}
% \bryan{We would obviously love to provide individual overview-detail for each user, so they don't have to keep customizing to their needs. but we can at least provide better defaults for individual groups. So they can select specific defaults set to their wishes.}


% \subsubsection{Revealers and Removers}
\subsubsection{Hoarders and Minimalists}
\label{results:hoarders-minimalists}
% \paragraph{Removers, Revealers, and Restorers}
% In addition to observing how participants surfaced attributes, 
Prior research has identified tendencies when managing digital information, along the spectrum of two extremes: hoarding and minimalism \cite{Vitale2018HoardingAndMinimalism}. We found that this behavior also emerged when customizing malleable overview-detail interfaces, when users were given the ability to surface or hide attributes from the overview (Fig. \ref{fig:attributes-logs}):
% \bryan{TODO: Rephrase this section}
% https://dl.acm.org/doi/10.1145/3411764.3445585
% Fileweaver
% While all participants added attributes to the overviews with both design probes, we observed distinct behaviors in how they \textit{remove} attributes (Fig. \ref{fig:attributes-logs}). We identified two common groups:
\begin{enumerate}
    \item Hoarders (P2, P4, P10): Participants who did not hide any attributes from the overview.
    \item Minimalists (P1, P3, P6, P7): Participants who deliberately hid attributes from the overview.
\end{enumerate}

P2 (Hoarder) did not hide any attributes in the overview, including ones they surfaced manually from the detail view or by using AI . They reasoned, ``\textit{hiding it has a bigger inertia for me to overcome because if I want it back, I would feel like I wasted more effort to remove it and bring it back again.}'' They further explained that this is their natural tendency, as they also clutter their screen with many tabs. On the contrary, P3 (Minimalist), who hid five default attributes from the shopping website and one default attribute on the hotel booking website, admitted to the higher effort, but also advocated for the reward, stating, ``\textit{it probably takes longer to set it up the way I want it, but also then it's easier to look through because I'm not getting irrelevant stuff.}''

% \bryan{Aligned with literature on hoarding and minimalism \cite{Vitale2018HoardingAndMinimalism}}
Perhaps Hoarders are more resilient to clutter in the overview and less resilient to the cost of repeatedly retrieving information from the detail view. For them, an overview interface that packs information from the start, allowing them to sift through the information themselves, would be more preferable.
On the other hand, Minimalists value the limited space the overview interface can provide and want to ``keep this space clean''. For them, a blank slate in the overview, allowing them to choose which attributes they want to see would be more preferable.

% \paragraph{Participants utilize multiple overviews for different workflows}
% \paragraph{Participants use multiple overviews to break down tasks}
% \subsubsection{Participants use multiple overviews to break down tasks}
\subsubsection{Utilizing the overview composition and layout to structure tasks}
% While 3/12 participants used the default overviews provided to them (Search Results, Cart), the remaining nine
Among the 10/12 participants that utilized multiple overviews to perform the shopping task, five of them (P1, P2, P6, P7, P12) created two overviews---one for each monitor type (work and home). P12, who created these two overviews, approached their task by opening only one overview at a time to find monitors for each type. This setup allowed them to offload important information for later, saying, ``\textit{It gives me some mental space where I can preserve it.}'' They also appreciated how they could open both spaces at once when they needed to compare between the two overviews. P6 also split their budget into each overview, allocating \$150 for the work monitor and \$100 for the home monitor.

The behaviors of these participants hint at a pattern of utilizing the overview composition and layout to reflect and manage sub-tasks.
To support this usage pattern, malleable overview-detail interfaces may provide functionalities that allow users to create nested or linked overviews based on their high-level tasks, manually or leveraging AI. For example, the interface can use hierarchical structures to break complex tasks into more manageable sub-tasks or linearly order overviews to queue sequentially dependent tasks. This aligns with literature that take the task-centric approach to provide hierarchically organized browser tabs \cite{tabsdo}, dedicated desktop spaces \cite{henderson1986rooms}, and dynamically linked email threads \cite{bellotti2003taskEmailThrasks}.
% Approaches to designing task-centric interfaces have been explored by providing hierarchical organizations of tabs \cite{tabsdo}, dedicated desktop spaces on the operating system \cite{henderson1986rooms}, or dynamically linked threads of emails \cite{bellotti2003taskEmailThrasks}.

% Just as Tabs.do reflects the task structure into a hierarchical organization of tabs, users may similarly configure their overview layouts into a hierarchical structure if needed \cite{tabsdo}.
% Other tasks that may involve a more sequential process (e.g., project management), may lead users to produce overview arrangements that resemble a Gantt chart or a Kanban board.



%  ------


% P12 - , especially when I I can compare the home and the work in different spaces by opening them, opening up them together.

% This reveals a group of users who prefer to match their overview-detail interface to how they organize their task.
% suggests that this group utilizes multiple overviews to break down their task into sub-tasks.
% broke down their task into two subtasks: finding a monitor for work and finding a monitor for home. With their organization, they


\subsection{RQ3. What additional customizations did users seek that were not supported by our design probes?}
% \textit{What additional customizations did users seek that were not supported by our design probes?}

\subsubsection{Choose how detail views are invoked (P6)}
% P6 shared how they wanted to change how 
% shared a notable dimension our design space did not include: navigation. 
While our design probes were implemented to open detail views by clicking, P6 suggested the probes to allow users to open details by hovering. They further described how they would also want a ``less maximized'' view of the details, suggesting the desire to invoke multiple detail views with \textit{different sets of attributes} in different ways.

% P6 - different ways to invoked details
% if you could hover over it and just like have it pop up instead of having to click on it. Like the less clicks I have to do the better just because it's like faster for me. Or if there was like a way for it to like be minimized and then be maximized instead of like it all being this like it's all being displayed and I appreciate it all being displayed. But if it was like displayed so I could like actually see the numbers or prices for all of them, would that be nice?

\subsubsection{Attributes about all items in the overview (P6, P10, P12)}
Participants wanted details across all items in the overview, in addition to individual ones for each item. For instance, P6 wanted to calculate the total price of the hotels in their bookmarks bar, while P10 wanted to find a ``best price'' by balancing multiple criteria they surfaced. 
Indeed, if the detail view can have attributes about an item, the overview should also have attributes about the entire collection \cite{Xia2017CollectionObjects}. Since the shopping website provided a title of the overview, it is certainly reasonable for users to also need more attributes that describe the overview itself. 

% \subsubsection{Receive recommended attributes (P2, P11, P12)}
% Three participants also wished to see recommended attributes to surface into the overview in addition to directly surfacing and prompting AI. P11 suggested a sidebar that shows attributes relevant to what they were looking for. This could perhaps better scaffold users in information-seeking tasks, as explored in prior research that explored providing contextually relevant search query suggestions to facilitate exploratory search \cite{Selenite, Srishti2022InterWeave}.











% P2, P11 - Recommended attributes to grab
% instead of you grabbing a detail from an existing entry, I would probably prefer there to be a sidebar showing details that are relevant, like showing fields that are relevant to this thing I'm looking for
% Selenite, CoNotate


% P6, P10 - calculations across overview items
% that would be so nice if there was like a way to have like the budget, like if you could add the budget somehow and like just because I was like using my calculator. But if like there was like a way to like do the math of like, oh, your total sum of hotels is like this much, that'd be nice.


% \paragraph{Further explanations with AI (P6, P8)}
% P8 - AI makes deeper judgments, answering questions about certain attributes


% - Way to invoke detail view --> wanted to just hover over something to peek instead of having to click. Perhaps both can be provided at the same time.. How to let users easily customize this without getting in the way of their work? How to lower that friction/barrier? \cite{Mackay1991TriggersAndBarriers}



% \bryan{Were there some things users tried to do, but then didn't work? Want to ask AI for filters or sorts.}

% \bryan{Participants also wanted features that we introduce in the interaction techniques section... Maybe this is not necessary---reviewers would say: ``Then why didn't you implement that into the probe?''}

% \bryan{Since we provided hotel booking website first---which only provided the content dimension to customize---users brought up dimensions that we had prepared for the shopping website. For instance, wanting to ....? }





% RQ1 DUMP


% AI-enthusiasts

% \subsubsection{AI-enthusiasts iteratively refine their attributes}
% P8's behavior also reveals another finding with AI-assisted \technique. While P8 over-generalized their initial prompts before reaching their desired response---a tendency commonly found in non-AI expert prompters \cite{whyjonnycantprompt}, our design probe still allowed them to iterate towards their desired attribute. Similar behaviors were also observed with P12, who initially generated the attribute \textit{High Resolution}, then landed on the attribute \textit{Is 4k}.
% P12, who surfaced 5/6 attributes in the shopping website by prompting AI, found prompting the interface the most convenient as it gave them direct answers, stating: ``\textit{I'm a very lazy person, so I'll rely on this feature because I don't want to click on each [item] and check whether they are 4k monitors.}''
% appreciated how they could prompt AI for direct answers
% This presents opportunities to provide AI-enthusiasts 

% % Also could be named Restorers
% The third group, Refiners, did not hide any default attributes but hid attributes they generated themselves. For example, P8 initially asked for free shipping, first prompting with ``free,'' which led the AI to generate the attribute \textit{Free}. This did not give them the attribute they wanted, so they prompted again, this time specifying ``free shipping,'' upon which AI generated \textit{Free Shipping}. However, they were not satisfied with the attribute, so they prompted for a third attribute, \textit{Total Price}. After generating the attribute they wanted, they hid both \textit{Free} and \textit{Free Shipping}.

% This behavior differed from the other two groups. Revealers did not hide excess attributes after iterating towards their desired attribute with AI (P2, P10). Removers on the other hand did hide excess attributes, including AI-generated ones (P3). Although Refiners did not deliberately hide default attributes, they did hide excess ones they created, suggesting a unique tendency for Refiners to ``clean up after themselves''.
% % . They instead only made an effort to hide the excess attributes
% % Although Refiners did not deliberately hide default attributes as how Removers did, they did make the effort to hide attributes they generated and no longer needed, suggesting this group's tendency to ``clean up after themselves''.
% When asked why P8 hid excess attributes but left the default attributes in the overview throughout their task, they explained that the excess attributes were distracting because they provided no more information for them. However, default attributes such as \textit{Ratings} were ``\textit{ignorable}'' enough to be kept in case they might be useful in the future.
% % This indicates that Refiners' decision to hide attributes is conditional, with specific criteria determining whether an attribute should be hidden or left visible.




%  So I think it is more adaptive to my own preference and practices.
% Like just make the correct correlation of if I'm looking for this, this is the price I'm going to be looking at. Or like if I want to include these things, this is like but I also need to be like connecting multiple details with each other.

% humble myself --> participant was talking about this when they were 
% P1 even described how customizing content encouraged them to ``\textit{humble myself}'' and tell themselves, ``\textit{Yeah, this is what I actually need to look at}'', suggesting that granular control over content on websites may have better helped P1 reflect on their criteria and needs during the task.
% This suggest providing more granular control over the attributes users may additionally 

% \bryan{Need quotes on AI attributes utility}

% \paragraph{Utility of customizing composition}
% \bryan{Todo}
% \bryan{Must find quotes about how it was useful to add new overviews. Especially how you can add as many as you want.}


% Participants made diverse customizations
% 1. Diverse attributes (Fig \ref{fig:attributes-logs}) were surfaced and hidden -- You can see that there are a lot of commonalities, there are some attributes some people surfaced, but there were quite a few attributes that no one had surfaced. Note the hotel booking as example.
% 2. Composition? but how did they use these different overviews?
% 3. Layout? but how did they use these different layouts?

% P10 added a lot in the map, but not that much in shopping

% Also, why did people surface many different things? Why were the attributes diverse, even when given the same task?




% % I can just customize what information I really want to focus. For example. I personally really prefer the ratings. So I think it is more adaptive to my own like preference and practices.''
% % So I think like what Airbnb and traditional map driven search engine usually just zoom in by only one or two section. For example, them like they're stars or like how far are they from the locations I want or the money like the rent per night. But I think the difference between this one, the concept of it is like 


% % \textbf{Starting to think more about criteria and attributes}
% % P12 - I think I kind of after reading the information, I kind of have some criteria review my mind of which which kind of features I probably want. So I will only concentrate on these features. So I think like what Airbnb and traditional map driven search engine usually just zoom in by only one or two section. For example, them like they're stars or like how far are they from the locations I want or the money like the rent per night. But I think the difference between this one, the concept of it is like I can just customize what information I really want to focus. For example. I personally really prefer the ratings. So I think it is more adaptive to my own like preference and practices. So which makes easier to use?

% % \textbf{Humble oneself; choosing what they actually need to look at}
% % P1 - I got to see all the options that made that a lot easier to do. And I could like, humble myself and be like, yeah, this is what I actually need to look at.



% % appreciated being able to ``\textit{customize what information I really want to focus on}'' (P12), 




% P1 - Being able to like look at this whole thing and see like, oh, this doesn't have a desk or oh, this has a tennis court. The fact that it's visible in multiple places is really nice. I don't have to like search through something to get to it.




% P12 - \textbf{the difference between this one, the concept of it is like I can just customize what information I really want to focus. For example, I personally really prefer the ratings. So I think it is more adaptive to my own like preference and practices. So which makes it easier to use.}



% X/12 particiapnts it was easy to use. They mention it was a bit of understanding, but once they got it, it was quick and intuitive. or something that says that.


% \textbf{You need to literally look for each and everything. This, you don't have to...}
% P4 - it was definitely very useful because most of the UK booking websites, if we see like the booking.com and the Expedia and the Airbnb, they don't have these options. I mean, there are specific things that you want to see and filter out, but then in those websites you have to literally look for each and everything. And in some of the hotels, something is good, something is bad. And in some of the hotels if something is bad, something is good. So deciding between these offsets and whether that extra price is justified or not, those decision like it's very difficult to take in the normal website versus especially the bookmarking option which you had in the booking website where you have only like only the options which you want to be displayed that is getting displayed.





% You have to look for everything manually, and some hotels are good in some ways but bad in others. Deciding if the extra price is worth it is difficult. But with the bookmarking option on your website, only the options I want are displayed, making it much easier. I’d love to have that feature soon, so selecting hotels won’t be such a hassle or take hours."

%  it was definitely very useful because most of the UK booking websites, if we see like the booking.com and the Expedia and the Airbnb, they don't have these options. I mean, there are specific things that you want to see and filter out, but then in those websites you have to literally look for each and everything. And in some of the hotels, something is good, something is bad. And in some of the hotels if something is bad, something is good. So deciding between these offsets and whether that extra price is justified or not, those decision like it's very difficult to take in the normal website versus especially the bookmarking option which you had in the booking website where you have only like only the options which you want to be displayed that is getting displayed. That is like very easy. So yeah, that's makes things definitely very useful for me to use it. So yeah, I would love to have that website hop soon so that yeah, it will be easier every time to select for the hotels, not like the hassle thing and taking like multiple hours.

% P4 - But yeah, these side by side options and also the grid ones, which typical websites don't provide, that makes things very easy. And also the I think the main benefit of both the website is selecting only the useful details and it's starting the rest


% P4 - that's makes things definitely very useful for me to use it. So yeah, I would love to have that website hop soon so that yeah, it will be easier every time to select for the hotels, not like the hassle thing and taking like multiple hours.

% P4 -  I would love to have that website soon so that it will be easier every time to select hotels, it's not a hassle and taking multiple hours.

% P4 said, "That definitely makes it very useful for me. I’d love to have that feature soon, so it’ll be easier to select hotels without the hassle of spending multiple hours."

% P5 -  I think it's just more convenient than what eBay currently has right now just because yeah, eBay is you go to, you click on something, you go to a separate page. And I don't like going back and forth.


% P5 - the options to filter [in booking] are a lot more useful than shopping just because one is like where you're going to live versus like something you're going to buy, I guess. So like the whole thing with if you want like someone who speaks Chinese, I think that's very important. And like I'm surprised it's not been implemented, I guess because that that would be very convenient for someone.


% \textbf{Needing to use other applications -- not a very strong quote though}
% P6 - ``Please make this available tomorrow. I've gone on trips with friends and looking for a place to say, and it's so tough. We end up making an excel spreadsheet [with] all of our options, like costs and everything we need. So if this layout was able to be implemented with the booking site it would be so nice, because you can see a grid instead of making an excel sheet on the side.''



% P3 - it was nice to be able to see like the things that I was looking for on each location. Yeah, Because it prevented like me from having to scroll through every place separately.


% P3 - I really like being able to customize it for both because I think if I were to get like really used to like really used to using it in a certain way, like with the list view or the grid view, then it would be a lot easier to like shop for things with like looking for specific specific criteria.





% P1 - Being able to like look at this whole thing and see like, oh, this doesn't have a desk or oh, this has a tennis court. The fact that it's visible in multiple places is really nice. I don't have to like search through something to get to it.

% P1 - Same thing with like being able to drag over the exact details I want, and then I actually really like being able to remove information I didn't need 'cause then I could just like glance through exactly what I wanted and I didn't have to like read through other stuff.




% \bryan{@Allen: Quotes on why the customizations were useful}


% \bryan{@Allen: How many participants mentioned \technique was their favorite feature?}

% \bryan{@Allen: Quotes on what their favorite feature was and why.}

% P3 - it probably takes longer to like set it up the way I want it, but also then it's easier to look through and I'm not getting like irrelevant stuff.


% P5, who does not like going back and forth between separate pages, also preferred the side-by-side layout, stating 

% , and stated this option was more convenient than standard sites because they didn
% compared the shopping website to other shopping websites, and 

% ``It's just more convenient than what eBay currently has right now just because, with eBay, you click on something, 

% a layout they individually wanted, P9 stating, ``

% As shown in Figure \ref{fig:dimensions-logs}, most participants made two or three customizations in layout and composition, likely because they were able to quickly converger

% ``I found a layout that I liked, which was the side by side and I just stuck to using that.''

% P9 - I kind of found like a layout that I liked, which was the side by side and then I'm just like, OK, I'll just stick to using that. So I guess that's sort of like customization really helps because it's like everybody has like a different way of like doing different things.

% % People talked about how they liked using multiple views, it let them do some things...
% % People liked how they could view multiple different layouts

% P6 - 

% P6 - t's like as much as as like the table, like you're saying like, oh, it's like so terrible. But I actually feel like it's like, it reminds me of like Notion and like Excel. So it's really like structured. And when you're looking for like certain qualities or like certain like features that you want, like specific like requirements that you want to meet, it's so nice to be able to just like see that instead of like making it pretty or like, oh, like I want like, I feel that the grid is like visually like more appealing. But because I was looking for these qualities that's sort of like mix and match like, oh, this goes with this and this goes with this. So just like the mental framework was very intuitive. So that's what I really liked from this. So I really strongly agree with this. I think it's really, really nice. That's awesome, yes. And the interface helped me complete the shopping task better than typical. Yes. I wish all the websites were like this. It was so nice. So nice. I'm so glad to hear that. Yeah. So I'm going to strongly agree with this because like, honestly, I wish like, I am so used to this and like, yes, this isn't pretty, but like for my own sake, if I am customizing it and I have like certain like departments I have to meet, it's like so useful to just like for me to have like mental clarity of like, yes, this is within my budget. This is like, there's my resolution. It's like like taking of things of like A to do list.


% P5 directly compared the shopping website with eBay stating: ``I think it's just more convenient than what eBay currently has right now just because, with eBay, you click on something, you go to a separate page, and I don't like going back and forth.

% But PX preferred the table because of ...

% PX preferred having both a table and a grid because of...


% 11/12 participants stated they preferred the side-by-side view for the shopping website. P3 preferred a popup instead. \bryan{Why?} P12 initially started with a dropdown, then switched to side-by-side. \bryan{Why}

% Ultimately, participants were able to find a preference in the interface, suggesting that participants were able to effectively make use of the options provided by the malleable overview-detail interface.


% RQ2 DUMP



% ---- START SYNCHRONIZERS AND SEPARATORS SECTION ----
% \paragraph{Participants either surface the same or different set of attributes across different overviews}


% \paragraph{Synchronizers and Separators}

% The hotel booking interface utilized two different forms of overviews: the bookmarks bar and the map, which allowed users to either surface attributes to both overviews or just one. We observed that the 12 participants were evenly divided between two distinct usage patterns:
% \begin{enumerate}
%     \item Synchronizers (P1\textasciitilde P3, P5\textasciitilde P9, P12): Participants who surfaced the same attributes into both overviews.
%     \item Separators (P4, P10, P11): Participants who surfaced different attributes in each overview.
% \end{enumerate}

% Synchronizers surfaced all attributes to both overviews, sometimes before opening the bookmarks bar. P12, a Synchronizer, preferred to surface attributes to all overviews with the expectation that the information ``\textit{will be important in the future}''. 

% Although surfacing too many attributes can clutter the map, 

% P8 surfaced both ways, 

% realized to surface it everywhere, if need info i prob need everywhere
% surfaced images in the tutorial
% didn't surface any of the big elements
% didn't use bookmark view


% This aligned with P8, also a Synchronizer

% surfaced all attributes with the mind that ``\textit{this will be important in the future}''

% Not aware of the feature (or just Synchronizer by default...)
% P1, P2, P5, P6, P9

% Aware of choices
% P3 - Synchronizer (Hid choice after surfacing everywhere)
% P4 - Separator (She used the bookmarks bar as a comparison space; map as viewing information) (surfaced rankings and amenities)
% P7 - Synchronizer
% P8 - Synchronizer
% P10 - Separator (Only Map)
% P11 - Separator (Only Map except one in bookmark
% P12 - Synchronizer (This will be important in the future)

% Synchronizers surfaced the same attributes in both overviews, <what motivated them to do that?>
% PX stated ``Something about surfacing the same set of attributes''
% P7 even went as far to surfacing the rating of the hotels to the bookmarks bar, even though it had already been surfaced in the map. (They must have surfaced, hid, then surfaced. Maybe don't use this, it's a little risky)

% Synchronizers:
% P8 - can I get more insights from him?
% P12 - a bit cluttered for sure, but 
% P10
% - less in bookmarks, more in map --> actually no.
% Says it did get cluttered, but they didn't find it a huge issue to zoom in and out for it.
% - Yeah, I think I would still prioritize the the criteria. It's not too bad. I think it's just because they're so close together. The hotels, it's a little cluttered, but it's not like a huge issue like I would just have to zoom in and zoom out for it.
% - Likes having pictures on the map

% Separators chose to surface attributes to 
% - To overcome the clutter issue on the map, P3 added the photo only to the bookmarks bar
% - P4 was an avid bookmarks user. Only surfaced number of reviews to the map (while keeping the default, hotel rating), and surfaced price value, ranking, and amenities about breakfast to the bookmarks bar.
% - Similarly, 

% Same
% 1 2 6 8 9 12

% More in Bookmark
% 4 5 6 11

% More in Map
% 10

% P1
% - same

% P2
% - same

% P3
% - photos
% - 

% P4
% - price, number of reviews, ranking, amenitie, a LOT more in the bookmarks
% - rating, number of reviews

% P5: morein th ebookmkars
% - languages
% - breakfast, room service, description

% P6
% - photos, price level, value
% - breakfast

% P6
% - same

% P8 -- didn't care, but used same
% - same

% P9
% - same

% P10
% - less in bookmarks, more in map --> actually no.
% Says it did get cluttered, but they didn't find it a huge issue to zoom in and out for it.
% - Yeah, I think I would still prioritize the the criteria. It's not too bad. I think it's just because they're so close together. The hotels, it's a little cluttered, but it's not like a huge issue like I would just have to zoom in and zoom out for it.
% - Likes having pictures on the map

% P11
% - More in bookmarks, less in map
% - b: photos, more ameniteies

% P12
% - same

% ---- END SYNCHRONIZERS AND SEPARATORS SECTION ----



% This suggests users who heavily rely on AI to find information 
% This suggests that users who rely on AI will leverage 
% of malleable overview-detail interfaces may

% \paragraph{Reliants}

% \bryan{TODO: Instead of restorers, it's people who were more reliant on AI.}

% \bryan{Move this to AI-assisted section right below. Talk about AI people in one group. Avid AI users}
% so it's not about how they chose not to hide any default attributes, but through refining their prompt with AI, they worked towards a final attribute they wanted.

% From this explanation, it may be reason


% \bryan{This suggests integrating AI-assisted \technique into malleable overview-detail interfaces can provide a workspace to make granular changes while still having the controls to undo those changes, make revisions, or build upon them---\technique provides this entire set of interactions.}
% This process may also be preferred over manually navigating around the overview-detail interface for some users. 

%  And sometimes I don’t care about the details I don’t fully understand, like the model number or similar specifics.

% ``I particularly like the AI feature because it helps me give me direct answers.''

% Want to say this iteration is still eventually good for the user, 

% I think it seems I have the full control over all the criteria, potential criteria I can choose.

% when users inevitably stumble upon getting the right response, 

% \bryan{What does this suggest???}



% P12 - I particularly like the AI feature because it helps me give me direct answers. I, I'm a very lazy person, so I rely on these things that I don't want to click on each tab and check whether they are four key monitors. So I think that feature really help. And sometimes I don't care about the things, the numbers that don't really understand, such as such as these things, the model, OK, these are things I don't care about. So I like how the IT only features two specific item details 4 three of them, and then I can make a decision.

% P8 started their shopping task by asking for three attributes: \textit{Total Price}, which added shipping costs to the item price, \textit{Free Shipping}, whether an item provided free shipping, and \textit{Free}, another request if the. After viewing the values of the three attributes, they then hid \textit{Free Shipping} and \textit{Free}, with \textit{Total Price} remaining in the overview.
% While P8 surfaced attributes about shipping costs, whether there's free shipping or not, P9 instead asked AI for the total cost of each item, which computed the price and shipping cost into one value.


% P2 asked for the size of the monitors...

% We gave participants the criterion ``4k or better'' monitor.
% We saw some participants surfaced the attributes such as \textit{Maximum Resolution}, but many instead asked AI, producing attributes \textit{Is 4k}, \textit{Is 4k Resolution}. P12 initially (?) asked for \textit{High Resolution}, but instead hid that attribute and generated the new attribute \textit{Is 4k}.

% While some participants (P1, P7, P12) asked AI whether monitors included a monitor stand, P11 instead made a new search, ``Monitor with monitor stand'' \bryan{or something like this!}

% P7 also asked for the condition, even though it had already been surfaced in the overview. Looks like P7 used AI to also search for attributes. This may suggest implications on the reliance of AI for other tasks



% But why didn't they hide other attributes given to them by defaut?

% , introduced by using AI to generate attributes, were Restorers: participants who generated AI attributes, but removed them as an iterative step towards their desired attribute. P8 first generated three attributes
% \bryan{What does this suggest? Does this align with other literature? Need to dig deeper into this insight.}





% Revealers: P2, P4, P10
% - people who didn't said, it's not worth their effort, you can see everything, so you may as well just keep it there. (basically, you can just ignore it)
% Removers: P1, P3, P7
% - people who wanted to hide attributes say it's too cluttered, and I just want to focus on my information
% Restorers: P11, P12
% - What did restorers say? What's their reason for hiding back attributes?
% People surfaced details, but didn't hide defaults. Does this mean they liked the defaults? or did they not bother to hide? or did they really want to hide the things they surfaced?
% look into P8, who surfaced Free Shipping but hid it back


% We also observed participants who appeared to be primarily Revealers until they wanted to remove an AI-generated attribute they did not want. For instance, P8 first generated the attribute \textit{Free}, then \textit{Free Shipping}, then finally \textit{Total Price}. 




% For instance, P8 first generated the attribute \textit{Total Price} to see the total price of the item including shipping fees, then generated \textit{Free Shipping} and \textit{Free}. They then sorted by \textit{Free}, until finally removing it and instead grabbing the actual shipping value. That's because AI just didn't work here man.


% P2 - ``I just didn't really want to waste effort of hiding it because I already took effort to add it.''
% P2 - I just didn't really want to waste effort of like because I took effort to add it. And so like hiding it has a bigger kind of like. Inertia for me to overcome because like, what if I want it back then I have to go back and then like, feel like, oh, wasted, you know, like more effort to remove it and bring it back again.


% PX did not hide default attributes, but did hide attributes they had surfaced before. 

% * does this align with past literature?

% \paragraph{Opening and closing attributes over opening and closing views}
% P8 added a lot of filters. interesting user.
% P3 and P8 surfaced attributes, then hid them. \textbf{Does this suggest a behavior of users ``opening'' and ``closing'' attributes, rather than full web pages?}
% \textbf{Perhaps, more granular control over the information on their websites allows them to still effectively find information they want?}
% Look at P3 -- They hid a lot of things. They surfaced, and then hid back a few things as well.



% We observed that 10/12 participants utilized multiple overviews to approach the shopping task in two distinct approaches:
% \begin{enumerate}
%     \item  5/12 participants (P1, P2, P6, P7, P12) created two overviews, one for each monitor type (work and home)
%     % \item ---by creating a separate overview for each.
%     \item 5/12 participants (P3, P4, P8, P9, P10) created an intermediate collection for items that best satisfied their criteria, assigning names such as ``Save for Later'', ``Wishlist'', or ``Maybe''.
%     % \item prioritized criteria, adding items that best satisfied their criteria into an intermediate collection (). Another collection was then used to add and remove finalists from the intermediate collection.
% \end{enumerate}

% divided their interface into two subtasks

% P12 - The different space is very important for me, especially when I I can compare the home and the work in different spaces by opening them, opening up them together.

% P12, who created two separated overviews for work and home, sometimes opened only one of the overviews to focus on one sub-task, but 

% P12, who created separate overviews for work and home, focused on finding a monitor for one location at a time by hiding the other overview. This setup allowed them to switch their attention between the two tasks, stating, ``It gives me some mental space where I can preserve it.'' P6, who also created two overviews, even split their budget for each overview, allocating \$150 for the work monitor and \$100 for the home monitor.
% This suggests that this group utilizes multiple overviews to break down their task into sub-tasks.
% % broke down their task into two subtasks: finding a monitor for work and finding a monitor for home. With their organization, they

% On the other hand, some participants P4, who utilized an intermediate overview, began their task by collecting items into their intermediate overview based on key criteria—such as resolution, brand, and model. They used this overview to add and remove candidates, while dedicating their Cart overview as the final collection, suggesting that other users utilize multiple overviews as a way to sift through the results to find items with the best criteria first.

% to sift through items primarily based on criteria


% On the other hand, P4, who utilized an intermediate overview, began their task by looking for items with the best resolution, best brand, and newest model of monitors. They added the monitors that best matched these criteria into their intermediate collection, then among the candidates, saved the best candidates for work and for home. They dedicated the Cart overview as their final collection, while using the intermediate space as a workspace to add and remove items, suggesting another group of users that prioritize criteria and utilize multiple overviews to sift through items that best match their criteria.



% another group of users that prioritize criteria and utilize multiple overviews to sift through items that best match their criteria.


% This approach highlights the benefit of using multiple stages of overview to enhance decision accuracy and efficiency. For design implications, consider incorporating features that support intermediate evaluations and allow users to refine their selections progressively, improving their overall experience and satisfaction.


% Among the options, P4 was willing to compromise the condition for their home monitor, so 
% P10 approached this similarly, and also mentioned, if they had much more options the would have added more lists. \bryan{But to do what? what would be the purpose to add more lists?}


% because participants oftentimes kept both the intermediate overview and Cart overview open at the same time, suggesting the value of maintaining a visual context


% P5 and P11

% While this usage pattern is similar to using the Cart overview, 

% This usage pattern differs from the the use of not using additional overviews (only using the Cart overview) 
% Cart, they added 

% P5 only used the cart, but not 


% This approach differed from

% collected items that best fit one or more of their criteria. 

% P4 - First of all I wanted to go with the like the maximum resolution, the best brand and the newest model. What's the price? Since I have the limited budget, what's the price? So since I saw that the 4K ones are like pretty expensive that itself cost like more than 250. So I cannot ever buy 2 laptops considering one having the 4K. So I just opted that option out at all. I was not choosing at all in my next steps in the maximum resolution. Then I went to the 2K. The 2K models what I saw and I wanted the condition to be new because first of all I was selecting for the workplace. So for the workplace I want something new and then the next resolution was 2K. So for the 2K then I selected what were the options in the search result. Then in the search result I found three options. One was over budget. I opted that out. I then there was two options out of that too. One was the good brand, so I selected that and discard the rest. So with the work option I have, I had the best price, newest, best resolution and also the good model.

% P4 - Then whatever the money I had left, I can compromise on my like home monitor. I see. Yeah. So then I chose the condition as used or like certified. So first I chose the certified one, the level level down one by one. I chose the open box and certified. If I'm not getting anything there, then I chose the used one. But then whatever I have, I segregate that in the list, like the non work one, the home ones. And then I made this mind that if I have more money than I can buy the open box and if I have strict budget, if I'm like poor, then I can buy the used one. Yeah.

% criteria over subtasks.

% P4 added items in their intermedi
% which led them to collect items that best satisfied one or more of their criteria. Then used the intermediate step to collect items with the best criteria



% On the other hand, P9 utilized an intermediate overview to 
% compare and contrast between all possibly options, and used another overview as a ``\textit{final list}''. 

% \bryan{Separate their space is one way to help make decisions}
% The group that separates their final spaces may work to separate their collections based on subtasks,




% P9 - adding different lists. I think for me, having one list work at like store stuff for like, OK, I like different options and then I can compare and contrast between each of those different options. And then the card is more of like a final list of like. Out of the ones that I chose, I think the list feature was the most helpful.

% P4 - So for the workplace I want something new and then the next resolution was 2K. So for the 2K then I selected what were the options in the search result. Then in the search result I found three options. One was over budget. I opted that out. I then there was two options out of that too. One was the good brand, so I selected that and discard the rest. So with the work option I have, I had the best price, newest, best resolution and also the good model.

% P11 - like the idea of having other lists as essentially like a part. And I think there are some like slight UI issues with it with kind of like, OK, let's say like I feel that because of the shopping website, the cart should always be treated specially. Yeah, instead of just a list like like list would just be less in part because like a car, you actually could like it's like you're essentially checking out. You're in the couture line, you're going to pay for it. Yeah, yeah. Whereas list is like wish list, you can just look more casual.


% \bryan{To best benefit these groups, a default MOD could be provided to allow users how many types of items they will purchase, providing enough spaces to compare within the options. Perhaps even allowing comparison between combinations of items can be provided.}
% \bryan{For the other group who organize items into intermediate collections, providing stronger synrchonization or something..... }
% \bryan{But these are like design recommendations. So all of these should just be foreshadowed... maybe?}


% \bryan{Different content in different overviews}
% Hotel booking site provided two overviews: bookmarks list and the map view. We noticed participants surfaced different attributes for the two different overviews.

% For instance, PX surfaced this on the map, but surfaced this on the bookmark.

% PX surfaced both these on map and bookmark, but the bookmark additionally had this attribute.

% P11 -- hide image in the map, but instead added to the bookmark. Didn't want clutter.

% Use of different customizations across different overviews were also observed on the shopping website. In the shopping interface, creating a new overview carried all surfaced attribute settings to the new one. By default, all add to list buttons were added in each overview. P7 instead removed add to list buttons that were not for that particular list, leaving each overview to only have a button that removed from its own list, serving as a ``delete'' button. Others used different layouts for different overviews, such as P4, who used a grid and a list and P11, who used a grid and a table.



% P2 
% P3 used maybe and then cart

% consdier candidates for the two locations

% Considered candidates in one space, as an intermediate space.
% Intermediate space contained both monitors for the two different spaces.

% This suggests, people do have different working patterns, able to customize the overviews for their different cases

% P10 - 

% ``The different space is very important for me, especially when I can compare the home and work in different spaces''

% P12 - The different space is very important for me, especially when I I can compare the home and the work in different spaces by opening them, opening up them together.

% P12 - It gives me like it gives me some mental space that I can preserve it.



% \paragraph{Surface to sort}
% \bryan{Another visual showing all the cases where participant sorts right after surfacing attribte or right after filtering}
% We commonly observed participants surface attributes, then sort or filter them right away.
% \bryan{I saw that there's a correlation in the number of attributes surfaced and the number of attributes sorted. I wonder if there's a common Surface + Sort mechanic happening?}
% \bryan{I think there's a common usage pattern of surfacing, then sorting right after.}
% \bryan{There is also one quote saying they feel they can sort by anything}
% \bryan{If you know you're able to sort or filter by every attribute possible, then there's no point it having a dedicated filter/sort area. Instead, you can just directly sort any attribute or value.}
% \bryan{This suggests an interface can support: if user surfaces an attribute, a sorting and filtering functionality shows up in the UI.}
% \bryan{Another options is to also be able to sort or filter from the detail view rather than only in the overview.}

% \textbf{Different in layout?}
% Did they use differnt layouts for different views, or did they constantly switch between many?

% What were the different layouts people created for their search? did people use two different views? Did people use the same view across different overviews? 



==> versions/initial_submission/99_conclusion.tex <==
\section{Conclusion}
\label{section:conclusion}

This research explored malleable overview-detail interfaces, ones that end-users can customize to address individual needs. We conducted a content analysis of overview-detail interfaces in the wild and identified three dimensions of variation: content, composition, and layout. Based on these dimensions, we developed interaction techniques to support customization along these dimensions. Most notably, we introduced a novel interaction technique, \technique, that enables users to choose which, where, and how attributes are displayed in each view, sort and filter items by any attribute, and generate new attributes and reformat existing ones by leveraging AI. Our user study found that participants produced diverse customizations and surfaced usage patterns in how they managed attributes and organized multiple overviews. We hope our work paves the way for further exploration of malleable overview-detail interfaces in new contexts and inspires the expansion of malleable interfaces to additional design patterns.



==> versions/initial_submission/9_discussion.tex <==
\section{Discussion and Future Work}
\label{section:discussion}

Our exploration of design probes and observations from our user study reveal opportunities to further investigate malleable overview-detail interfaces. We discuss potential directions for supporting additional aspects of in our probes and in future systems, studying their prolonged use, and exploring practical approaches to implement them in real-world websites. Finally, we explore the potential for malleable overview-detail interfaces may have for user-defined abstractions.


% \subsection{Even more malleable overview-detail interfaces}
% \subsection{Even More Malleable Overview-Detail Interfaces}
% EMMODs

\subsection{Supporting More Variations for Malleable Overview-Detail Interfaces}
In this research, we focused primarily on the utility of the malleability of overview-detail interfaces, rather than the utility of each individual variation. As a result, we did not implement all possible variations within the design space. However, implementing the full range of variations---and potentially more variations outside of our design space---could provide a more comprehensive understanding of the value each design option offers. 
Probes could also be implemented in different contexts beyond shopping and hotel booking to offer insights into which variations and instances users prefer in diverse scenarios and gain stronger evidence of diverse usage patterns of malleable overview-detail interfaces.
% A larger set of provided variations and contexts could open opportunities to uncover more usage patterns of malleable overview-detail interfaces than what we identified.
Future work should explore the full range of design variations, including those beyond our design space, and investigate their utility across different contexts.



% Another value that long-term studies could provide is the opportunity to uncover more usage patterns we identified.

% \bryan{Explore deeper into what kinds of variations could be possible}
% \bryan{Being able to change axes and navigation, could become these transformation primitives, which AI can get change and generate UI and functionality for it to make those transformations work, for instance, generating brand new overviews, or generating more overview-detail layouts beyond those mentioned in the design space}
% Future studies could also include more probes across different contexts beyond shopping and hotel booking, offering insights into which variations and instances users prefer in diverse scenarios and why.


% \bryan{Direct manipulation to communicate AI operations}
% \bryan{Our stuff focused on direct manipulation of attributes to basically move them or filter. And most of AI was triggered by prompting.}
% \bryan{We did have one feature where you can surface, and AI would essentailly autofill values of items that aren't there.}
% \bryan{maybe somehting with direct manupulation, but these actions communicate the intent to AI, resulting in some operation.}
% \bryan{What could happen if you could drag an attribute onto another attribute}
% \bryan{What could happen if you could an attribute onto a different item?}
% \bryan{What coyld happen if you select multiple attributes and drag them to an empty space?}
% \bryan{Maybe this is backwards thinking... maybe you need to flip the thinking to needs-based, then provide DM opporunities}
% \bryan{This relates to more variations because this could make it possbile to create more variations in MOD...}



%  Moreover, there are opportunities to deeply explore these additional variations beyond the ones implemented in our probes, such as customizing how one might invoke detail views from the overview (e.g., clicking, hovering, highlighting).

% \subsection{}

% \bryan{What are other usage patterns out there?}
% \bryan{We could discover more with a prolonged study.}


% \subsection{vs or +  Defaults for malleable overview-detail interfaces}
% \subsection{Malleable overview-detail defaults: will we reach convergence or an alternating cycle?}
% \subsection{To converge or to alternate between overview-detail customizations}
\subsection{Customizing Overview-Detail Interfaces: To Settle or To Switch?}
% \subsection{Against or for malleable overview-detail defaults?}
% \subsection{Malleable overview-detail defaults: Yes or No?}

% Our study found that some users only surface attributes to the overview while others also hide them. We also found that users will compose multiple overviews to better structure their tasks. 
Our insights offered recommendations for better defaults by observing usage patterns of malleable overview-detail interfaces.
Indeed, some users may only need better defaults, as they perceive customizations as merely a short-term task. 
% tehy see customizations as one-and-done thing...
As P11 commented, ``\textit{Personally, I'd like a customization page or a separate menu for customization, something I can customize once and be done.}''
However, other users may want to keep this power throughout, as P1 expressed a desire to stay in Attributes Mode for their task.
%rather than toggling.
% When asked about desired features of our probes, P2 wanted to see recommendations of attributes to surface, explaining, ``\textit{Given so much power, I don't like many options to customize. I wasn't sure which ones might be more important for me for this specific task.}'' 

These preferences suggest two potential directions for malleable overview-detail interfaces: 1) users may settle on an optimal default setting, or 2) they may continuously switch between different customizations as they navigate their tasks. This raises several questions: \textit{What factors influence users to settle on a setting, and what factors drive them to frequently customize? Does this behavior vary with different customizable dimensions? How does this behavior evolve over time?}
One way to answer these questions is to study the prolonged use of malleable overview-detail interfaces with a larger population. Future work could involve developing and deploying a robust probe to observe when and how frequently users make overview-detail customizations. Such a study would provide insights into whether and when users find an optimal setting, or if they continue to leverage various customizations in different contexts.


% \subsection{Malleable overview-detail interfaces for the real world}
% \subsection{Are malleable overview-detail interfaces worth it?}
\subsection{How Do We Bring Malleable Overview-Detail Interfaces to the Real World?}
% \subsection{Are malleable overview-detail interfaces ready for the real world?}

Our user study showed promising signs of the utility and value of malleable overview-detail interfaces for end-users. Our design probes further demonstrated that such interfaces can be effectively implemented on websites. However, the decision to implement these designs ultimately rests with the developers---from individual providers to large corporations. Increasing customizability requires additional development, which demands significant time and effort. Therefore, the critical question becomes: \textit{How can we practically bring malleable overview-detail interfaces to the real world?}
% \textit{How can we make it practical for developers to implement malleable overview-detail interfaces?}

Perhaps an approach to address this challenge is to forego the development cost entirely by creating an end-user tool as a browser extension or plug-in, similar to existing end-user customization tools explored in prior research \cite{Zhang2018Fusion, Visbug2024, Kim2022Stylette}. This tool could scrape the currently active website to identify overviews and detail views along with their associated attributes. By leveraging AI, the tool can fill in missing attributes to provide more consistent data. However, there are challenges to consider: websites are constantly evolving, requiring that the tool also adapt continuously to support as many sites as possible. Additionally, the tool would be limited by the data provided by the browser-compiled website data, potentially limiting the customization capabilities for the end-user.
% This solution is currently scoped for browser environments.

Another approach is to build a developer toolkit, such as a library or framework. This toolkit could offer all the variations and customizations outlined in our design space and enable our proposed interaction techniques out of the box. While integrating this tool into websites incurs a cost for developers, it could potentially reduce this cost if the toolkit provides default layouts that developers want to implement from the start. However, providing a broadly implementable toolkit requires engineering this tool to interoperate with existing websites and become reliably extensible to more overview-detail customizations in the future.

Both approaches present their own engineering challenges worth investigating. Future work should delve deeper into the benefits and challenges to effectively bring our malleable overview-detail interfaces into the real world.


\subsection{Malleable Interfaces: Beyond the Overview-Detail Design Pattern}
This research focuses on making overview-detail interfaces malleable. While the overview-detail pattern is widely implemented across many interface systems, it is not the only design pattern in use. Research has explored the challenges and opportunities for end-users to customize various interface elements, including dashboard interfaces \cite{Sarikaya2019ReviewDashboards}, item collections in lists and spreadsheets \cite{Huynh2006Sifter,Litt2020Wildcard}, and menu list interfaces \cite{Park2007AdaptableVersusAdaptive}. We have also investigated how different representations of the overview interface can be customized in relation to the overview-detail interface. We believe that exploring other design patterns and their design spaces can offer new opportunities for making more interfaces malleable. This approach of investigating the variations and nuances of each design pattern may help us move closer to developing a general malleable interface.


% \bryan{There are these other patterns}


% \bryan{By explore how we can make other design patterns malleable, we believe this research contributes an approach towards finding ways to make other design patterns malleable, ultimately working towards general malleable interfaces.}
% \bryan{We believe this research shares an approach to making more }

% \bryan{There's }

% \subsection{A Language for End-users to Customize Malleable Interfaces}

% There seems to be a common misconception that malleable software implies open code and an open architecture. End-users being able to manipulate and tweak their own software doesn’t necessarily mean they should use the same language developers and engineers use. End-users need to be able to use their own language* to manipulate and tweak their own software whenever they want to. 

% \bryan{Opening the code for users to grow acclimated to programming}
% \bryan{Using AI for prompts}
% \bryan{But what we want is a language for the end-users, }

% \subsection{Further Exploring User-Defined Abstractions}
% \subsection{Towards Malleable Interfaces with User-Defined Abstractions}
% \subsection{Towards Malleable Interfaces with User-Defined Abstractions}

% Bret Victor talks about ladder of abstraction to be able to climb up and down to facilitate understanding of systems. This argues that \textit{a single representation is not enough}, but rather interfaces must provide multiple representations. Indeed, our user study observed that users effectively leveraged the various overviews and sets of attributes provided to them. However, our user study also found that users surfaced diverse sets of attributes we could not have fully anticipated.

% Bret Victor discusses the concept of the ``ladder of abstraction,''which allows users to move up and down levels of abstraction to better understand complex systems \cite{Victor2011LadderOfAbstraction}. This perspective argues that a single representation is not sufficient; instead, interfaces must offer multiple representations to support diverse user needs. In line with this, our user study observed that participants effectively utilized the various overviews and sets of attributes provided to them. However, the study also revealed that users surfaced diverse sets of attributes that we could not have fully anticipated.

% Not only is a single representation enough, but \textit{providing} multiple representations is not enough either. Instead, we must provide \textit{user-defined abstractions}---abstractions that end-users can customize or create on their own, enabling them to engage with information in ways that best suit their needs. For instance, if a user is new to a city and wants to know popular areas for lively restaurants, the user should be able to easily augment their map to display a heat map based on restaurant the number of reviews they have. 

% However, this scenario raises two core questions. First, how does the interface provide any possible representation the user wants? One user may want a heat map, while another may want an animation illustrating change in liveliness throughout the day. Perhaps generative AI could help create these abstractions, with emerging systems being able to generate and render user interfaces on the fly \cite{anthropic2024claude35, vercelGenUI}. Though, the challenge still remains in allowing the end-user to understand and change this generated code when it inevitably fails to address the user's exact needs \cite{whyjonnycantprompt, sarkar2022like, designguidelinesforpromptengineering}. Second, how would the user know \textit{what kinds} of abstractions would best help them in their context? Our approach in this paper was to provide default abstractions that can kick-start users' path towards creating their own. However, these defaults may inevitably be insufficient in supporting all user needs. 





% Perhaps the techniques for manipulating attributes explored in this paper may provide the means to elicit the most suitable representations.

% Perhaps these defaults can be iteratively customized kick-start their path towards creating their own abstractions.




% While this makes it high potential, it is challenging to address \textit{all} possible diverse needs we can not anticipate. We identify two hurdles to fully achieve the types of

% Participants surfacing diverse attributes hints at the potential for user-defined abstractions

% , forming diverse and unique abstractions---abstractions users formed to their own preferences, sets of attributes we could not anticipate users to surface.

% Thus, not only is a single representation enough, but \textit{providing} multiple representations to the end-user is not enough either. Instead, end-users must be able to create their own abstractions in diverse forms beyond what we can anticipate. While this goal is 



% Our study found that users could customize ....
% Self constructed, and diverse variations of overviews demonstrating that user-defined abstractions
% custom abstractions users can create on their own.
% We cannot possibly provide more representations for them. Providing multiple representations may not be enough to support understanding.
% Rather, they should form any own abstractions on their own. We envision an expressive way for users to form their own abstractions, beyond just surfacing specific attributes and forming overviews provided to them.
% But create their own abstractions of any form.




% Our study found that users could effectively customize which kinds of information they wanted to surface from the detail view to the overview with \technique.
% and which overview layout they wanted to see items in.
% At the core of the overview-detail pattern is the need to view information at different levels of abstraction, for different sets of details, and in different spatial arrangements during information tasks. 
% Their self-constructed overviews demonstrated their capability to choose which information to abstract away from the detailed views of all items.
% We believe this hints at the potential for \textit{user-defined abstractions}---abstractions that end-users can customize or create on their own, enabling them to engage with information in ways that best suit their needs.

% We believe this points to the potential for user-defined abstractions—customizable abstractions that allow end-users to tailor and shape their interactions to meet their specific needs, enabling them to engage with information in ways that best suit their preferences.
% For instance, if a user is new to a city and wants to know popular areas for lively restaurants, the user should be able to augment their map to display a heat map based on restaurant attributes such as \textit{Review Count}.

% While we propose a step forward with \technique, we identify two hurdles to fully achieve the types of user-defined abstractions we envision.
% lightweight, reliable, and expressive
%  to be communicate to the interface in a lightweight, reliable, and expressive way to produce
% First, we need to effectively support the diverse forms of abstractions end-users need. One approach can be through generative AI, with emerging systems being able to generate and render user interfaces on the fly \cite{anthropic2024claude35, vercelGenUI}. Though, the challenge still remains in allowing the end-user to understand and change this generated code when it inevitably fails to address the user's exact needs \cite{whyjonnycantprompt, sarkar2022like, designguidelinesforpromptengineering}.
% Second, and arguably more importantly, end-users must know \textit{what kinds} of abstractions they need to form. One avenue can be to provide recommendations and default abstractions users can use to kick-start their path towards creating their own abstractions.
% , by first modifying the defaults.
% We believe this direction can lead to promising insights in how the end-user can form and utilize dynamic representations to suit their needs.
% We believe this direction can lead to promising insights in how the end-user can form and utilize dynamic representations to suit their needs.
%  of overview-detail interfaces 



% % \subsection{Towards user-defined abstractions}
% \subsection{Malleable Interfaces: Beyond the Overview-Detail Interface}

% \bryan{To write or not to write?}
% \bryan{This section is not very clear to me right now, but this would lay down the long term vision of malleable interfaces that we want.}

% \textbf{Outline}
% \begin{itemize}
%     \item Can our design approach extend to more design patterns? Does this work provide a step towards making more interfaces malleable?
%     \begin{itemize}
%         \item Pattern 1: Collections
%         \item Pattern 2: 
%     \end{itemize}
% \end{itemize}


% We explored the interaction technique \technique.

% We are curious whether this can apply to other interface design patterns. 

% For a collection of items, definitely. selecting by attribute

% What is my argument in this section though? I don't even know what I want to talk about here, That's the problem

% Our goal: Malleable interfaces. We want to achieve this. We want end-user customization of anything they want, including functionality or whatever. 

% Our question is actually: Does our research approach work for other design patterns?

% What are other design patterns out there?

% viewports

% dashboards

% WYSIWYG



% In this research, we were primarily interested in the utility of the malleability of overview-detail interfaces, rather than the utility of each individual variation. Therefore, we did not implement all variations in the design space. However, implementing all variations into a system could provide a more comprehensive understanding of the utility of each design option within the design space. Additionally, there are opportunities to explore and implement more dimensions beyond the ones in this paper.
% A future study could also include more probes beyond shopping and hotel booking, which could offer valuable insights into which variations and instances users prefer and why in various scenarios.

% We only implemented a few of the variations because we were interested in utility of malleability of ODs, instaed of trying to evaluate the utility of each feature and each variation.
% Implementing all variations into a system  would give us a more comprehensive understanding of the utility of each variation in the design space.
% We could also expand this to more probes in different contexts beyond shopping and hotel booking.
% Studying this may offer insights to which variations and which instances users prefer in which contexts.

% Our two design probes do not implement all variations in our entire design space.
% we don’t implement our entire design space so we don’t claim utility or ease of use of all the variations we collected
% This paper explored three dimensions of variation in malleable overview-detail interfaces and provided interaction techniques for end-users to customize them.



% Furthermore, end-users must know \textit{what kinds} of abstractions to make. When
% Thus we ask the following questions: 

% In the case of \technique, we observed that end-users, such as P12, felt the attributes they surfaced better aligned with their decisino-making criteria.

% This can lead to future designs of malleable overview-detail interfaces that support more ways to abstract information from their details.

% Questions
% 1. How do we enable end-users to create their own abstractions?
% 2. How do we enable end-users to know what kinds of abstractions they need?

% * Our design space observed more forms of abstractions that attributes took, especially visual
% * There are various other forms of overviews that could be achieved, such as
% * 


% \textbf{Outline}
% \begin{itemize}
%     \item Study findings hinted at the value of user-defined abstractions---end-users being able to customize given abstractions and even form their own---through MODs.
%     \begin{itemize}
%         \item How can we further support user-defined abstractions? Can AI support this?
%     \end{itemize}
%     \item More dimensions for MODs
%     \begin{itemize}
%         \item axis, navigation, synchronization
%     \end{itemize}
%     \item Using AI to generate and customize more aspects of MODs
% \end{itemize}

% * We proposed an interaction technique of reformatting titles of items in shopping websites to make them more consistent and easier to read. There are opportunities to reformat more things. Even re-style things, re-arrange attributes to show certain things before others. You can change the size, so you can see specific details easier than others....


% - Towards user-defined abstractions
% \bryan{Our interface hinted at the potential that users can begin to create their own abstractions to suit their needs. Our probes specifically studied how users surface and hide their own details, this being Judy Fan's definition of abstraction. While it's limited, \technique was able to support users in creating their own abstractions that overview items represented for details.}

% \bryan{How can AI help create these different abstractions that people need?}

% % \subsection{There was this one section I wanted to write about, but I don't remember...}
% % \bryan{It was something about the findings from the user study... some result or something....}


% \bryan{Different definitions of abstraction: traditional definition, as well as Judy Fan's definition (more and less details)}

% \bryan{Talk about all the work on abstractions, Damien Masson, Bret Victor, Ian's Notational Programming}

% \bryan{But creating new abstractions are still tough. An initial challenge is that people cannot easily create our own abstractions. Programming is hard. Sketching is hard. To create abstractions, it takes time and effort, costs that people most likely do not afford to spend (This is why research is such a great incubator for novel abstractions). A more crucial challenge that precedes the previous is that people may not even know \textit{what kinds} of abstractions they need.}

% \bryan{Our study has shown signs that suggest user-defined abstractions---when provided the ability to choose which attributes they want to surface---can be achieved. ... Creating different kinds of abstractions in the same interface as well. In the hotel booking website, X/12 participants finished their task with different attributes surfaced in the bookmarks overview and the map overview. When asked about }

% \bryan{Creating more visual abstractions through AI could be possible. While multiple representations are fixed in our probes, generative AI tools have the potential to construct custom abstractions based on attributes people surface in the overview.}





% Our exploration of design probes and observations from our user study reveal opportunities to support more variations of overview-detail interfaces. We discuss future steps to study these opportunities in the long term, identifying practical approaches to implement malleable overview-detail interfaces in real-world websites.

% Our exploration of our design probes and observations from our user study ---> there are opportunities to support more variations of overview-detail interfaces, future steps to further study ... in the long run, and approaches to take to practically implement malleable overview-detail interfaces in realworld websites


% In this section, we discuss how customization behaviors may differ with prolonged use of malleable overview-detail interfaces and provide how future work can further study these behaviors. We then discuss how malleable overview-detail interfaces could be practically implemented in real-world websites, and then finally explore approaches to making overview-detail interfaces even more malleable.


% Perhaps an approach to take is to scrap the plan to convince developers entirely by doing it ourselves and making an end-user tool in browsers, following the many end-user customization extensions tools from prior research \cite{}.
% + We can scrape the currently active website to identify the overview and detail view as well as all their attributes
% + Leverage AI to cover for missing attributes and make data more consistent.
% - Websites are also constantly evolving, which will require the extension to constantly evolve to support as many websites as possible.
% - We are limited by the data provided in compiled code through the browser, forcing us to reconstruct the data already constructed by the website providers
% - This is only scoped for the browser. (I might remove this argument, cause framework also scoped to browser)

% \textbf{Outline}
% \begin{itemize}
%     \item We find MODs are very useful and people really want it. How do we practically bring this to the real world?
%     \begin{itemize}
%         \item It's about reducing the burden for developers --- developer toolkit
%     \end{itemize}
% \end{itemize}


% - Practical value of malleable overview-detail interfaces
% \bryan{Transition to ``Well, inevitably, everyone is different, even within our identified groups. This means we still need malleability. How do we practically implement malleable overview-detail interfaces?''}
% But we also need these customizations to become easily accessible, become defaults of the overview-detail interface.

% \bryan{We have demonstrated that end-users can and will customize overview-detail interfaces.}
% \bryan{We have also demonstrated---through our design probes---malleable overview-detail interfaces can be built effectively.}
% \bryan{But the question remains: Is it practical to invest the time and effort to provide such malleability in real websites? Will corporations and website providers actually build this?}
% \bryan{Certainly, creating more customization features requires more time and effort to develop, which costs money. The incentive for corporations and independent website providers to create a more malleable overview-detail interface is not necessarily in their best financial or personal interest.}
% \bryan{However, the financial and user experience benefits may exceed the initial cost to build. Improved user experience increases retention, retention increases likelihood of sales (cite? more logic?).}
% \bryan{The bottleneck lies in the burden for designers and developers to build these customizations to lower the barrier to bringing malleability to these sites.}
% \bryan{One way to achieve this is to provide a developer toolkit---a library or a development framework that provides a more malleable overview-detail interfaces out of the box.}
% \bryan{Note: Mention how overview representations have the potential to be interoverable with overview-detail interfaces now, through attributes}

% \bryan{Also, how do we actually get AI into the mix of things in these websites? We're already seeing many websites use AI as chatbots with LLMs being so powerful. Websites are using LLMs to return UI components within the conversational UI. But this means you lose the interface you designed to be used --- there's a disconnect. But with AI integrated into overview-detail, it's possible to directly change the UI. (But that's already been convinced in the past sections). }


% We found in our user study that participants had strongly agreed of the utility of our customizations, suggesting that users
% Our user study showed optimistic signs of the utility and value in malleable overview-detail interfaces for end-users. We have also demonstrated through our design probes that malleable overview-detail interfaces can indeed be built in websites.
% However, providing more customizability does require more development, and for all website builders---individual website providers to large corporations---costs in time and effort are extremely valuable.

% Our designs are valuable, and we provide results that signal the utility of these customizations.
% But ultimately, the decision to implement these designs fall to the hands of the developers---individual website providers to large corporations. And providing more customizability requires more development, which costs time and effort---extremely valuable resources for orgs and businesses.
% Thus, our question then becomes: How do we make it practical for developers to bring malleable overview-detail interfaces

% Our user study showed promising signs of the utility and value of malleable overview-detail interfaces for end-users. Our design probes further demonstrated that such interfaces can be effectively implemented on websites. However, adding more customization options requires additional development, which translates to significant time and effort—valuable resources for both individual website providers and large corporations.

% Thus, the key question becomes: How can we make it practical for developers to integrate malleable overview-detail interfaces into their systems?


% \paragraph{Developer toolkit for malleable overview-detail interfaces}



% \subsection{Seamless customization}
% We proposed \technique, which allowed users to easily surface, hide, sort, and filter attributes of interest.

% Filtering and sorting aren't really considered customizations, but they are configurations on the website. Similarly, reordering tabs on a browser is so lightweight that it's not a customization basically.
% Can \technique achieve this level of seamlessness in the interface?



% slowly dwindle or remain cyclical. 

% Regardless of the outcome, the need for malleable overview-detail interfaces remains unchanged. If users continue to alternate between various customizations based on different contexts, we indeed confirm the need for malleable overview-detail interfaces in our everyday use. If users converge towards an optimal overview-detail setting, the very tool needed to reach this optimal setting is through the malleable overview-detail interface.

% Perhaps we may converge to find out that users eventually reach a final default they like and never switch away from for all dimensions. Nevertheless, the value of malleable overview-detail interfaces still remain in \textit{enabling} users to reach this optimal convergence.




% * On the other hand, other participants had mentioned the utility of customizations, for instance P1 stated they wished they could stay in ``Attributes Mode''



% \textbf{Outline}
% \begin{itemize}
%     \item We don't want participants to customize all the time. We need to provide defaults that fit user groups.
%                     \begin{itemize}
%                         \item P11 said they will customize and just be done with it.
%                         \item P2 said they didn't like too many options to customize.
%                         \item Possible defaults we can provide to these groups?
%                         \item Need to figure this out. What are some defaults that might best benefit these groups? (Groups being Revealers, Removers, and Refiners; AI-enthusiasts; sub-task creators)
%                     \end{itemize}
% \item In addition to default MOD settings, we found participants who wanted some customizations to be default.
%     \begin{itemize}
%         \item P1 wanted to just stay in Attributes Mode.
%         \item Perhaps \technique is more ``seamless'' than the others, hinting at this customization being a necessary feature for user workflows. Similar to filtering and sorting---they are customizations, but so lightweight and so necessary, it's a default way to configure the interface.
%     \end{itemize}
% \item If we do give better defaults for MODs, will users still customize? If so, what will they customize? Is there a convergence towards a user-optimal set of features, or is there an alternating cycle?
%     \begin{itemize}
%         \item Future work could study this.
%     \end{itemize}
% \end{itemize}

% From these two needs, we find that there are people who want good defaults, but there are also people who want customizations by default.
% What are the features that users want as better defaults? What are features that users will inevitably still customize?
% Future work could design and implement better defaults for usage groups, and study user behaviors of these better default probes.


% - Design implications and recommendations for the user groups we identified
% \bryan{There are barriers to customization \cite{Mackay1991TriggersAndBarriers}, and thus would be most beneficial to provide more general defaults that tailor toward these groups.}
% \bryan{This talks about for these groups, what may be the default that will help them the most}

% \bryan{X/12 participants mentioned they would have liked to stay on Attributes Mode during the whole task, PX stating, ``....'''}
% \bryan{Another participant (PX) wished to be able to right-click to select the attributes instead to access the attribute even more in-situ.}






% One way to answer these questions can be to study the prolonged use of malleable overview-detail interfaces. Future work could build and deploy a robust probe to observe when and how frequently users make customizations. 
% This study would provide insights to the if and when users will find an optimal setting or continue to leverage various customizations in different contexts.

% We could use this probe to observe whether the a long-term use will lead to users finding their optimal default or continue to leverage various customizations in different contexts.



% These preferences can take us in two directions for malleable overview-detail interfaces: 1) users either converge towards an optimal default setting or 2) users constantly alternate between various customizations throughout their tasks.

% Users' desires to stay in

% that they would prefer a ``customization page'' where they can customize once and 
% these better defaults may be the desired ultimate outcome, .

% P11 commented on the matter of convenience/, ``\textit{Personally, I'd like a customization page or a separate menu for customization, something I can customize once and be done.}'' 


% * Rec default designs
% * This may be the desired outcome, that people simply want better defaults.
% * P11 says they want to customize and just be done with it
% * P2 says they don't like being given too many options to customize.
% * Then, this might show that providing better defaults for these groups would certainly be beneficial.
% * Other participants, however, mentioned that they wanted ``Attributes Mode'' to be a default for their interface, suggesting that users may constantly use \technique throughout their task. This means other participants would want to keep customizing, changing the various dimensions.
% * These decisions can take us in two trajectories: 1) Eventual convergence towards an optimal default setting or 2) an alternating cycle between customizations based on task.
% * The behaviors after we give these user groups improved defaults can take two trajectories: User needs and overview-detail defaults can converge
% perhaps we can provide them the defaults they want, and run the study once more. Will users still customize?




% P11 - Customize and done
% It might be like personally I think I like, I like like a customization page possibly or a a separate menu for customization that I feel like I customize once and then I'm done. Yeah. But for featuring customization like the hide on and off, yeah, I if I were to hope for a way to do it, I just, I want like maybe a check box or maybe some like keywords I can type into it, Yeah.

% P2 - given so much power, I don't like like many options to customize. I think I wasn't sure which ones might be like, I have an idea like what might be more important for me, like for this specific task, but like, I don't know if I'm choosing the right ones for those, if that makes sense. I see, like, yeah, maybe I want like a recommendation of like most people sorted by price, size and weight or something like that. And like, oh, I didn't think about weight. Like I want a heavy like monitor or not, or yeah. And so like I'd want to also filter by that or like, yeah, I don't know, like being able to not only choose what filters I want to use, but also explore other useful filters for me in my use case. But I guess that's more of the like the kind of like AI powered suggestion, kind of like functionality, but maybe not what we're talking about for customization. 










% \bryan{AI Limitation: Refining Prompts}
% We also found participants who appeared to be primarily Revealers ended up hiding AI-generated attributes they no longer wanted. Likely due to the attribute and value being incorrect... they didn't want the value to distract them. However, some eventually did land on an attribute they wanted, but just through iteration. Allowing users to refine their prompt likely resolves this challenge.



% \bryan{Suggesting an equilibrium of attributes?}
% Hotel booking and shopping websites provided different number of attributes by default. The hotel booking website provided only the rating of the hotel, while the shopping website provided eight default attributes. This explains why participants hid more attributes on the shopping website as opposed to the hotel booking website, uncovering the behavior group of removers. However, some still did not remove attributes on the shopping website. This raises the question: regardless of provided defaults, will the end-user inevitably surface attributes they need, or is there a large enough barrier to stop users from surfacing all details they would need? Answering this may provide implications to the design of the defaults of malleable overview-detail interfaces.
% Although websites may converge to a subset of attributes most users may need



% \subsection{Isn't it always better to let people customize?}

% Diverse customizations can simply mean they make different changes to the interface. Giving them the same task does control, but diverse changes could just be because everyone does different things.

% Our study suggests users want diverse customizations of overview-detail, but it could also be because people just make a lot of different choices?

% \bryan{It is true. Having the option is better. But there are barriers to customization that aren't necessarily worth it. Wendy shares these barriers to customizing software, and a key barrier is simply how easy it is to customize.}
% \bryan{During our study, X/12 participants raised their score from the hotel booking website to the shopping website when rating Ease of Use on the content dimension (this might not be a valid argument). But X/12 participants DID state that \technique got easier to use because they became familiar with it during the hotel booking task.}
% \bryan{So ease of use and ease of learning are important. This might sacrifice discoverability, but once discovered, could be powerful.....? this reads weird}



% \subsection{Guidelines for practically implementing malleable overview-detail interfaces}

% \subsubsection{Practically Implementing \TechNique}
% \bryan{When designing \technique, we considered multiple interactions for users to easily select attributes. We explored area selection, standard in-browser text selection, and even simply right-clicking to open a context menu. We opted for a toggle button that highlighted all attributes to prioritize discoverability of the novel interaction technique.}
% \bryan{During our user study, while all 12 participants either agreed or strongly agreed that \technique useful, some wished for an easier way to manipulate attributes.}
% \bryan{X/12 participants mentioned they would have liked to stay on Attributes Mode during the whole task, PX stating, ``....'''}
% \bryan{Another participant (PX) wished to be able to right-click to select the attributes instead to access the attribute even more in-situ.}
% \bryan{Thus, our findings recommend designers to provide multiple ways---for discoverability and ease of access---for selecting attributes, when practically implementing \technique on websites}

% \subsubsection{Practically Implementing AI-assisted \TechNique}
% ...




% \subsection{How much malleability is enough malleability?}
% End-user customization can go as far as being able to edit the code \bryan{Reference what Geoffrey Litt and Clemens referenced in their talks --- MyWebstrates or Wildcard? Climbing step by step towards more code...?}



==> versions/initial_submission/9_limitations_future_work.tex <==
% \section{Limitations and Future Work}
% \label{section:limitation-future-work}


% \subsection{Content Analysis Limitations}

% \subsection{User Study}

% There may have been a learning bias from the hotel booking website to the shopping website, 


% Diverse customizations can simply mean they make different changes to the interface. Giving them the same task does control, but diverse changes could just be because everyone does different things.

% Our study suggests users want diverse customizations of overview-detail, but it could also be because people just make a lot of different choices?




% \subsection{Studying the Prolonged Use Malleable Overview-Detail Interfaces}

% % Certainly, a system with too many features becomes too complex for users to learn within the given time of a controlled study.
% % The purpose of our probes is to study the diverse customizations people make, rather if they utilize all customizations in a given time-frame. To this end, ...
% % % However, we do not undermine the importance of providing more customizability options malleable overview-detail interfaces.
% % Many other features in a practical setting, could be implemented to be more discoverable through a prolonged use of the system.


% % Since the purpose of the probes is to study the how people make diverse customizations when provided, rather than evaluating whether they can make effectively make and utilize every customization in the interface, we implemented a subset of our interaction techniques into our probes. 

% % Certainly, a system with too many features becomes too complex for users to learn within the given time of a controlled study.
% % The purpose of our probes is to study the diverse customizations people make, rather if they utilize all customizations in a given time-frame. To this end, ...
% % However, we do not undermine the importance of malleable overview-detail interfaces.
% % Many other features in a practical setting, could be implemented to be more discoverable through a prolonged use of the system.



% \subsection{Developer Toolkit for Malleable Overview-Detail Interfaces}
